The California-Kepler Survey. I. High Resolution Spectroscopy of 1305 Stars Hosting Kepler Transiting Planets

The California-Kepler Survey (CKS) is an observational program to improve our knowledge of the properties of stars found to host transiting planets by NASA's Kepler Mission. The improvement stems from new high-resolution optical spectra obtained using HIRES at the W. M. Keck Observatory. The CKS stellar sample comprises 1305 stars classified as Kepler Objects of Interest, hosting a total of 2075 transiting planets. The primary sample is magnitude-limited (Kp < 14.2) and contains 960 stars with 1385 planets. The sample was extended to include some fainter stars that host multiple planets, ultra short period planets, or habitable zone planets. The spectroscopic parameters were determined with two different codes, one based on template matching and the other on direct spectral synthesis using radiative transfer. We demonstrate a precision of 60 K in effective temperature, 0.10 dex in surface gravity, 0.04 dex in [Fe/H], and 1.0 km/s in projected rotational velocity. In this paper we describe the CKS project and present a uniform catalog of spectroscopic parameters. Subsequent papers in this series present catalogs of derived stellar properties such as mass, radius and age; revised planet properties; and statistical explorations of the ensemble. CKS is the largest survey to determine the properties of Kepler stars using a uniform set of high-resolution, high signal-to-noise ratio spectra. The HIRES spectra are available to the community for independent analyses.

==> tab_cks.tex <==
K00001 & 5819 & 4.40 & $+$0.01 & 1.3 &  & 5853 & 4.43 & $+$0.02 & 1.3 &  & 5785 & 4.37 & $+$0.01 & 4.3 & $+$0.5\\ 
K00002 & 6449 & 4.13 & $+$0.20 & 5.2 &  & 6376 & 4.13 & $+$0.21 & 5.2 &  & 6521 & 4.14 & $+$0.20 & 6.1 & $-$10.4\\ 
K00003 & 4864 & 4.50 & $+$0.33 & 3.2 &  & 4864 & 4.50 & $+$0.33 & 3.2 &  & 4696 & 3.97 & $-$0.36 & 3.1 & $-$63.4\\ 
K00006 & 6348 & 4.36 & $+$0.04 & 11.8 &  & 6348 & 4.36 & $+$0.04 & 11.8 &  & \nodata & \nodata & \nodata & \nodata & $-$42.8\\ 
K00007 & 5827 & 4.09 & $+$0.18 & 2.8 &  & 5813 & 4.03 & $+$0.17 & 2.8 &  & 5841 & 4.15 & $+$0.18 & 4.6 & $-$60.8\\ 
K00008 & 5891 & 4.53 & $-$0.07 & 3.0 &  & 5891 & 4.53 & $-$0.07 & 3.0 &  & \nodata & \nodata & \nodata & \nodata & $-$54.7\\ 
K00010 & 6181 & 4.24 & $-$0.08 & 10.2 &  & 6195 & 4.20 & $-$0.09 & 10.2 &  & 6167 & 4.27 & $-$0.07 & 10.9 & $-$52.5\\ 
K00017 & 5660 & 4.15 & $+$0.36 & 2.6 &  & 5671 & 4.11 & $+$0.36 & 2.6 &  & 5648 & 4.20 & $+$0.36 & 4.6 & $-$49.2\\ 
K00018 & 6332 & 4.12 & $+$0.02 & 4.4 &  & 6308 & 4.13 & $+$0.02 & 4.4 &  & 6355 & 4.11 & $+$0.03 & 6.1 & $-$18.4\\ 
K00020 & 5926 & 4.01 & $+$0.03 & 1.7 &  & 5926 & 4.01 & $+$0.03 & 1.7 &  & \nodata & \nodata & \nodata & \nodata & $+$1.7\\ 
K00022 & 5891 & 4.21 & $+$0.21 & 1.9 &  & 5903 & 4.20 & $+$0.22 & 1.9 &  & 5880 & 4.22 & $+$0.20 & 4.8 & $-$12.0\\ 
K00041 & 5854 & 4.07 & $+$0.10 & 2.7 &  & 5859 & 4.05 & $+$0.10 & 2.7 &  & 5850 & 4.09 & $+$0.10 & 5.2 & $-$61.4\\ 
K00042 & 6306 & 4.28 & $-$0.01 & 13.0 &  & 6351 & 4.33 & $+$0.01 & 13.0 &  & 6260 & 4.23 & $-$0.02 & 13.7 & $-$40.2\\ 
K00046 & 5661 & 4.07 & $+$0.39 & 2.5 &  & 5622 & 3.95 & $+$0.39 & 2.5 &  & 5700 & 4.19 & $+$0.40 & 4.3 & $-$77.7\\ 
K00049 & 5779 & 4.34 & $-$0.06 & 7.7 &  & 5804 & 4.33 & $-$0.06 & 7.7 &  & 5755 & 4.35 & $-$0.07 & 8.6 & $-$111.2\\ 
K00063 & 5673 & 4.68 & $+$0.25 & 4.8 &  & 5636 & 4.61 & $+$0.23 & 4.8 &  & 5710 & 4.75 & $+$0.26 & 6.6 & $-$22.3\\ 
K00064 & 5357 & 3.86 & $+$0.09 & 2.0 &  & 5319 & 3.90 & $+$0.06 & 2.0 &  & 5395 & 3.81 & $+$0.13 & 5.0 & $-$29.8\\ 
K00069 & 5594 & 4.41 & $-$0.09 & 0.0 &  & 5615 & 4.43 & $-$0.10 & 0.0 &  & 5572 & 4.39 & $-$0.08 & 4.4 & $+$27.2\\ 
K00070 & 5508 & 4.47 & $+$0.11 & 0.0 &  & 5511 & 4.47 & $+$0.10 & 0.0 &  & 5505 & 4.46 & $+$0.12 & 4.4 & $-$21.2\\ 
K00072 & 5599 & 4.28 & $-$0.11 & 0.0 &  & 5629 & 4.26 & $-$0.11 & 0.0 &  & 5569 & 4.29 & $-$0.12 & 4.4 & $-$99.1\\ 
K00075 & 5940 & 3.86 & $-$0.04 & 5.0 &  & 5857 & 3.80 & $-$0.09 & 5.0 &  & 6023 & 3.93 & $+$0.00 & 6.8 & $-$12.4\\ 
K00082 & 4909 & 4.62 & $+$0.11 & 0.7 &  & 4870 & 4.61 & $+$0.10 & 0.7 &  & 4949 & 4.64 & $+$0.11 & 4.3 & $-$28.4\\ 
K00084 & 5520 & 4.49 & $-$0.03 & 0.0 &  & 5508 & 4.46 & $-$0.05 & 0.0 &  & 5533 & 4.51 & $-$0.02 & 4.1 & $-$10.6\\ 
K00085 & 6220 & 4.21 & $+$0.13 & 8.7 &  & 6217 & 4.21 & $+$0.15 & 8.7 &  & 6222 & 4.22 & $+$0.11 & 9.7 & $-$17.3\\ 
K00087 & 5528 & 4.51 & $-$0.20 & 0.0 &  & 5547 & 4.54 & $-$0.23 & 0.0 &  & 5509 & 4.48 & $-$0.18 & 4.5 & $-$4.3\\ 
K00092 & 5923 & 4.39 & $+$0.09 & 2.7 &  & 5931 & 4.38 & $+$0.09 & 2.7 &  & 5915 & 4.41 & $+$0.08 & 4.7 & $-$34.0\\ 
K00094 & 6181 & 4.23 & $+$0.07 & 7.4 &  & 6159 & 4.21 & $+$0.07 & 7.4 &  & 6203 & 4.26 & $+$0.07 & 8.6 & $-$19.7\\ 
K00097 & 6084 & 3.99 & $+$0.19 & 3.7 &  & 6035 & 3.94 & $+$0.18 & 3.7 &  & 6133 & 4.04 & $+$0.21 & 5.1 & $+$0.2\\ 
K00098 & 6500 & 4.23 & $+$0.05 & 7.4 &  & 6483 & 4.28 & $+$0.05 & 7.4 &  & 6517 & 4.17 & $+$0.05 & 10.3 & $+$7.1\\ 
K00099 & 4935 & 4.42 & $-$0.28 & 0.4 &  & 4937 & 4.44 & $-$0.27 & 0.4 &  & 4933 & 4.40 & $-$0.30 & 4.0 & $-$71.4\\ 
K00102 & 5759 & 4.34 & $+$0.24 & 1.7 &  & 5782 & 4.30 & $+$0.24 & 1.7 &  & 5735 & 4.37 & $+$0.24 & 4.3 & $-$18.8\\ 
K00103 & 5565 & 4.54 & $+$0.01 & 0.2 &  & 5575 & 4.53 & $+$0.00 & 0.2 &  & 5556 & 4.54 & $+$0.02 & 4.3 & $+$9.9\\ 
K00104 & 4728 & 4.38 & $+$0.32 & 1.3 &  & 4728 & 4.38 & $+$0.32 & 1.3 &  & 4959 & 3.89 & $+$0.36 & 4.7 & $-$51.2\\ 
K00105 & 5567 & 4.38 & $-$0.35 & 0.0 &  & 5559 & 4.28 & $-$0.37 & 0.0 &  & 5574 & 4.47 & $-$0.34 & 3.7 & $-$58.1\\ 
K00107 & 5920 & 4.10 & $+$0.26 & 3.9 &  & 5934 & 4.08 & $+$0.28 & 3.9 &  & 5906 & 4.12 & $+$0.25 & 5.3 & $-$50.8\\ 
K00108 & 5886 & 4.08 & $+$0.13 & 3.1 &  & 5903 & 4.08 & $+$0.14 & 3.1 &  & 5869 & 4.08 & $+$0.12 & 5.6 & $-$28.1\\ 
K00110 & 6207 & 4.35 & $-$0.16 & 7.0 &  & 6238 & 4.37 & $-$0.16 & 7.0 &  & 6177 & 4.33 & $-$0.17 & 8.1 & $-$32.4\\ 
K00111 & 5760 & 4.36 & $-$0.42 & 0.0 &  & 5805 & 4.39 & $-$0.43 & 0.0 &  & 5716 & 4.34 & $-$0.42 & 4.4 & $+$1.7\\ 
K00112 & 5805 & 4.34 & $-$0.03 & 2.9 &  & 5827 & 4.34 & $-$0.03 & 2.9 &  & 5783 & 4.33 & $-$0.02 & 4.9 & $-$1.2\\ 
K00113 & 5591 & 4.10 & $+$0.40 & 2.3 &  & 5569 & 4.03 & $+$0.40 & 2.3 &  & 5614 & 4.17 & $+$0.40 & 4.4 & $-$84.0\\ 
K00115 & 5933 & 4.40 & $-$0.09 & 2.9 &  & 5955 & 4.39 & $-$0.09 & 2.9 &  & 5911 & 4.41 & $-$0.09 & 4.8 & $+$0.4\\ 
K00116 & 5860 & 4.36 & $-$0.09 & 0.6 &  & 5876 & 4.36 & $-$0.09 & 0.6 &  & 5843 & 4.36 & $-$0.08 & 4.5 & $-$57.9\\ 
K00117 & 5867 & 4.11 & $+$0.32 & 3.1 &  & 5856 & 4.08 & $+$0.33 & 3.1 &  & 5877 & 4.15 & $+$0.32 & 4.9 & $+$5.6\\ 
K00118 & 5764 & 4.17 & $+$0.07 & 2.1 &  & 5772 & 4.14 & $+$0.08 & 2.1 &  & 5756 & 4.20 & $+$0.06 & 4.4 & $-$26.9\\ 
K00119 & 5681 & 3.86 & $+$0.37 & 3.2 &  & 5644 & 3.79 & $+$0.36 & 3.2 &  & 5718 & 3.93 & $+$0.38 & 5.0 & $-$14.8\\ 
K00122 & 5654 & 4.09 & $+$0.27 & 0.9 &  & 5659 & 4.03 & $+$0.27 & 0.9 &  & 5649 & 4.15 & $+$0.27 & 4.7 & $-$31.6\\ 
K00123 & 5917 & 4.17 & $-$0.02 & 2.8 &  & 5930 & 4.17 & $-$0.02 & 2.8 &  & 5904 & 4.17 & $-$0.01 & 5.1 & $-$37.4\\ 
K00124 & 5956 & 4.27 & $-$0.10 & 3.3 &  & 5973 & 4.27 & $-$0.10 & 3.3 &  & 5939 & 4.28 & $-$0.10 & 5.1 & $+$0.1\\ 
K00127 & 5596 & 4.37 & $+$0.37 & 2.0 &  & 5575 & 4.33 & $+$0.36 & 2.0 &  & 5616 & 4.41 & $+$0.38 & 4.6 & $-$24.9\\ 
K00128 & 5662 & 4.19 & $+$0.27 & 2.9 &  & 5648 & 4.13 & $+$0.27 & 2.9 &  & 5677 & 4.25 & $+$0.27 & 4.6 & $-$20.5\\ 
K00134 & 6236 & 4.14 & $+$0.28 & 11.1 &  & 6255 & 4.16 & $+$0.30 & 11.1 &  & 6216 & 4.12 & $+$0.27 & 11.9 & $-$17.1\\ 
K00135 & 5957 & 4.20 & $+$0.34 & 5.4 &  & 5950 & 4.13 & $+$0.36 & 5.4 &  & 5964 & 4.26 & $+$0.33 & 6.4 & $-$37.7\\ 
K00137 & 5441 & 4.42 & $+$0.28 & 0.0 &  & 5436 & 4.37 & $+$0.28 & 0.0 &  & 5446 & 4.47 & $+$0.29 & 4.5 & $-$18.8\\ 
K00139 & 5905 & 4.28 & $+$0.22 & 2.8 &  & 5918 & 4.29 & $+$0.22 & 2.8 &  & 5893 & 4.27 & $+$0.22 & 5.0 & $-$18.9\\ 
K00141 & 5321 & 4.42 & $+$0.31 & 3.0 &  & 5274 & 4.36 & $+$0.29 & 3.0 &  & 5367 & 4.48 & $+$0.34 & 4.8 & $-$21.1\\ 
K00142 & 5466 & 4.42 & $+$0.27 & 0.0 &  & 5471 & 4.39 & $+$0.27 & 0.0 &  & 5460 & 4.44 & $+$0.27 & 3.5 & $-$20.5\\ 
K00144 & 4932 & 4.48 & $+$0.29 & 2.9 &  & 4920 & 4.48 & $+$0.28 & 2.9 &  & 4944 & 4.49 & $+$0.29 & 4.6 & $-$9.0\\ 
K00145 & 4923 & 3.26 & $+$0.05 & 2.4 &  & 4923 & 3.26 & $+$0.05 & 2.4 &  & \nodata & \nodata & \nodata & \nodata & $-$35.7\\ 
K00148 & 5235 & 4.46 & $+$0.26 & 0.3 &  & 5204 & 4.40 & $+$0.24 & 0.3 &  & 5266 & 4.52 & $+$0.28 & 4.4 & $-$14.0\\ 
K00149 & 5708 & 3.95 & $+$0.03 & 2.6 &  & 5699 & 3.93 & $+$0.03 & 2.6 &  & 5717 & 3.98 & $+$0.04 & 4.6 & $-$23.0\\ 
K00150 & 5501 & 4.49 & $-$0.40 & 0.8 &  & 5562 & 4.49 & $-$0.40 & 0.8 &  & 5439 & 4.49 & $-$0.41 & 4.1 & $-$84.4\\ 
K00152 & 6389 & 4.33 & $+$0.06 & 14.0 &  & 6426 & 4.39 & $+$0.07 & 14.0 &  & 6351 & 4.26 & $+$0.05 & 15.0 & $-$24.4\\ 
K00153 & 4791 & 4.48 & $+$0.13 & 2.2 &  & 4733 & 4.42 & $+$0.11 & 2.2 &  & 4849 & 4.54 & $+$0.14 & 4.3 & $+$1.6\\ 
K00155 & 5667 & 4.13 & $-$0.17 & 1.4 &  & 5672 & 4.06 & $-$0.17 & 1.4 &  & 5662 & 4.21 & $-$0.17 & 4.0 & $+$4.4\\ 
K00156 & 4661 & 4.50 & $+$0.10 & 3.1 &  & 4661 & 4.50 & $+$0.10 & 3.1 &  & 5755 & 4.13 & $+$0.90 & 7.4 & $-$57.6\\ 
K00157 & 5763 & 4.28 & $+$0.05 & 0.9 &  & 5763 & 4.28 & $+$0.05 & 0.9 &  & \nodata & \nodata & \nodata & \nodata & $-$56.6\\ 
K00159 & 6000 & 4.37 & $-$0.02 & 3.5 &  & 6024 & 4.36 & $-$0.02 & 3.5 &  & 5975 & 4.38 & $-$0.02 & 5.3 & $-$56.1\\ 
K00161 & 4995 & 4.51 & $+$0.34 & 1.3 &  & 4976 & 4.50 & $+$0.33 & 1.3 &  & 5014 & 4.51 & $+$0.34 & 4.1 & $-$14.9\\ 
K00162 & 5863 & 4.27 & $+$0.22 & 3.1 &  & 5841 & 4.21 & $+$0.22 & 3.1 &  & 5885 & 4.34 & $+$0.21 & 4.9 & $-$21.8\\ 
K00163 & 5035 & 4.56 & $-$0.37 & 0.9 &  & 5037 & 4.63 & $-$0.37 & 0.9 &  & 5033 & 4.49 & $-$0.38 & 3.8 & $-$9.7\\ 
K00165 & 5154 & 4.52 & $-$0.20 & 1.7 &  & 5121 & 4.55 & $-$0.21 & 1.7 &  & 5187 & 4.49 & $-$0.19 & 4.5 & $+$14.9\\ 
K00166 & 5159 & 4.56 & $-$0.21 & 0.6 &  & 5171 & 4.63 & $-$0.22 & 0.6 &  & 5146 & 4.50 & $-$0.21 & 4.0 & $-$32.5\\ 
K00167 & 6231 & 4.16 & $+$0.05 & 2.4 &  & 6224 & 4.17 & $+$0.05 & 2.4 &  & 6238 & 4.16 & $+$0.06 & 4.4 & $-$22.5\\ 
K00168 & 5823 & 4.06 & $-$0.09 & 1.4 &  & 5790 & 4.01 & $-$0.12 & 1.4 &  & 5857 & 4.11 & $-$0.06 & 4.4 & $-$26.1\\ 
K00171 & 6220 & 4.28 & $+$0.07 & 7.9 &  & 6225 & 4.29 & $+$0.10 & 7.9 &  & 6215 & 4.27 & $+$0.05 & 8.6 & $-$12.7\\ 
K00172 & 5630 & 4.29 & $-$0.22 & 1.4 &  & 5659 & 4.22 & $-$0.22 & 1.4 &  & 5601 & 4.36 & $-$0.22 & 4.3 & $-$38.7\\ 
K00173 & 5676 & 4.21 & $+$0.01 & 2.0 &  & 5667 & 4.16 & $-$0.00 & 2.0 &  & 5685 & 4.25 & $+$0.01 & 4.5 & $+$5.8\\ 
K00174 & 4734 & 4.41 & $-$0.27 & 2.2 &  & 4692 & 4.39 & $-$0.25 & 2.2 &  & 4775 & 4.44 & $-$0.30 & 4.5 & $-$99.4\\ 
K00176 & 6319 & 4.35 & $-$0.22 & 11.1 &  & 6381 & 4.40 & $-$0.21 & 11.1 &  & 6256 & 4.30 & $-$0.22 & 11.8 & $-$47.6\\ 
K00177 & 5741 & 4.38 & $-$0.00 & 1.9 &  & 5733 & 4.36 & $-$0.00 & 1.9 &  & 5749 & 4.40 & $+$0.00 & 4.2 & $-$8.1\\ 
K00179 & 6218 & 4.07 & $+$0.25 & 9.3 &  & 6126 & 4.02 & $+$0.23 & 9.3 &  & 6309 & 4.12 & $+$0.27 & 10.2 & $+$7.8\\ 
K00180 & 5652 & 4.58 & $+$0.06 & 0.8 &  & 5635 & 4.58 & $+$0.04 & 0.8 &  & 5668 & 4.58 & $+$0.08 & 4.7 & $-$2.3\\ 
K00186 & 5802 & 4.37 & $+$0.19 & 2.1 &  & 5802 & 4.37 & $+$0.19 & 2.1 &  & \nodata & \nodata & \nodata & \nodata & $-$8.2\\ 
K00191 & 5456 & 4.47 & $+$0.11 & 1.0 &  & 5469 & 4.44 & $+$0.13 & 1.0 &  & 5444 & 4.49 & $+$0.08 & 4.1 & $-$62.8\\ 
K00193 & 5628 & 3.93 & $+$0.03 & 303.4 &  & 5677 & 3.63 & $+$0.11 & 303.4 &  & 5578 & 4.23 & $-$0.05 & 6.1 & $-$25.5\\ 
K00195 & 5535 & 4.48 & $-$0.17 & 0.1 &  & 5535 & 4.48 & $-$0.17 & 0.1 &  & \nodata & \nodata & \nodata & \nodata & $-$78.2\\ 
K00197 & 4938 & 4.50 & $+$0.02 & 1.9 &  & 4936 & 4.49 & $+$0.06 & 1.9 &  & 4939 & 4.52 & $-$0.01 & 4.6 & $-$15.8\\ 
K00201 & 5522 & 4.23 & $+$0.37 & 2.1 &  & 5551 & 4.24 & $+$0.39 & 2.1 &  & 5493 & 4.21 & $+$0.35 & 4.7 & $-$60.1\\ 
K00203 & 5722 & 4.53 & $+$0.33 & 4.5 &  & 5705 & 4.51 & $+$0.32 & 4.5 &  & 5740 & 4.56 & $+$0.34 & 6.0 & $-$24.8\\ 
K00209 & 6085 & 4.14 & $+$0.03 & 7.4 &  & 6059 & 4.14 & $+$0.01 & 7.4 &  & 6111 & 4.14 & $+$0.04 & 8.3 & $-$12.4\\ 
K00211 & 5830 & 4.06 & $-$0.05 & 3.7 &  & 5765 & 3.89 & $-$0.09 & 3.7 &  & 5895 & 4.23 & $-$0.00 & 5.4 & $-$1.6\\ 
K00214 & 5482 & 4.32 & $+$0.42 & 2.5 &  & 5466 & 4.23 & $+$0.42 & 2.5 &  & 5498 & 4.40 & $+$0.41 & 4.6 & $-$27.3\\ 
K00232 & 5917 & 4.27 & $-$0.08 & 4.0 &  & 6008 & 4.26 & $-$0.05 & 4.0 &  & 5825 & 4.28 & $-$0.11 & 5.5 & $+$20.4\\ 
K00237 & 5748 & 4.22 & $+$0.24 & 2.8 &  & 5762 & 4.25 & $+$0.26 & 2.8 &  & 5734 & 4.19 & $+$0.23 & 4.8 & $-$21.9\\ 
K00238 & 6154 & 4.28 & $-$0.08 & 5.9 &  & 6132 & 4.27 & $-$0.10 & 5.9 &  & 6175 & 4.28 & $-$0.06 & 7.1 & $-$21.3\\ 
K00241 & 4960 & 4.45 & $-$0.46 & 1.3 &  & 4935 & 4.44 & $-$0.44 & 1.3 &  & 4984 & 4.46 & $-$0.48 & 4.2 & $-$68.9\\ 
K00244 & 6285 & 4.29 & $-$0.04 & 9.3 &  & 6269 & 4.30 & $-$0.03 & 9.3 &  & 6302 & 4.28 & $-$0.05 & 10.2 & $-$8.3\\ 
K00245 & 5348 & 4.59 & $-$0.25 & 0.0 &  & 5366 & 4.65 & $-$0.26 & 0.0 &  & 5329 & 4.53 & $-$0.24 & 4.1 & $-$30.9\\ 
K00246 & 5789 & 4.20 & $+$0.14 & 0.0 &  & 5773 & 4.12 & $+$0.13 & 0.0 &  & 5805 & 4.28 & $+$0.14 & 4.4 & $-$21.0\\ 
K00257 & 6163 & 4.30 & $+$0.10 & 7.5 &  & 6191 & 4.35 & $+$0.11 & 7.5 &  & 6134 & 4.26 & $+$0.09 & 8.5 & $-$12.1\\ 
K00260 & 6270 & 4.30 & $-$0.16 & 8.7 &  & 6281 & 4.31 & $-$0.15 & 8.7 &  & 6259 & 4.28 & $-$0.17 & 9.7 & $-$20.9\\ 
K00261 & 5751 & 4.50 & $+$0.10 & 0.2 &  & 5738 & 4.49 & $+$0.08 & 0.2 &  & 5763 & 4.52 & $+$0.12 & 4.3 & $-$47.5\\ 
K00262 & 6162 & 4.14 & $-$0.09 & 10.0 &  & 6140 & 4.13 & $-$0.10 & 10.0 &  & 6184 & 4.14 & $-$0.08 & 11.1 & $-$2.8\\ 
K00263 & 5771 & 4.03 & $-$0.11 & 0.8 &  & 5768 & 4.01 & $-$0.13 & 0.8 &  & 5773 & 4.06 & $-$0.10 & 4.8 & $+$1.5\\ 
K00265 & 6030 & 4.24 & $+$0.14 & 2.3 &  & 6012 & 4.17 & $+$0.14 & 2.3 &  & 6048 & 4.30 & $+$0.14 & 4.6 & $-$6.7\\ 
K00266 & 6150 & 4.35 & $-$0.06 & 5.6 &  & 6197 & 4.40 & $-$0.04 & 5.6 &  & 6102 & 4.31 & $-$0.08 & 7.1 & $+$15.8\\ 
K00268 & 6389 & 4.35 & $-$0.02 & 8.5 &  & 6475 & 4.39 & $+$0.02 & 8.5 &  & 6302 & 4.32 & $-$0.05 & 9.6 & $-$41.9\\ 
K00269 & 6303 & 4.25 & $-$0.07 & 11.8 &  & 6299 & 4.28 & $-$0.08 & 11.8 &  & 6306 & 4.22 & $-$0.07 & 12.7 & $-$10.8\\ 
K00270 & 5633 & 4.18 & $-$0.13 & 3.7 &  & 5619 & 4.10 & $-$0.15 & 3.7 &  & 5647 & 4.26 & $-$0.12 & 5.3 & $+$13.7\\ 
K00271 & 6125 & 4.22 & $+$0.24 & 6.6 &  & 6157 & 4.23 & $+$0.27 & 6.6 &  & 6093 & 4.20 & $+$0.21 & 7.5 & $-$21.1\\ 
K00273 & 5678 & 4.24 & $+$0.28 & 0.5 &  & 5674 & 4.21 & $+$0.28 & 0.5 &  & 5682 & 4.26 & $+$0.28 & 4.6 & $-$71.6\\ 
K00274 & 6081 & 4.09 & $-$0.03 & 6.1 &  & 6044 & 4.04 & $-$0.06 & 6.1 &  & 6119 & 4.14 & $-$0.01 & 7.6 & $-$22.0\\ 
K00275 & 5809 & 4.02 & $+$0.26 & 2.9 &  & 5814 & 4.01 & $+$0.26 & 2.9 &  & 5804 & 4.02 & $+$0.25 & 4.7 & $-$21.8\\ 
K00276 & 5952 & 4.28 & $-$0.02 & 2.4 &  & 5991 & 4.33 & $-$0.01 & 2.4 &  & 5913 & 4.23 & $-$0.04 & 4.6 & $-$19.1\\ 
K00277 & 5979 & 4.11 & $-$0.18 & 4.9 &  & 5948 & 4.10 & $-$0.21 & 4.9 &  & 6010 & 4.11 & $-$0.15 & 6.0 & $+$8.5\\ 
K00279 & 6298 & 4.22 & $+$0.17 & 12.9 &  & 6286 & 4.26 & $+$0.17 & 12.9 &  & 6310 & 4.17 & $+$0.17 & 13.8 & $-$18.1\\ 
K00280 & 6002 & 4.41 & $-$0.27 & 3.0 &  & 6077 & 4.50 & $-$0.27 & 3.0 &  & 5928 & 4.32 & $-$0.27 & 5.2 & $-$40.6\\ 
K00281 & 5699 & 4.28 & $-$0.36 & 0.1 &  & 5711 & 4.16 & $-$0.35 & 0.1 &  & 5688 & 4.40 & $-$0.36 & 3.9 & $-$58.6\\ 
K00282 & 5887 & 4.34 & $-$0.16 & 0.9 &  & 5903 & 4.30 & $-$0.16 & 0.9 &  & 5870 & 4.37 & $-$0.16 & 3.9 & $+$19.3\\ 
K00283 & 5787 & 4.44 & $+$0.19 & 0.3 &  & 5786 & 4.41 & $+$0.19 & 0.3 &  & 5788 & 4.48 & $+$0.19 & 4.3 & $-$22.0\\ 
K00284 & 5910 & 4.41 & $-$0.20 & 3.5 &  & 5966 & 4.48 & $-$0.19 & 3.5 &  & 5853 & 4.35 & $-$0.21 & 5.4 & $-$29.1\\ 
K00285 & 5946 & 4.06 & $+$0.19 & 4.0 &  & 5932 & 4.01 & $+$0.19 & 4.0 &  & 5960 & 4.11 & $+$0.19 & 5.3 & $-$40.9\\ 
K00288 & 6221 & 4.05 & $+$0.22 & 7.9 &  & 6184 & 4.02 & $+$0.22 & 7.9 &  & 6258 & 4.08 & $+$0.21 & 8.6 & $-$16.6\\ 
K00289 & 5837 & 4.16 & $-$0.35 & 1.9 &  & 5829 & 4.08 & $-$0.37 & 1.9 &  & 5845 & 4.24 & $-$0.33 & 5.3 & $+$1.0\\ 
K00291 & 5712 & 4.15 & $+$0.29 & 4.0 &  & 5672 & 4.06 & $+$0.28 & 4.0 &  & 5752 & 4.24 & $+$0.30 & 5.4 & $+$7.1\\ 
K00292 & 5773 & 4.45 & $-$0.15 & 0.0 &  & 5777 & 4.45 & $-$0.18 & 0.0 &  & 5769 & 4.45 & $-$0.13 & 4.4 & $+$6.3\\ 
K00294 & 6051 & 4.36 & $+$0.04 & 4.4 &  & 6074 & 4.36 & $+$0.05 & 4.4 &  & 6028 & 4.36 & $+$0.04 & 5.9 & $-$25.4\\ 
K00295 & 5918 & 4.49 & $-$0.17 & 2.0 &  & 5945 & 4.51 & $-$0.18 & 2.0 &  & 5890 & 4.47 & $-$0.15 & 4.7 & $-$26.9\\ 
K00296 & 5748 & 4.33 & $-$0.11 & 1.8 &  & 5753 & 4.29 & $-$0.13 & 1.8 &  & 5742 & 4.36 & $-$0.10 & 4.4 & $-$9.4\\ 
K00297 & 6155 & 4.30 & $+$0.11 & 7.0 &  & 6149 & 4.27 & $+$0.11 & 7.0 &  & 6161 & 4.33 & $+$0.11 & 8.0 & $-$11.6\\ 
K00299 & 5567 & 4.54 & $+$0.20 & 0.2 &  & 5534 & 4.50 & $+$0.18 & 0.2 &  & 5600 & 4.58 & $+$0.22 & 4.1 & $-$30.7\\ 
K00301 & 6014 & 4.13 & $-$0.07 & 5.5 &  & 5983 & 4.08 & $-$0.09 & 5.5 &  & 6046 & 4.17 & $-$0.05 & 6.7 & $-$40.5\\ 
K00303 & 5563 & 4.37 & $-$0.16 & 1.3 &  & 5611 & 4.36 & $-$0.14 & 1.3 &  & 5514 & 4.37 & $-$0.18 & 4.1 & $-$75.9\\ 
K00304 & 5802 & 4.56 & $-$0.14 & 1.5 &  & 5802 & 4.56 & $-$0.17 & 1.5 &  & 5801 & 4.55 & $-$0.11 & 4.4 & $+$23.7\\ 
K00305 & 4852 & 4.55 & $+$0.23 & 0.9 &  & 4807 & 4.49 & $+$0.23 & 0.9 &  & 4897 & 4.61 & $+$0.24 & 4.1 & $-$26.2\\ 
K00306 & 5347 & 4.66 & $+$0.18 & 2.6 &  & 5338 & 4.66 & $+$0.18 & 2.6 &  & 5356 & 4.65 & $+$0.18 & 4.7 & $-$21.5\\ 
K00307 & 6009 & 4.45 & $-$0.09 & 5.4 &  & 6029 & 4.41 & $-$0.08 & 5.4 &  & 5990 & 4.50 & $-$0.09 & 6.7 & $+$19.6\\ 
K00308 & 6237 & 4.37 & $+$0.02 & 10.0 &  & 6254 & 4.41 & $+$0.03 & 10.0 &  & 6219 & 4.33 & $+$0.01 & 10.9 & $-$36.2\\ 
K00312 & 6248 & 4.27 & $+$0.07 & 9.6 &  & 6242 & 4.26 & $+$0.07 & 9.6 &  & 6253 & 4.29 & $+$0.07 & 10.4 & $-$38.8\\ 
K00313 & 5237 & 4.49 & $+$0.05 & 0.1 &  & 5224 & 4.53 & $+$0.04 & 0.1 &  & 5250 & 4.46 & $+$0.05 & 3.6 & $-$29.2\\ 
K00315 & 4816 & 4.61 & $-$0.22 & 1.8 &  & 4793 & 4.68 & $-$0.21 & 1.8 &  & 4840 & 4.54 & $-$0.22 & 4.1 & $+$17.7\\ 
K00316 & 5631 & 4.28 & $+$0.35 & 1.4 &  & 5649 & 4.26 & $+$0.38 & 1.4 &  & 5612 & 4.31 & $+$0.32 & 4.2 & $-$27.9\\ 
K00317 & 6563 & 4.24 & $+$0.06 & 15.9 &  & 6558 & 4.32 & $+$0.07 & 15.9 &  & 6568 & 4.15 & $+$0.05 & 17.2 & $+$11.0\\ 
K00318 & 6338 & 4.17 & $+$0.26 & 13.5 &  & 6342 & 4.16 & $+$0.26 & 13.5 &  & 6335 & 4.18 & $+$0.25 & 14.5 & $-$1.9\\ 
K00319 & 5956 & 3.98 & $+$0.17 & 5.3 &  & 5922 & 3.95 & $+$0.15 & 5.3 &  & 5990 & 4.01 & $+$0.20 & 6.6 & $-$8.6\\ 
K00321 & 5656 & 4.32 & $+$0.28 & 0.3 &  & 5659 & 4.26 & $+$0.28 & 0.3 &  & 5654 & 4.38 & $+$0.27 & 4.3 & $-$58.4\\ 
K00323 & 5529 & 4.72 & $+$0.10 & 4.7 &  & 5458 & 4.72 & $+$0.06 & 4.7 &  & 5599 & 4.72 & $+$0.15 & 5.9 & $+$10.8\\ 
K00327 & 6024 & 4.32 & $-$0.03 & 4.4 &  & 6025 & 4.28 & $-$0.03 & 4.4 &  & 6023 & 4.36 & $-$0.02 & 5.8 & $-$27.8\\ 
K00328 & 5766 & 4.48 & $-$0.09 & 2.3 &  & 5766 & 4.48 & $-$0.09 & 2.3 &  & \nodata & \nodata & \nodata & \nodata & $-$30.5\\ 
K00330 & 5838 & 4.09 & $+$0.01 & 3.4 &  & 5856 & 4.06 & $+$0.02 & 3.4 &  & 5820 & 4.12 & $-$0.00 & 5.1 & $-$43.0\\ 
K00331 & 5506 & 3.90 & $+$0.11 & 2.4 &  & 5512 & 3.93 & $+$0.11 & 2.4 &  & 5500 & 3.87 & $+$0.11 & 4.5 & $-$25.8\\ 
K00332 & 5799 & 4.16 & $+$0.38 & 2.9 &  & 5794 & 4.09 & $+$0.38 & 2.9 &  & 5803 & 4.23 & $+$0.39 & 4.8 & $-$60.5\\ 
K00333 & 6209 & 4.42 & $+$0.11 & 8.3 &  & 6197 & 4.39 & $+$0.09 & 8.3 &  & 6220 & 4.45 & $+$0.13 & 9.3 & $+$8.9\\ 
K00337 & 5724 & 4.25 & $+$0.07 & 1.9 &  & 5755 & 4.27 & $+$0.09 & 1.9 &  & 5692 & 4.23 & $+$0.06 & 4.6 & $-$60.7\\ 
K00338 & 5019 & 4.54 & $+$0.33 & 1.9 &  & 4996 & 4.47 & $+$0.34 & 1.9 &  & 5043 & 4.61 & $+$0.33 & 4.2 & $-$19.3\\ 
K00339 & 5966 & 4.45 & $-$0.17 & 4.9 &  & 5983 & 4.51 & $-$0.19 & 4.9 &  & 5949 & 4.39 & $-$0.15 & 6.4 & $-$13.7\\ 
K00340 & 5701 & 4.08 & $+$0.35 & 7.1 &  & 5688 & 4.08 & $+$0.35 & 7.1 &  & 5714 & 4.08 & $+$0.35 & 8.0 & $-$93.2\\ 
K00341 & 5567 & 4.57 & $+$0.18 & 1.9 &  & 5549 & 4.55 & $+$0.17 & 1.9 &  & 5585 & 4.58 & $+$0.19 & 4.2 & $-$28.5\\ 
K00343 & 5759 & 4.31 & $+$0.05 & 2.1 &  & 5755 & 4.27 & $+$0.04 & 2.1 &  & 5763 & 4.36 & $+$0.05 & 4.2 & $-$47.6\\ 
K00344 & 5600 & 4.54 & $-$0.18 & 0.0 &  & 5608 & 4.57 & $-$0.20 & 0.0 &  & 5593 & 4.52 & $-$0.16 & 3.7 & $+$11.5\\ 
K00345 & 4935 & 4.62 & $+$0.05 & 0.9 &  & 4909 & 4.61 & $+$0.06 & 0.9 &  & 4960 & 4.63 & $+$0.04 & 3.5 & $-$23.4\\ 
K00346 & 5120 & 4.68 & $+$0.10 & 2.4 &  & 5083 & 4.67 & $+$0.08 & 2.4 &  & 5157 & 4.68 & $+$0.11 & 4.3 & $+$12.4\\ 
K00348 & 4790 & 4.55 & $+$0.07 & 2.6 &  & 4731 & 4.53 & $+$0.08 & 2.6 &  & 4850 & 4.56 & $+$0.06 & 4.4 & $+$0.9\\ 
K00349 & 5752 & 4.23 & $+$0.34 & 4.2 &  & 5728 & 4.21 & $+$0.33 & 4.2 &  & 5776 & 4.25 & $+$0.35 & 5.6 & $+$3.1\\ 
K00350 & 5785 & 4.45 & $+$0.06 & 1.4 &  & 5792 & 4.44 & $+$0.06 & 1.4 &  & 5778 & 4.47 & $+$0.06 & 4.0 & $-$29.3\\ 
K00351 & 6015 & 4.26 & $+$0.10 & 3.7 &  & 5967 & 4.22 & $+$0.08 & 3.7 &  & 6064 & 4.31 & $+$0.12 & 5.5 & $-$17.4\\ 
K00352 & 5802 & 4.18 & $-$0.01 & 2.4 &  & 5812 & 4.15 & $-$0.02 & 2.4 &  & 5792 & 4.21 & $-$0.01 & 4.6 & $-$32.2\\ 
K00355 & 6128 & 4.31 & $+$0.20 & 4.9 &  & 6114 & 4.24 & $+$0.20 & 4.9 &  & 6141 & 4.37 & $+$0.21 & 6.3 & $+$9.8\\ 
K00356 & 5485 & 4.48 & $+$0.03 & 1.6 &  & 5462 & 4.46 & $+$0.03 & 1.6 &  & 5508 & 4.50 & $+$0.03 & 4.0 & $-$13.1\\ 
K00360 & 5991 & 4.30 & $-$0.09 & 2.9 &  & 6016 & 4.28 & $-$0.10 & 2.9 &  & 5966 & 4.31 & $-$0.09 & 4.9 & $-$22.1\\ 
K00361 & 5697 & 4.43 & $+$0.14 & 0.7 &  & 5699 & 4.43 & $+$0.15 & 0.7 &  & 5695 & 4.43 & $+$0.14 & 3.6 & $-$14.7\\ 
K00364 & 5808 & 4.10 & $+$0.27 & 0.7 &  & 5786 & 4.05 & $+$0.25 & 0.7 &  & 5829 & 4.14 & $+$0.28 & 4.7 & $+$3.3\\ 
K00365 & 5498 & 4.49 & $-$0.08 & 0.0 &  & 5488 & 4.50 & $-$0.10 & 0.0 &  & 5508 & 4.48 & $-$0.06 & 4.0 & $-$37.4\\ 
K00367 & 5731 & 4.37 & $+$0.19 & 2.8 &  & 5742 & 4.37 & $+$0.19 & 2.8 &  & 5721 & 4.38 & $+$0.18 & 4.6 & $-$39.5\\ 
K00369 & 6182 & 4.33 & $-$0.13 & 6.8 &  & 6225 & 4.37 & $-$0.12 & 6.8 &  & 6140 & 4.28 & $-$0.14 & 8.0 & $-$1.8\\ 
K00370 & 6110 & 4.04 & $+$0.06 & 6.7 &  & 6080 & 4.07 & $+$0.06 & 6.7 &  & 6140 & 4.01 & $+$0.06 & 7.6 & $-$26.0\\ 
K00371 & 5183 & 3.68 & $+$0.14 & 2.3 &  & 5182 & 3.69 & $+$0.14 & 2.3 &  & 5183 & 3.67 & $+$0.14 & 4.5 & $-$59.0\\ 
K00372 & 5816 & 4.60 & $-$0.02 & 3.0 &  & 5772 & 4.54 & $-$0.04 & 3.0 &  & 5859 & 4.66 & $+$0.00 & 5.1 & $+$10.6\\ 
K00373 & 5738 & 4.47 & $-$0.33 & 1.3 &  & 5793 & 4.52 & $-$0.33 & 1.3 &  & 5683 & 4.42 & $-$0.32 & 4.3 & $+$4.9\\ 
K00374 & 5842 & 4.35 & $-$0.18 & 0.5 &  & 5873 & 4.31 & $-$0.18 & 0.5 &  & 5812 & 4.39 & $-$0.18 & 3.9 & $+$5.9\\ 
K00375 & 5804 & 4.03 & $+$0.22 & 2.7 &  & 5772 & 3.99 & $+$0.20 & 2.7 &  & 5837 & 4.07 & $+$0.23 & 4.6 & $-$20.6\\ 
K00377 & 5788 & 4.47 & $+$0.08 & 1.1 &  & 5788 & 4.47 & $+$0.08 & 1.1 &  & \nodata & \nodata & \nodata & \nodata & $+$2.2\\ 
K00379 & 6176 & 4.06 & $+$0.17 & 7.5 &  & 6135 & 3.98 & $+$0.18 & 7.5 &  & 6216 & 4.13 & $+$0.16 & 8.2 & $-$20.2\\ 
K00384 & 6178 & 4.01 & $+$0.03 & 5.7 &  & 6134 & 3.97 & $+$0.02 & 5.7 &  & 6223 & 4.05 & $+$0.05 & 6.9 & $-$16.4\\ 
K00385 & 5475 & 4.47 & $+$0.12 & 0.4 &  & 5481 & 4.46 & $+$0.12 & 0.4 &  & 5470 & 4.47 & $+$0.12 & 3.7 & $-$20.4\\ 
K00386 & 6001 & 4.41 & $+$0.08 & 3.6 &  & 5982 & 4.40 & $+$0.06 & 3.6 &  & 6019 & 4.42 & $+$0.10 & 5.4 & $+$7.6\\ 
K00387 & 4791 & 4.70 & $-$0.01 & 3.2 &  & 4716 & 4.64 & $-$0.03 & 3.2 &  & 4865 & 4.76 & $+$0.02 & 4.3 & $-$26.4\\ 
K00388 & 5781 & 3.96 & $+$0.12 & 3.9 &  & 5765 & 3.93 & $+$0.12 & 3.9 &  & 5798 & 3.99 & $+$0.12 & 5.3 & $-$22.8\\ 
K00392 & 5943 & 4.09 & $+$0.10 & 4.1 &  & 5899 & 4.06 & $+$0.08 & 4.1 &  & 5988 & 4.11 & $+$0.12 & 5.6 & $-$1.9\\ 
K00393 & 6241 & 4.29 & $-$0.20 & 8.0 &  & 6280 & 4.33 & $-$0.18 & 8.0 &  & 6201 & 4.24 & $-$0.21 & 9.1 & $-$19.3\\ 
K00399 & 6142 & 4.49 & $+$0.01 & 6.4 &  & 6142 & 4.49 & $+$0.01 & 6.4 &  & \nodata & \nodata & \nodata & \nodata & $-$8.3\\ 
K00401 & 5455 & 4.42 & $+$0.35 & 1.2 &  & 5464 & 4.38 & $+$0.36 & 1.2 &  & 5446 & 4.45 & $+$0.34 & 4.0 & $-$6.3\\ 
K00403 & 6223 & 4.21 & $+$0.04 & 10.1 &  & 6228 & 4.23 & $+$0.04 & 10.1 &  & 6218 & 4.19 & $+$0.04 & 11.2 & $-$25.5\\ 
K00408 & 5588 & 4.58 & $+$0.12 & 1.8 &  & 5594 & 4.59 & $+$0.11 & 1.8 &  & 5583 & 4.57 & $+$0.12 & 4.4 & $-$16.1\\ 
K00409 & 5845 & 4.38 & $+$0.18 & 1.7 &  & 5858 & 4.34 & $+$0.18 & 1.7 &  & 5832 & 4.43 & $+$0.17 & 4.5 & $+$0.6\\ 
K00415 & 5656 & 4.23 & $-$0.20 & 1.0 &  & 5688 & 4.18 & $-$0.20 & 1.0 &  & 5623 & 4.28 & $-$0.19 & 4.4 & $-$1.6\\ 
K00416 & 5065 & 4.61 & $-$0.12 & 1.7 &  & 5065 & 4.61 & $-$0.12 & 1.7 &  & \nodata & \nodata & \nodata & \nodata & $-$4.4\\ 
K00427 & 5333 & 4.58 & $+$0.14 & 1.3 &  & 5333 & 4.58 & $+$0.14 & 1.3 &  & \nodata & \nodata & \nodata & \nodata & $+$4.0\\ 
K00431 & 5178 & 4.74 & $-$0.27 & 0.3 &  & 5178 & 4.74 & $-$0.27 & 0.3 &  & \nodata & \nodata & \nodata & \nodata & $+$19.1\\ 
K00433 & 5182 & 4.39 & $+$0.18 & 2.4 &  & 5182 & 4.39 & $+$0.18 & 2.4 &  & \nodata & \nodata & \nodata & \nodata & $-$15.0\\ 
K00435 & 5666 & 4.35 & $+$0.02 & 1.1 &  & 5693 & 4.34 & $+$0.00 & 1.1 &  & 5639 & 4.35 & $+$0.04 & 4.6 & $-$8.7\\ 
K00439 & 5458 & 4.37 & $+$0.34 & 1.7 &  & 5467 & 4.33 & $+$0.35 & 1.7 &  & 5449 & 4.40 & $+$0.33 & 4.4 & $-$76.4\\ 
K00440 & 5078 & 4.53 & $+$0.17 & 2.6 &  & 5074 & 4.54 & $+$0.18 & 2.6 &  & 5082 & 4.53 & $+$0.16 & 4.6 & $-$25.6\\ 
K00442 & 5791 & 4.34 & $-$0.04 & 1.5 &  & 5811 & 4.32 & $-$0.03 & 1.5 &  & 5771 & 4.37 & $-$0.05 & 4.1 & $-$39.7\\ 
K00444 & 5641 & 4.43 & $-$0.07 & 0.8 &  & 5627 & 4.43 & $-$0.09 & 0.8 &  & 5655 & 4.42 & $-$0.04 & 4.0 & $-$20.3\\ 
K00446 & 4618 & 4.68 & $-$0.30 & 2.6 &  & 4618 & 4.68 & $-$0.30 & 2.6 &  & \nodata & \nodata & \nodata & \nodata & $-$20.3\\ 
K00448 & 4653 & 4.70 & $-$0.04 & 4.4 &  & 4653 & 4.70 & $-$0.04 & 4.4 &  & \nodata & \nodata & \nodata & \nodata & $-$1.1\\ 
K00456 & 5616 & 4.34 & $+$0.20 & 1.3 &  & 5616 & 4.34 & $+$0.20 & 1.3 &  & \nodata & \nodata & \nodata & \nodata & $-$23.1\\ 
K00457 & 5108 & 4.54 & $+$0.24 & 2.4 &  & 5107 & 4.55 & $+$0.25 & 2.4 &  & 5108 & 4.54 & $+$0.23 & 4.4 & $-$34.4\\ 
K00459 & 5870 & 4.28 & $+$0.11 & 3.0 &  & 5870 & 4.28 & $+$0.11 & 3.0 &  & \nodata & \nodata & \nodata & \nodata & $-$11.1\\ 
K00464 & 5479 & 4.48 & $+$0.26 & 1.6 &  & 5479 & 4.48 & $+$0.26 & 1.6 &  & \nodata & \nodata & \nodata & \nodata & $-$18.5\\ 
K00465 & 5967 & 4.10 & $-$0.01 & 3.9 &  & 6019 & 4.19 & $-$0.01 & 3.9 &  & 5915 & 4.01 & $-$0.01 & 6.1 & $-$25.8\\ 
K00466 & 5957 & 4.19 & $+$0.03 & 6.0 &  & 5957 & 4.19 & $+$0.03 & 6.0 &  & \nodata & \nodata & \nodata & \nodata & $-$64.1\\ 
K00474 & 5923 & 4.40 & $+$0.00 & 3.3 &  & 5977 & 4.42 & $+$0.02 & 3.3 &  & 5869 & 4.37 & $-$0.02 & 5.2 & $+$10.9\\ 
K00475 & 5100 & 4.74 & $-$0.25 & 1.3 &  & 5100 & 4.74 & $-$0.25 & 1.3 &  & \nodata & \nodata & \nodata & \nodata & $+$0.0\\ 
K00479 & 5560 & 4.42 & $-$0.06 & 0.7 &  & 5558 & 4.44 & $-$0.07 & 0.7 &  & 5563 & 4.41 & $-$0.06 & 3.9 & $-$51.2\\ 
K00481 & 5175 & 4.60 & $-$0.08 & 0.5 &  & 5175 & 4.60 & $-$0.08 & 0.5 &  & \nodata & \nodata & \nodata & \nodata & $-$29.7\\ 
K00486 & 5624 & 4.36 & $-$0.30 & 0.6 &  & 5653 & 4.34 & $-$0.30 & 0.6 &  & 5595 & 4.37 & $-$0.29 & 4.0 & $-$28.1\\ 
K00490 & 4868 & 4.57 & $+$0.03 & 2.1 &  & 4828 & 4.56 & $+$0.02 & 2.1 &  & 4908 & 4.58 & $+$0.05 & 4.3 & $-$29.7\\ 
K00500 & 4665 & 4.59 & $+$0.06 & 3.5 &  & 4631 & 4.54 & $+$0.06 & 3.5 &  & 4699 & 4.63 & $+$0.05 & 4.8 & $-$5.9\\ 
K00505 & 5046 & 4.60 & $+$0.17 & 2.7 &  & 5030 & 4.59 & $+$0.17 & 2.7 &  & 5062 & 4.61 & $+$0.17 & 4.5 & $-$40.8\\ 
K00508 & 5573 & 4.29 & $+$0.38 & 1.8 &  & 5573 & 4.29 & $+$0.38 & 1.8 &  & \nodata & \nodata & \nodata & \nodata & $-$39.0\\ 
K00509 & 5529 & 4.51 & $+$0.17 & 1.5 &  & 5529 & 4.51 & $+$0.17 & 1.5 &  & \nodata & \nodata & \nodata & \nodata & $-$50.8\\ 
K00510 & 5613 & 4.34 & $+$0.39 & 2.2 &  & 5603 & 4.30 & $+$0.40 & 2.2 &  & 5624 & 4.37 & $+$0.37 & 4.6 & $-$12.4\\ 
K00511 & 5941 & 4.43 & $+$0.07 & 3.6 &  & 5941 & 4.43 & $+$0.07 & 3.6 &  & \nodata & \nodata & \nodata & \nodata & $+$14.9\\ 
K00517 & 5542 & 4.55 & $+$0.26 & 2.8 &  & 5549 & 4.55 & $+$0.27 & 2.8 &  & 5536 & 4.55 & $+$0.26 & 4.8 & $-$13.9\\ 
K00518 & 4693 & 4.53 & $-$0.56 & 2.1 &  & 4693 & 4.53 & $-$0.56 & 2.1 &  & \nodata & \nodata & \nodata & \nodata & $-$98.4\\ 
K00519 & 5735 & 4.21 & $+$0.04 & 2.3 &  & 5735 & 4.21 & $+$0.04 & 2.3 &  & \nodata & \nodata & \nodata & \nodata & $-$28.5\\ 
K00520 & 5106 & 4.58 & $+$0.13 & 1.4 &  & 5106 & 4.58 & $+$0.13 & 1.4 &  & \nodata & \nodata & \nodata & \nodata & $-$4.3\\ 
K00523 & 5732 & 4.11 & $-$0.11 & 1.7 &  & 5732 & 4.11 & $-$0.11 & 1.7 &  & \nodata & \nodata & \nodata & \nodata & $-$115.0\\ 
K00528 & 5386 & 4.50 & $-$0.04 & 0.8 &  & 5386 & 4.50 & $-$0.04 & 0.8 &  & \nodata & \nodata & \nodata & \nodata & $-$29.6\\ 
K00534 & 5257 & 4.50 & $+$0.12 & 1.8 &  & 5257 & 4.50 & $+$0.12 & 1.8 &  & \nodata & \nodata & \nodata & \nodata & $-$33.5\\ 
K00543 & 5120 & 4.54 & $-$0.05 & 2.0 &  & 5120 & 4.54 & $-$0.05 & 2.0 &  & \nodata & \nodata & \nodata & \nodata & $-$42.7\\ 
K00546 & 5960 & 4.21 & $+$0.11 & 3.6 &  & 5960 & 4.21 & $+$0.11 & 3.6 &  & \nodata & \nodata & \nodata & \nodata & $-$46.8\\ 
K00548 & 5984 & 4.26 & $-$0.06 & 3.0 &  & 5996 & 4.23 & $-$0.06 & 3.0 &  & 5971 & 4.30 & $-$0.05 & 5.2 & $-$33.5\\ 
K00550 & 5695 & 4.45 & $+$0.16 & 1.7 &  & 5711 & 4.47 & $+$0.17 & 1.7 &  & 5679 & 4.44 & $+$0.14 & 4.3 & $-$23.7\\ 
K00551 & 5686 & 4.37 & $+$0.11 & 1.6 &  & 5686 & 4.37 & $+$0.11 & 1.6 &  & \nodata & \nodata & \nodata & \nodata & $-$38.2\\ 
K00555 & 5274 & 4.46 & $+$0.07 & 1.0 &  & 5293 & 4.49 & $+$0.10 & 1.0 &  & 5255 & 4.43 & $+$0.05 & 4.0 & $-$36.1\\ 
K00561 & 5048 & 4.50 & $-$0.15 & 0.6 &  & 5034 & 4.53 & $-$0.15 & 0.6 &  & 5062 & 4.47 & $-$0.15 & 3.8 & $-$28.7\\ 
K00564 & 5855 & 4.01 & $+$0.34 & 4.6 &  & 5855 & 4.01 & $+$0.34 & 4.6 &  & \nodata & \nodata & \nodata & \nodata & $-$20.3\\ 
K00567 & 5530 & 4.60 & $-$0.15 & 0.4 &  & 5530 & 4.60 & $-$0.15 & 0.4 &  & \nodata & \nodata & \nodata & \nodata & $-$45.9\\ 
K00568 & 5350 & 4.49 & $+$0.05 & 1.3 &  & 5324 & 4.47 & $+$0.05 & 1.3 &  & 5375 & 4.51 & $+$0.06 & 4.0 & $-$10.0\\ 
K00569 & 5037 & 4.69 & $-$0.14 & 1.2 &  & 5037 & 4.69 & $-$0.14 & 1.2 &  & \nodata & \nodata & \nodata & \nodata & $-$47.9\\ 
K00572 & 5997 & 4.15 & $-$0.04 & 4.3 &  & 5996 & 4.15 & $-$0.06 & 4.3 &  & 5997 & 4.15 & $-$0.02 & 6.0 & $+$6.6\\ 
K00573 & 5707 & 4.37 & $+$0.15 & 2.1 &  & 5707 & 4.37 & $+$0.15 & 2.1 &  & \nodata & \nodata & \nodata & \nodata & $-$8.3\\ 
K00574 & 5045 & 4.58 & $-$0.04 & 1.8 &  & 5045 & 4.58 & $-$0.04 & 1.8 &  & \nodata & \nodata & \nodata & \nodata & $-$8.8\\ 
K00577 & 5079 & 4.52 & $+$0.12 & 1.4 &  & 5079 & 4.52 & $+$0.12 & 1.4 &  & \nodata & \nodata & \nodata & \nodata & $-$221.6\\ 
K00579 & 5138 & 4.64 & $+$0.06 & 1.7 &  & 5133 & 4.66 & $+$0.06 & 1.7 &  & 5144 & 4.62 & $+$0.06 & 4.2 & $-$42.1\\ 
K00582 & 5191 & 4.69 & $+$0.13 & 1.8 &  & 5191 & 4.69 & $+$0.13 & 1.8 &  & \nodata & \nodata & \nodata & \nodata & $+$6.7\\ 
K00584 & 5527 & 4.36 & $+$0.31 & 1.3 &  & 5520 & 4.34 & $+$0.31 & 1.3 &  & 5535 & 4.38 & $+$0.31 & 4.3 & $-$10.2\\ 
K00590 & 5975 & 4.42 & $-$0.00 & 3.7 &  & 5975 & 4.42 & $-$0.00 & 3.7 &  & \nodata & \nodata & \nodata & \nodata & $-$12.0\\ 
K00597 & 5710 & 4.31 & $-$0.03 & 0.9 &  & 5710 & 4.31 & $-$0.03 & 0.9 &  & \nodata & \nodata & \nodata & \nodata & $-$20.8\\ 
K00598 & 5232 & 4.64 & $+$0.04 & 0.4 &  & 5232 & 4.64 & $+$0.04 & 0.4 &  & \nodata & \nodata & \nodata & \nodata & $-$20.7\\ 
K00600 & 5742 & 4.28 & $-$0.04 & 1.0 &  & 5742 & 4.28 & $-$0.04 & 1.0 &  & \nodata & \nodata & \nodata & \nodata & $-$28.9\\ 
K00601 & 5816 & 4.60 & $+$0.08 & 4.2 &  & 5816 & 4.60 & $+$0.08 & 4.2 &  & \nodata & \nodata & \nodata & \nodata & $+$3.6\\ 
K00611 & 6350 & 4.35 & $+$0.11 & 12.4 &  & 6420 & 4.39 & $+$0.14 & 12.4 &  & 6280 & 4.31 & $+$0.08 & 13.2 & $-$15.5\\ 
K00612 & 5146 & 4.55 & $+$0.03 & 1.7 &  & 5132 & 4.57 & $+$0.02 & 1.7 &  & 5160 & 4.52 & $+$0.04 & 4.3 & $+$23.2\\ 
K00620 & 5674 & 4.70 & $+$0.05 & 5.5 &  & 5674 & 4.70 & $+$0.05 & 5.5 &  & \nodata & \nodata & \nodata & \nodata & $-$4.3\\ 
K00623 & 5945 & 4.32 & $-$0.40 & 0.6 &  & 5966 & 4.37 & $-$0.43 & 0.6 &  & 5924 & 4.27 & $-$0.38 & 4.3 & $+$3.3\\ 
K00624 & 5681 & 4.61 & $+$0.13 & 3.1 &  & 5660 & 4.59 & $+$0.12 & 3.1 &  & 5702 & 4.63 & $+$0.15 & 4.7 & $-$25.0\\ 
K00626 & 6070 & 4.28 & $-$0.18 & 4.0 &  & 6129 & 4.32 & $-$0.17 & 4.0 &  & 6011 & 4.24 & $-$0.20 & 5.5 & $-$16.5\\ 
K00627 & 6042 & 4.19 & $+$0.17 & 5.4 &  & 6028 & 4.16 & $+$0.18 & 5.4 &  & 6056 & 4.22 & $+$0.17 & 6.5 & $+$8.2\\ 
K00628 & 5721 & 4.49 & $-$0.31 & 0.6 &  & 5765 & 4.52 & $-$0.32 & 0.6 &  & 5677 & 4.46 & $-$0.30 & 4.3 & $+$36.3\\ 
K00629 & 6006 & 4.24 & $-$0.27 & 2.7 &  & 6031 & 4.29 & $-$0.30 & 2.7 &  & 5980 & 4.19 & $-$0.24 & 5.2 & $+$8.4\\ 
K00632 & 5406 & 4.61 & $+$0.12 & 0.6 &  & 5402 & 4.61 & $+$0.12 & 0.6 &  & 5410 & 4.60 & $+$0.13 & 3.8 & $-$50.1\\ 
K00633 & 5755 & 4.17 & $-$0.16 & 1.9 &  & 5758 & 4.12 & $-$0.17 & 1.9 &  & 5752 & 4.23 & $-$0.14 & 4.4 & $-$39.0\\ 
K00635 & 6087 & 4.43 & $+$0.05 & 6.0 &  & 6114 & 4.46 & $+$0.04 & 6.0 &  & 6061 & 4.39 & $+$0.05 & 7.3 & $-$37.9\\ 
K00638 & 5721 & 4.50 & $-$0.00 & 1.4 &  & 5733 & 4.52 & $-$0.01 & 1.4 &  & 5709 & 4.48 & $+$0.00 & 4.2 & $+$14.0\\ 
K00639 & 6158 & 4.34 & $+$0.04 & 7.4 &  & 6179 & 4.34 & $+$0.05 & 7.4 &  & 6137 & 4.35 & $+$0.04 & 8.3 & $-$22.5\\ 
K00640 & 5274 & 4.49 & $+$0.14 & 0.9 &  & 5285 & 4.48 & $+$0.15 & 0.9 &  & 5263 & 4.50 & $+$0.13 & 3.9 & $-$23.6\\ 
K00644 & 5685 & 4.16 & $-$0.10 & 1.6 &  & 5721 & 4.24 & $-$0.09 & 1.6 &  & 5648 & 4.07 & $-$0.10 & 4.7 & $-$73.5\\ 
K00645 & 5856 & 4.15 & $-$0.18 & 2.3 &  & 5843 & 4.16 & $-$0.21 & 2.3 &  & 5869 & 4.15 & $-$0.14 & 4.9 & $+$4.3\\ 
K00647 & 6109 & 4.32 & $-$0.37 & 2.6 &  & 6150 & 4.34 & $-$0.36 & 2.6 &  & 6068 & 4.30 & $-$0.39 & 5.0 & $-$53.4\\ 
K00649 & 6282 & 4.07 & $+$0.22 & 7.8 &  & 6230 & 4.09 & $+$0.22 & 7.8 &  & 6333 & 4.05 & $+$0.22 & 8.8 & $-$13.7\\ 
K00650 & 5058 & 4.53 & $+$0.05 & 0.8 &  & 5050 & 4.54 & $+$0.06 & 0.8 &  & 5067 & 4.51 & $+$0.03 & 3.7 & $-$21.8\\ 
K00654 & 5785 & 4.48 & $-$0.03 & 1.3 &  & 5823 & 4.51 & $-$0.01 & 1.3 &  & 5747 & 4.44 & $-$0.05 & 4.3 & $-$38.9\\ 
K00655 & 6152 & 4.22 & $-$0.03 & 2.7 &  & 6148 & 4.20 & $-$0.04 & 2.7 &  & 6156 & 4.24 & $-$0.02 & 4.6 & $+$9.5\\ 
K00657 & 4762 & 4.58 & $-$0.21 & 1.6 &  & 4705 & 4.63 & $-$0.21 & 1.6 &  & 4819 & 4.53 & $-$0.20 & 3.9 & $-$7.9\\ 
K00658 & 5887 & 4.41 & $+$0.08 & 2.8 &  & 5897 & 4.42 & $+$0.08 & 2.8 &  & 5876 & 4.40 & $+$0.08 & 5.0 & $-$34.7\\ 
K00659 & 6281 & 4.37 & $-$0.05 & 8.8 &  & 6344 & 4.43 & $-$0.04 & 8.8 &  & 6218 & 4.31 & $-$0.06 & 10.1 & $-$39.2\\ 
K00660 & 5319 & 3.89 & $-$0.07 & 1.7 &  & 5305 & 3.85 & $-$0.08 & 1.7 &  & 5334 & 3.92 & $-$0.06 & 4.2 & $-$56.7\\ 
K00661 & 5877 & 4.43 & $+$0.07 & 2.6 &  & 5898 & 4.43 & $+$0.07 & 2.6 &  & 5857 & 4.43 & $+$0.06 & 4.8 & $+$20.9\\ 
K00662 & 5834 & 4.05 & $-$0.02 & 2.0 &  & 5777 & 3.97 & $-$0.04 & 2.0 &  & 5891 & 4.14 & $+$0.01 & 3.9 & $-$18.0\\ 
K00664 & 5691 & 4.29 & $+$0.06 & 0.7 &  & 5722 & 4.29 & $+$0.06 & 0.7 &  & 5660 & 4.30 & $+$0.05 & 4.0 & $-$11.3\\ 
K00665 & 5969 & 4.09 & $+$0.29 & 5.3 &  & 5973 & 4.07 & $+$0.30 & 5.3 &  & 5966 & 4.11 & $+$0.29 & 6.4 & $-$47.6\\ 
K00666 & 5600 & 4.40 & $+$0.14 & 1.8 &  & 5627 & 4.41 & $+$0.15 & 1.8 &  & 5573 & 4.39 & $+$0.14 & 4.3 & $-$41.1\\ 
K00670 & 5605 & 4.00 & $+$0.17 & 2.3 &  & 5624 & 3.99 & $+$0.19 & 2.3 &  & 5586 & 4.02 & $+$0.16 & 4.5 & $-$69.3\\ 
K00671 & 6054 & 4.24 & $+$0.02 & 5.1 &  & 6058 & 4.21 & $+$0.01 & 5.1 &  & 6049 & 4.26 & $+$0.03 & 6.5 & $-$5.8\\ 
K00672 & 5564 & 4.48 & $+$0.14 & 0.6 &  & 5567 & 4.47 & $+$0.13 & 0.6 &  & 5561 & 4.50 & $+$0.15 & 4.2 & $-$10.7\\ 
K00673 & 6380 & 4.47 & $+$0.04 & 12.7 &  & 6472 & 4.52 & $+$0.10 & 12.7 &  & 6289 & 4.41 & $-$0.02 & 13.5 & $-$28.0\\ 
K00674 & 4933 & 3.66 & $+$0.25 & 3.1 &  & 4920 & 3.59 & $+$0.25 & 3.1 &  & 4946 & 3.73 & $+$0.24 & 4.6 & $-$50.4\\ 
K00678 & 5193 & 4.63 & $+$0.18 & 2.8 &  & 5190 & 4.63 & $+$0.19 & 2.8 &  & 5197 & 4.63 & $+$0.18 & 4.4 & $-$26.9\\ 
K00679 & 5880 & 4.14 & $+$0.22 & 3.8 &  & 5863 & 4.10 & $+$0.21 & 3.8 &  & 5896 & 4.19 & $+$0.23 & 5.5 & $-$146.3\\ 
K00680 & 6238 & 4.05 & $+$0.05 & 6.4 &  & 6178 & 4.02 & $+$0.03 & 6.4 &  & 6298 & 4.08 & $+$0.07 & 7.5 & $-$26.1\\ 
K00682 & 5620 & 4.30 & $+$0.34 & 2.0 &  & 5663 & 4.31 & $+$0.36 & 2.0 &  & 5578 & 4.30 & $+$0.31 & 4.6 & $-$69.3\\ 
K00683 & 5869 & 4.32 & $+$0.15 & 1.4 &  & 5907 & 4.36 & $+$0.17 & 1.4 &  & 5832 & 4.28 & $+$0.13 & 4.2 & $-$8.7\\ 
K00684 & 5287 & 3.84 & $+$0.10 & 2.7 &  & 5263 & 3.82 & $+$0.10 & 2.7 &  & 5312 & 3.85 & $+$0.11 & 4.6 & $-$79.9\\ 
K00685 & 6540 & 4.26 & $-$0.05 & 14.9 &  & 6605 & 4.39 & $-$0.02 & 14.9 &  & 6475 & 4.13 & $-$0.09 & 15.7 & $-$27.7\\ 
K00686 & 5599 & 4.33 & $+$0.00 & 1.3 &  & 5640 & 4.33 & $+$0.02 & 1.3 &  & 5558 & 4.32 & $-$0.01 & 4.3 & $-$33.3\\ 
K00687 & 5879 & 4.39 & $+$0.08 & 4.5 &  & 5849 & 4.40 & $+$0.06 & 4.5 &  & 5910 & 4.38 & $+$0.11 & 6.1 & $-$44.6\\ 
K00688 & 6192 & 4.28 & $-$0.05 & 8.9 &  & 6188 & 4.25 & $-$0.07 & 8.9 &  & 6195 & 4.31 & $-$0.04 & 10.0 & $+$20.3\\ 
K00689 & 5334 & 4.54 & $-$0.44 & 0.5 &  & 5359 & 4.54 & $-$0.45 & 0.5 &  & 5308 & 4.54 & $-$0.44 & 3.9 & $-$95.0\\ 
K00691 & 5914 & 4.18 & $-$0.30 & 2.5 &  & 5932 & 4.18 & $-$0.31 & 2.5 &  & 5896 & 4.17 & $-$0.29 & 4.8 & $-$29.7\\ 
K00692 & 5658 & 4.28 & $+$0.15 & 2.3 &  & 5665 & 4.25 & $+$0.16 & 2.3 &  & 5651 & 4.30 & $+$0.15 & 4.3 & $-$78.7\\ 
K00693 & 6052 & 4.12 & $-$0.02 & 6.5 &  & 6011 & 4.08 & $-$0.03 & 6.5 &  & 6093 & 4.17 & $-$0.01 & 7.5 & $-$35.5\\ 
K00694 & 5693 & 4.41 & $+$0.23 & 1.6 &  & 5701 & 4.43 & $+$0.23 & 1.6 &  & 5686 & 4.40 & $+$0.22 & 4.4 & $-$19.9\\ 
K00695 & 5694 & 4.47 & $-$0.40 & 0.0 &  & 5725 & 4.49 & $-$0.42 & 0.0 &  & 5663 & 4.45 & $-$0.38 & 3.8 & $-$8.1\\ 
K00697 & 5848 & 4.15 & $+$0.14 & 2.1 &  & 5829 & 4.06 & $+$0.13 & 2.1 &  & 5867 & 4.24 & $+$0.15 & 4.2 & $-$63.5\\ 
K00700 & 5648 & 4.55 & $-$0.43 & 0.6 &  & 5703 & 4.57 & $-$0.44 & 0.6 &  & 5593 & 4.53 & $-$0.43 & 4.1 & $+$17.4\\ 
K00701 & 4859 & 4.59 & $-$0.34 & 0.6 &  & 4851 & 4.66 & $-$0.34 & 0.6 &  & 4867 & 4.52 & $-$0.34 & 4.1 & $+$16.8\\ 
K00703 & 6386 & 4.11 & $+$0.26 & 7.5 &  & 6379 & 4.17 & $+$0.26 & 7.5 &  & 6393 & 4.06 & $+$0.25 & 8.7 & $-$15.9\\ 
K00704 & 5266 & 4.61 & $-$0.08 & 1.8 &  & 5277 & 4.65 & $-$0.07 & 1.8 &  & 5255 & 4.57 & $-$0.08 & 4.3 & $-$29.9\\ 
K00707 & 5947 & 4.05 & $+$0.14 & 4.4 &  & 5930 & 4.05 & $+$0.13 & 4.4 &  & 5964 & 4.06 & $+$0.16 & 5.8 & $+$14.1\\ 
K00708 & 6119 & 4.19 & $-$0.07 & 7.1 &  & 6081 & 4.17 & $-$0.11 & 7.1 &  & 6156 & 4.21 & $-$0.03 & 8.2 & $+$4.9\\ 
K00709 & 5349 & 4.51 & $-$0.14 & 0.3 &  & 5385 & 4.58 & $-$0.13 & 0.3 &  & 5313 & 4.44 & $-$0.15 & 4.0 & $-$36.7\\ 
K00710 & 6554 & 4.17 & $-$0.07 & 15.0 &  & 6533 & 4.26 & $-$0.06 & 15.0 &  & 6576 & 4.08 & $-$0.09 & 15.7 & $-$14.6\\ 
K00711 & 5594 & 4.32 & $+$0.37 & 1.4 &  & 5629 & 4.29 & $+$0.40 & 1.4 &  & 5559 & 4.34 & $+$0.35 & 4.3 & $-$55.4\\ 
K00712 & 5474 & 4.56 & $+$0.02 & 1.4 &  & 5464 & 4.58 & $+$0.02 & 1.4 &  & 5483 & 4.55 & $+$0.02 & 4.0 & $-$46.4\\ 
K00714 & 5393 & 4.58 & $+$0.14 & 0.6 &  & 5373 & 4.56 & $+$0.15 & 0.6 &  & 5413 & 4.61 & $+$0.13 & 3.6 & $-$52.5\\ 
K00717 & 5612 & 4.24 & $+$0.33 & 1.3 &  & 5640 & 4.20 & $+$0.34 & 1.3 &  & 5585 & 4.27 & $+$0.31 & 4.0 & $-$8.1\\ 
K00718 & 5873 & 4.28 & $+$0.36 & 3.5 &  & 5906 & 4.27 & $+$0.37 & 3.5 &  & 5841 & 4.29 & $+$0.34 & 5.5 & $-$16.6\\ 
K00719 & 4665 & 4.58 & $-$0.01 & 3.1 &  & 4665 & 4.58 & $-$0.01 & 3.1 &  & 4048 & 4.48 & $-$0.56 & 4.7 & $+$17.7\\ 
K00720 & 5260 & 4.68 & $+$0.04 & 4.5 &  & 5205 & 4.68 & $+$0.01 & 4.5 &  & 5315 & 4.67 & $+$0.08 & 5.8 & $+$2.8\\ 
K00721 & 5846 & 4.08 & $+$0.13 & 2.0 &  & 5815 & 4.02 & $+$0.12 & 2.0 &  & 5878 & 4.14 & $+$0.13 & 4.1 & $-$49.5\\ 
K00722 & 6145 & 4.36 & $-$0.11 & 5.6 &  & 6173 & 4.37 & $-$0.12 & 5.6 &  & 6117 & 4.34 & $-$0.10 & 7.1 & $-$26.5\\ 
K00723 & 5315 & 4.55 & $+$0.33 & 4.2 &  & 5315 & 4.55 & $+$0.33 & 4.2 &  & \nodata & \nodata & \nodata & \nodata & $-$21.0\\ 
K00730 & 5697 & 3.84 & $+$0.11 & 2.2 &  & 5697 & 3.84 & $+$0.11 & 2.2 &  & \nodata & \nodata & \nodata & \nodata & $-$31.0\\ 
K00732 & 5251 & 4.41 & $+$0.30 & 1.7 &  & 5251 & 4.41 & $+$0.30 & 1.7 &  & \nodata & \nodata & \nodata & \nodata & $-$15.9\\ 
K00733 & 5046 & 4.60 & $-$0.06 & 2.8 &  & 5038 & 4.68 & $-$0.08 & 2.8 &  & 5054 & 4.52 & $-$0.05 & 4.7 & $+$10.8\\ 
K00734 & 5904 & 4.14 & $+$0.24 & 2.6 &  & 5904 & 4.14 & $+$0.24 & 2.6 &  & \nodata & \nodata & \nodata & \nodata & $-$36.9\\ 
K00738 & 5378 & 4.64 & $-$0.44 & 1.1 &  & 5378 & 4.64 & $-$0.44 & 1.1 &  & \nodata & \nodata & \nodata & \nodata & $-$49.5\\ 
K00749 & 5356 & 4.47 & $+$0.09 & 0.6 &  & 5356 & 4.47 & $+$0.09 & 0.6 &  & \nodata & \nodata & \nodata & \nodata & $-$35.8\\ 
K00752 & 5539 & 4.44 & $+$0.10 & 0.8 &  & 5539 & 4.44 & $+$0.10 & 0.8 &  & \nodata & \nodata & \nodata & \nodata & $-$32.1\\ 
K00756 & 5660 & 4.26 & $+$0.18 & 2.6 &  & 5660 & 4.26 & $+$0.18 & 2.6 &  & \nodata & \nodata & \nodata & \nodata & $-$64.4\\ 
K00757 & 5002 & 4.68 & $+$0.06 & 2.1 &  & 5002 & 4.68 & $+$0.06 & 2.1 &  & \nodata & \nodata & \nodata & \nodata & $+$5.1\\ 
K00759 & 5253 & 4.61 & $-$0.21 & 0.6 &  & 5253 & 4.61 & $-$0.21 & 0.6 &  & \nodata & \nodata & \nodata & \nodata & $+$0.9\\ 
K00760 & 5742 & 4.36 & $+$0.10 & 1.2 &  & 5742 & 4.36 & $+$0.10 & 1.2 &  & \nodata & \nodata & \nodata & \nodata & $-$36.2\\ 
K00771 & 5652 & 4.33 & $+$0.17 & 2.5 &  & 5652 & 4.33 & $+$0.17 & 2.5 &  & \nodata & \nodata & \nodata & \nodata & $-$14.3\\ 
K00800 & 5911 & 4.25 & $+$0.22 & 3.5 &  & 5911 & 4.25 & $+$0.22 & 3.5 &  & \nodata & \nodata & \nodata & \nodata & $-$33.6\\ 
K00806 & 5464 & 4.66 & $+$0.16 & 2.3 &  & 5464 & 4.66 & $+$0.16 & 2.3 &  & \nodata & \nodata & \nodata & \nodata & $-$6.9\\ 
K00825 & 4897 & 4.48 & $+$0.22 & 2.0 &  & 4897 & 4.48 & $+$0.22 & 2.0 &  & \nodata & \nodata & \nodata & \nodata & $-$26.8\\ 
K00829 & 5766 & 4.28 & $+$0.00 & 2.4 &  & 5766 & 4.28 & $+$0.00 & 2.4 &  & \nodata & \nodata & \nodata & \nodata & $-$57.1\\ 
K00834 & 5800 & 4.07 & $+$0.34 & 3.0 &  & 5761 & 4.05 & $+$0.33 & 3.0 &  & 5838 & 4.10 & $+$0.35 & 4.9 & $-$14.0\\ 
K00835 & 4939 & 4.57 & $+$0.17 & 1.7 &  & 4939 & 4.57 & $+$0.17 & 1.7 &  & \nodata & \nodata & \nodata & \nodata & $-$20.3\\ 
K00837 & 4918 & 4.38 & $+$0.40 & 2.8 &  & 4918 & 4.38 & $+$0.40 & 2.8 &  & \nodata & \nodata & \nodata & \nodata & $-$40.7\\ 
K00841 & 5264 & 4.65 & $+$0.12 & 2.4 &  & 5264 & 4.65 & $+$0.12 & 2.4 &  & \nodata & \nodata & \nodata & \nodata & $-$85.7\\ 
K00853 & 4876 & 4.73 & $-$0.02 & 3.0 &  & 4876 & 4.73 & $-$0.02 & 3.0 &  & \nodata & \nodata & \nodata & \nodata & $-$16.0\\ 
K00857 & 5149 & 4.51 & $+$0.26 & 2.4 &  & 5149 & 4.51 & $+$0.26 & 2.4 &  & \nodata & \nodata & \nodata & \nodata & $-$47.4\\ 
K00864 & 5498 & 4.53 & $+$0.08 & 1.2 &  & 5498 & 4.53 & $+$0.08 & 1.2 &  & \nodata & \nodata & \nodata & \nodata & $-$5.5\\ 
K00869 & 5105 & 4.67 & $+$0.12 & 3.1 &  & 5096 & 4.68 & $+$0.11 & 3.1 &  & 5114 & 4.66 & $+$0.13 & 4.7 & $-$42.2\\ 
K00870 & 4674 & 4.59 & $+$0.02 & 3.8 &  & 4674 & 4.59 & $+$0.02 & 3.8 &  & 5871 & 2.81 & $-$1.21 & 4.1 & $-$35.5\\ 
K00872 & 5162 & 4.59 & $+$0.17 & 1.3 &  & 5162 & 4.59 & $+$0.17 & 1.3 &  & \nodata & \nodata & \nodata & \nodata & $-$20.2\\ 
K00874 & 5089 & 4.58 & $+$0.20 & 2.4 &  & 5089 & 4.58 & $+$0.20 & 2.4 &  & \nodata & \nodata & \nodata & \nodata & $-$13.9\\ 
K00880 & 5401 & 4.37 & $+$0.20 & 2.4 &  & 5419 & 4.38 & $+$0.21 & 2.4 &  & 5382 & 4.36 & $+$0.19 & 4.7 & $-$44.3\\ 
K00881 & 4927 & 4.09 & $-$0.08 & 1.2 &  & 4927 & 4.09 & $-$0.08 & 1.2 &  & \nodata & \nodata & \nodata & \nodata & $-$21.4\\ 
K00884 & 5060 & 4.48 & $+$0.30 & 1.6 &  & 5060 & 4.48 & $+$0.30 & 1.6 &  & \nodata & \nodata & \nodata & \nodata & $-$56.3\\ 
K00889 & 5305 & 4.49 & $+$0.23 & 3.1 &  & 5339 & 4.50 & $+$0.26 & 3.1 &  & 5272 & 4.47 & $+$0.20 & 4.9 & $-$64.0\\ 
K00892 & 5064 & 4.70 & $-$0.06 & 2.6 &  & 5064 & 4.70 & $-$0.06 & 2.6 &  & \nodata & \nodata & \nodata & \nodata & $+$10.6\\ 
K00896 & 4973 & 3.94 & $+$0.17 & 1.1 &  & 4973 & 3.94 & $+$0.17 & 1.1 &  & \nodata & \nodata & \nodata & \nodata & $-$21.3\\ 
K00906 & 5007 & 4.58 & $+$0.01 & 2.1 &  & 5007 & 4.58 & $+$0.01 & 2.1 &  & \nodata & \nodata & \nodata & \nodata & $-$8.7\\ 
K00907 & 5492 & 4.47 & $-$0.06 & 1.7 &  & 5545 & 4.54 & $-$0.04 & 1.7 &  & 5440 & 4.39 & $-$0.08 & 4.5 & $-$2.7\\ 
K00918 & 5399 & 4.62 & $+$0.13 & 2.2 &  & 5399 & 4.62 & $+$0.13 & 2.2 &  & \nodata & \nodata & \nodata & \nodata & $-$54.0\\ 
K00921 & 5081 & 4.57 & $+$0.15 & 0.6 &  & 5081 & 4.57 & $+$0.15 & 0.6 &  & \nodata & \nodata & \nodata & \nodata & $-$56.1\\ 
K00934 & 5503 & 4.52 & $-$0.13 & 0.4 &  & 5503 & 4.52 & $-$0.13 & 0.4 &  & \nodata & \nodata & \nodata & \nodata & $+$10.7\\ 
K00935 & 6088 & 4.15 & $-$0.09 & 112.1 &  & 6088 & 4.15 & $-$0.09 & 112.1 &  & 5722 & 4.03 & $-$0.26 & 7.9 & $-$171.6\\ 
K00939 & 5607 & 4.32 & $+$0.26 & 1.8 &  & 5665 & 4.34 & $+$0.29 & 1.8 &  & 5550 & 4.29 & $+$0.23 & 4.5 & $-$9.9\\ 
K00941 & 5118 & 4.42 & $+$0.40 & 2.0 &  & 5118 & 4.42 & $+$0.40 & 2.0 &  & \nodata & \nodata & \nodata & \nodata & $-$7.2\\ 
K00954 & 5511 & 4.51 & $-$0.09 & 1.2 &  & 5511 & 4.51 & $-$0.09 & 1.2 &  & \nodata & \nodata & \nodata & \nodata & $-$11.9\\ 
K00958 & 4925 & 4.60 & $-$0.01 & 3.1 &  & 4903 & 4.68 & $+$0.01 & 3.1 &  & 4948 & 4.53 & $-$0.03 & 4.7 & $-$26.8\\ 
K00974 & 6318 & 4.12 & $-$0.05 & 7.8 &  & 6319 & 4.12 & $-$0.04 & 7.8 &  & 6317 & 4.11 & $-$0.06 & 8.5 & $-$20.7\\ 
K00975 & 6203 & 4.08 & $-$0.04 & 7.3 &  & 6174 & 4.07 & $-$0.05 & 7.3 &  & 6231 & 4.09 & $-$0.03 & 8.7 & $-$18.7\\ 
K00981 & 5050 & 3.30 & $-$0.14 & 2.1 &  & 5018 & 3.31 & $-$0.15 & 2.1 &  & 5082 & 3.30 & $-$0.13 & 4.6 & $-$32.8\\ 
K00986 & 5541 & 4.52 & $+$0.29 & 2.1 &  & 5542 & 4.50 & $+$0.29 & 2.1 &  & 5539 & 4.54 & $+$0.28 & 4.5 & $-$25.1\\ 
K00987 & 5509 & 4.59 & $+$0.12 & 0.6 &  & 5490 & 4.56 & $+$0.10 & 0.6 &  & 5528 & 4.62 & $+$0.13 & 3.9 & $-$4.9\\ 
K00988 & 5121 & 4.69 & $+$0.11 & 3.3 &  & 5092 & 4.70 & $+$0.10 & 3.3 &  & 5150 & 4.67 & $+$0.13 & 4.8 & $-$23.5\\ 
K00991 & 5495 & 4.51 & $-$0.14 & 1.6 &  & 5535 & 4.54 & $-$0.14 & 1.6 &  & 5456 & 4.48 & $-$0.15 & 4.3 & $-$1.7\\ 
K00993 & 5549 & 4.60 & $-$0.32 & 0.5 &  & 5549 & 4.60 & $-$0.32 & 0.5 &  & \nodata & \nodata & \nodata & \nodata & $-$26.5\\ 
K00999 & 5113 & 4.71 & $-$0.08 & 2.1 &  & 5113 & 4.71 & $-$0.08 & 2.1 &  & \nodata & \nodata & \nodata & \nodata & $-$39.6\\ 
K01001 & 6284 & 4.10 & $+$0.13 & 9.0 &  & 6254 & 4.10 & $+$0.12 & 9.0 &  & 6314 & 4.09 & $+$0.15 & 9.9 & $-$19.2\\ 
K01002 & 5405 & 4.40 & $+$0.12 & 1.7 &  & 5387 & 4.39 & $+$0.12 & 1.7 &  & 5422 & 4.40 & $+$0.13 & 4.5 & $-$50.0\\ 
K01010 & 6104 & 4.20 & $-$0.06 & 7.5 &  & 6068 & 4.13 & $-$0.07 & 7.5 &  & 6139 & 4.27 & $-$0.06 & 8.2 & $-$38.7\\ 
K01015 & 5948 & 4.15 & $-$0.10 & 4.4 &  & 5948 & 4.15 & $-$0.10 & 4.4 &  & \nodata & \nodata & \nodata & \nodata & $+$10.8\\ 
K01019 & 5018 & 3.55 & $+$0.17 & 2.1 &  & 4968 & 3.49 & $+$0.13 & 2.1 &  & 5068 & 3.61 & $+$0.21 & 4.7 & $-$20.9\\ 
K01032 & 4921 & 3.62 & $+$0.08 & 3.2 &  & 4882 & 3.51 & $+$0.05 & 3.2 &  & 4960 & 3.74 & $+$0.10 & 4.7 & $-$27.4\\ 
K01050 & 5067 & 4.58 & $+$0.08 & 2.1 &  & 5061 & 4.59 & $+$0.09 & 2.1 &  & 5072 & 4.57 & $+$0.08 & 4.4 & $-$44.4\\ 
K01052 & 5871 & 4.39 & $-$0.11 & 1.7 &  & 5922 & 4.38 & $-$0.10 & 1.7 &  & 5819 & 4.40 & $-$0.13 & 4.6 & $-$19.3\\ 
K01054 & 5946 & 3.52 & $-$0.41 & 5.5 &  & 5475 & 3.39 & $-$0.69 & 5.5 &  & 5946 & 3.52 & $-$0.41 & 6.6 & $-$141.5\\ 
K01060 & 6360 & 4.42 & $-$0.21 & 456.7 &  & 6503 & 4.49 & $-$0.15 & 456.7 &  & 6216 & 4.35 & $-$0.28 & 13.3 & $+$0.6\\ 
K01069 & 5239 & 4.46 & $+$0.30 & 1.8 &  & 5239 & 4.46 & $+$0.30 & 1.8 &  & \nodata & \nodata & \nodata & \nodata & $-$36.9\\ 
K01089 & 5848 & 4.37 & $+$0.15 & 2.5 &  & 5848 & 4.37 & $+$0.15 & 2.5 &  & \nodata & \nodata & \nodata & \nodata & $-$18.6\\ 
K01102 & 6022 & 4.13 & $-$0.04 & 25.2 &  & 6137 & 3.96 & $-$0.00 & 25.2 &  & 5907 & 4.31 & $-$0.08 & 7.3 & $-$81.4\\ 
K01113 & 6097 & 4.29 & $+$0.04 & 5.2 &  & 6098 & 4.27 & $+$0.04 & 5.2 &  & 6096 & 4.32 & $+$0.04 & 6.6 & $+$17.1\\ 
K01115 & 5641 & 3.97 & $+$0.12 & 2.6 &  & 5632 & 3.99 & $+$0.11 & 2.6 &  & 5651 & 3.96 & $+$0.13 & 4.6 & $-$35.7\\ 
K01116 & 5736 & 4.32 & $+$0.04 & 2.3 &  & 5754 & 4.33 & $+$0.04 & 2.3 &  & 5719 & 4.31 & $+$0.05 & 4.8 & $-$20.9\\ 
K01117 & 6513 & 4.16 & $-$0.02 & 9.6 &  & 6445 & 4.18 & $-$0.03 & 9.6 &  & 6581 & 4.14 & $-$0.01 & 10.6 & $+$0.5\\ 
K01118 & 6010 & 4.25 & $-$0.04 & 3.5 &  & 6029 & 4.24 & $-$0.05 & 3.5 &  & 5991 & 4.26 & $-$0.04 & 5.4 & $+$18.3\\ 
K01120 & 4929 & 3.58 & $+$0.17 & 4.8 &  & 4929 & 3.58 & $+$0.17 & 4.8 &  & \nodata & \nodata & \nodata & \nodata & $-$15.4\\ 
K01126 & 5283 & 4.50 & $+$0.04 & 1.4 &  & 5283 & 4.50 & $+$0.04 & 1.4 &  & \nodata & \nodata & \nodata & \nodata & $+$5.6\\ 
K01127 & 5619 & 4.07 & $+$0.40 & 2.4 &  & 5619 & 4.07 & $+$0.40 & 2.4 &  & \nodata & \nodata & \nodata & \nodata & $-$36.7\\ 
K01128 & 5354 & 4.51 & $-$0.04 & 0.7 &  & 5352 & 4.51 & $-$0.03 & 0.7 &  & 5356 & 4.51 & $-$0.05 & 3.9 & $-$2.7\\ 
K01145 & 6007 & 4.43 & $+$0.09 & 4.1 &  & 5989 & 4.38 & $+$0.08 & 4.1 &  & 6025 & 4.48 & $+$0.09 & 5.6 & $+$6.7\\ 
K01148 & 6099 & 4.28 & $+$0.15 & 5.5 &  & 6116 & 4.26 & $+$0.16 & 5.5 &  & 6081 & 4.30 & $+$0.15 & 6.8 & $-$38.7\\ 
K01150 & 5754 & 4.32 & $+$0.10 & 3.8 &  & 5731 & 4.28 & $+$0.08 & 3.8 &  & 5776 & 4.36 & $+$0.13 & 5.5 & $-$3.8\\ 
K01151 & 5470 & 4.52 & $-$0.17 & 0.6 &  & 5477 & 4.52 & $-$0.18 & 0.6 &  & 5463 & 4.52 & $-$0.17 & 4.0 & $+$10.4\\ 
K01161 & 5439 & 4.40 & $+$0.04 & 2.7 &  & 5439 & 4.40 & $+$0.04 & 2.7 &  & \nodata & \nodata & \nodata & \nodata & $+$31.0\\ 
K01162 & 5684 & 4.36 & $-$0.22 & 1.0 &  & 5745 & 4.33 & $-$0.20 & 1.0 &  & 5622 & 4.38 & $-$0.24 & 4.3 & $-$68.8\\ 
K01163 & 5217 & 4.62 & $-$0.28 & 0.4 &  & 5217 & 4.62 & $-$0.28 & 0.4 &  & \nodata & \nodata & \nodata & \nodata & $-$15.1\\ 
K01165 & 5381 & 4.49 & $-$0.01 & 1.0 &  & 5397 & 4.52 & $+$0.00 & 1.0 &  & 5365 & 4.46 & $-$0.01 & 4.1 & $-$9.9\\ 
K01168 & 6141 & 4.12 & $+$0.06 & 6.4 &  & 6104 & 4.15 & $+$0.04 & 6.4 &  & 6177 & 4.08 & $+$0.08 & 7.9 & $-$7.6\\ 
K01169 & 5638 & 4.36 & $+$0.12 & 0.2 &  & 5642 & 4.29 & $+$0.13 & 0.2 &  & 5634 & 4.43 & $+$0.11 & 3.8 & $-$38.4\\ 
K01175 & 5640 & 3.80 & $+$0.10 & 4.4 &  & 5578 & 3.78 & $+$0.08 & 4.4 &  & 5701 & 3.82 & $+$0.12 & 5.6 & $+$0.9\\ 
K01196 & 5684 & 4.15 & $-$0.16 & 1.6 &  & 5684 & 4.15 & $-$0.16 & 1.6 &  & \nodata & \nodata & \nodata & \nodata & $-$59.8\\ 
K01198 & 6179 & 4.32 & $+$0.08 & 8.3 &  & 6328 & 4.40 & $+$0.10 & 8.3 &  & 6030 & 4.24 & $+$0.06 & 9.7 & $-$26.3\\ 
K01199 & 4772 & 4.53 & $+$0.11 & 2.3 &  & 4772 & 4.53 & $+$0.11 & 2.3 &  & \nodata & \nodata & \nodata & \nodata & $-$42.1\\ 
K01203 & 5693 & 4.58 & $-$0.29 & 0.7 &  & 5693 & 4.58 & $-$0.29 & 0.7 &  & \nodata & \nodata & \nodata & \nodata & $+$6.0\\ 
K01206 & 5834 & 3.82 & $+$0.12 & 5.3 &  & 5764 & 3.75 & $+$0.09 & 5.3 &  & 5905 & 3.88 & $+$0.14 & 6.3 & $-$48.4\\ 
K01208 & 6417 & 4.16 & $-$0.07 & 8.1 &  & 6372 & 4.26 & $-$0.07 & 8.1 &  & 6462 & 4.05 & $-$0.06 & 9.2 & $+$6.0\\ 
K01209 & 5774 & 4.37 & $+$0.06 & 1.5 &  & 5774 & 4.37 & $+$0.06 & 1.5 &  & \nodata & \nodata & \nodata & \nodata & $-$16.7\\ 
K01215 & 6065 & 4.03 & $+$0.09 & 2.9 &  & 6047 & 4.01 & $+$0.09 & 2.9 &  & 6083 & 4.04 & $+$0.10 & 4.7 & $-$63.1\\ 
K01216 & 5995 & 4.10 & $-$0.06 & 3.5 &  & 5939 & 4.03 & $-$0.09 & 3.5 &  & 6051 & 4.17 & $-$0.03 & 5.0 & $-$35.9\\ 
K01218 & 5582 & 4.33 & $-$0.02 & 2.2 &  & 5571 & 4.30 & $-$0.03 & 2.2 &  & 5592 & 4.36 & $-$0.00 & 4.6 & $-$35.2\\ 
K01220 & 5319 & 3.83 & $+$0.17 & 2.8 &  & 5283 & 3.80 & $+$0.16 & 2.8 &  & 5356 & 3.86 & $+$0.19 & 4.6 & $-$33.2\\ 
K01221 & 5002 & 3.62 & $+$0.33 & 2.1 &  & 4978 & 3.57 & $+$0.34 & 2.1 &  & 5026 & 3.66 & $+$0.33 & 4.4 & $-$46.8\\ 
K01222 & 5082 & 3.54 & $+$0.09 & 3.1 &  & 5044 & 3.54 & $+$0.07 & 3.1 &  & 5120 & 3.53 & $+$0.11 & 4.7 & $+$1.8\\ 
K01230 & 5119 & 3.35 & $+$0.01 & 3.9 &  & 5023 & 3.26 & $-$0.04 & 3.9 &  & 5216 & 3.45 & $+$0.06 & 5.2 & $-$29.2\\ 
K01239 & 5747 & 4.37 & $-$0.05 & 1.5 &  & 5747 & 4.37 & $-$0.05 & 1.5 &  & \nodata & \nodata & \nodata & \nodata & $-$16.9\\ 
K01240 & 5541 & 4.35 & $+$0.14 & 0.9 &  & 5541 & 4.35 & $+$0.14 & 0.9 &  & \nodata & \nodata & \nodata & \nodata & $+$5.2\\ 
K01241 & 4912 & 3.38 & $+$0.40 & 3.2 &  & 4840 & 3.22 & $+$0.37 & 3.2 &  & 4983 & 3.54 & $+$0.43 & 4.7 & $-$54.3\\ 
K01242 & 6139 & 4.26 & $-$0.01 & 5.5 &  & 6148 & 4.26 & $-$0.02 & 5.5 &  & 6130 & 4.25 & $+$0.00 & 6.9 & $-$5.3\\ 
K01257 & 5501 & 4.29 & $+$0.32 & 3.5 &  & 5490 & 4.23 & $+$0.31 & 3.5 &  & 5511 & 4.36 & $+$0.33 & 5.4 & $+$9.6\\ 
K01270 & 5203 & 4.56 & $+$0.08 & 1.6 &  & 5203 & 4.56 & $+$0.08 & 1.6 &  & \nodata & \nodata & \nodata & \nodata & $-$20.4\\ 
K01271 & 6263 & 4.21 & $-$0.28 & 6.9 &  & 6272 & 4.26 & $-$0.30 & 6.9 &  & 6255 & 4.16 & $-$0.25 & 8.4 & $+$6.7\\ 
K01274 & 5224 & 4.57 & $-$0.23 & 1.4 &  & 5236 & 4.61 & $-$0.22 & 1.4 &  & 5211 & 4.53 & $-$0.23 & 4.3 & $-$25.5\\ 
K01275 & 5854 & 4.25 & $+$0.03 & 2.7 &  & 5886 & 4.28 & $+$0.04 & 2.7 &  & 5822 & 4.23 & $+$0.01 & 4.9 & $-$24.5\\ 
K01276 & 5486 & 4.39 & $+$0.14 & 1.4 &  & 5486 & 4.39 & $+$0.14 & 1.4 &  & \nodata & \nodata & \nodata & \nodata & $-$26.0\\ 
K01278 & 5656 & 4.30 & $-$0.20 & 0.7 &  & 5697 & 4.26 & $-$0.21 & 0.7 &  & 5616 & 4.34 & $-$0.19 & 4.5 & $+$2.1\\ 
K01279 & 5705 & 4.32 & $-$0.02 & 1.3 &  & 5696 & 4.28 & $-$0.03 & 1.3 &  & 5713 & 4.35 & $-$0.01 & 4.1 & $-$11.5\\ 
K01282 & 6112 & 4.14 & $-$0.12 & 6.2 &  & 6100 & 4.15 & $-$0.12 & 6.2 &  & 6124 & 4.13 & $-$0.12 & 7.3 & $-$9.3\\ 
K01283 & 5737 & 4.13 & $-$0.25 & 0.3 &  & 5776 & 4.16 & $-$0.26 & 0.3 &  & 5699 & 4.11 & $-$0.25 & 4.2 & $-$65.1\\ 
K01288 & 6026 & 4.27 & $+$0.06 & 1.7 &  & 6070 & 4.33 & $+$0.07 & 1.7 &  & 5982 & 4.21 & $+$0.06 & 4.7 & $+$5.7\\ 
K01299 & 5002 & 3.42 & $+$0.07 & 3.0 &  & 4960 & 3.41 & $+$0.06 & 3.0 &  & 5045 & 3.44 & $+$0.09 & 4.6 & $-$35.7\\ 
K01300 & 4759 & 4.52 & $+$0.03 & 2.4 &  & 4759 & 4.52 & $+$0.03 & 2.4 &  & \nodata & \nodata & \nodata & \nodata & $+$8.7\\ 
K01301 & 5219 & 4.61 & $-$0.26 & 0.9 &  & 5219 & 4.61 & $-$0.26 & 0.9 &  & \nodata & \nodata & \nodata & \nodata & $-$7.3\\ 
K01305 & 5296 & 4.60 & $+$0.17 & 0.5 &  & 5296 & 4.60 & $+$0.17 & 0.5 &  & \nodata & \nodata & \nodata & \nodata & $+$8.2\\ 
K01306 & 5559 & 4.46 & $-$0.25 & 0.0 &  & 5622 & 4.53 & $-$0.26 & 0.0 &  & 5496 & 4.40 & $-$0.25 & 4.5 & $-$50.8\\ 
K01307 & 5547 & 4.49 & $+$0.12 & 0.8 &  & 5547 & 4.49 & $+$0.12 & 0.8 &  & \nodata & \nodata & \nodata & \nodata & $-$14.1\\ 
K01308 & 5639 & 4.12 & $+$0.02 & 2.5 &  & 5637 & 4.02 & $+$0.02 & 2.5 &  & 5642 & 4.21 & $+$0.02 & 4.6 & $-$6.1\\ 
K01311 & 5864 & 4.37 & $-$0.24 & 2.2 &  & 5865 & 4.36 & $-$0.27 & 2.2 &  & 5862 & 4.39 & $-$0.21 & 4.8 & $-$2.9\\ 
K01314 & 5074 & 3.56 & $+$0.12 & 2.9 &  & 5057 & 3.58 & $+$0.12 & 2.9 &  & 5091 & 3.54 & $+$0.13 & 4.7 & $-$36.2\\ 
K01315 & 6079 & 4.31 & $+$0.05 & 4.7 &  & 6094 & 4.30 & $+$0.06 & 4.7 &  & 6065 & 4.33 & $+$0.04 & 6.0 & $+$3.1\\ 
K01316 & 5847 & 3.97 & $+$0.32 & 3.9 &  & 5849 & 3.93 & $+$0.33 & 3.9 &  & 5845 & 4.00 & $+$0.31 & 5.5 & $-$54.0\\ 
K01332 & 5698 & 4.36 & $-$0.24 & 0.9 &  & 5698 & 4.36 & $-$0.24 & 0.9 &  & \nodata & \nodata & \nodata & \nodata & $-$35.1\\ 
K01335 & 6443 & 4.20 & $+$0.15 & 12.9 &  & 6432 & 4.19 & $+$0.18 & 12.9 &  & 6454 & 4.21 & $+$0.13 & 13.7 & $-$12.6\\ 
K01336 & 5776 & 4.47 & $+$0.10 & 2.1 &  & 5776 & 4.47 & $+$0.10 & 2.1 &  & \nodata & \nodata & \nodata & \nodata & $-$18.7\\ 
K01338 & 5680 & 4.34 & $-$0.16 & 1.7 &  & 5680 & 4.34 & $-$0.16 & 1.7 &  & \nodata & \nodata & \nodata & \nodata & $-$3.1\\ 
K01344 & 6010 & 4.26 & $-$0.32 & 2.5 &  & 6078 & 4.33 & $-$0.32 & 2.5 &  & 5942 & 4.20 & $-$0.33 & 5.1 & $-$34.3\\ 
K01353 & 5989 & 4.60 & $+$0.03 & 5.8 &  & 5973 & 4.56 & $+$0.01 & 5.8 &  & 6005 & 4.63 & $+$0.04 & 7.0 & $-$17.3\\ 
K01356 & 5719 & 3.94 & $+$0.22 & 3.6 &  & 5719 & 3.94 & $+$0.22 & 3.6 &  & \nodata & \nodata & \nodata & \nodata & $+$11.7\\ 
K01359 & 5756 & 4.49 & $-$0.18 & 0.2 &  & 5756 & 4.49 & $-$0.18 & 0.2 &  & \nodata & \nodata & \nodata & \nodata & $-$12.2\\ 
K01360 & 4962 & 4.71 & $-$0.10 & 2.4 &  & 4962 & 4.71 & $-$0.10 & 2.4 &  & \nodata & \nodata & \nodata & \nodata & $-$22.9\\ 
K01363 & 5637 & 4.23 & $+$0.23 & 2.2 &  & 5637 & 4.23 & $+$0.23 & 2.2 &  & \nodata & \nodata & \nodata & \nodata & $+$0.8\\ 
K01364 & 5248 & 4.45 & $+$0.04 & 1.4 &  & 5306 & 4.51 & $+$0.08 & 1.4 &  & 5191 & 4.38 & $-$0.01 & 4.3 & $+$169.5\\ 
K01366 & 5483 & 4.53 & $+$0.10 & 0.7 &  & 5483 & 4.53 & $+$0.10 & 0.7 &  & \nodata & \nodata & \nodata & \nodata & $-$21.4\\ 
K01367 & 4965 & 4.69 & $-$0.08 & 1.3 &  & 4965 & 4.69 & $-$0.08 & 1.3 &  & \nodata & \nodata & \nodata & \nodata & $-$26.0\\ 
K01375 & 6202 & 4.28 & $-$0.19 & 8.8 &  & 6214 & 4.30 & $-$0.20 & 8.8 &  & 6190 & 4.25 & $-$0.18 & 9.9 & $-$1.8\\ 
K01378 & 5582 & 4.04 & $-$0.25 & 2.2 &  & 5599 & 4.01 & $-$0.26 & 2.2 &  & 5565 & 4.06 & $-$0.24 & 4.8 & $-$39.4\\ 
K01379 & 5688 & 4.37 & $-$0.08 & 1.6 &  & 5682 & 4.35 & $-$0.09 & 1.6 &  & 5694 & 4.40 & $-$0.06 & 4.5 & $-$27.0\\ 
K01396 & 5513 & 4.54 & $+$0.11 & 1.5 &  & 5513 & 4.54 & $+$0.11 & 1.5 &  & \nodata & \nodata & \nodata & \nodata & $-$5.4\\ 
K01411 & 5672 & 4.22 & $+$0.34 & 2.6 &  & 5699 & 4.21 & $+$0.36 & 2.6 &  & 5644 & 4.23 & $+$0.32 & 4.7 & $-$62.0\\ 
K01412 & 5936 & 4.12 & $+$0.14 & 3.7 &  & 5938 & 4.12 & $+$0.12 & 3.7 &  & 5934 & 4.12 & $+$0.15 & 5.4 & $+$16.6\\ 
K01413 & 5253 & 3.79 & $-$0.03 & 2.8 &  & 5253 & 3.79 & $-$0.03 & 2.8 &  & \nodata & \nodata & \nodata & \nodata & $-$32.8\\ 
K01421 & 5623 & 4.33 & $+$0.03 & 2.2 &  & 5623 & 4.33 & $+$0.03 & 2.2 &  & \nodata & \nodata & \nodata & \nodata & $-$45.1\\ 
K01426 & 5693 & 4.51 & $-$0.11 & 1.3 &  & 5689 & 4.52 & $-$0.12 & 1.3 &  & 5696 & 4.51 & $-$0.09 & 4.2 & $-$9.9\\ 
K01428 & 4773 & 4.60 & $-$0.11 & 2.3 &  & 4773 & 4.60 & $-$0.11 & 2.3 &  & \nodata & \nodata & \nodata & \nodata & $+$5.9\\ 
K01431 & 5532 & 4.37 & $+$0.27 & 0.3 &  & 5528 & 4.34 & $+$0.26 & 0.3 &  & 5536 & 4.41 & $+$0.27 & 4.6 & $-$36.1\\ 
K01432 & 5678 & 4.35 & $+$0.12 & 1.9 &  & 5669 & 4.34 & $+$0.11 & 1.9 &  & 5688 & 4.37 & $+$0.13 & 4.6 & $+$12.4\\ 
K01436 & 5656 & 4.46 & $+$0.18 & 1.5 &  & 5656 & 4.46 & $+$0.18 & 1.5 &  & \nodata & \nodata & \nodata & \nodata & $-$12.0\\ 
K01438 & 5722 & 3.94 & $+$0.19 & 3.9 &  & 5677 & 3.89 & $+$0.17 & 3.9 &  & 5767 & 3.99 & $+$0.21 & 5.2 & $-$38.5\\ 
K01439 & 5979 & 4.03 & $+$0.14 & 4.9 &  & 5972 & 4.00 & $+$0.13 & 4.9 &  & 5985 & 4.05 & $+$0.15 & 6.4 & $-$29.2\\ 
K01442 & 5556 & 4.25 & $+$0.41 & 0.6 &  & 5553 & 4.19 & $+$0.42 & 0.6 &  & 5559 & 4.32 & $+$0.40 & 4.6 & $-$24.9\\ 
K01444 & 6236 & 4.11 & $+$0.11 & 8.3 &  & 6206 & 4.12 & $+$0.10 & 8.3 &  & 6267 & 4.11 & $+$0.12 & 9.4 & $-$16.9\\ 
K01445 & 6318 & 4.25 & $+$0.12 & 13.8 &  & 6334 & 4.25 & $+$0.13 & 13.8 &  & 6302 & 4.26 & $+$0.10 & 14.6 & $-$18.2\\ 
K01463 & 6532 & 4.19 & $-$0.04 & 10.3 &  & 6486 & 4.29 & $-$0.04 & 10.3 &  & 6578 & 4.08 & $-$0.04 & 11.7 & $-$25.9\\ 
K01466 & 4817 & 4.41 & $+$0.26 & 2.8 &  & 4817 & 4.41 & $+$0.26 & 2.8 &  & \nodata & \nodata & \nodata & \nodata & $-$150.2\\ 
K01474 & 6383 & 4.18 & $+$0.17 & 13.6 &  & 6413 & 4.20 & $+$0.18 & 13.6 &  & 6354 & 4.16 & $+$0.15 & 14.4 & $-$25.1\\ 
K01477 & 5259 & 4.69 & $-$0.02 & 2.4 &  & 5259 & 4.69 & $-$0.02 & 2.4 &  & \nodata & \nodata & \nodata & \nodata & $-$10.8\\ 
K01478 & 5511 & 4.38 & $+$0.02 & 0.7 &  & 5531 & 4.38 & $+$0.03 & 0.7 &  & 5492 & 4.38 & $+$0.00 & 3.9 & $-$27.9\\ 
K01480 & 4923 & 4.70 & $-$0.19 & 2.7 &  & 4923 & 4.70 & $-$0.19 & 2.7 &  & \nodata & \nodata & \nodata & \nodata & $-$8.3\\ 
K01483 & 5801 & 4.01 & $+$0.29 & 1.9 &  & 5801 & 4.01 & $+$0.29 & 1.9 &  & \nodata & \nodata & \nodata & \nodata & $-$13.8\\ 
K01486 & 5703 & 4.28 & $+$0.16 & 1.7 &  & 5703 & 4.28 & $+$0.16 & 1.7 &  & \nodata & \nodata & \nodata & \nodata & $+$5.3\\ 
K01528 & 5320 & 4.46 & $+$0.08 & 1.5 &  & 5326 & 4.47 & $+$0.08 & 1.5 &  & 5314 & 4.45 & $+$0.08 & 4.3 & $+$10.3\\ 
K01529 & 5884 & 4.18 & $-$0.20 & 1.9 &  & 5884 & 4.18 & $-$0.20 & 1.9 &  & \nodata & \nodata & \nodata & \nodata & $-$40.3\\ 
K01530 & 5953 & 4.33 & $-$0.43 & 1.0 &  & 6004 & 4.39 & $-$0.44 & 1.0 &  & 5903 & 4.28 & $-$0.42 & 4.6 & $-$18.5\\ 
K01531 & 5747 & 4.39 & $-$0.09 & 3.1 &  & 5796 & 4.42 & $-$0.06 & 3.1 &  & 5698 & 4.35 & $-$0.11 & 4.9 & $-$30.5\\ 
K01532 & 6133 & 4.18 & $+$0.14 & 6.6 &  & 6142 & 4.21 & $+$0.15 & 6.6 &  & 6124 & 4.16 & $+$0.13 & 7.7 & $-$30.5\\ 
K01533 & 5857 & 4.49 & $-$0.21 & 0.9 &  & 5879 & 4.51 & $-$0.23 & 0.9 &  & 5834 & 4.48 & $-$0.18 & 4.5 & $+$2.6\\ 
K01534 & 6207 & 4.28 & $+$0.04 & 8.1 &  & 6189 & 4.27 & $+$0.03 & 8.1 &  & 6225 & 4.30 & $+$0.05 & 9.1 & $-$2.9\\ 
K01535 & 5739 & 4.51 & $-$0.32 & 0.4 &  & 5774 & 4.53 & $-$0.34 & 0.4 &  & 5704 & 4.49 & $-$0.31 & 4.1 & $-$42.8\\ 
K01536 & 5885 & 4.09 & $+$0.22 & 3.1 &  & 5900 & 4.09 & $+$0.22 & 3.1 &  & 5870 & 4.09 & $+$0.21 & 5.2 & $-$17.0\\ 
K01537 & 6219 & 4.15 & $-$0.13 & 6.2 &  & 6206 & 4.16 & $-$0.14 & 6.2 &  & 6231 & 4.13 & $-$0.13 & 7.4 & $-$28.0\\ 
K01546 & 6179 & 4.31 & $-$0.00 & 4.9 &  & 6179 & 4.31 & $-$0.00 & 4.9 &  & \nodata & \nodata & \nodata & \nodata & $+$6.8\\ 
K01557 & 4843 & 4.70 & $+$0.03 & 3.5 &  & 4796 & 4.70 & $+$0.02 & 3.5 &  & 4889 & 4.71 & $+$0.04 & 4.7 & $-$26.9\\ 
K01563 & 5080 & 4.57 & $+$0.09 & 2.0 &  & 5099 & 4.59 & $+$0.10 & 2.0 &  & 5061 & 4.54 & $+$0.08 & 4.4 & $-$3.3\\ 
K01567 & 4908 & 4.43 & $-$0.13 & 2.2 &  & 4912 & 4.48 & $-$0.08 & 2.2 &  & 4904 & 4.37 & $-$0.17 & 4.3 & $-$20.4\\ 
K01576 & 5559 & 4.42 & $+$0.23 & 2.0 &  & 5584 & 4.42 & $+$0.25 & 2.0 &  & 5535 & 4.41 & $+$0.21 & 4.7 & $-$45.2\\ 
K01581 & 5437 & 3.98 & $+$0.24 & 2.6 &  & 5437 & 3.98 & $+$0.24 & 2.6 &  & \nodata & \nodata & \nodata & \nodata & $-$20.0\\ 
K01589 & 6026 & 4.56 & $-$0.11 & 4.5 &  & 6032 & 4.62 & $-$0.12 & 4.5 &  & 6021 & 4.51 & $-$0.10 & 5.8 & $+$12.8\\ 
K01590 & 4867 & 4.65 & $-$0.08 & 2.9 &  & 4867 & 4.65 & $-$0.08 & 2.9 &  & \nodata & \nodata & \nodata & \nodata & $-$40.3\\ 
K01596 & 4786 & 4.49 & $+$0.27 & 2.2 &  & 4786 & 4.49 & $+$0.27 & 2.2 &  & \nodata & \nodata & \nodata & \nodata & $-$52.8\\ 
K01598 & 5451 & 4.57 & $-$0.12 & 0.4 &  & 5451 & 4.57 & $-$0.12 & 0.4 &  & \nodata & \nodata & \nodata & \nodata & $-$27.5\\ 
K01601 & 5555 & 3.94 & $-$0.10 & 1.7 &  & 5555 & 3.94 & $-$0.10 & 1.7 &  & \nodata & \nodata & \nodata & \nodata & $-$72.2\\ 
K01606 & 5435 & 4.51 & $+$0.14 & 1.6 &  & 5442 & 4.53 & $+$0.14 & 1.6 &  & 5427 & 4.50 & $+$0.15 & 4.1 & $-$17.6\\ 
K01608 & 5897 & 4.29 & $-$0.03 & 2.8 &  & 5905 & 4.27 & $-$0.03 & 2.8 &  & 5890 & 4.31 & $-$0.02 & 4.9 & $-$36.6\\ 
K01609 & 5956 & 4.45 & $-$0.40 & 2.7 &  & 5967 & 4.50 & $-$0.44 & 2.7 &  & 5944 & 4.39 & $-$0.37 & 5.1 & $-$3.9\\ 
K01612 & 6089 & 4.30 & $-$0.15 & 2.8 &  & 6092 & 4.27 & $-$0.14 & 2.8 &  & 6086 & 4.34 & $-$0.15 & 5.5 & $-$54.6\\ 
K01615 & 6053 & 4.49 & $+$0.21 & 7.9 &  & 6008 & 4.42 & $+$0.21 & 7.9 &  & 6098 & 4.55 & $+$0.21 & 8.7 & $-$23.5\\ 
K01616 & 6042 & 4.26 & $+$0.17 & 5.3 &  & 6042 & 4.26 & $+$0.17 & 5.3 &  & \nodata & \nodata & \nodata & \nodata & $-$28.0\\ 
K01618 & 6229 & 4.16 & $+$0.14 & 10.1 &  & 6199 & 4.16 & $+$0.13 & 10.1 &  & 6260 & 4.17 & $+$0.15 & 11.0 & $-$4.6\\ 
K01619 & 4847 & 4.61 & $-$0.26 & 2.7 &  & 4837 & 4.69 & $-$0.25 & 2.7 &  & 4857 & 4.53 & $-$0.26 & 4.7 & $-$6.2\\ 
K01621 & 6079 & 4.04 & $+$0.01 & 5.9 &  & 6079 & 4.04 & $+$0.01 & 5.9 &  & \nodata & \nodata & \nodata & \nodata & $-$47.4\\ 
K01623 & 5667 & 4.05 & $+$0.02 & 2.1 &  & 5698 & 4.03 & $+$0.03 & 2.1 &  & 5635 & 4.06 & $+$0.01 & 5.0 & $+$7.2\\ 
K01628 & 6224 & 4.48 & $+$0.15 & 10.4 &  & 6241 & 4.49 & $+$0.14 & 10.4 &  & 6206 & 4.48 & $+$0.15 & 11.2 & $-$23.3\\ 
K01629 & 5804 & 4.17 & $+$0.26 & 3.2 &  & 5800 & 4.14 & $+$0.26 & 3.2 &  & 5809 & 4.20 & $+$0.25 & 5.0 & $-$27.2\\ 
K01632 & 6081 & 4.16 & $+$0.02 & 7.6 &  & 6073 & 4.15 & $+$0.02 & 7.6 &  & 6089 & 4.18 & $+$0.03 & 8.5 & $+$0.4\\ 
K01639 & 6203 & 3.90 & $+$0.11 & 5.9 &  & 6150 & 3.87 & $+$0.12 & 5.9 &  & 6256 & 3.93 & $+$0.10 & 7.1 & $-$30.6\\ 
K01647 & 5709 & 4.18 & $+$0.26 & 3.7 &  & 5690 & 4.12 & $+$0.26 & 3.7 &  & 5728 & 4.24 & $+$0.26 & 5.1 & $-$38.6\\ 
K01655 & 5534 & 4.44 & $-$0.07 & 0.3 &  & 5537 & 4.44 & $-$0.09 & 0.3 &  & 5530 & 4.43 & $-$0.06 & 4.1 & $+$21.1\\ 
K01665 & 5987 & 4.17 & $+$0.32 & 3.0 &  & 5965 & 4.11 & $+$0.32 & 3.0 &  & 6008 & 4.23 & $+$0.31 & 4.8 & $-$18.0\\ 
K01666 & 6435 & 4.38 & $+$0.12 & 14.2 &  & 6435 & 4.38 & $+$0.12 & 14.2 &  & \nodata & \nodata & \nodata & \nodata & $+$0.0\\ 
K01669 & 6162 & 4.25 & $-$0.04 & 6.9 &  & 6133 & 4.23 & $-$0.05 & 6.9 &  & 6191 & 4.28 & $-$0.03 & 7.9 & $-$4.1\\ 
K01688 & 5988 & 4.07 & $+$0.18 & 5.6 &  & 5988 & 4.07 & $+$0.18 & 5.6 &  & \nodata & \nodata & \nodata & \nodata & $-$27.0\\ 
K01692 & 5440 & 4.45 & $+$0.38 & 2.7 &  & 5440 & 4.45 & $+$0.38 & 2.7 &  & \nodata & \nodata & \nodata & \nodata & $-$21.5\\ 
K01695 & 5856 & 4.13 & $+$0.13 & 3.7 &  & 5881 & 4.14 & $+$0.14 & 3.7 &  & 5830 & 4.12 & $+$0.12 & 5.8 & $-$14.6\\ 
K01706 & 5166 & 4.35 & $+$0.07 & 2.4 &  & 5103 & 4.19 & $+$0.02 & 2.4 &  & 5228 & 4.50 & $+$0.13 & 4.4 & $-$53.0\\ 
K01707 & 5683 & 4.42 & $-$0.27 & 0.6 &  & 5683 & 4.42 & $-$0.27 & 0.6 &  & \nodata & \nodata & \nodata & \nodata & $+$0.0\\ 
K01715 & 5789 & 4.30 & $-$0.23 & 1.1 &  & 5825 & 4.32 & $-$0.25 & 1.1 &  & 5753 & 4.28 & $-$0.22 & 4.3 & $-$24.8\\ 
K01726 & 4768 & 4.48 & $+$0.08 & 2.9 &  & 4746 & 4.47 & $+$0.09 & 2.9 &  & 4789 & 4.50 & $+$0.06 & 4.6 & $-$39.4\\ 
K01738 & 5287 & 4.46 & $+$0.24 & 2.3 &  & 5307 & 4.46 & $+$0.26 & 2.3 &  & 5267 & 4.46 & $+$0.22 & 4.5 & $-$17.2\\ 
K01739 & 5794 & 4.20 & $+$0.08 & 2.6 &  & 5794 & 4.20 & $+$0.08 & 2.6 &  & \nodata & \nodata & \nodata & \nodata & $-$30.9\\ 
K01751 & 5130 & 4.68 & $-$0.01 & 2.5 &  & 5130 & 4.68 & $-$0.01 & 2.5 &  & \nodata & \nodata & \nodata & \nodata & $-$36.6\\ 
K01754 & 6157 & 4.36 & $-$0.04 & 6.9 &  & 6164 & 4.38 & $-$0.06 & 6.9 &  & 6150 & 4.34 & $-$0.02 & 8.3 & $-$9.5\\ 
K01779 & 5873 & 4.56 & $+$0.33 & 7.0 &  & 5857 & 4.55 & $+$0.33 & 7.0 &  & 5889 & 4.57 & $+$0.33 & 8.0 & $-$24.9\\ 
K01781 & 4961 & 4.69 & $+$0.21 & 3.8 &  & 4906 & 4.62 & $+$0.19 & 3.8 &  & 5016 & 4.75 & $+$0.24 & 5.7 & $-$19.7\\ 
K01783 & 5923 & 4.29 & $+$0.11 & 3.1 &  & 5933 & 4.28 & $+$0.12 & 3.1 &  & 5913 & 4.30 & $+$0.10 & 5.0 & $-$3.1\\ 
K01792 & 5460 & 4.01 & $+$0.03 & 3.8 &  & 5468 & 4.10 & $+$0.01 & 3.8 &  & 5452 & 3.92 & $+$0.05 & 5.8 & $-$25.6\\ 
K01796 & 6013 & 4.48 & $-$0.01 & 4.3 &  & 6045 & 4.49 & $-$0.01 & 4.3 &  & 5981 & 4.48 & $-$0.01 & 5.9 & $+$1.2\\ 
K01797 & 5030 & 4.73 & $+$0.20 & 4.3 &  & 4973 & 4.67 & $+$0.18 & 4.3 &  & 5087 & 4.78 & $+$0.22 & 5.5 & $-$23.7\\ 
K01800 & 5620 & 4.69 & $+$0.07 & 6.9 &  & 5562 & 4.67 & $+$0.05 & 6.9 &  & 5679 & 4.70 & $+$0.10 & 7.7 & $+$1.6\\ 
K01802 & 5918 & 4.49 & $+$0.05 & 3.3 &  & 5901 & 4.52 & $+$0.03 & 3.3 &  & 5936 & 4.47 & $+$0.08 & 5.4 & $-$3.7\\ 
K01803 & 4979 & 4.68 & $+$0.07 & 2.8 &  & 4922 & 4.66 & $+$0.05 & 2.8 &  & 5037 & 4.69 & $+$0.08 & 4.5 & $-$7.4\\ 
K01805 & 5599 & 4.65 & $+$0.06 & 3.4 &  & 5562 & 4.66 & $+$0.03 & 3.4 &  & 5636 & 4.63 & $+$0.08 & 5.0 & $+$10.1\\ 
K01806 & 6134 & 4.28 & $-$0.06 & 6.9 &  & 6152 & 4.28 & $-$0.05 & 6.9 &  & 6117 & 4.28 & $-$0.08 & 8.1 & $-$46.7\\ 
K01808 & 6143 & 4.44 & $+$0.04 & 6.7 &  & 6183 & 4.43 & $+$0.06 & 6.7 &  & 6103 & 4.46 & $+$0.03 & 7.7 & $-$3.7\\ 
K01809 & 5741 & 4.39 & $+$0.12 & 2.9 &  & 5748 & 4.40 & $+$0.12 & 2.9 &  & 5734 & 4.39 & $+$0.12 & 4.8 & $-$12.2\\ 
K01812 & 5941 & 4.21 & $-$0.04 & 2.4 &  & 5974 & 4.24 & $-$0.04 & 2.4 &  & 5908 & 4.19 & $-$0.05 & 4.7 & $-$16.9\\ 
K01813 & 5419 & 4.62 & $+$0.06 & 2.1 &  & 5413 & 4.63 & $+$0.06 & 2.1 &  & 5425 & 4.61 & $+$0.06 & 4.4 & $+$0.8\\ 
K01815 & 4773 & 4.64 & $+$0.06 & 2.5 &  & 4747 & 4.61 & $+$0.07 & 2.5 &  & 4799 & 4.67 & $+$0.05 & 4.4 & $-$22.0\\ 
K01818 & 5560 & 4.64 & $+$0.05 & 2.4 &  & 5515 & 4.62 & $+$0.02 & 2.4 &  & 5605 & 4.65 & $+$0.08 & 4.6 & $+$15.2\\ 
K01819 & 5450 & 4.68 & $+$0.05 & 3.3 &  & 5447 & 4.71 & $+$0.05 & 3.3 &  & 5453 & 4.65 & $+$0.05 & 4.9 & $-$3.4\\ 
K01820 & 5414 & 4.65 & $+$0.13 & 2.5 &  & 5413 & 4.65 & $+$0.12 & 2.5 &  & 5415 & 4.64 & $+$0.13 & 4.6 & $-$23.8\\ 
K01822 & 6090 & 4.45 & $-$0.20 & 4.5 &  & 6104 & 4.47 & $-$0.22 & 4.5 &  & 6077 & 4.43 & $-$0.18 & 6.1 & $-$4.9\\ 
K01824 & 5935 & 4.34 & $-$0.16 & 3.1 &  & 5959 & 4.31 & $-$0.17 & 3.1 &  & 5911 & 4.36 & $-$0.14 & 5.2 & $+$13.4\\ 
K01825 & 5391 & 4.69 & $+$0.13 & 4.5 &  & 5370 & 4.68 & $+$0.14 & 4.5 &  & 5411 & 4.69 & $+$0.12 & 5.6 & $-$21.6\\ 
K01826 & 5881 & 4.32 & $-$0.05 & 2.9 &  & 5914 & 4.33 & $-$0.05 & 2.9 &  & 5847 & 4.30 & $-$0.05 & 5.1 & $-$12.7\\ 
K01831 & 5233 & 4.47 & $+$0.18 & 2.1 &  & 5228 & 4.46 & $+$0.17 & 2.1 &  & 5237 & 4.47 & $+$0.18 & 4.5 & $-$70.3\\ 
K01832 & 5541 & 4.74 & $+$0.02 & 2.9 &  & 5541 & 4.74 & $+$0.02 & 2.9 &  & \nodata & \nodata & \nodata & \nodata & $-$18.9\\ 
K01835 & 5184 & 4.67 & $+$0.21 & 4.7 &  & 5132 & 4.65 & $+$0.18 & 4.7 &  & 5235 & 4.69 & $+$0.24 & 5.9 & $-$16.7\\ 
K01837 & 5243 & 4.63 & $+$0.15 & 2.9 &  & 5215 & 4.62 & $+$0.14 & 2.9 &  & 5271 & 4.64 & $+$0.16 & 4.6 & $-$20.9\\ 
K01839 & 5517 & 4.66 & $+$0.17 & 7.1 &  & 5453 & 4.61 & $+$0.12 & 7.1 &  & 5581 & 4.72 & $+$0.21 & 8.2 & $-$21.2\\ 
K01841 & 5181 & 4.59 & $+$0.04 & 2.0 &  & 5169 & 4.60 & $+$0.04 & 2.0 &  & 5193 & 4.58 & $+$0.04 & 4.3 & $-$21.7\\ 
K01845 & 4801 & 4.37 & $+$0.32 & 2.8 &  & 4801 & 4.37 & $+$0.32 & 2.8 &  & \nodata & \nodata & \nodata & \nodata & $-$9.9\\ 
K01848 & 5996 & 4.39 & $-$0.10 & 6.1 &  & 6023 & 4.46 & $-$0.10 & 6.1 &  & 5970 & 4.31 & $-$0.11 & 7.4 & $+$20.3\\ 
K01850 & 5831 & 4.19 & $+$0.01 & 2.9 &  & 5847 & 4.17 & $+$0.01 & 2.9 &  & 5814 & 4.22 & $+$0.01 & 4.9 & $+$0.4\\ 
K01852 & 6333 & 4.28 & $-$0.20 & 4.2 &  & 6347 & 4.26 & $-$0.21 & 4.2 &  & 6318 & 4.30 & $-$0.19 & 5.8 & $-$9.2\\ 
K01854 & 5601 & 4.49 & $+$0.04 & 1.3 &  & 5592 & 4.49 & $+$0.04 & 1.3 &  & 5610 & 4.50 & $+$0.04 & 4.1 & $-$23.0\\ 
K01856 & 5251 & 4.58 & $+$0.02 & 1.9 &  & 5238 & 4.60 & $+$0.02 & 1.9 &  & 5264 & 4.56 & $+$0.03 & 4.4 & $-$24.5\\ 
K01857 & 5743 & 4.42 & $-$0.03 & 2.8 &  & 5774 & 4.43 & $-$0.01 & 2.8 &  & 5712 & 4.41 & $-$0.05 & 4.9 & $-$30.5\\ 
K01858 & 5425 & 4.67 & $+$0.00 & 1.9 &  & 5425 & 4.67 & $+$0.00 & 1.9 &  & \nodata & \nodata & \nodata & \nodata & $-$18.0\\ 
K01860 & 5718 & 4.44 & $+$0.12 & 2.6 &  & 5728 & 4.45 & $+$0.13 & 2.6 &  & 5709 & 4.44 & $+$0.12 & 4.8 & $-$15.9\\ 
K01861 & 6020 & 4.58 & $+$0.03 & 7.7 &  & 6043 & 4.59 & $+$0.03 & 7.7 &  & 5997 & 4.57 & $+$0.02 & 8.7 & $+$14.5\\ 
K01862 & 5611 & 4.38 & $+$0.25 & 1.8 &  & 5605 & 4.33 & $+$0.25 & 1.8 &  & 5616 & 4.42 & $+$0.25 & 4.3 & $+$3.2\\ 
K01863 & 5989 & 4.42 & $+$0.20 & 4.7 &  & 5983 & 4.40 & $+$0.21 & 4.7 &  & 5994 & 4.43 & $+$0.18 & 6.0 & $-$19.1\\ 
K01864 & 5620 & 3.93 & $+$0.12 & 2.1 &  & 5615 & 3.96 & $+$0.13 & 2.1 &  & 5625 & 3.89 & $+$0.11 & 4.6 & $-$48.9\\ 
K01871 & 4628 & 4.34 & $+$0.18 & 3.1 &  & 4628 & 4.34 & $+$0.18 & 3.1 &  & \nodata & \nodata & \nodata & \nodata & $-$62.4\\ 
K01875 & 5577 & 4.37 & $-$0.11 & 1.5 &  & 5577 & 4.37 & $-$0.11 & 1.5 &  & \nodata & \nodata & \nodata & \nodata & $-$32.3\\ 
K01877 & 4914 & 4.63 & $+$0.02 & 2.8 &  & 4891 & 4.64 & $+$0.03 & 2.8 &  & 4937 & 4.62 & $-$0.00 & 4.4 & $-$14.8\\ 
K01878 & 6190 & 4.28 & $+$0.15 & 6.9 &  & 6207 & 4.27 & $+$0.17 & 6.9 &  & 6174 & 4.29 & $+$0.13 & 8.0 & $-$11.4\\ 
K01883 & 6059 & 4.15 & $+$0.06 & 6.6 &  & 6009 & 4.11 & $+$0.04 & 6.6 &  & 6109 & 4.18 & $+$0.07 & 7.7 & $-$29.8\\ 
K01886 & 6201 & 4.19 & $+$0.04 & 10.5 &  & 6226 & 4.18 & $+$0.05 & 10.5 &  & 6176 & 4.21 & $+$0.03 & 11.2 & $-$51.8\\ 
K01888 & 6421 & 4.23 & $+$0.10 & 17.1 &  & 6400 & 4.29 & $+$0.10 & 17.1 &  & 6442 & 4.17 & $+$0.11 & 18.0 & $-$1.3\\ 
K01889 & 5440 & 4.65 & $+$0.04 & 2.1 &  & 5440 & 4.65 & $+$0.04 & 2.1 &  & \nodata & \nodata & \nodata & \nodata & $+$4.8\\ 
K01890 & 6120 & 4.19 & $+$0.12 & 7.2 &  & 6071 & 4.15 & $+$0.10 & 7.2 &  & 6168 & 4.23 & $+$0.14 & 8.2 & $-$46.2\\ 
K01891 & 5028 & 4.52 & $+$0.16 & 1.1 &  & 5028 & 4.52 & $+$0.16 & 1.1 &  & \nodata & \nodata & \nodata & \nodata & $-$5.4\\ 
K01893 & 5672 & 4.25 & $-$0.30 & 2.0 &  & 5718 & 4.17 & $-$0.29 & 2.0 &  & 5625 & 4.32 & $-$0.31 & 4.8 & $-$87.1\\ 
K01894 & 5007 & 3.49 & $+$0.19 & 3.1 &  & 4990 & 3.49 & $+$0.18 & 3.1 &  & 5025 & 3.48 & $+$0.19 & 4.9 & $-$38.2\\ 
K01897 & 5880 & 4.30 & $-$0.09 & 2.2 &  & 5893 & 4.31 & $-$0.11 & 2.2 &  & 5867 & 4.29 & $-$0.08 & 4.6 & $+$22.3\\ 
K01898 & 5728 & 4.31 & $+$0.02 & 1.6 &  & 5755 & 4.29 & $+$0.01 & 1.6 &  & 5702 & 4.33 & $+$0.03 & 4.5 & $-$48.9\\ 
K01901 & 5999 & 4.30 & $+$0.14 & 4.4 &  & 6003 & 4.26 & $+$0.14 & 4.4 &  & 5994 & 4.34 & $+$0.14 & 6.0 & $-$24.6\\ 
K01904 & 5045 & 4.61 & $-$0.03 & 2.7 &  & 5053 & 4.66 & $+$0.01 & 2.7 &  & 5038 & 4.56 & $-$0.06 & 4.8 & $+$9.5\\ 
K01905 & 4955 & 4.66 & $-$0.13 & 1.3 &  & 4948 & 4.72 & $-$0.11 & 1.3 &  & 4962 & 4.59 & $-$0.15 & 4.1 & $-$36.3\\ 
K01909 & 5866 & 4.44 & $+$0.01 & 2.4 &  & 5901 & 4.45 & $+$0.02 & 2.4 &  & 5830 & 4.43 & $+$0.00 & 4.8 & $-$34.7\\ 
K01913 & 5500 & 4.53 & $+$0.23 & 2.7 &  & 5497 & 4.51 & $+$0.23 & 2.7 &  & 5503 & 4.54 & $+$0.23 & 4.7 & $-$11.2\\ 
K01915 & 6000 & 4.04 & $+$0.34 & 6.5 &  & 5958 & 4.00 & $+$0.33 & 6.5 &  & 6041 & 4.09 & $+$0.35 & 7.7 & $+$13.5\\ 
K01916 & 5888 & 4.40 & $+$0.22 & 5.8 &  & 5869 & 4.36 & $+$0.22 & 5.8 &  & 5907 & 4.44 & $+$0.22 & 6.8 & $-$27.6\\ 
K01917 & 5936 & 4.34 & $-$0.06 & 3.2 &  & 5943 & 4.33 & $-$0.07 & 3.2 &  & 5928 & 4.35 & $-$0.05 & 5.1 & $-$4.7\\ 
K01921 & 6443 & 4.30 & $+$0.03 & 18.6 &  & 6495 & 4.35 & $+$0.04 & 18.6 &  & 6392 & 4.25 & $+$0.03 & 19.8 & $+$12.2\\ 
K01922 & 5781 & 4.40 & $+$0.04 & 1.7 &  & 5781 & 4.40 & $+$0.04 & 1.7 &  & \nodata & \nodata & \nodata & \nodata & $-$2.8\\ 
K01923 & 5400 & 4.50 & $+$0.20 & 2.0 &  & 5377 & 4.45 & $+$0.19 & 2.0 &  & 5423 & 4.54 & $+$0.22 & 4.4 & $+$11.4\\ 
K01924 & 5948 & 3.81 & $+$0.34 & 4.7 &  & 5948 & 3.81 & $+$0.34 & 4.7 &  & \nodata & \nodata & \nodata & \nodata & $-$13.0\\ 
K01925 & 5416 & 4.43 & $+$0.12 & 2.4 &  & 5419 & 4.43 & $+$0.12 & 2.4 &  & 5413 & 4.43 & $+$0.11 & 4.5 & $-$28.2\\ 
K01928 & 5860 & 4.40 & $+$0.23 & 2.9 &  & 5867 & 4.36 & $+$0.25 & 2.9 &  & 5853 & 4.45 & $+$0.22 & 4.8 & $-$50.3\\ 
K01929 & 5634 & 3.96 & $+$0.07 & 2.1 &  & 5649 & 3.96 & $+$0.07 & 2.1 &  & 5620 & 3.96 & $+$0.06 & 4.5 & $-$62.8\\ 
K01930 & 5897 & 4.02 & $-$0.01 & 5.1 &  & 5847 & 3.96 & $-$0.04 & 5.1 &  & 5948 & 4.09 & $+$0.02 & 6.5 & $-$17.2\\ 
K01931 & 5446 & 4.68 & $-$0.00 & 1.8 &  & 5446 & 4.68 & $-$0.00 & 1.8 &  & \nodata & \nodata & \nodata & \nodata & $-$15.0\\ 
K01938 & 5109 & 4.59 & $-$0.23 & 1.6 &  & 5110 & 4.64 & $-$0.22 & 1.6 &  & 5109 & 4.54 & $-$0.23 & 4.3 & $-$20.0\\ 
K01944 & 5739 & 4.58 & $+$0.07 & 3.2 &  & 5732 & 4.59 & $+$0.07 & 3.2 &  & 5747 & 4.58 & $+$0.08 & 5.2 & $-$36.2\\ 
K01945 & 5354 & 4.42 & $+$0.26 & 1.4 &  & 5354 & 4.42 & $+$0.26 & 1.4 &  & \nodata & \nodata & \nodata & \nodata & $-$5.2\\ 
K01947 & 5944 & 3.95 & $+$0.22 & 3.1 &  & 5945 & 3.96 & $+$0.22 & 3.1 &  & 5942 & 3.95 & $+$0.22 & 5.1 & $-$59.2\\ 
K01951 & 6031 & 4.26 & $-$0.22 & 4.3 &  & 6091 & 4.34 & $-$0.20 & 4.3 &  & 5971 & 4.18 & $-$0.23 & 6.2 & $-$40.2\\ 
K01952 & 5722 & 4.19 & $+$0.07 & 1.9 &  & 5722 & 4.19 & $+$0.07 & 1.9 &  & \nodata & \nodata & \nodata & \nodata & $-$95.6\\ 
K01955 & 6272 & 4.25 & $+$0.10 & 9.5 &  & 6241 & 4.24 & $+$0.09 & 9.5 &  & 6304 & 4.26 & $+$0.11 & 10.5 & $-$27.3\\ 
K01958 & 5786 & 4.57 & $+$0.06 & 4.1 &  & 5850 & 4.63 & $+$0.07 & 4.1 &  & 5721 & 4.52 & $+$0.06 & 6.2 & $+$7.0\\ 
K01960 & 5781 & 4.17 & $+$0.18 & 3.0 &  & 5795 & 4.16 & $+$0.18 & 3.0 &  & 5768 & 4.18 & $+$0.18 & 5.0 & $-$84.7\\ 
K01961 & 5404 & 4.62 & $+$0.05 & 3.5 &  & 5382 & 4.61 & $+$0.03 & 3.5 &  & 5425 & 4.62 & $+$0.07 & 5.2 & $-$5.1\\ 
K01962 & 5910 & 4.12 & $-$0.05 & 4.6 &  & 5898 & 4.08 & $-$0.06 & 4.6 &  & 5921 & 4.16 & $-$0.05 & 5.9 & $-$56.7\\ 
K01963 & 5876 & 4.21 & $+$0.09 & 4.6 &  & 5876 & 4.21 & $+$0.09 & 4.6 &  & 6163 & 4.78 & $+$0.09 & 5.1 & $-$37.0\\ 
K01964 & 5535 & 4.47 & $+$0.05 & 2.4 &  & 5535 & 4.48 & $+$0.04 & 2.4 &  & 5534 & 4.46 & $+$0.05 & 4.7 & $-$19.8\\ 
K01970 & 5459 & 4.41 & $+$0.08 & 0.3 &  & 5459 & 4.41 & $+$0.08 & 0.3 &  & \nodata & \nodata & \nodata & \nodata & $-$35.3\\ 
K01978 & 5511 & 4.54 & $+$0.10 & 1.1 &  & 5511 & 4.54 & $+$0.10 & 1.1 &  & \nodata & \nodata & \nodata & \nodata & $-$19.8\\ 
K01979 & 5737 & 4.33 & $+$0.19 & 2.7 &  & 5721 & 4.26 & $+$0.20 & 2.7 &  & 5754 & 4.40 & $+$0.19 & 4.6 & $-$60.2\\ 
K01980 & 5476 & 4.55 & $+$0.18 & 2.3 &  & 5491 & 4.56 & $+$0.19 & 2.3 &  & 5461 & 4.54 & $+$0.18 & 4.6 & $-$40.6\\ 
K01984 & 6000 & 4.31 & $+$0.13 & 4.2 &  & 6010 & 4.31 & $+$0.14 & 4.2 &  & 5991 & 4.30 & $+$0.12 & 5.7 & $-$35.0\\ 
K01985 & 4950 & 4.64 & $+$0.01 & 2.7 &  & 4928 & 4.67 & $+$0.02 & 2.7 &  & 4972 & 4.60 & $+$0.01 & 4.5 & $-$2.4\\ 
K01988 & 4766 & 4.57 & $+$0.13 & 3.0 &  & 4696 & 4.50 & $+$0.13 & 3.0 &  & 4837 & 4.64 & $+$0.14 & 4.5 & $+$5.8\\ 
K01989 & 5697 & 4.48 & $+$0.09 & 2.2 &  & 5706 & 4.48 & $+$0.09 & 2.2 &  & 5687 & 4.47 & $+$0.09 & 4.5 & $-$5.5\\ 
K01992 & 5704 & 4.03 & $-$0.14 & 1.7 &  & 5704 & 4.03 & $-$0.14 & 1.7 &  & \nodata & \nodata & \nodata & \nodata & $-$66.9\\ 
K02001 & 5170 & 4.64 & $+$0.09 & 3.1 &  & 5144 & 4.68 & $+$0.08 & 3.1 &  & 5196 & 4.61 & $+$0.10 & 4.8 & $-$11.9\\ 
K02002 & 6004 & 4.50 & $+$0.04 & 4.8 &  & 6014 & 4.50 & $+$0.03 & 4.8 &  & 5995 & 4.50 & $+$0.04 & 6.3 & $-$1.5\\ 
K02004 & 5659 & 4.23 & $+$0.29 & 4.6 &  & 5666 & 4.20 & $+$0.30 & 4.6 &  & 5651 & 4.27 & $+$0.28 & 6.0 & $-$34.6\\ 
K02007 & 5846 & 4.42 & $+$0.10 & 2.5 &  & 5901 & 4.50 & $+$0.14 & 2.5 &  & 5791 & 4.34 & $+$0.06 & 4.9 & $-$20.4\\ 
K02009 & 5618 & 4.37 & $-$0.23 & 1.3 &  & 5654 & 4.34 & $-$0.23 & 1.3 &  & 5582 & 4.40 & $-$0.24 & 4.5 & $-$2.8\\ 
K02010 & 6417 & 4.25 & $-$0.02 & 10.0 &  & 6424 & 4.28 & $-$0.00 & 10.0 &  & 6409 & 4.22 & $-$0.03 & 11.0 & $+$11.6\\ 
K02011 & 6421 & 4.38 & $-$0.03 & 15.2 &  & 6444 & 4.43 & $-$0.03 & 15.2 &  & 6398 & 4.33 & $-$0.03 & 16.3 & $-$25.3\\ 
K02012 & 5738 & 4.60 & $+$0.12 & 3.3 &  & 5738 & 4.60 & $+$0.12 & 3.3 &  & \nodata & \nodata & \nodata & \nodata & $-$26.1\\ 
K02016 & 5909 & 4.18 & $+$0.35 & 4.0 &  & 5885 & 4.12 & $+$0.34 & 4.0 &  & 5933 & 4.25 & $+$0.35 & 5.6 & $-$7.8\\ 
K02017 & 5682 & 4.62 & $+$0.06 & 3.9 &  & 5642 & 4.62 & $+$0.04 & 3.9 &  & 5722 & 4.63 & $+$0.08 & 5.5 & $-$3.3\\ 
K02022 & 5884 & 4.58 & $+$0.21 & 6.3 &  & 5884 & 4.58 & $+$0.21 & 6.3 &  & \nodata & \nodata & \nodata & \nodata & $-$22.4\\ 
K02026 & 5994 & 4.52 & $-$0.09 & 4.5 &  & 5997 & 4.50 & $-$0.10 & 4.5 &  & 5992 & 4.53 & $-$0.08 & 6.0 & $-$6.6\\ 
K02029 & 5224 & 4.71 & $-$0.11 & 3.0 &  & 5216 & 4.77 & $-$0.11 & 3.0 &  & 5232 & 4.65 & $-$0.11 & 5.0 & $-$6.9\\ 
K02033 & 5051 & 4.53 & $-$0.12 & 1.6 &  & 5053 & 4.57 & $-$0.11 & 1.6 &  & 5049 & 4.48 & $-$0.14 & 4.3 & $-$10.0\\ 
K02035 & 5558 & 4.67 & $+$0.10 & 6.0 &  & 5508 & 4.65 & $+$0.07 & 6.0 &  & 5607 & 4.69 & $+$0.13 & 7.1 & $-$10.0\\ 
K02037 & 4883 & 4.64 & $+$0.21 & 4.0 &  & 4883 & 4.64 & $+$0.21 & 4.0 &  & \nodata & \nodata & \nodata & \nodata & $-$22.8\\ 
K02038 & 5520 & 4.55 & $+$0.12 & 2.1 &  & 5509 & 4.57 & $+$0.12 & 2.1 &  & 5531 & 4.53 & $+$0.12 & 4.5 & $-$15.2\\ 
K02039 & 5584 & 4.61 & $+$0.28 & 2.3 &  & 5584 & 4.61 & $+$0.28 & 2.3 &  & \nodata & \nodata & \nodata & \nodata & $-$41.5\\ 
K02040 & 5656 & 4.38 & $+$0.01 & 1.3 &  & 5666 & 4.39 & $+$0.02 & 1.3 &  & 5646 & 4.37 & $+$0.01 & 4.2 & $-$18.8\\ 
K02043 & 5816 & 4.23 & $+$0.01 & 2.4 &  & 5821 & 4.24 & $+$0.01 & 2.4 &  & 5812 & 4.21 & $+$0.02 & 5.1 & $-$52.0\\ 
K02044 & 5684 & 4.50 & $+$0.19 & 2.0 &  & 5670 & 4.45 & $+$0.20 & 2.0 &  & 5698 & 4.56 & $+$0.17 & 4.1 & $+$6.6\\ 
K02046 & 5579 & 4.07 & $+$0.23 & 2.7 &  & 5566 & 3.96 & $+$0.22 & 2.7 &  & 5592 & 4.18 & $+$0.24 & 4.8 & $+$0.1\\ 
K02047 & 6090 & 4.37 & $-$0.05 & 5.3 &  & 6187 & 4.38 & $-$0.02 & 5.3 &  & 5994 & 4.35 & $-$0.08 & 6.9 & $-$42.2\\ 
K02048 & 5167 & 4.66 & $+$0.15 & 2.8 &  & 5167 & 4.66 & $+$0.15 & 2.8 &  & \nodata & \nodata & \nodata & \nodata & $+$0.0\\ 
K02049 & 6004 & 4.19 & $+$0.09 & 4.1 &  & 5967 & 4.15 & $+$0.07 & 4.1 &  & 6042 & 4.24 & $+$0.11 & 5.7 & $-$19.6\\ 
K02051 & 5769 & 4.30 & $-$0.06 & 1.4 &  & 5769 & 4.30 & $-$0.06 & 1.4 &  & \nodata & \nodata & \nodata & \nodata & $-$42.1\\ 
K02053 & 6140 & 4.25 & $+$0.05 & 6.8 &  & 6148 & 4.24 & $+$0.06 & 6.8 &  & 6132 & 4.27 & $+$0.04 & 8.0 & $-$41.6\\ 
K02071 & 5273 & 4.49 & $+$0.18 & 1.7 &  & 5266 & 4.50 & $+$0.17 & 1.7 &  & 5279 & 4.48 & $+$0.19 & 4.4 & $-$10.6\\ 
K02072 & 5847 & 4.15 & $-$0.13 & 1.6 &  & 5806 & 4.14 & $-$0.16 & 1.6 &  & 5887 & 4.15 & $-$0.09 & 4.9 & $-$24.1\\ 
K02073 & 4935 & 4.59 & $+$0.06 & 1.8 &  & 4935 & 4.59 & $+$0.06 & 1.8 &  & \nodata & \nodata & \nodata & \nodata & $+$3.9\\ 
K02076 & 5856 & 4.30 & $+$0.22 & 1.9 &  & 5856 & 4.30 & $+$0.22 & 1.9 &  & \nodata & \nodata & \nodata & \nodata & $-$4.6\\ 
K02079 & 5476 & 4.39 & $+$0.40 & 1.6 &  & 5467 & 4.34 & $+$0.39 & 1.6 &  & 5486 & 4.44 & $+$0.41 & 4.4 & $-$44.8\\ 
K02081 & 5078 & 3.57 & $+$0.18 & 2.8 &  & 5075 & 3.59 & $+$0.19 & 2.8 &  & 5080 & 3.55 & $+$0.17 & 4.9 & $-$14.4\\ 
K02082 & 6005 & 4.23 & $+$0.32 & 3.9 &  & 6011 & 4.16 & $+$0.34 & 3.9 &  & 5998 & 4.29 & $+$0.31 & 5.5 & $-$31.3\\ 
K02083 & 6033 & 4.37 & $-$0.03 & 5.6 &  & 6020 & 4.41 & $-$0.05 & 5.6 &  & 6046 & 4.33 & $-$0.02 & 7.0 & $-$18.2\\ 
K02086 & 5834 & 4.11 & $-$0.04 & 3.0 &  & 5819 & 4.01 & $-$0.05 & 3.0 &  & 5849 & 4.20 & $-$0.03 & 4.9 & $-$35.4\\ 
K02087 & 5943 & 4.45 & $+$0.01 & 3.6 &  & 5983 & 4.46 & $+$0.03 & 3.6 &  & 5903 & 4.43 & $-$0.00 & 5.2 & $-$16.6\\ 
K02092 & 5585 & 4.50 & $-$0.29 & 1.0 &  & 5585 & 4.50 & $-$0.29 & 1.0 &  & \nodata & \nodata & \nodata & \nodata & $+$5.8\\ 
K02093 & 5958 & 4.36 & $+$0.02 & 3.4 &  & 5958 & 4.36 & $+$0.02 & 3.4 &  & \nodata & \nodata & \nodata & \nodata & $+$0.6\\ 
K02094 & 5325 & 4.71 & $+$0.01 & 2.2 &  & 5325 & 4.71 & $+$0.01 & 2.2 &  & \nodata & \nodata & \nodata & \nodata & $-$19.7\\ 
K02098 & 6314 & 4.26 & $-$0.14 & 11.4 &  & 6296 & 4.32 & $-$0.13 & 11.4 &  & 6332 & 4.20 & $-$0.15 & 12.5 & $-$5.7\\ 
K02105 & 5882 & 4.39 & $-$0.06 & 2.6 &  & 5920 & 4.41 & $-$0.05 & 2.6 &  & 5845 & 4.38 & $-$0.07 & 4.8 & $-$5.0\\ 
K02109 & 6085 & 4.09 & $+$0.07 & 7.4 &  & 6018 & 4.07 & $+$0.04 & 7.4 &  & 6151 & 4.12 & $+$0.11 & 8.5 & $-$41.0\\ 
K02110 & 6386 & 4.26 & $+$0.21 & 16.4 &  & 6391 & 4.27 & $+$0.23 & 16.4 &  & 6381 & 4.25 & $+$0.19 & 17.7 & $-$32.9\\ 
K02111 & 5604 & 4.59 & $+$0.15 & 3.7 &  & 5604 & 4.59 & $+$0.15 & 3.7 &  & \nodata & \nodata & \nodata & \nodata & $-$18.3\\ 
K02115 & 5238 & 4.71 & $+$0.13 & 2.7 &  & 5219 & 4.73 & $+$0.08 & 2.7 &  & 5258 & 4.68 & $+$0.18 & 4.7 & $+$8.2\\ 
K02119 & 5137 & 4.59 & $+$0.20 & 3.6 &  & 5097 & 4.59 & $+$0.18 & 3.6 &  & 5177 & 4.60 & $+$0.21 & 5.0 & $-$14.1\\ 
K02120 & 5027 & 4.63 & $-$0.07 & 2.7 &  & 5025 & 4.69 & $-$0.05 & 2.7 &  & 5030 & 4.56 & $-$0.09 & 4.5 & $-$50.2\\ 
K02135 & 6145 & 4.17 & $+$0.04 & 7.6 &  & 6161 & 4.20 & $+$0.05 & 7.6 &  & 6129 & 4.14 & $+$0.03 & 8.5 & $+$10.1\\ 
K02137 & 5269 & 4.55 & $-$0.13 & 1.4 &  & 5290 & 4.59 & $-$0.12 & 1.4 &  & 5248 & 4.51 & $-$0.15 & 4.2 & $-$3.5\\ 
K02143 & 5429 & 4.48 & $+$0.22 & 2.3 &  & 5435 & 4.46 & $+$0.23 & 2.3 &  & 5422 & 4.50 & $+$0.21 & 4.5 & $-$26.6\\ 
K02147 & 5626 & 4.42 & $-$0.12 & 2.0 &  & 5626 & 4.42 & $-$0.12 & 2.0 &  & \nodata & \nodata & \nodata & \nodata & $-$2.8\\ 
K02148 & 5648 & 4.00 & $+$0.44 & 3.2 &  & 5610 & 3.92 & $+$0.42 & 3.2 &  & 5687 & 4.09 & $+$0.47 & 4.9 & $-$70.6\\ 
K02149 & 6213 & 4.21 & $+$0.20 & 8.8 &  & 6204 & 4.21 & $+$0.21 & 8.8 &  & 6221 & 4.20 & $+$0.18 & 9.7 & $-$36.4\\ 
K02153 & 6090 & 4.25 & $-$0.04 & 5.8 &  & 6033 & 4.21 & $-$0.06 & 5.8 &  & 6147 & 4.30 & $-$0.02 & 6.8 & $-$7.0\\ 
K02158 & 5330 & 4.35 & $+$0.00 & 1.8 &  & 5354 & 4.32 & $+$0.02 & 1.8 &  & 5307 & 4.37 & $-$0.02 & 4.4 & $-$91.1\\ 
K02159 & 5761 & 4.42 & $+$0.12 & 2.4 &  & 5760 & 4.45 & $+$0.12 & 2.4 &  & 5761 & 4.40 & $+$0.13 & 4.7 & $-$159.0\\ 
K02162 & 5644 & 4.49 & $-$0.41 & 1.4 &  & 5670 & 4.53 & $-$0.44 & 1.4 &  & 5619 & 4.44 & $-$0.38 & 4.4 & $-$65.7\\ 
K02167 & 5707 & 4.53 & $+$0.11 & 3.1 &  & 5707 & 4.53 & $+$0.11 & 3.1 &  & \nodata & \nodata & \nodata & \nodata & $+$14.1\\ 
K02168 & 5938 & 4.31 & $-$0.06 & 3.7 &  & 5938 & 4.31 & $-$0.06 & 3.7 &  & \nodata & \nodata & \nodata & \nodata & $-$45.8\\ 
K02169 & 5402 & 4.54 & $+$0.18 & 0.3 &  & 5396 & 4.53 & $+$0.18 & 0.3 &  & 5407 & 4.55 & $+$0.19 & 4.6 & $+$7.0\\ 
K02173 & 4859 & 4.70 & $+$0.11 & 3.2 &  & 4799 & 4.64 & $+$0.10 & 3.2 &  & 4919 & 4.76 & $+$0.12 & 4.6 & $-$23.0\\ 
K02175 & 5459 & 3.91 & $+$0.13 & 3.0 &  & 5424 & 3.89 & $+$0.10 & 3.0 &  & 5494 & 3.92 & $+$0.15 & 4.9 & $+$1.3\\ 
K02183 & 5649 & 4.41 & $+$0.12 & 0.3 &  & 5649 & 4.41 & $+$0.12 & 0.3 &  & \nodata & \nodata & \nodata & \nodata & $-$35.4\\ 
K02188 & 5640 & 4.50 & $-$0.57 & 0.0 &  & 5640 & 4.50 & $-$0.57 & 0.0 &  & \nodata & \nodata & \nodata & \nodata & $-$184.0\\ 
K02194 & 5710 & 4.19 & $-$0.21 & 2.0 &  & 5758 & 4.17 & $-$0.21 & 2.0 &  & 5661 & 4.22 & $-$0.21 & 4.8 & $+$22.2\\ 
K02195 & 6121 & 4.24 & $-$0.13 & 5.0 &  & 6121 & 4.24 & $-$0.13 & 5.0 &  & \nodata & \nodata & \nodata & \nodata & $-$28.2\\ 
K02201 & 6120 & 4.14 & $+$0.20 & 7.4 &  & 6090 & 4.13 & $+$0.20 & 7.4 &  & 6150 & 4.16 & $+$0.20 & 8.4 & $-$6.8\\ 
K02202 & 5310 & 4.51 & $+$0.34 & 2.5 &  & 5306 & 4.45 & $+$0.35 & 2.5 &  & 5313 & 4.57 & $+$0.33 & 4.6 & $-$10.5\\ 
K02208 & 5837 & 4.27 & $+$0.10 & 3.3 &  & 5846 & 4.25 & $+$0.10 & 3.3 &  & 5828 & 4.29 & $+$0.10 & 5.1 & $-$56.6\\ 
K02218 & 5602 & 4.47 & $+$0.14 & 3.0 &  & 5602 & 4.47 & $+$0.14 & 3.0 &  & \nodata & \nodata & \nodata & \nodata & $-$5.3\\ 
K02219 & 4996 & 4.53 & $+$0.14 & 1.7 &  & 4996 & 4.56 & $+$0.15 & 1.7 &  & 4996 & 4.51 & $+$0.14 & 4.3 & $-$13.8\\ 
K02220 & 5730 & 4.17 & $+$0.15 & 2.4 &  & 5730 & 4.17 & $+$0.15 & 2.4 &  & \nodata & \nodata & \nodata & \nodata & $+$5.6\\ 
K02228 & 6656 & 4.19 & $-$0.10 & 12.7 &  & 6631 & 4.36 & $-$0.10 & 12.7 &  & 6682 & 4.02 & $-$0.10 & 14.0 & $-$11.9\\ 
K02236 & 5483 & 4.40 & $-$0.03 & 0.5 &  & 5483 & 4.40 & $-$0.03 & 0.5 &  & \nodata & \nodata & \nodata & \nodata & $-$22.4\\ 
K02246 & 5667 & 4.50 & $-$0.19 & 0.8 &  & 5726 & 4.54 & $-$0.18 & 0.8 &  & 5609 & 4.45 & $-$0.20 & 4.4 & $-$27.9\\ 
K02248 & 5148 & 4.57 & $+$0.12 & 2.9 &  & 5213 & 4.67 & $+$0.13 & 2.9 &  & 5084 & 4.48 & $+$0.11 & 5.0 & $-$19.9\\ 
K02250 & 4958 & 4.63 & $+$0.13 & 2.8 &  & 4958 & 4.63 & $+$0.13 & 2.8 &  & \nodata & \nodata & \nodata & \nodata & $-$66.4\\ 
K02252 & 6184 & 4.03 & $+$0.10 & 7.6 &  & 6109 & 4.01 & $+$0.08 & 7.6 &  & 6259 & 4.05 & $+$0.12 & 8.5 & $-$23.5\\ 
K02260 & 6208 & 4.21 & $+$0.02 & 7.9 &  & 6183 & 4.22 & $+$0.01 & 7.9 &  & 6233 & 4.20 & $+$0.04 & 9.1 & $-$45.7\\ 
K02261 & 5176 & 4.70 & $+$0.06 & 3.1 &  & 5155 & 4.70 & $+$0.06 & 3.1 &  & 5197 & 4.69 & $+$0.06 & 4.9 & $-$20.8\\ 
K02273 & 6028 & 4.27 & $+$0.23 & 4.5 &  & 6038 & 4.25 & $+$0.25 & 4.5 &  & 6018 & 4.30 & $+$0.21 & 5.9 & $-$54.9\\ 
K02278 & 5846 & 4.10 & $-$0.12 & 2.6 &  & 5860 & 4.09 & $-$0.13 & 2.6 &  & 5832 & 4.12 & $-$0.11 & 4.7 & $-$54.8\\ 
K02279 & 5924 & 4.27 & $+$0.05 & 2.6 &  & 5952 & 4.25 & $+$0.05 & 2.6 &  & 5897 & 4.28 & $+$0.04 & 4.8 & $-$12.9\\ 
K02281 & 5076 & 4.53 & $+$0.17 & 1.9 &  & 5062 & 4.53 & $+$0.17 & 1.9 &  & 5090 & 4.53 & $+$0.16 & 4.3 & $+$3.5\\ 
K02287 & 4695 & 4.52 & $+$0.03 & 3.4 &  & 4695 & 4.52 & $+$0.03 & 3.4 &  & 5124 & 3.30 & $-$0.54 & 8.5 & $-$61.8\\ 
K02289 & 6060 & 4.32 & $+$0.09 & 4.9 &  & 6045 & 4.27 & $+$0.09 & 4.9 &  & 6076 & 4.36 & $+$0.08 & 6.2 & $-$10.1\\ 
K02290 & 4966 & 4.70 & $-$0.24 & 1.7 &  & 4966 & 4.70 & $-$0.24 & 1.7 &  & \nodata & \nodata & \nodata & \nodata & $-$34.0\\ 
K02295 & 5430 & 4.53 & $-$0.12 & 4.1 &  & 5422 & 4.54 & $-$0.13 & 4.1 &  & 5437 & 4.52 & $-$0.11 & 5.9 & $-$16.3\\ 
K02300 & 5133 & 4.63 & $-$0.12 & 1.0 &  & 5142 & 4.70 & $-$0.10 & 1.0 &  & 5124 & 4.57 & $-$0.13 & 4.2 & $-$27.0\\ 
K02312 & 6328 & 3.91 & $-$0.28 & 6.5 &  & 6257 & 3.87 & $-$0.33 & 6.5 &  & 6399 & 3.95 & $-$0.22 & 7.8 & $-$13.9\\ 
K02319 & 6097 & 4.31 & $-$0.02 & 4.7 &  & 6086 & 4.30 & $-$0.03 & 4.7 &  & 6109 & 4.33 & $-$0.01 & 6.1 & $-$5.2\\ 
K02331 & 5851 & 4.15 & $+$0.09 & 3.6 &  & 5853 & 4.13 & $+$0.10 & 3.6 &  & 5849 & 4.16 & $+$0.08 & 5.2 & $-$12.7\\ 
K02332 & 5190 & 3.86 & $-$0.05 & 2.3 &  & 5193 & 3.81 & $-$0.04 & 2.3 &  & 5186 & 3.90 & $-$0.06 & 4.5 & $-$54.2\\ 
K02333 & 6031 & 4.29 & $-$0.16 & 3.7 &  & 6072 & 4.34 & $-$0.16 & 3.7 &  & 5990 & 4.24 & $-$0.16 & 5.5 & $-$9.1\\ 
K02335 & 5566 & 4.41 & $+$0.01 & 1.8 &  & 5560 & 4.43 & $-$0.01 & 1.8 &  & 5572 & 4.39 & $+$0.03 & 4.5 & $-$6.9\\ 
K02339 & 4762 & 4.57 & $+$0.17 & 3.9 &  & 4762 & 4.57 & $+$0.17 & 3.9 &  & \nodata & \nodata & \nodata & \nodata & $-$21.0\\ 
K02342 & 5843 & 4.25 & $-$0.38 & 2.3 &  & 5883 & 4.29 & $-$0.39 & 2.3 &  & 5804 & 4.20 & $-$0.37 & 5.0 & $-$43.7\\ 
K02352 & 6346 & 4.19 & $-$0.16 & 7.2 &  & 6374 & 4.28 & $-$0.15 & 7.2 &  & 6319 & 4.10 & $-$0.16 & 8.6 & $-$3.2\\ 
K02357 & 5640 & 4.21 & $+$0.03 & 1.2 &  & 5640 & 4.21 & $+$0.03 & 1.2 &  & \nodata & \nodata & \nodata & \nodata & $-$11.3\\ 
K02358 & 6282 & 4.13 & $+$0.21 & 13.6 &  & 6284 & 4.16 & $+$0.21 & 13.6 &  & 6280 & 4.10 & $+$0.20 & 14.7 & $-$43.6\\ 
K02365 & 5936 & 4.18 & $+$0.20 & 3.7 &  & 5948 & 4.16 & $+$0.21 & 3.7 &  & 5923 & 4.20 & $+$0.19 & 5.5 & $-$26.5\\ 
K02366 & 6150 & 4.33 & $+$0.00 & 6.6 &  & 6171 & 4.32 & $+$0.02 & 6.6 &  & 6130 & 4.33 & $-$0.01 & 7.6 & $-$27.5\\ 
K02367 & 6065 & 4.14 & $+$0.16 & 6.3 &  & 6049 & 4.13 & $+$0.15 & 6.3 &  & 6080 & 4.14 & $+$0.17 & 7.4 & $-$9.8\\ 
K02369 & 5787 & 4.16 & $+$0.10 & 2.9 &  & 5787 & 4.16 & $+$0.10 & 2.9 &  & \nodata & \nodata & \nodata & \nodata & $-$15.3\\ 
K02370 & 6447 & 4.39 & $-$0.13 & 19.1 &  & 6464 & 4.46 & $-$0.14 & 19.1 &  & 6430 & 4.32 & $-$0.11 & 20.4 & $+$14.7\\ 
K02372 & 5941 & 4.12 & $-$0.08 & 3.9 &  & 5965 & 4.17 & $-$0.09 & 3.9 &  & 5916 & 4.07 & $-$0.07 & 5.8 & $-$54.7\\ 
K02374 & 5719 & 4.33 & $+$0.13 & 2.3 &  & 5719 & 4.33 & $+$0.13 & 2.3 &  & \nodata & \nodata & \nodata & \nodata & $-$54.7\\ 
K02389 & 5832 & 4.10 & $-$0.06 & 2.4 &  & 5829 & 4.05 & $-$0.08 & 2.4 &  & 5835 & 4.14 & $-$0.05 & 4.7 & $-$5.9\\ 
K02390 & 6003 & 3.92 & $+$0.14 & 5.5 &  & 5943 & 3.91 & $+$0.12 & 5.5 &  & 6062 & 3.94 & $+$0.16 & 6.6 & $+$5.0\\ 
K02393 & 4835 & 4.63 & $-$0.07 & 1.1 &  & 4835 & 4.63 & $-$0.07 & 1.1 &  & \nodata & \nodata & \nodata & \nodata & $+$3.6\\ 
K02396 & 5230 & 4.60 & $+$0.10 & 1.4 &  & 5230 & 4.60 & $+$0.10 & 1.4 &  & \nodata & \nodata & \nodata & \nodata & $-$9.2\\ 
K02398 & 6165 & 4.15 & $-$0.30 & 8.2 &  & 6151 & 4.23 & $-$0.32 & 8.2 &  & 6180 & 4.06 & $-$0.28 & 9.2 & $-$8.7\\ 
K02399 & 5065 & 4.59 & $-$0.06 & 1.5 &  & 5053 & 4.61 & $-$0.06 & 1.5 &  & 5078 & 4.56 & $-$0.07 & 4.2 & $-$19.0\\ 
K02403 & 6125 & 4.32 & $+$0.14 & 5.3 &  & 6184 & 4.37 & $+$0.18 & 5.3 &  & 6067 & 4.28 & $+$0.10 & 6.9 & $-$26.9\\ 
K02407 & 6000 & 4.18 & $+$0.20 & 5.2 &  & 5956 & 4.11 & $+$0.19 & 5.2 &  & 6044 & 4.25 & $+$0.20 & 6.3 & $+$0.9\\ 
K02408 & 5485 & 4.50 & $-$0.07 & 1.5 &  & 5480 & 4.49 & $-$0.08 & 1.5 &  & 5490 & 4.52 & $-$0.06 & 4.2 & $+$18.9\\ 
K02409 & 4767 & 4.51 & $-$0.61 & 2.1 &  & 4767 & 4.51 & $-$0.61 & 2.1 &  & \nodata & \nodata & \nodata & \nodata & $-$86.5\\ 
K02410 & 5648 & 4.49 & $-$0.09 & 1.0 &  & 5648 & 4.49 & $-$0.09 & 1.0 &  & \nodata & \nodata & \nodata & \nodata & $-$11.3\\ 
K02414 & 5541 & 4.10 & $-$0.29 & 1.6 &  & 5580 & 4.06 & $-$0.29 & 1.6 &  & 5502 & 4.15 & $-$0.30 & 4.5 & $-$36.8\\ 
K02422 & 5214 & 4.60 & $-$0.02 & 1.3 &  & 5214 & 4.60 & $-$0.02 & 1.3 &  & \nodata & \nodata & \nodata & \nodata & $+$18.8\\ 
K02426 & 5327 & 4.33 & $+$0.08 & 1.1 &  & 5346 & 4.32 & $+$0.09 & 1.1 &  & 5308 & 4.34 & $+$0.08 & 4.4 & $+$19.3\\ 
K02433 & 5837 & 4.18 & $+$0.01 & 2.8 &  & 5837 & 4.18 & $+$0.01 & 2.8 &  & \nodata & \nodata & \nodata & \nodata & $-$4.6\\ 
K02440 & 5670 & 4.17 & $+$0.33 & 2.1 &  & 5672 & 4.12 & $+$0.33 & 2.1 &  & 5668 & 4.23 & $+$0.32 & 4.5 & $-$30.5\\ 
K02442 & 5058 & 4.59 & $+$0.06 & 1.9 &  & 5058 & 4.59 & $+$0.06 & 1.9 &  & \nodata & \nodata & \nodata & \nodata & $-$12.0\\ 
K02443 & 5789 & 4.31 & $-$0.30 & 1.3 &  & 5788 & 4.29 & $-$0.34 & 1.3 &  & 5790 & 4.33 & $-$0.26 & 4.6 & $-$24.5\\ 
K02462 & 5975 & 4.04 & $+$0.09 & 5.7 &  & 5961 & 4.01 & $+$0.06 & 5.7 &  & 5989 & 4.08 & $+$0.12 & 6.9 & $-$7.6\\ 
K02463 & 6069 & 4.25 & $+$0.19 & 5.8 &  & 6058 & 4.23 & $+$0.19 & 5.8 &  & 6081 & 4.26 & $+$0.19 & 7.0 & $+$5.6\\ 
K02469 & 4838 & 4.64 & $-$0.01 & 1.7 &  & 4838 & 4.64 & $-$0.01 & 1.7 &  & \nodata & \nodata & \nodata & \nodata & $-$37.8\\ 
K02470 & 5847 & 4.22 & $+$0.30 & 3.0 &  & 5858 & 4.19 & $+$0.31 & 3.0 &  & 5836 & 4.24 & $+$0.29 & 4.9 & $-$9.0\\ 
K02473 & 5072 & 4.65 & $-$0.10 & 0.9 &  & 5072 & 4.65 & $-$0.10 & 0.9 &  & \nodata & \nodata & \nodata & \nodata & $-$56.9\\ 
K02474 & 5320 & 4.64 & $-$0.26 & 2.0 &  & 5326 & 4.70 & $-$0.27 & 2.0 &  & 5315 & 4.58 & $-$0.25 & 4.6 & $-$1.5\\ 
K02479 & 5372 & 3.88 & $+$0.08 & 2.9 &  & 5369 & 3.88 & $+$0.07 & 2.9 &  & 5375 & 3.87 & $+$0.08 & 4.7 & $+$26.3\\ 
K02481 & 4807 & 3.09 & $+$0.16 & 4.1 &  & 4682 & 2.90 & $+$0.11 & 4.1 &  & 4932 & 3.28 & $+$0.21 & 5.1 & $+$10.3\\ 
K02484 & 5711 & 4.20 & $-$0.33 & 1.8 &  & 5762 & 4.17 & $-$0.32 & 1.8 &  & 5660 & 4.23 & $-$0.33 & 4.7 & $-$44.7\\ 
K02486 & 6035 & 4.20 & $+$0.09 & 5.8 &  & 6035 & 4.17 & $+$0.09 & 5.8 &  & 6035 & 4.22 & $+$0.09 & 6.9 & $-$4.6\\ 
K02488 & 5994 & 4.13 & $-$0.01 & 5.0 &  & 5905 & 4.05 & $-$0.06 & 5.0 &  & 6082 & 4.21 & $+$0.04 & 6.0 & $+$16.7\\ 
K02492 & 5627 & 4.32 & $-$0.33 & 1.2 &  & 5654 & 4.21 & $-$0.33 & 1.2 &  & 5600 & 4.44 & $-$0.33 & 4.1 & $-$61.3\\ 
K02498 & 5128 & 4.48 & $-$0.11 & 1.8 &  & 5131 & 4.50 & $-$0.10 & 1.8 &  & 5125 & 4.46 & $-$0.13 & 4.2 & $-$49.2\\ 
K02503 & 4885 & 4.51 & $+$0.18 & 2.1 &  & 4885 & 4.51 & $+$0.18 & 2.1 &  & 4776 & 4.18 & $-$0.20 & 4.3 & $-$11.7\\ 
K02516 & 5431 & 3.91 & $+$0.30 & 2.6 &  & 5422 & 3.90 & $+$0.29 & 2.6 &  & 5441 & 3.91 & $+$0.32 & 5.0 & $-$50.5\\ 
K02517 & 5606 & 4.63 & $-$0.08 & 1.1 &  & 5606 & 4.63 & $-$0.08 & 1.1 &  & \nodata & \nodata & \nodata & \nodata & $+$9.8\\ 
K02521 & 4976 & 4.68 & $-$0.24 & 1.4 &  & 4976 & 4.68 & $-$0.24 & 1.4 &  & \nodata & \nodata & \nodata & \nodata & $+$3.4\\ 
K02522 & 4983 & 4.55 & $+$0.23 & 2.5 &  & 4944 & 4.52 & $+$0.25 & 2.5 &  & 5021 & 4.58 & $+$0.22 & 4.2 & $-$22.3\\ 
K02529 & 4734 & 4.79 & $-$0.09 & 3.2 &  & 4734 & 4.79 & $-$0.09 & 3.2 &  & \nodata & \nodata & \nodata & \nodata & $-$12.2\\ 
K02530 & 5937 & 4.01 & $+$0.15 & 4.5 &  & 5910 & 4.01 & $+$0.13 & 4.5 &  & 5964 & 4.00 & $+$0.16 & 5.7 & $-$27.2\\ 
K02533 & 5005 & 3.57 & $+$0.03 & 3.2 &  & 4959 & 3.57 & $+$0.01 & 3.2 &  & 5051 & 3.56 & $+$0.06 & 4.7 & $+$14.5\\ 
K02534 & 6099 & 4.34 & $+$0.02 & 4.4 &  & 6112 & 4.35 & $+$0.02 & 4.4 &  & 6086 & 4.33 & $+$0.03 & 6.1 & $-$4.8\\ 
K02538 & 4972 & 4.54 & $-$0.23 & 6.5 &  & 4962 & 4.60 & $-$0.23 & 6.5 &  & 4981 & 4.47 & $-$0.22 & 7.6 & $+$29.7\\ 
K02541 & 5090 & 3.70 & $+$0.15 & 2.9 &  & 5055 & 3.68 & $+$0.13 & 2.9 &  & 5126 & 3.73 & $+$0.16 & 4.7 & $+$21.4\\ 
K02545 & 6197 & 4.04 & $+$0.17 & 6.8 &  & 6120 & 3.99 & $+$0.15 & 6.8 &  & 6275 & 4.08 & $+$0.19 & 7.9 & $-$10.1\\ 
K02547 & 5925 & 4.36 & $-$0.13 & 2.2 &  & 5953 & 4.38 & $-$0.13 & 2.2 &  & 5897 & 4.35 & $-$0.14 & 4.5 & $+$26.7\\ 
K02555 & 6145 & 4.35 & $-$0.06 & 6.2 &  & 6151 & 4.35 & $-$0.08 & 6.2 &  & 6139 & 4.34 & $-$0.05 & 7.7 & $-$31.3\\ 
K02556 & 5478 & 4.53 & $-$0.17 & 1.3 &  & 5516 & 4.55 & $-$0.15 & 1.3 &  & 5440 & 4.50 & $-$0.18 & 4.2 & $-$42.9\\ 
K02559 & 5860 & 4.31 & $+$0.12 & 2.7 &  & 5876 & 4.30 & $+$0.14 & 2.7 &  & 5843 & 4.32 & $+$0.10 & 4.7 & $-$36.2\\ 
K02561 & 6010 & 4.18 & $+$0.03 & 4.2 &  & 5984 & 4.14 & $+$0.02 & 4.2 &  & 6036 & 4.21 & $+$0.03 & 5.5 & $-$16.6\\ 
K02563 & 6174 & 4.03 & $+$0.12 & 7.5 &  & 6130 & 4.00 & $+$0.12 & 7.5 &  & 6217 & 4.06 & $+$0.13 & 8.6 & $+$8.5\\ 
K02564 & 6137 & 4.09 & $-$0.11 & 9.1 &  & 6079 & 4.03 & $-$0.14 & 9.1 &  & 6194 & 4.15 & $-$0.09 & 9.9 & $-$13.3\\ 
K02571 & 5268 & 4.50 & $+$0.26 & 6.1 &  & 5268 & 4.50 & $+$0.26 & 6.1 &  & \nodata & \nodata & \nodata & \nodata & $-$13.8\\ 
K02581 & 5483 & 4.46 & $+$0.28 & 2.1 &  & 5498 & 4.44 & $+$0.28 & 2.1 &  & 5468 & 4.48 & $+$0.28 & 4.5 & $+$1.5\\ 
K02582 & 5857 & 4.16 & $+$0.30 & 3.5 &  & 5876 & 4.12 & $+$0.31 & 3.5 &  & 5838 & 4.20 & $+$0.28 & 5.0 & $-$30.5\\ 
K02583 & 5605 & 4.40 & $+$0.11 & 0.4 &  & 5609 & 4.40 & $+$0.11 & 0.4 &  & 5602 & 4.40 & $+$0.11 & 3.9 & $-$27.3\\ 
K02585 & 5951 & 4.38 & $-$0.35 & 1.8 &  & 6008 & 4.44 & $-$0.36 & 1.8 &  & 5894 & 4.33 & $-$0.35 & 4.6 & $-$70.8\\ 
K02590 & 6206 & 4.00 & $-$0.01 & 10.2 &  & 6134 & 3.97 & $-$0.02 & 10.2 &  & 6278 & 4.02 & $+$0.00 & 10.9 & $-$1.9\\ 
K02593 & 6213 & 4.26 & $+$0.19 & 7.4 &  & 6225 & 4.27 & $+$0.22 & 7.4 &  & 6200 & 4.25 & $+$0.17 & 8.4 & $-$3.5\\ 
K02595 & 6330 & 4.29 & $+$0.05 & 14.4 &  & 6331 & 4.31 & $+$0.04 & 14.4 &  & 6329 & 4.28 & $+$0.05 & 15.3 & $-$21.5\\ 
K02597 & 5871 & 4.48 & $-$0.30 & 2.0 &  & 5871 & 4.48 & $-$0.30 & 2.0 &  & \nodata & \nodata & \nodata & \nodata & $-$7.4\\ 
K02603 & 6278 & 4.09 & $-$0.05 & 9.7 &  & 6202 & 4.13 & $-$0.09 & 9.7 &  & 6353 & 4.06 & $-$0.01 & 10.7 & $+$7.2\\ 
K02607 & 5776 & 4.42 & $+$0.21 & 3.1 &  & 5776 & 4.42 & $+$0.21 & 3.1 &  & \nodata & \nodata & \nodata & \nodata & $-$17.8\\ 
K02608 & 6431 & 4.34 & $+$0.03 & 18.1 &  & 6424 & 4.40 & $+$0.06 & 18.1 &  & 6439 & 4.28 & $+$0.00 & 18.7 & $-$24.6\\ 
K02612 & 5544 & 4.27 & $+$0.32 & 2.4 &  & 5544 & 4.27 & $+$0.32 & 2.4 &  & \nodata & \nodata & \nodata & \nodata & $-$19.0\\ 
K02623 & 6219 & 4.13 & $+$0.13 & 7.2 &  & 6175 & 4.10 & $+$0.12 & 7.2 &  & 6263 & 4.17 & $+$0.13 & 8.0 & $-$40.3\\ 
K02631 & 5754 & 4.18 & $-$0.40 & 2.2 &  & 5757 & 4.18 & $-$0.44 & 2.2 &  & 5752 & 4.18 & $-$0.37 & 4.8 & $-$27.1\\ 
K02632 & 6238 & 4.06 & $-$0.02 & 10.3 &  & 6164 & 4.00 & $-$0.04 & 10.3 &  & 6312 & 4.11 & $-$0.00 & 11.0 & $-$31.5\\ 
K02635 & 6021 & 4.01 & $-$0.15 & 7.0 &  & 6052 & 4.09 & $-$0.14 & 7.0 &  & 5990 & 3.94 & $-$0.16 & 8.3 & $-$30.1\\ 
K02636 & 5858 & 4.40 & $+$0.07 & 3.0 &  & 5890 & 4.46 & $+$0.09 & 3.0 &  & 5825 & 4.35 & $+$0.05 & 5.4 & $-$17.7\\ 
K02639 & 5583 & 3.89 & $-$0.02 & 2.5 &  & 5583 & 3.89 & $-$0.02 & 2.5 &  & \nodata & \nodata & \nodata & \nodata & $-$36.7\\ 
K02640 & 4895 & 3.03 & $-$0.13 & 3.6 &  & 4836 & 2.97 & $-$0.21 & 3.6 &  & 4955 & 3.08 & $-$0.06 & 5.1 & $-$64.7\\ 
K02641 & 5797 & 4.07 & $-$0.00 & 2.9 &  & 5800 & 4.04 & $-$0.00 & 2.9 &  & 5793 & 4.10 & $-$0.00 & 4.9 & $-$32.7\\ 
K02657 & 5434 & 4.50 & $-$0.15 & 0.8 &  & 5470 & 4.54 & $-$0.13 & 0.8 &  & 5398 & 4.46 & $-$0.17 & 4.2 & $-$35.1\\ 
K02659 & 5077 & 3.40 & $+$0.24 & 2.9 &  & 5033 & 3.51 & $+$0.24 & 2.9 &  & 5121 & 3.29 & $+$0.24 & 5.0 & $+$3.1\\ 
K02668 & 5463 & 4.57 & $-$0.04 & 1.1 &  & 5490 & 4.59 & $-$0.02 & 1.1 &  & 5437 & 4.54 & $-$0.07 & 4.4 & $-$11.6\\ 
K02672 & 5656 & 4.57 & $+$0.18 & 3.6 &  & 5649 & 4.56 & $+$0.18 & 3.6 &  & 5663 & 4.57 & $+$0.19 & 5.3 & $-$14.5\\ 
K02674 & 5754 & 4.06 & $+$0.10 & 1.8 &  & 5701 & 4.01 & $+$0.07 & 1.8 &  & 5807 & 4.11 & $+$0.13 & 4.4 & $-$13.9\\ 
K02675 & 5756 & 4.63 & $+$0.13 & 7.7 &  & 5723 & 4.61 & $+$0.11 & 7.7 &  & 5789 & 4.66 & $+$0.15 & 8.7 & $-$8.4\\ 
K02676 & 6329 & 3.97 & $-$0.07 & 4.6 &  & 6211 & 3.95 & $-$0.11 & 4.6 &  & 6448 & 4.00 & $-$0.03 & 6.0 & $-$24.5\\ 
K02677 & 6130 & 4.05 & $+$0.03 & 6.6 &  & 6115 & 4.04 & $+$0.04 & 6.6 &  & 6145 & 4.05 & $+$0.02 & 7.5 & $+$9.0\\ 
K02678 & 5416 & 4.70 & $+$0.12 & 6.8 &  & 5372 & 4.69 & $+$0.08 & 6.8 &  & 5459 & 4.72 & $+$0.15 & 7.8 & $-$29.5\\ 
K02681 & 5316 & 4.59 & $-$0.06 & 1.7 &  & 5316 & 4.59 & $-$0.06 & 1.7 &  & \nodata & \nodata & \nodata & \nodata & $-$35.0\\ 
K02686 & 4713 & 4.62 & $-$0.05 & 2.6 &  & 4684 & 4.59 & $-$0.03 & 2.6 &  & 4742 & 4.64 & $-$0.07 & 4.5 & $-$6.2\\ 
K02687 & 5788 & 4.51 & $+$0.07 & 2.3 &  & 5765 & 4.49 & $+$0.05 & 2.3 &  & 5812 & 4.54 & $+$0.08 & 5.0 & $+$10.2\\ 
K02690 & 5516 & 4.66 & $+$0.14 & 3.7 &  & 5472 & 4.64 & $+$0.13 & 3.7 &  & 5561 & 4.69 & $+$0.15 & 5.2 & $-$11.2\\ 
K02694 & 4780 & 4.45 & $+$0.24 & 2.4 &  & 4780 & 4.45 & $+$0.24 & 2.4 &  & \nodata & \nodata & \nodata & \nodata & $-$10.9\\ 
K02698 & 5936 & 4.28 & $+$0.11 & 3.0 &  & 5943 & 4.28 & $+$0.12 & 3.0 &  & 5930 & 4.29 & $+$0.11 & 4.9 & $-$10.5\\ 
K02706 & 6337 & 4.18 & $+$0.11 & 10.8 &  & 6333 & 4.17 & $+$0.13 & 10.8 &  & 6340 & 4.18 & $+$0.09 & 11.4 & $-$35.9\\ 
K02707 & 5581 & 4.51 & $-$0.09 & 1.5 &  & 5581 & 4.51 & $-$0.09 & 1.5 &  & \nodata & \nodata & \nodata & \nodata & $-$13.2\\ 
K02711 & 5950 & 4.48 & $+$0.10 & 4.0 &  & 5945 & 4.50 & $+$0.09 & 4.0 &  & 5955 & 4.47 & $+$0.10 & 5.6 & $+$15.7\\ 
K02712 & 6354 & 4.19 & $+$0.26 & 13.2 &  & 6329 & 4.17 & $+$0.27 & 13.2 &  & 6380 & 4.20 & $+$0.24 & 14.1 & $-$19.5\\ 
K02714 & 6045 & 4.04 & $+$0.00 & 5.8 &  & 5972 & 4.01 & $-$0.03 & 5.8 &  & 6117 & 4.08 & $+$0.03 & 7.0 & $-$12.4\\ 
K02717 & 6063 & 4.30 & $+$0.00 & 4.6 &  & 6024 & 4.25 & $-$0.02 & 4.6 &  & 6102 & 4.35 & $+$0.02 & 6.0 & $+$2.2\\ 
K02720 & 5926 & 4.03 & $-$0.13 & 2.6 &  & 5941 & 4.07 & $-$0.13 & 2.6 &  & 5911 & 3.98 & $-$0.12 & 5.5 & $-$9.3\\ 
K02722 & 6119 & 4.38 & $-$0.05 & 6.3 &  & 6129 & 4.38 & $-$0.07 & 6.3 &  & 6109 & 4.39 & $-$0.04 & 7.7 & $+$0.7\\ 
K02729 & 5646 & 4.38 & $-$0.27 & 1.5 &  & 5613 & 4.28 & $-$0.31 & 1.5 &  & 5679 & 4.48 & $-$0.23 & 4.5 & $+$0.3\\ 
K02730 & 5597 & 4.16 & $-$0.02 & 2.0 &  & 5620 & 4.08 & $-$0.00 & 2.0 &  & 5574 & 4.24 & $-$0.05 & 4.5 & $-$57.3\\ 
K02732 & 6094 & 4.06 & $+$0.09 & 4.9 &  & 6082 & 4.06 & $+$0.08 & 4.9 &  & 6106 & 4.07 & $+$0.10 & 6.4 & $-$32.0\\ 
K02733 & 4849 & 4.72 & $+$0.04 & 3.7 &  & 4816 & 4.68 & $+$0.02 & 3.7 &  & 4883 & 4.75 & $+$0.05 & 5.2 & $+$7.2\\ 
K02737 & 5641 & 4.04 & $+$0.36 & 2.3 &  & 5665 & 4.02 & $+$0.37 & 2.3 &  & 5617 & 4.06 & $+$0.35 & 4.5 & $-$86.7\\ 
K02740 & 5988 & 4.27 & $-$0.27 & 6.8 &  & 6033 & 4.35 & $-$0.29 & 6.8 &  & 5943 & 4.19 & $-$0.26 & 8.3 & $-$28.7\\ 
K02741 & 5852 & 4.38 & $+$0.06 & 0.8 &  & 5875 & 4.39 & $+$0.07 & 0.8 &  & 5829 & 4.36 & $+$0.06 & 4.2 & $-$52.1\\ 
K02743 & 5581 & 4.57 & $-$0.01 & 1.0 &  & 5568 & 4.55 & $-$0.02 & 1.0 &  & 5594 & 4.59 & $+$0.00 & 4.2 & $-$33.0\\ 
K02748 & 5499 & 4.00 & $-$0.06 & 2.5 &  & 5463 & 3.91 & $-$0.09 & 2.5 &  & 5535 & 4.10 & $-$0.03 & 4.7 & $+$2.2\\ 
K02749 & 6260 & 4.06 & $+$0.02 & 9.5 &  & 6172 & 4.02 & $-$0.01 & 9.5 &  & 6347 & 4.10 & $+$0.05 & 10.4 & $-$26.5\\ 
K02750 & 5952 & 3.98 & $-$0.10 & 88.6 &  & 5952 & 3.98 & $-$0.10 & 88.6 &  & \nodata & \nodata & \nodata & \nodata & $+$19.9\\ 
K02752 & 6092 & 4.27 & $+$0.15 & 7.6 &  & 6057 & 4.22 & $+$0.13 & 7.6 &  & 6127 & 4.31 & $+$0.16 & 8.4 & $-$4.9\\ 
K02753 & 5834 & 4.17 & $+$0.22 & 2.3 &  & 5811 & 4.17 & $+$0.22 & 2.3 &  & 5857 & 4.17 & $+$0.22 & 4.6 & $+$6.8\\ 
K02754 & 5874 & 4.38 & $-$0.08 & 3.2 &  & 5894 & 4.41 & $-$0.09 & 3.2 &  & 5855 & 4.35 & $-$0.08 & 5.3 & $-$48.5\\ 
K02755 & 5741 & 4.44 & $-$0.15 & 2.2 &  & 5785 & 4.47 & $-$0.15 & 2.2 &  & 5698 & 4.41 & $-$0.16 & 4.7 & $-$23.1\\ 
K02756 & 5909 & 4.40 & $+$0.11 & 3.1 &  & 5909 & 4.40 & $+$0.11 & 3.1 &  & \nodata & \nodata & \nodata & \nodata & $-$29.1\\ 
K02758 & 5219 & 3.75 & $+$0.34 & 4.0 &  & 5210 & 3.72 & $+$0.35 & 4.0 &  & 5228 & 3.77 & $+$0.33 & 5.3 & $-$59.2\\ 
K02762 & 4683 & 4.42 & $+$0.28 & 2.5 &  & 4683 & 4.42 & $+$0.28 & 2.5 &  & \nodata & \nodata & \nodata & \nodata & $-$15.5\\ 
K02763 & 4725 & 4.62 & $-$0.01 & 2.9 &  & 4725 & 4.62 & $-$0.01 & 2.9 &  & \nodata & \nodata & \nodata & \nodata & $-$45.4\\ 
K02765 & 6230 & 4.06 & $+$0.09 & 3.4 &  & 6183 & 4.04 & $+$0.08 & 3.4 &  & 6278 & 4.08 & $+$0.11 & 5.1 & $+$4.4\\ 
K02768 & 5326 & 4.62 & $-$0.03 & 1.1 &  & 5326 & 4.62 & $-$0.03 & 1.1 &  & \nodata & \nodata & \nodata & \nodata & $-$30.0\\ 
K02769 & 5787 & 3.96 & $-$0.02 & 2.8 &  & 5767 & 3.96 & $-$0.05 & 2.8 &  & 5806 & 3.95 & $-$0.00 & 4.9 & $-$17.7\\ 
K02771 & 6165 & 4.44 & $-$0.06 & 4.2 &  & 6250 & 4.52 & $-$0.03 & 4.2 &  & 6080 & 4.36 & $-$0.09 & 6.1 & $-$17.6\\ 
K02781 & 5701 & 4.16 & $-$0.44 & 1.4 &  & 5734 & 4.12 & $-$0.45 & 1.4 &  & 5668 & 4.21 & $-$0.43 & 4.6 & $-$62.2\\ 
K02785 & 5815 & 4.31 & $-$0.00 & 2.4 &  & 5854 & 4.30 & $+$0.02 & 2.4 &  & 5776 & 4.33 & $-$0.02 & 4.6 & $-$3.5\\ 
K02786 & 6333 & 4.10 & $-$0.16 & 7.5 &  & 6364 & 4.27 & $-$0.13 & 7.5 &  & 6302 & 3.92 & $-$0.19 & 8.4 & $-$8.8\\ 
K02790 & 5103 & 4.37 & $-$0.22 & 1.6 &  & 5079 & 4.38 & $-$0.22 & 1.6 &  & 5127 & 4.35 & $-$0.21 & 4.5 & $-$28.4\\ 
K02792 & 5970 & 4.24 & $+$0.20 & 4.2 &  & 5975 & 4.17 & $+$0.22 & 4.2 &  & 5964 & 4.30 & $+$0.18 & 5.7 & $-$29.3\\ 
K02796 & 5687 & 4.34 & $-$0.01 & 1.8 &  & 5687 & 4.34 & $-$0.01 & 1.8 &  & \nodata & \nodata & \nodata & \nodata & $+$18.8\\ 
K02801 & 6057 & 4.14 & $+$0.04 & 3.6 &  & 6021 & 4.12 & $+$0.02 & 3.6 &  & 6093 & 4.16 & $+$0.05 & 5.1 & $+$7.9\\ 
K02803 & 5575 & 4.35 & $+$0.17 & 2.7 &  & 5591 & 4.36 & $+$0.17 & 2.7 &  & 5560 & 4.33 & $+$0.17 & 4.9 & $+$11.5\\ 
K02805 & 5870 & 4.28 & $-$0.22 & 1.7 &  & 5876 & 4.28 & $-$0.24 & 1.7 &  & 5864 & 4.27 & $-$0.19 & 4.4 & $-$42.0\\ 
K02807 & 6400 & 4.29 & $+$0.16 & 13.8 &  & 6407 & 4.33 & $+$0.18 & 13.8 &  & 6393 & 4.24 & $+$0.14 & 14.7 & $-$14.4\\ 
K02815 & 5876 & 4.28 & $-$0.05 & 1.9 &  & 5891 & 4.26 & $-$0.06 & 1.9 &  & 5861 & 4.30 & $-$0.05 & 4.6 & $-$30.8\\ 
K02828 & 4699 & 4.65 & $-$0.03 & 3.2 &  & 4699 & 4.65 & $-$0.03 & 3.2 &  & \nodata & \nodata & \nodata & \nodata & $-$14.4\\ 
K02829 & 5875 & 4.14 & $+$0.00 & 3.4 &  & 5880 & 4.11 & $+$0.00 & 3.4 &  & 5870 & 4.16 & $+$0.00 & 5.2 & $-$27.4\\ 
K02831 & 5752 & 3.92 & $-$0.01 & 4.5 &  & 5721 & 3.93 & $-$0.03 & 4.5 &  & 5784 & 3.92 & $+$0.01 & 5.9 & $-$22.0\\ 
K02832 & 5037 & 4.52 & $+$0.08 & 1.5 &  & 5040 & 4.53 & $+$0.11 & 1.5 &  & 5034 & 4.51 & $+$0.06 & 4.4 & $-$33.6\\ 
K02833 & 6193 & 4.38 & $-$0.19 & 5.0 &  & 6236 & 4.44 & $-$0.18 & 5.0 &  & 6150 & 4.32 & $-$0.20 & 6.4 & $+$11.6\\ 
K02838 & 5700 & 4.06 & $+$0.15 & 1.8 &  & 5685 & 4.01 & $+$0.15 & 1.8 &  & 5714 & 4.10 & $+$0.16 & 4.4 & $-$36.8\\ 
K02840 & 5621 & 4.01 & $-$0.03 & 1.8 &  & 5630 & 3.97 & $-$0.02 & 1.8 &  & 5613 & 4.05 & $-$0.04 & 4.4 & $-$15.9\\ 
K02841 & 5161 & 4.49 & $-$0.11 & 0.8 &  & 5161 & 4.49 & $-$0.11 & 0.8 &  & \nodata & \nodata & \nodata & \nodata & $-$13.9\\ 
K02848 & 5704 & 4.16 & $+$0.32 & 2.8 &  & 5723 & 4.13 & $+$0.33 & 2.8 &  & 5684 & 4.18 & $+$0.31 & 4.8 & $-$80.6\\ 
K02857 & 6190 & 4.17 & $+$0.22 & 6.3 &  & 6168 & 4.13 & $+$0.23 & 6.3 &  & 6213 & 4.20 & $+$0.21 & 7.4 & $-$12.2\\ 
K02859 & 5260 & 4.51 & $-$0.07 & 1.5 &  & 5259 & 4.53 & $-$0.07 & 1.5 &  & 5260 & 4.49 & $-$0.07 & 4.3 & $-$26.3\\ 
K02863 & 5660 & 4.36 & $-$0.25 & 0.7 &  & 5694 & 4.29 & $-$0.25 & 0.7 &  & 5625 & 4.43 & $-$0.24 & 4.2 & $-$61.6\\ 
K02864 & 5779 & 4.38 & $-$0.15 & 0.8 &  & 5812 & 4.42 & $-$0.13 & 0.8 &  & 5746 & 4.34 & $-$0.17 & 4.3 & $-$41.9\\ 
K02866 & 6280 & 4.28 & $+$0.07 & 5.4 &  & 6284 & 4.34 & $+$0.10 & 5.4 &  & 6275 & 4.22 & $+$0.05 & 7.1 & $-$7.7\\ 
K02874 & 5234 & 4.46 & $-$0.09 & 1.5 &  & 5268 & 4.52 & $-$0.06 & 1.5 &  & 5201 & 4.41 & $-$0.11 & 4.8 & $-$25.9\\ 
K02875 & 4966 & 4.61 & $-$0.10 & 2.1 &  & 4989 & 4.71 & $-$0.06 & 2.1 &  & 4942 & 4.51 & $-$0.14 & 4.8 & $-$12.4\\ 
K02879 & 5475 & 4.57 & $-$0.01 & 1.8 &  & 5458 & 4.58 & $-$0.01 & 1.8 &  & 5493 & 4.55 & $-$0.01 & 4.3 & $-$5.1\\ 
K02884 & 5729 & 3.91 & $-$0.00 & 3.5 &  & 5674 & 3.93 & $-$0.04 & 3.5 &  & 5785 & 3.88 & $+$0.03 & 5.1 & $-$38.4\\ 
K02885 & 5492 & 3.93 & $-$0.36 & 1.8 &  & 5492 & 3.95 & $-$0.40 & 1.8 &  & 5492 & 3.90 & $-$0.33 & 4.8 & $-$25.4\\ 
K02891 & 6142 & 4.02 & $+$0.14 & 5.7 &  & 6110 & 4.02 & $+$0.14 & 5.7 &  & 6174 & 4.03 & $+$0.15 & 7.0 & $-$23.1\\ 
K02896 & 6233 & 4.47 & $-$0.02 & 14.9 &  & 6179 & 4.45 & $-$0.03 & 14.9 &  & 6287 & 4.50 & $-$0.02 & 14.8 & $-$15.8\\ 
K02904 & 6139 & 4.01 & $+$0.29 & 7.5 &  & 6073 & 3.96 & $+$0.30 & 7.5 &  & 6205 & 4.07 & $+$0.29 & 8.4 & $-$37.4\\ 
K02906 & 6093 & 4.14 & $-$0.24 & 6.0 &  & 6086 & 4.14 & $-$0.28 & 6.0 &  & 6100 & 4.14 & $-$0.20 & 7.5 & $+$23.3\\ 
K02913 & 5727 & 4.18 & $+$0.32 & 2.2 &  & 5740 & 4.16 & $+$0.33 & 2.2 &  & 5714 & 4.20 & $+$0.31 & 4.6 & $-$11.7\\ 
K02915 & 5618 & 4.45 & $+$0.02 & 0.8 &  & 5613 & 4.43 & $+$0.01 & 0.8 &  & 5622 & 4.46 & $+$0.03 & 4.1 & $-$22.4\\ 
K02916 & 4973 & 4.54 & $-$0.01 & 1.8 &  & 4986 & 4.56 & $+$0.02 & 1.8 &  & 4959 & 4.52 & $-$0.03 & 4.7 & $+$4.8\\ 
K02925 & 5444 & 4.51 & $+$0.20 & 1.4 &  & 5448 & 4.49 & $+$0.19 & 1.4 &  & 5439 & 4.52 & $+$0.21 & 4.4 & $+$15.0\\ 
K02926 & 5052 & 3.52 & $-$0.50 & 2.4 &  & 5052 & 3.52 & $-$0.50 & 2.4 &  & \nodata & \nodata & \nodata & \nodata & $-$37.9\\ 
K02931 & 4962 & 4.65 & $-$0.11 & 2.2 &  & 4962 & 4.65 & $-$0.11 & 2.2 &  & \nodata & \nodata & \nodata & \nodata & $+$17.1\\ 
K02943 & 5781 & 4.07 & $+$0.34 & 2.7 &  & 5783 & 4.01 & $+$0.34 & 2.7 &  & 5780 & 4.12 & $+$0.33 & 4.8 & $-$12.7\\ 
K02949 & 5913 & 4.16 & $+$0.08 & 2.8 &  & 5896 & 4.11 & $+$0.07 & 2.8 &  & 5930 & 4.21 & $+$0.08 & 4.7 & $-$23.0\\ 
K02951 & 5602 & 4.49 & $-$0.17 & 2.3 &  & 5626 & 4.54 & $-$0.18 & 2.3 &  & 5578 & 4.44 & $-$0.16 & 4.9 & $+$23.1\\ 
K02956 & 6421 & 3.95 & $-$0.01 & 9.9 &  & 6333 & 3.87 & $-$0.03 & 9.9 &  & 6510 & 4.03 & $+$0.02 & 10.9 & $+$14.8\\ 
K02960 & 5913 & 4.21 & $+$0.07 & 3.0 &  & 5945 & 4.23 & $+$0.09 & 3.0 &  & 5882 & 4.19 & $+$0.05 & 5.2 & $-$41.1\\ 
K02961 & 6069 & 4.31 & $+$0.12 & 5.2 &  & 6076 & 4.27 & $+$0.12 & 5.2 &  & 6062 & 4.36 & $+$0.12 & 6.5 & $-$13.9\\ 
K02964 & 6123 & 4.16 & $-$0.33 & 8.2 &  & 6151 & 4.21 & $-$0.34 & 8.2 &  & 6095 & 4.12 & $-$0.32 & 9.4 & $-$24.4\\ 
K02968 & 6212 & 4.00 & $-$0.11 & 7.4 &  & 6165 & 4.03 & $-$0.14 & 7.4 &  & 6259 & 3.97 & $-$0.08 & 8.6 & $-$19.8\\ 
K02969 & 6024 & 4.05 & $+$0.19 & 5.2 &  & 5953 & 3.98 & $+$0.18 & 5.2 &  & 6094 & 4.13 & $+$0.21 & 6.2 & $+$3.8\\ 
K02970 & 6130 & 4.37 & $-$0.07 & 5.1 &  & 6154 & 4.36 & $-$0.07 & 5.1 &  & 6107 & 4.39 & $-$0.07 & 6.7 & $+$20.3\\ 
K02971 & 6273 & 4.20 & $+$0.18 & 14.9 &  & 6246 & 4.16 & $+$0.18 & 14.9 &  & 6301 & 4.24 & $+$0.19 & 15.6 & $+$7.5\\ 
K02974 & 6547 & 4.14 & $+$0.09 & 13.2 &  & 6524 & 4.16 & $+$0.12 & 13.2 &  & 6570 & 4.12 & $+$0.05 & 13.7 & $-$63.5\\ 
K02977 & 5969 & 4.23 & $-$0.04 & 3.3 &  & 5897 & 4.14 & $-$0.09 & 3.3 &  & 6042 & 4.31 & $+$0.00 & 5.0 & $-$30.9\\ 
K02979 & 5957 & 4.26 & $-$0.17 & 1.9 &  & 5969 & 4.26 & $-$0.20 & 1.9 &  & 5945 & 4.27 & $-$0.15 & 4.5 & $-$28.8\\ 
K02984 & 6123 & 4.09 & $+$0.09 & 6.3 &  & 6092 & 4.07 & $+$0.09 & 6.3 &  & 6155 & 4.11 & $+$0.09 & 7.4 & $-$5.0\\ 
K03008 & 6018 & 4.12 & $-$0.07 & 5.4 &  & 5985 & 4.07 & $-$0.08 & 5.4 &  & 6051 & 4.17 & $-$0.05 & 6.6 & $-$30.1\\ 
K03009 & 5113 & 4.62 & $+$0.18 & 3.4 &  & 5113 & 4.62 & $+$0.18 & 3.4 &  & \nodata & \nodata & \nodata & \nodata & $+$0.0\\ 
K03012 & 5493 & 4.16 & $-$0.50 & 1.5 &  & 5434 & 4.03 & $-$0.52 & 1.5 &  & 5551 & 4.28 & $-$0.48 & 4.3 & $-$61.5\\ 
K03015 & 5759 & 4.10 & $-$0.03 & 2.4 &  & 5726 & 4.03 & $-$0.05 & 2.4 &  & 5792 & 4.17 & $-$0.01 & 4.5 & $-$3.2\\ 
K03017 & 5532 & 4.48 & $-$0.16 & 0.7 &  & 5565 & 4.51 & $-$0.16 & 0.7 &  & 5499 & 4.46 & $-$0.17 & 4.2 & $-$43.1\\ 
K03021 & 5879 & 4.44 & $+$0.21 & 2.9 &  & 5873 & 4.40 & $+$0.19 & 2.9 &  & 5884 & 4.48 & $+$0.22 & 4.9 & $-$5.1\\ 
K03023 & 6215 & 4.41 & $-$0.10 & 6.9 &  & 6313 & 4.42 & $-$0.08 & 6.9 &  & 6118 & 4.41 & $-$0.12 & 8.2 & $-$31.6\\ 
K03032 & 5200 & 4.39 & $+$0.37 & 1.6 &  & 5200 & 4.39 & $+$0.37 & 1.6 &  & \nodata & \nodata & \nodata & \nodata & $-$28.7\\ 
K03039 & 5693 & 4.07 & $-$0.28 & 2.8 &  & 5730 & 4.02 & $-$0.26 & 2.8 &  & 5657 & 4.11 & $-$0.30 & 5.1 & $-$14.8\\ 
K03046 & 5672 & 4.23 & $+$0.28 & 2.5 &  & 5673 & 4.17 & $+$0.28 & 2.5 &  & 5670 & 4.28 & $+$0.28 & 4.6 & $-$35.8\\ 
K03052 & 5371 & 4.60 & $-$0.12 & 3.4 &  & 5386 & 4.65 & $-$0.12 & 3.4 &  & 5355 & 4.56 & $-$0.12 & 5.3 & $-$12.3\\ 
K03057 & 5461 & 4.47 & $-$0.06 & 0.0 &  & 5461 & 4.47 & $-$0.06 & 0.0 &  & \nodata & \nodata & \nodata & \nodata & $+$23.5\\ 
K03060 & 6190 & 4.05 & $-$0.06 & 6.2 &  & 6193 & 4.11 & $-$0.05 & 6.2 &  & 6186 & 4.00 & $-$0.06 & 7.6 & $-$56.2\\ 
K03065 & 5718 & 4.56 & $-$0.00 & 2.8 &  & 5718 & 4.56 & $-$0.00 & 2.8 &  & \nodata & \nodata & \nodata & \nodata & $+$15.2\\ 
K03075 & 5321 & 4.52 & $-$0.45 & 0.1 &  & 5353 & 4.51 & $-$0.44 & 0.1 &  & 5289 & 4.52 & $-$0.46 & 4.2 & $-$91.6\\ 
K03083 & 5829 & 4.28 & $+$0.32 & 2.3 &  & 5861 & 4.26 & $+$0.34 & 2.3 &  & 5797 & 4.30 & $+$0.30 & 4.8 & $-$23.4\\ 
K03086 & 5226 & 4.56 & $-$0.16 & 0.8 &  & 5226 & 4.56 & $-$0.16 & 0.8 &  & \nodata & \nodata & \nodata & \nodata & $-$43.4\\ 
K03087 & 5320 & 4.55 & $+$0.28 & 0.9 &  & 5316 & 4.52 & $+$0.29 & 0.9 &  & 5324 & 4.58 & $+$0.26 & 4.2 & $-$15.6\\ 
K03093 & 5879 & 4.44 & $+$0.05 & 0.9 &  & 5843 & 4.42 & $+$0.03 & 0.9 &  & 5914 & 4.47 & $+$0.07 & 3.9 & $-$14.5\\ 
K03096 & 5477 & 4.02 & $-$0.06 & 2.1 &  & 5465 & 3.88 & $-$0.05 & 2.1 &  & 5489 & 4.16 & $-$0.08 & 4.4 & $-$73.8\\ 
K03097 & 5976 & 4.10 & $-$0.01 & 5.2 &  & 5907 & 4.02 & $-$0.05 & 5.2 &  & 6045 & 4.18 & $+$0.02 & 6.5 & $-$10.2\\ 
K03100 & 5955 & 4.06 & $+$0.27 & 3.0 &  & 5937 & 4.02 & $+$0.28 & 3.0 &  & 5974 & 4.09 & $+$0.27 & 5.0 & $-$15.8\\ 
K03103 & 5883 & 4.25 & $+$0.28 & 3.4 &  & 5895 & 4.23 & $+$0.29 & 3.4 &  & 5872 & 4.27 & $+$0.27 & 5.1 & $-$12.4\\ 
K03109 & 6285 & 4.02 & $+$0.11 & 17.3 &  & 6298 & 4.09 & $+$0.11 & 17.3 &  & 6273 & 3.95 & $+$0.11 & 18.2 & $+$4.4\\ 
K03111 & 5917 & 4.36 & $-$0.06 & 2.6 &  & 5923 & 4.36 & $-$0.07 & 2.6 &  & 5911 & 4.35 & $-$0.06 & 4.8 & $-$17.3\\ 
K03114 & 6218 & 4.04 & $+$0.20 & 8.7 &  & 6180 & 4.04 & $+$0.19 & 8.7 &  & 6255 & 4.04 & $+$0.21 & 9.7 & $-$18.4\\ 
K03117 & 5563 & 4.54 & $+$0.10 & 1.8 &  & 5551 & 4.54 & $+$0.11 & 1.8 &  & 5575 & 4.54 & $+$0.10 & 4.2 & $-$42.2\\ 
K03122 & 6251 & 4.06 & $+$0.24 & 10.1 &  & 6188 & 4.03 & $+$0.23 & 10.1 &  & 6314 & 4.10 & $+$0.25 & 11.0 & $-$24.8\\ 
K03125 & 6234 & 4.27 & $-$0.14 & 9.6 &  & 6276 & 4.31 & $-$0.11 & 9.6 &  & 6192 & 4.23 & $-$0.16 & 10.4 & $-$12.2\\ 
K03128 & 6142 & 4.00 & $-$0.05 & 5.3 &  & 6090 & 4.00 & $-$0.09 & 5.3 &  & 6194 & 4.00 & $-$0.01 & 7.0 & $-$22.4\\ 
K03130 & 4866 & 4.64 & $-$0.47 & 1.6 &  & 4877 & 4.76 & $-$0.46 & 1.6 &  & 4855 & 4.51 & $-$0.48 & 4.6 & $-$15.0\\ 
K03132 & 6257 & 4.07 & $+$0.43 & 12.0 &  & 6219 & 4.02 & $+$0.43 & 12.0 &  & 6295 & 4.12 & $+$0.44 & 12.9 & $-$16.5\\ 
K03146 & 5654 & 4.01 & $+$0.22 & 2.4 &  & 5667 & 4.00 & $+$0.22 & 2.4 &  & 5640 & 4.01 & $+$0.21 & 5.1 & $-$71.6\\ 
K03158 & 4947 & 4.45 & $-$0.48 & 0.5 &  & 4963 & 4.46 & $-$0.46 & 0.5 &  & 4930 & 4.45 & $-$0.51 & 4.2 & $-$121.3\\ 
K03165 & 6267 & 4.15 & $-$0.17 & 7.9 &  & 6244 & 4.16 & $-$0.19 & 7.9 &  & 6291 & 4.14 & $-$0.15 & 9.0 & $-$10.1\\ 
K03167 & 5588 & 4.69 & $+$0.04 & 3.4 &  & 5539 & 4.66 & $+$0.01 & 3.4 &  & 5637 & 4.73 & $+$0.07 & 5.1 & $+$7.2\\ 
K03168 & 5803 & 4.12 & $-$0.14 & 2.7 &  & 5800 & 4.09 & $-$0.16 & 2.7 &  & 5806 & 4.15 & $-$0.11 & 4.8 & $-$35.3\\ 
K03172 & 6086 & 4.00 & $-$0.01 & 6.4 &  & 6003 & 3.95 & $-$0.06 & 6.4 &  & 6169 & 4.05 & $+$0.03 & 7.5 & $+$12.5\\ 
K03179 & 5731 & 4.51 & $+$0.08 & 2.3 &  & 5713 & 4.51 & $+$0.08 & 2.3 &  & 5748 & 4.52 & $+$0.08 & 4.4 & $-$39.8\\ 
K03180 & 6139 & 3.91 & $+$0.11 & 4.9 &  & 6062 & 3.87 & $+$0.08 & 4.9 &  & 6217 & 3.96 & $+$0.13 & 6.0 & $+$18.3\\ 
K03184 & 5907 & 4.19 & $+$0.27 & 4.1 &  & 5869 & 4.13 & $+$0.25 & 4.1 &  & 5945 & 4.25 & $+$0.28 & 5.6 & $+$5.0\\ 
K03190 & 5999 & 4.34 & $-$0.17 & 1.5 &  & 6010 & 4.33 & $-$0.19 & 1.5 &  & 5988 & 4.36 & $-$0.16 & 4.4 & $+$2.3\\ 
K03193 & 4990 & 3.25 & $+$0.13 & 3.8 &  & 4953 & 3.24 & $+$0.09 & 3.8 &  & 5028 & 3.26 & $+$0.17 & 5.2 & $-$5.9\\ 
K03194 & 6361 & 4.13 & $+$0.17 & 6.9 &  & 6386 & 4.19 & $+$0.21 & 6.9 &  & 6336 & 4.08 & $+$0.13 & 7.9 & $-$42.0\\ 
K03195 & 6040 & 3.95 & $-$0.32 & 3.6 &  & 5944 & 3.92 & $-$0.39 & 3.6 &  & 6135 & 3.98 & $-$0.26 & 5.3 & $-$15.4\\ 
K03196 & 6109 & 4.27 & $-$0.01 & 3.7 &  & 6094 & 4.24 & $-$0.01 & 3.7 &  & 6123 & 4.31 & $+$0.00 & 5.3 & $-$16.6\\ 
K03197 & 6187 & 4.43 & $-$0.06 & 7.4 &  & 6167 & 4.40 & $-$0.09 & 7.4 &  & 6208 & 4.46 & $-$0.03 & 8.6 & $+$4.8\\ 
K03201 & 5700 & 4.47 & $-$0.41 & 0.9 &  & 5748 & 4.51 & $-$0.43 & 0.9 &  & 5651 & 4.42 & $-$0.40 & 4.4 & $-$25.0\\ 
K03202 & 5262 & 3.80 & $+$0.03 & 3.2 &  & 5235 & 3.82 & $+$0.02 & 3.2 &  & 5288 & 3.78 & $+$0.04 & 4.9 & $-$49.8\\ 
K03203 & 6570 & 4.16 & $-$0.16 & 16.3 &  & 6550 & 4.32 & $-$0.15 & 16.3 &  & 6591 & 4.00 & $-$0.18 & 17.5 & $-$11.2\\ 
K03208 & 5846 & 4.45 & $-$0.12 & 2.5 &  & 5860 & 4.45 & $-$0.12 & 2.5 &  & 5832 & 4.45 & $-$0.12 & 4.7 & $-$34.7\\ 
K03214 & 5935 & 4.06 & $-$0.06 & 5.0 &  & 5881 & 4.00 & $-$0.08 & 5.0 &  & 5989 & 4.13 & $-$0.03 & 6.3 & $-$12.0\\ 
K03215 & 5602 & 4.29 & $+$0.12 & 2.2 &  & 5549 & 4.53 & $+$0.18 & 2.2 &  & 5656 & 4.04 & $+$0.05 & 4.6 & $-$18.8\\ 
K03218 & 5962 & 4.40 & $+$0.02 & 3.9 &  & 5996 & 4.43 & $+$0.04 & 3.9 &  & 5929 & 4.37 & $+$0.01 & 5.4 & $-$39.5\\ 
K03220 & 6388 & 4.20 & $+$0.15 & 12.8 &  & 6369 & 4.23 & $+$0.13 & 12.8 &  & 6407 & 4.18 & $+$0.16 & 14.1 & $+$10.7\\ 
K03224 & 5380 & 4.58 & $+$0.07 & 2.6 &  & 5373 & 4.59 & $+$0.07 & 2.6 &  & 5388 & 4.56 & $+$0.08 & 4.6 & $-$18.4\\ 
K03225 & 5409 & 4.54 & $+$0.19 & 2.3 &  & 5413 & 4.54 & $+$0.19 & 2.3 &  & 5405 & 4.55 & $+$0.19 & 4.6 & $-$19.5\\ 
K03227 & 5919 & 4.30 & $+$0.03 & 3.1 &  & 5935 & 4.29 & $+$0.03 & 3.1 &  & 5903 & 4.30 & $+$0.03 & 5.2 & $-$4.9\\ 
K03232 & 5738 & 4.48 & $+$0.06 & 3.8 &  & 5763 & 4.53 & $+$0.05 & 3.8 &  & 5712 & 4.43 & $+$0.07 & 5.7 & $-$25.7\\ 
K03233 & 5731 & 4.41 & $-$0.00 & 1.7 &  & 5754 & 4.44 & $+$0.01 & 1.7 &  & 5708 & 4.37 & $-$0.01 & 4.4 & $-$34.4\\ 
K03234 & 6344 & 4.48 & $-$0.07 & 11.6 &  & 6388 & 4.50 & $-$0.06 & 11.6 &  & 6300 & 4.47 & $-$0.08 & 12.9 & $+$2.7\\ 
K03236 & 6298 & 4.23 & $+$0.07 & 13.4 &  & 6266 & 4.19 & $+$0.05 & 13.4 &  & 6330 & 4.27 & $+$0.09 & 14.2 & $+$12.1\\ 
K03237 & 5875 & 4.57 & $+$0.21 & 4.9 &  & 5853 & 4.55 & $+$0.20 & 4.9 &  & 5897 & 4.59 & $+$0.23 & 6.3 & $-$30.3\\ 
K03239 & 5668 & 4.66 & $+$0.09 & 5.7 &  & 5637 & 4.66 & $+$0.06 & 5.7 &  & 5698 & 4.66 & $+$0.12 & 6.9 & $-$28.0\\ 
K03240 & 6073 & 3.87 & $+$0.25 & 5.4 &  & 6016 & 3.85 & $+$0.24 & 5.4 &  & 6130 & 3.90 & $+$0.26 & 6.6 & $-$24.2\\ 
K03244 & 4969 & 3.13 & $-$0.03 & 3.9 &  & 4886 & 3.04 & $-$0.10 & 3.9 &  & 5053 & 3.22 & $+$0.04 & 5.2 & $-$7.8\\ 
K03245 & 6078 & 4.29 & $-$0.10 & 3.6 &  & 6088 & 4.30 & $-$0.11 & 3.6 &  & 6068 & 4.28 & $-$0.09 & 5.3 & $-$17.8\\ 
K03246 & 4848 & 4.64 & $+$0.14 & 3.8 &  & 4798 & 4.59 & $+$0.14 & 3.8 &  & 4898 & 4.68 & $+$0.13 & 4.9 & $-$31.2\\ 
K03248 & 5729 & 4.30 & $-$0.02 & 1.6 &  & 5732 & 4.30 & $-$0.02 & 1.6 &  & 5726 & 4.31 & $-$0.01 & 4.3 & $-$5.2\\ 
K03249 & 6012 & 4.28 & $+$0.04 & 4.1 &  & 5984 & 4.24 & $+$0.02 & 4.1 &  & 6041 & 4.31 & $+$0.05 & 5.7 & $-$20.7\\ 
K03251 & 5897 & 4.15 & $+$0.09 & 3.8 &  & 5916 & 4.18 & $+$0.08 & 3.8 &  & 5877 & 4.12 & $+$0.09 & 5.6 & $+$15.3\\ 
K03254 & 5576 & 4.24 & $+$0.31 & 2.7 &  & 5589 & 4.21 & $+$0.32 & 2.7 &  & 5563 & 4.26 & $+$0.31 & 5.0 & $+$14.4\\ 
K03277 & 6045 & 3.98 & $+$0.00 & 7.3 &  & 5976 & 3.93 & $-$0.03 & 7.3 &  & 6114 & 4.02 & $+$0.03 & 8.4 & $-$46.1\\ 
K03278 & 5468 & 4.55 & $+$0.20 & 3.6 &  & 5468 & 4.55 & $+$0.20 & 3.6 &  & \nodata & \nodata & \nodata & \nodata & $-$9.0\\ 
K03283 & 4836 & 4.74 & $-$0.04 & 3.4 &  & 4836 & 4.74 & $-$0.04 & 3.4 &  & \nodata & \nodata & \nodata & \nodata & $-$1.4\\ 
K03287 & 5846 & 4.17 & $-$0.12 & 3.0 &  & 5888 & 4.19 & $-$0.10 & 3.0 &  & 5803 & 4.14 & $-$0.14 & 5.0 & $-$37.6\\ 
K03288 & 5414 & 4.62 & $+$0.05 & 2.3 &  & 5436 & 4.67 & $+$0.07 & 2.3 &  & 5391 & 4.57 & $+$0.03 & 4.9 & $-$13.8\\ 
K03301 & 5769 & 3.94 & $+$0.27 & 2.9 &  & 5755 & 3.92 & $+$0.28 & 2.9 &  & 5783 & 3.96 & $+$0.26 & 5.1 & $-$33.2\\ 
K03308 & 5845 & 4.06 & $+$0.01 & 3.2 &  & 5855 & 4.07 & $+$0.02 & 3.2 &  & 5835 & 4.06 & $+$0.00 & 5.3 & $-$25.9\\ 
K03310 & 5456 & 4.49 & $+$0.21 & 0.3 &  & 5440 & 4.46 & $+$0.21 & 0.3 &  & 5473 & 4.52 & $+$0.21 & 3.9 & $-$13.1\\ 
K03315 & 5552 & 4.47 & $-$0.43 & 0.2 &  & 5604 & 4.44 & $-$0.42 & 0.2 &  & 5499 & 4.50 & $-$0.44 & 4.5 & $-$95.7\\ 
K03338 & 6138 & 4.30 & $-$0.17 & 2.1 &  & 6194 & 4.36 & $-$0.16 & 2.1 &  & 6082 & 4.23 & $-$0.18 & 5.1 & $-$3.7\\ 
K03340 & 6093 & 4.33 & $-$0.10 & 6.5 &  & 6104 & 4.35 & $-$0.09 & 6.5 &  & 6082 & 4.31 & $-$0.10 & 7.6 & $+$12.1\\ 
K03346 & 5902 & 4.28 & $-$0.02 & 2.7 &  & 5942 & 4.30 & $-$0.02 & 2.7 &  & 5862 & 4.27 & $-$0.02 & 5.0 & $-$38.1\\ 
K03358 & 5313 & 4.50 & $-$0.13 & 2.6 &  & 5389 & 4.60 & $-$0.09 & 2.6 &  & 5237 & 4.39 & $-$0.16 & 5.5 & $+$1.0\\ 
K03363 & 5713 & 4.22 & $-$0.05 & 1.0 &  & 5700 & 4.20 & $-$0.06 & 1.0 &  & 5727 & 4.24 & $-$0.04 & 4.5 & $-$99.6\\ 
K03371 & 5428 & 4.56 & $+$0.00 & 1.9 &  & 5409 & 4.59 & $+$0.00 & 1.9 &  & 5447 & 4.53 & $+$0.01 & 4.7 & $-$29.2\\ 
K03378 & 5557 & 4.49 & $-$0.39 & 0.0 &  & 5570 & 4.47 & $-$0.41 & 0.0 &  & 5543 & 4.51 & $-$0.37 & 3.8 & $-$37.2\\ 
K03382 & 5371 & 4.42 & $+$0.15 & 0.9 &  & 5422 & 4.45 & $+$0.20 & 0.9 &  & 5320 & 4.38 & $+$0.10 & 4.4 & $-$47.5\\ 
K03384 & 5980 & 4.21 & $+$0.05 & 3.9 &  & 5956 & 4.17 & $+$0.05 & 3.9 &  & 6005 & 4.25 & $+$0.06 & 5.3 & $-$9.8\\ 
K03403 & 5800 & 3.95 & $+$0.13 & 3.9 &  & 5748 & 3.92 & $+$0.10 & 3.9 &  & 5851 & 3.99 & $+$0.16 & 5.5 & $-$8.6\\ 
K03419 & 6150 & 3.71 & $-$0.46 & 4.5 &  & 6439 & 3.88 & $-$0.41 & 4.5 &  & 5861 & 3.54 & $-$0.52 & 6.7 & $-$54.3\\ 
K03421 & 6388 & 4.14 & $+$0.06 & 7.8 &  & 6356 & 4.24 & $+$0.10 & 7.8 &  & 6420 & 4.03 & $+$0.03 & 8.8 & $-$2.3\\ 
K03422 & 5879 & 4.56 & $+$0.16 & 5.2 &  & 5848 & 4.53 & $+$0.14 & 5.2 &  & 5910 & 4.59 & $+$0.18 & 6.4 & $+$2.6\\ 
K03425 & 6149 & 4.05 & $+$0.01 & 6.4 &  & 6118 & 4.07 & $+$0.02 & 6.4 &  & 6180 & 4.03 & $+$0.00 & 7.5 & $-$33.6\\ 
K03436 & 5042 & 4.62 & $+$0.19 & 3.4 &  & 5044 & 4.60 & $+$0.21 & 3.4 &  & 5040 & 4.64 & $+$0.18 & 5.2 & $-$26.8\\ 
K03438 & 6016 & 4.31 & $-$0.15 & 3.7 &  & 6055 & 4.38 & $-$0.14 & 3.7 &  & 5977 & 4.24 & $-$0.17 & 5.6 & $-$49.2\\ 
K03451 & 6003 & 4.39 & $+$0.04 & 3.1 &  & 6021 & 4.41 & $+$0.05 & 3.1 &  & 5985 & 4.37 & $+$0.02 & 5.1 & $-$13.4\\ 
K03456 & 5525 & 4.50 & $-$0.29 & 8.0 &  & 5587 & 4.58 & $-$0.28 & 8.0 &  & 5463 & 4.43 & $-$0.30 & 8.9 & $-$56.3\\ 
K03465 & 5297 & 4.56 & $+$0.05 & 2.8 &  & 5332 & 4.61 & $+$0.06 & 2.8 &  & 5262 & 4.51 & $+$0.03 & 5.3 & $-$28.3\\ 
K03473 & 5156 & 4.65 & $+$0.05 & 5.3 &  & 5145 & 4.72 & $+$0.04 & 5.3 &  & 5168 & 4.58 & $+$0.05 & 6.7 & $-$17.9\\ 
K03474 & 5871 & 4.19 & $-$0.17 & 4.8 &  & 5876 & 4.21 & $-$0.16 & 4.8 &  & 5865 & 4.18 & $-$0.18 & 6.2 & $-$48.3\\ 
K03497 & 4808 & 4.68 & $+$0.10 & 4.6 &  & 4776 & 4.62 & $+$0.10 & 4.6 &  & 4840 & 4.74 & $+$0.11 & 5.8 & $-$17.9\\ 
K03500 & 6080 & 4.00 & $+$0.20 & 6.9 &  & 6032 & 3.98 & $+$0.20 & 6.9 &  & 6127 & 4.02 & $+$0.19 & 8.0 & $-$36.4\\ 
K03503 & 6001 & 4.29 & $-$0.47 & 1.9 &  & 6085 & 4.45 & $-$0.47 & 1.9 &  & 5918 & 4.14 & $-$0.48 & 4.9 & $+$0.7\\ 
K03541 & 6230 & 4.16 & $-$0.21 & 6.6 &  & 6233 & 4.25 & $-$0.21 & 6.6 &  & 6227 & 4.08 & $-$0.22 & 7.9 & $-$9.7\\ 
K03608 & 5774 & 4.26 & $-$0.11 & 2.1 &  & 5846 & 4.33 & $-$0.08 & 2.1 &  & 5701 & 4.20 & $-$0.14 & 5.1 & $-$32.7\\ 
K03641 & 6184 & 4.24 & $-$0.09 & 3.3 &  & 6161 & 4.30 & $-$0.09 & 3.3 &  & 6208 & 4.19 & $-$0.09 & 5.3 & $-$15.9\\ 
K03663 & 5676 & 4.45 & $-$0.03 & 2.0 &  & 5723 & 4.52 & $-$0.01 & 2.0 &  & 5629 & 4.37 & $-$0.05 & 5.0 & $-$19.0\\ 
K03678 & 5469 & 4.45 & $+$0.16 & 1.5 &  & 5499 & 4.48 & $+$0.18 & 1.5 &  & 5439 & 4.43 & $+$0.13 & 4.6 & $-$1.5\\ 
K03680 & 5793 & 4.30 & $+$0.22 & 2.3 &  & 5793 & 4.30 & $+$0.22 & 2.3 &  & \nodata & \nodata & \nodata & \nodata & $-$51.9\\ 
K03681 & 6194 & 4.29 & $+$0.12 & 8.1 &  & 6228 & 4.32 & $+$0.16 & 8.1 &  & 6161 & 4.26 & $+$0.08 & 9.0 & $-$27.7\\ 
K03683 & 6339 & 4.27 & $-$0.03 & 10.7 &  & 6339 & 4.27 & $-$0.03 & 10.7 &  & 5768 & 4.20 & $-$0.22 & 11.1 & $-$37.0\\ 
K03689 & 5988 & 4.17 & $+$0.02 & 4.0 &  & 6001 & 4.20 & $+$0.03 & 4.0 &  & 5975 & 4.13 & $+$0.01 & 5.7 & $+$21.5\\ 
K03726 & 4920 & 4.64 & $-$0.22 & 15.0 &  & 4920 & 4.64 & $-$0.22 & 15.0 &  & \nodata & \nodata & \nodata & \nodata & $-$29.4\\ 
K03770 & 6150 & 4.13 & $-$0.04 & 6.3 &  & 6127 & 4.14 & $-$0.04 & 6.3 &  & 6173 & 4.11 & $-$0.05 & 7.5 & $-$24.9\\ 
K03780 & 6383 & 4.16 & $-$0.19 & 8.4 &  & 6424 & 4.26 & $-$0.17 & 8.4 &  & 6342 & 4.06 & $-$0.20 & 9.7 & $-$19.9\\ 
K03787 & 5673 & 4.44 & $+$0.11 & 1.1 &  & 5712 & 4.47 & $+$0.14 & 1.1 &  & 5633 & 4.40 & $+$0.08 & 4.5 & $-$18.3\\ 
K03791 & 6054 & 4.06 & $-$0.04 & 5.1 &  & 6057 & 4.03 & $-$0.01 & 5.1 &  & 6051 & 4.10 & $-$0.06 & 6.5 & $-$5.6\\ 
K03801 & 5601 & 4.11 & $+$0.32 & 2.9 &  & 5601 & 4.11 & $+$0.32 & 2.9 &  & \nodata & \nodata & \nodata & \nodata & $-$29.2\\ 
K03811 & 5715 & 4.34 & $-$0.19 & 4.4 &  & 5759 & 4.43 & $-$0.18 & 4.4 &  & 5672 & 4.24 & $-$0.21 & 6.3 & $-$47.1\\ 
K03823 & 5657 & 4.55 & $+$0.11 & 1.5 &  & 5657 & 4.55 & $+$0.11 & 1.5 &  & 4960 & 3.38 & $-$0.68 & 6.1 & $+$2.8\\ 
K03835 & 5013 & 4.70 & $+$0.04 & 4.9 &  & 4988 & 4.73 & $+$0.03 & 4.9 &  & 5039 & 4.67 & $+$0.06 & 6.3 & $-$22.6\\ 
K03853 & 4931 & 3.57 & $-$0.08 & 3.7 &  & 4872 & 3.56 & $-$0.08 & 3.7 &  & 4989 & 3.57 & $-$0.08 & 5.4 & $-$94.4\\ 
K03864 & 5050 & 4.69 & $+$0.08 & 4.4 &  & 5033 & 4.69 & $+$0.09 & 4.4 &  & 5068 & 4.68 & $+$0.08 & 5.8 & $+$10.0\\ 
K03867 & 5568 & 4.44 & $+$0.15 & 1.5 &  & 5568 & 4.44 & $+$0.15 & 1.5 &  & \nodata & \nodata & \nodata & \nodata & $-$30.4\\ 
K03871 & 5193 & 4.62 & $+$0.07 & 3.3 &  & 5183 & 4.64 & $+$0.08 & 3.3 &  & 5203 & 4.59 & $+$0.06 & 5.3 & $-$22.6\\ 
K03876 & 5720 & 4.64 & $+$0.11 & 9.9 &  & 5714 & 4.66 & $+$0.11 & 9.9 &  & 5726 & 4.61 & $+$0.12 & 10.7 & $-$26.7\\ 
K03880 & 6277 & 4.47 & $+$0.06 & 14.3 &  & 6317 & 4.49 & $+$0.10 & 14.3 &  & 6237 & 4.44 & $+$0.01 & 14.7 & $-$4.5\\ 
K03886 & 4760 & 2.94 & $+$0.20 & 5.3 &  & 4688 & 2.94 & $+$0.22 & 5.3 &  & 4831 & 2.95 & $+$0.18 & 6.6 & $-$24.4\\ 
K03889 & 5752 & 4.19 & $+$0.20 & 1.7 &  & 5792 & 4.22 & $+$0.22 & 1.7 &  & 5713 & 4.16 & $+$0.18 & 4.8 & $-$88.0\\ 
K03890 & 4773 & 3.11 & $-$0.12 & 3.3 &  & 4732 & 3.07 & $-$0.12 & 3.3 &  & 4814 & 3.15 & $-$0.11 & 5.2 & $-$24.8\\ 
K03891 & 5080 & 3.75 & $-$0.10 & 2.7 &  & 5085 & 3.76 & $-$0.08 & 2.7 &  & 5075 & 3.73 & $-$0.12 & 4.9 & $-$42.3\\ 
K03892 & 5605 & 4.27 & $+$0.25 & 2.4 &  & 5642 & 4.29 & $+$0.28 & 2.4 &  & 5569 & 4.25 & $+$0.21 & 4.9 & $-$21.5\\ 
K03907 & 6543 & 4.42 & $-$0.12 & 18.4 &  & 6517 & 4.54 & $-$0.08 & 18.4 &  & 6569 & 4.30 & $-$0.16 & 18.9 & $-$11.5\\ 
K03908 & 5721 & 3.88 & $+$0.03 & 4.3 &  & 5667 & 3.85 & $+$0.00 & 4.3 &  & 5774 & 3.90 & $+$0.05 & 5.8 & $+$8.9\\ 
K03913 & 5958 & 4.26 & $+$0.20 & 2.9 &  & 5958 & 4.26 & $+$0.20 & 2.9 &  & \nodata & \nodata & \nodata & \nodata & $+$0.8\\ 
K03925 & 5371 & 4.61 & $+$0.07 & 2.6 &  & 5371 & 4.66 & $+$0.08 & 2.6 &  & 5370 & 4.57 & $+$0.06 & 5.0 & $-$35.8\\ 
K03928 & 6184 & 4.30 & $-$0.05 & 6.6 &  & 6184 & 4.30 & $-$0.05 & 6.6 &  & 6421 & 4.74 & $-$0.02 & 7.2 & $-$19.1\\ 
K03936 & 5081 & 4.66 & $+$0.17 & 5.8 &  & 5048 & 4.66 & $+$0.14 & 5.8 &  & 5114 & 4.66 & $+$0.19 & 6.9 & $-$28.0\\ 
K03943 & 6175 & 4.23 & $-$0.07 & 7.8 &  & 6203 & 4.28 & $-$0.05 & 7.8 &  & 6148 & 4.17 & $-$0.09 & 8.9 & $-$45.1\\ 
K03946 & 6320 & 4.15 & $-$0.22 & 7.1 &  & 6335 & 4.26 & $-$0.21 & 7.1 &  & 6305 & 4.05 & $-$0.23 & 8.3 & $-$12.8\\ 
K03980 & 5765 & 4.30 & $+$0.17 & 2.0 &  & 5765 & 4.30 & $+$0.17 & 2.0 &  & \nodata & \nodata & \nodata & \nodata & $-$17.0\\ 
K03991 & 5606 & 4.62 & $-$0.02 & 6.6 &  & 5626 & 4.67 & $-$0.02 & 6.6 &  & 5586 & 4.57 & $-$0.03 & 7.8 & $-$19.1\\ 
K04002 & 5210 & 4.58 & $+$0.21 & 2.9 &  & 5210 & 4.58 & $+$0.21 & 2.9 &  & \nodata & \nodata & \nodata & \nodata & $-$10.3\\ 
K04004 & 5739 & 4.68 & $-$0.05 & 6.9 &  & 5734 & 4.66 & $-$0.02 & 6.9 &  & 5745 & 4.70 & $-$0.08 & 7.0 & $-$25.6\\ 
K04005 & 5498 & 4.46 & $+$0.10 & 1.7 &  & 5498 & 4.46 & $+$0.10 & 1.7 &  & \nodata & \nodata & \nodata & \nodata & $-$41.0\\ 
K04011 & 5908 & 4.19 & $+$0.17 & 3.8 &  & 5932 & 4.20 & $+$0.18 & 3.8 &  & 5884 & 4.17 & $+$0.16 & 5.9 & $-$22.4\\ 
K04014 & 5942 & 4.31 & $+$0.07 & 3.5 &  & 5971 & 4.34 & $+$0.09 & 3.5 &  & 5914 & 4.29 & $+$0.04 & 5.4 & $+$12.7\\ 
K04018 & 5483 & 4.61 & $-$0.01 & 1.8 &  & 5483 & 4.61 & $-$0.01 & 1.8 &  & \nodata & \nodata & \nodata & \nodata & $-$23.6\\ 
K04021 & 6344 & 4.44 & $+$0.00 & 19.1 &  & 6446 & 4.53 & $+$0.01 & 19.1 &  & 6243 & 4.34 & $-$0.01 & 21.2 & $-$1.7\\ 
K04022 & 5998 & 3.96 & $-$0.08 & 6.8 &  & 5975 & 4.00 & $-$0.08 & 6.8 &  & 6020 & 3.93 & $-$0.08 & 7.8 & $-$7.7\\ 
K04024 & 5210 & 4.56 & $-$0.07 & 3.8 &  & 5235 & 4.58 & $-$0.03 & 3.8 &  & 5185 & 4.55 & $-$0.10 & 5.7 & $+$52.7\\ 
K04032 & 5545 & 4.26 & $+$0.07 & 1.1 &  & 5580 & 4.25 & $+$0.09 & 1.1 &  & 5509 & 4.27 & $+$0.05 & 4.6 & $-$8.9\\ 
K04036 & 4852 & 4.61 & $+$0.01 & 2.9 &  & 4864 & 4.64 & $+$0.04 & 2.9 &  & 4840 & 4.57 & $-$0.02 & 5.0 & $-$18.5\\ 
K04037 & 6191 & 4.30 & $-$0.03 & 7.3 &  & 6236 & 4.40 & $-$0.01 & 7.3 &  & 6146 & 4.20 & $-$0.04 & 8.7 & $-$9.5\\ 
K04053 & 5966 & 4.38 & $-$0.13 & 4.4 &  & 6044 & 4.57 & $-$0.08 & 4.4 &  & 5888 & 4.20 & $-$0.19 & 5.8 & $-$24.0\\ 
K04054 & 5253 & 4.62 & $+$0.11 & 1.7 &  & 5253 & 4.62 & $+$0.11 & 1.7 &  & \nodata & \nodata & \nodata & \nodata & $-$24.1\\ 
K04060 & 5792 & 4.08 & $+$0.18 & 3.2 &  & 5792 & 4.08 & $+$0.18 & 3.2 &  & 5176 & 3.48 & $-$0.37 & 4.9 & $-$67.4\\ 
K04062 & 6049 & 4.18 & $+$0.02 & 4.3 &  & 6059 & 4.18 & $+$0.03 & 4.3 &  & 6038 & 4.19 & $+$0.02 & 6.0 & $-$7.5\\ 
K04066 & 6318 & 4.30 & $+$0.09 & 12.7 &  & 6400 & 4.41 & $+$0.13 & 12.7 &  & 6236 & 4.18 & $+$0.05 & 13.4 & $-$25.0\\ 
K04067 & 5970 & 4.32 & $+$0.08 & 3.8 &  & 5999 & 4.33 & $+$0.10 & 3.8 &  & 5941 & 4.32 & $+$0.07 & 5.7 & $-$20.2\\ 
K04070 & 4926 & 4.58 & $+$0.07 & 1.9 &  & 4926 & 4.58 & $+$0.07 & 1.9 &  & \nodata & \nodata & \nodata & \nodata & $-$12.6\\ 
K04072 & 5840 & 4.25 & $+$0.12 & 2.7 &  & 5865 & 4.21 & $+$0.14 & 2.7 &  & 5814 & 4.28 & $+$0.09 & 4.9 & $+$4.6\\ 
K04098 & 4986 & 4.65 & $-$0.07 & 3.3 &  & 4979 & 4.68 & $-$0.05 & 3.3 &  & 4994 & 4.61 & $-$0.09 & 5.1 & $-$5.1\\ 
K04103 & 5271 & 4.67 & $-$0.02 & 2.5 &  & 5271 & 4.67 & $-$0.02 & 2.5 &  & \nodata & \nodata & \nodata & \nodata & $-$15.8\\ 
K04109 & 4986 & 4.46 & $+$0.26 & 2.5 &  & 4986 & 4.46 & $+$0.26 & 2.5 &  & \nodata & \nodata & \nodata & \nodata & $-$32.5\\ 
K04121 & 5121 & 4.57 & $-$0.46 & 1.9 &  & 5121 & 4.57 & $-$0.46 & 1.9 &  & \nodata & \nodata & \nodata & \nodata & $-$68.7\\ 
K04123 & 6230 & 3.95 & $+$0.11 & 4.0 &  & 6170 & 3.94 & $+$0.12 & 4.0 &  & 6289 & 3.95 & $+$0.10 & 5.3 & $-$20.4\\ 
K04129 & 5078 & 4.51 & $+$0.15 & 1.7 &  & 5105 & 4.55 & $+$0.17 & 1.7 &  & 5052 & 4.47 & $+$0.12 & 4.7 & $-$48.3\\ 
K04136 & 5715 & 3.95 & $+$0.15 & 3.1 &  & 5705 & 3.93 & $+$0.16 & 3.1 &  & 5726 & 3.96 & $+$0.14 & 5.3 & $-$25.0\\ 
K04144 & 6000 & 4.39 & $-$0.12 & 3.1 &  & 6000 & 4.39 & $-$0.12 & 3.1 &  & \nodata & \nodata & \nodata & \nodata & $+$19.9\\ 
K04146 & 5092 & 4.65 & $+$0.24 & 3.7 &  & 5082 & 4.64 & $+$0.25 & 3.7 &  & 5102 & 4.65 & $+$0.24 & 5.4 & $-$25.1\\ 
K04156 & 5807 & 4.05 & $+$0.25 & 3.4 &  & 5754 & 3.93 & $+$0.25 & 3.4 &  & 5860 & 4.18 & $+$0.24 & 5.0 & $-$34.3\\ 
K04157 & 6246 & 4.35 & $+$0.00 & 10.2 &  & 6257 & 4.37 & $+$0.03 & 10.2 &  & 6234 & 4.33 & $-$0.02 & 11.0 & $-$17.0\\ 
K04159 & 5224 & 4.44 & $+$0.13 & 2.0 &  & 5224 & 4.44 & $+$0.13 & 2.0 &  & \nodata & \nodata & \nodata & \nodata & $-$85.9\\ 
K04160 & 5767 & 4.50 & $+$0.24 & 3.5 &  & 5791 & 4.53 & $+$0.26 & 3.5 &  & 5742 & 4.47 & $+$0.22 & 5.4 & $-$17.0\\ 
K04184 & 4885 & 4.57 & $-$0.02 & 5.0 &  & 4910 & 4.64 & $+$0.02 & 5.0 &  & 4860 & 4.49 & $-$0.07 & 6.3 & $-$23.7\\ 
K04188 & 5970 & 4.45 & $+$0.12 & 4.2 &  & 5986 & 4.50 & $+$0.14 & 4.2 &  & 5954 & 4.40 & $+$0.10 & 5.8 & $+$5.0\\ 
K04190 & 5651 & 4.05 & $+$0.30 & 3.0 &  & 5671 & 4.06 & $+$0.32 & 3.0 &  & 5631 & 4.05 & $+$0.29 & 5.1 & $-$39.8\\ 
K04198 & 6105 & 3.99 & $-$0.38 & 5.8 &  & 6061 & 4.02 & $-$0.41 & 5.8 &  & 6149 & 3.96 & $-$0.36 & 7.1 & $-$23.2\\ 
K04199 & 5109 & 4.64 & $-$0.13 & 0.9 &  & 5109 & 4.64 & $-$0.13 & 0.9 &  & \nodata & \nodata & \nodata & \nodata & $-$10.9\\ 
K04204 & 5848 & 4.18 & $+$0.13 & 3.3 &  & 5880 & 4.19 & $+$0.17 & 3.3 &  & 5816 & 4.17 & $+$0.10 & 5.2 & $-$50.4\\ 
K04212 & 6173 & 4.36 & $+$0.10 & 6.6 &  & 6219 & 4.36 & $+$0.15 & 6.6 &  & 6128 & 4.36 & $+$0.06 & 7.6 & $-$15.9\\ 
K04215 & 5367 & 3.93 & $-$0.28 & 2.1 &  & 5407 & 3.94 & $-$0.26 & 2.1 &  & 5326 & 3.93 & $-$0.31 & 5.0 & $-$72.6\\ 
K04222 & 5638 & 4.59 & $-$0.02 & 3.1 &  & 5611 & 4.60 & $-$0.02 & 3.1 &  & 5665 & 4.58 & $-$0.01 & 5.2 & $-$1.6\\ 
K04226 & 5844 & 3.87 & $+$0.35 & 4.9 &  & 5865 & 3.87 & $+$0.38 & 4.9 &  & 5822 & 3.86 & $+$0.31 & 6.4 & $-$27.3\\ 
K04230 & 5819 & 4.13 & $-$0.36 & 1.8 &  & 5835 & 4.15 & $-$0.39 & 1.8 &  & 5802 & 4.10 & $-$0.34 & 4.9 & $-$50.5\\ 
K04235 & 6300 & 4.25 & $-$0.00 & 13.6 &  & 6321 & 4.26 & $+$0.04 & 13.6 &  & 6278 & 4.25 & $-$0.04 & 14.2 & $-$26.9\\ 
K04245 & 6053 & 3.98 & $+$0.20 & 5.9 &  & 5983 & 3.94 & $+$0.20 & 5.9 &  & 6122 & 4.03 & $+$0.21 & 7.0 & $-$22.1\\ 
K04246 & 5723 & 4.62 & $+$0.28 & 6.4 &  & 5702 & 4.59 & $+$0.27 & 6.4 &  & 5745 & 4.66 & $+$0.28 & 7.5 & $-$19.2\\ 
K04251 & 5514 & 4.53 & $+$0.04 & 1.8 &  & 5543 & 4.59 & $+$0.06 & 1.8 &  & 5484 & 4.46 & $+$0.02 & 4.8 & $+$0.9\\ 
K04257 & 5476 & 3.80 & $+$0.02 & 3.0 &  & 5467 & 3.79 & $+$0.01 & 3.0 &  & 5484 & 3.81 & $+$0.02 & 5.1 & $+$3.6\\ 
K04269 & 4966 & 3.56 & $+$0.07 & 2.6 &  & 4947 & 3.60 & $+$0.07 & 2.6 &  & 4984 & 3.51 & $+$0.08 & 4.9 & $-$19.6\\ 
K04273 & 6152 & 4.13 & $+$0.10 & 5.7 &  & 6133 & 4.13 & $+$0.10 & 5.7 &  & 6170 & 4.13 & $+$0.10 & 7.2 & $-$18.1\\ 
K04276 & 6300 & 3.98 & $+$0.12 & 8.2 &  & 6220 & 4.00 & $+$0.12 & 8.2 &  & 6380 & 3.97 & $+$0.12 & 9.2 & $-$10.5\\ 
K04287 & 6260 & 4.25 & $-$0.05 & 8.3 &  & 6267 & 4.32 & $-$0.03 & 8.3 &  & 6254 & 4.17 & $-$0.07 & 9.4 & $-$34.0\\ 
K04288 & 5932 & 4.14 & $+$0.08 & 3.7 &  & 5922 & 4.14 & $+$0.08 & 3.7 &  & 5942 & 4.14 & $+$0.08 & 5.6 & $-$8.6\\ 
K04292 & 5471 & 4.25 & $-$0.01 & 1.9 &  & 5522 & 4.24 & $+$0.04 & 1.9 &  & 5421 & 4.27 & $-$0.06 & 4.4 & $-$75.3\\ 
K04296 & 5569 & 4.56 & $-$0.50 & 0.9 &  & 5666 & 4.51 & $-$0.47 & 0.9 &  & 5472 & 4.61 & $-$0.53 & 4.4 & $-$105.4\\ 
K04298 & 6173 & 4.24 & $-$0.34 & 2.9 &  & 6109 & 4.22 & $-$0.38 & 2.9 &  & 6238 & 4.27 & $-$0.30 & 5.0 & $-$48.8\\ 
K04301 & 6131 & 4.30 & $-$0.21 & 5.0 &  & 6251 & 4.45 & $-$0.15 & 5.0 &  & 6010 & 4.15 & $-$0.26 & 6.6 & $-$40.6\\ 
K04302 & 6073 & 4.16 & $-$0.13 & 5.5 &  & 6094 & 4.14 & $-$0.13 & 5.5 &  & 6053 & 4.18 & $-$0.13 & 7.0 & $+$0.2\\ 
K04304 & 5774 & 4.01 & $+$0.05 & 3.5 &  & 5841 & 4.07 & $+$0.07 & 3.5 &  & 5708 & 3.95 & $+$0.02 & 5.6 & $-$34.5\\ 
K04312 & 5659 & 4.16 & $-$0.22 & 1.2 &  & 5705 & 4.11 & $-$0.19 & 1.2 &  & 5613 & 4.20 & $-$0.25 & 4.4 & $-$19.6\\ 
K04318 & 6467 & 4.32 & $-$0.03 & 18.1 &  & 6480 & 4.45 & $-$0.02 & 18.1 &  & 6454 & 4.20 & $-$0.05 & 19.3 & $-$9.1\\ 
K04323 & 6217 & 4.18 & $-$0.10 & 11.0 &  & 6292 & 4.23 & $-$0.06 & 11.0 &  & 6142 & 4.14 & $-$0.14 & 11.7 & $-$49.5\\ 
K04329 & 6207 & 4.25 & $+$0.09 & 7.9 &  & 6265 & 4.32 & $+$0.12 & 7.9 &  & 6150 & 4.18 & $+$0.05 & 9.0 & $-$37.5\\ 
K04335 & 5707 & 4.36 & $-$0.31 & 0.3 &  & 5731 & 4.37 & $-$0.32 & 0.3 &  & 5684 & 4.34 & $-$0.30 & 4.4 & $-$36.2\\ 
K04343 & 5897 & 4.02 & $-$0.38 & 3.5 &  & 5874 & 4.09 & $-$0.40 & 3.5 &  & 5921 & 3.94 & $-$0.35 & 5.4 & $-$25.2\\ 
K04356 & 4757 & 4.60 & $+$0.07 & 3.9 &  & 4757 & 4.60 & $+$0.07 & 3.9 &  & \nodata & \nodata & \nodata & \nodata & $-$35.4\\ 
K04366 & 5271 & 4.54 & $-$0.12 & 0.4 &  & 5271 & 4.54 & $-$0.12 & 0.4 &  & \nodata & \nodata & \nodata & \nodata & $-$15.6\\ 
K04367 & 6165 & 4.11 & $-$0.15 & 7.7 &  & 6277 & 4.22 & $-$0.06 & 7.7 &  & 6053 & 4.01 & $-$0.23 & 8.3 & $-$27.2\\ 
K04368 & 5973 & 3.88 & $+$0.08 & 4.0 &  & 5935 & 3.88 & $+$0.09 & 4.0 &  & 6010 & 3.87 & $+$0.07 & 5.4 & $+$27.2\\ 
K04374 & 5372 & 4.44 & $+$0.02 & 1.3 &  & 5419 & 4.49 & $+$0.05 & 1.3 &  & 5325 & 4.39 & $-$0.02 & 4.6 & $-$12.0\\ 
K04382 & 6205 & 4.24 & $-$0.13 & 10.0 &  & 6208 & 4.24 & $-$0.13 & 10.0 &  & 6203 & 4.24 & $-$0.13 & 11.0 & $+$10.8\\ 
K04383 & 5763 & 4.52 & $+$0.05 & 2.7 &  & 5772 & 4.53 & $+$0.07 & 2.7 &  & 5754 & 4.50 & $+$0.04 & 5.0 & $+$8.1\\ 
K04385 & 5090 & 4.43 & $+$0.11 & 1.5 &  & 5090 & 4.43 & $+$0.11 & 1.5 &  & \nodata & \nodata & \nodata & \nodata & $-$58.4\\ 
K04399 & 5577 & 4.67 & $-$0.04 & 1.8 &  & 5498 & 4.64 & $-$0.05 & 1.8 &  & 5656 & 4.71 & $-$0.03 & 5.0 & $-$2.5\\ 
K04400 & 5752 & 4.34 & $+$0.02 & 2.1 &  & 5803 & 4.36 & $+$0.04 & 2.1 &  & 5701 & 4.32 & $-$0.01 & 5.0 & $-$16.1\\ 
K04407 & 6401 & 4.24 & $-$0.17 & 7.5 &  & 6448 & 4.38 & $-$0.14 & 7.5 &  & 6354 & 4.11 & $-$0.19 & 8.8 & $+$4.6\\ 
K04409 & 5894 & 4.23 & $+$0.21 & 3.8 &  & 5918 & 4.23 & $+$0.23 & 3.8 &  & 5870 & 4.22 & $+$0.20 & 5.8 & $-$12.1\\ 
K04411 & 6044 & 4.35 & $-$0.17 & 4.2 &  & 6118 & 4.44 & $-$0.14 & 4.2 &  & 5969 & 4.26 & $-$0.20 & 6.1 & $-$12.8\\ 
K04418 & 5844 & 4.18 & $+$0.24 & 1.2 &  & 5844 & 4.18 & $+$0.24 & 1.2 &  & \nodata & \nodata & \nodata & \nodata & $+$2.0\\ 
K04421 & 5997 & 4.16 & $+$0.05 & 5.2 &  & 5965 & 4.13 & $+$0.04 & 5.2 &  & 6029 & 4.18 & $+$0.06 & 6.5 & $-$4.6\\ 
K04423 & 6260 & 4.12 & $-$0.16 & 9.2 &  & 6260 & 4.14 & $-$0.14 & 9.2 &  & 6260 & 4.10 & $-$0.18 & 9.9 & $-$26.6\\ 
K04426 & 6169 & 4.08 & $+$0.07 & 7.6 &  & 6139 & 4.06 & $+$0.07 & 7.6 &  & 6198 & 4.10 & $+$0.08 & 8.8 & $-$1.6\\ 
K04430 & 5104 & 4.62 & $+$0.11 & 2.2 &  & 5104 & 4.62 & $+$0.11 & 2.2 &  & \nodata & \nodata & \nodata & \nodata & $+$14.7\\ 
K04431 & 6275 & 4.16 & $-$0.13 & 9.7 &  & 6247 & 4.21 & $-$0.14 & 9.7 &  & 6303 & 4.10 & $-$0.11 & 10.7 & $-$7.6\\ 
K04435 & 6254 & 4.17 & $+$0.12 & 8.8 &  & 6174 & 4.13 & $+$0.13 & 8.8 &  & 6334 & 4.22 & $+$0.12 & 9.2 & $-$15.3\\ 
K04441 & 4884 & 4.55 & $+$0.07 & 1.8 &  & 4893 & 4.57 & $+$0.10 & 1.8 &  & 4876 & 4.53 & $+$0.04 & 4.5 & $-$37.1\\ 
K04443 & 6354 & 4.19 & $-$0.07 & 9.6 &  & 6373 & 4.27 & $-$0.04 & 9.6 &  & 6334 & 4.12 & $-$0.11 & 10.5 & $-$38.2\\ 
K04446 & 5087 & 3.81 & $-$0.30 & 2.8 &  & 5084 & 3.80 & $-$0.28 & 2.8 &  & 5090 & 3.82 & $-$0.31 & 5.1 & $-$42.4\\ 
K04452 & 5748 & 4.08 & $-$0.28 & 1.8 &  & 5785 & 4.13 & $-$0.29 & 1.8 &  & 5711 & 4.02 & $-$0.27 & 5.1 & $-$30.3\\ 
K04457 & 6051 & 4.15 & $-$0.20 & 7.5 &  & 6055 & 4.27 & $-$0.20 & 7.5 &  & 6048 & 4.04 & $-$0.20 & 8.7 & $-$29.9\\ 
K04469 & 4909 & 4.59 & $+$0.07 & 1.9 &  & 4909 & 4.59 & $+$0.07 & 1.9 &  & \nodata & \nodata & \nodata & \nodata & $-$23.8\\ 
K04473 & 5987 & 3.96 & $+$0.04 & 5.8 &  & 5947 & 4.00 & $+$0.04 & 5.8 &  & 6028 & 3.91 & $+$0.04 & 7.1 & $-$16.9\\ 
K04480 & 5634 & 4.42 & $+$0.32 & 1.4 &  & 5678 & 4.44 & $+$0.35 & 1.4 &  & 5590 & 4.41 & $+$0.29 & 4.9 & $-$27.7\\ 
K04482 & 6241 & 4.27 & $-$0.05 & 6.5 &  & 6251 & 4.33 & $-$0.03 & 6.5 &  & 6231 & 4.22 & $-$0.06 & 7.7 & $+$0.8\\ 
K04505 & 6077 & 4.28 & $-$0.11 & 5.7 &  & 6112 & 4.29 & $-$0.10 & 5.7 &  & 6042 & 4.26 & $-$0.12 & 7.1 & $-$23.8\\ 
K04546 & 5881 & 4.17 & $+$0.00 & 3.4 &  & 5954 & 4.22 & $+$0.04 & 3.4 &  & 5809 & 4.11 & $-$0.04 & 5.0 & $-$12.7\\ 
K04556 & 5437 & 3.83 & $-$0.11 & 3.5 &  & 5402 & 3.76 & $-$0.13 & 3.5 &  & 5472 & 3.89 & $-$0.09 & 5.2 & $-$52.8\\ 
K04557 & 5909 & 4.06 & $-$0.01 & 3.8 &  & 5929 & 4.08 & $+$0.00 & 3.8 &  & 5889 & 4.04 & $-$0.03 & 5.6 & $-$14.7\\ 
K04561 & 6037 & 4.11 & $+$0.01 & 6.5 &  & 5995 & 4.10 & $+$0.01 & 6.5 &  & 6080 & 4.12 & $+$0.02 & 7.7 & $-$25.9\\ 
K04567 & 6369 & 4.24 & $-$0.11 & 10.5 &  & 6363 & 4.27 & $-$0.10 & 10.5 &  & 6374 & 4.20 & $-$0.13 & 11.7 & $-$12.6\\ 
K04575 & 6281 & 4.07 & $+$0.03 & 5.8 &  & 6254 & 4.11 & $+$0.04 & 5.8 &  & 6308 & 4.02 & $+$0.01 & 6.9 & $-$22.1\\ 
K04580 & 5892 & 4.20 & $-$0.18 & 2.0 &  & 5907 & 4.18 & $-$0.21 & 2.0 &  & 5876 & 4.22 & $-$0.15 & 4.8 & $-$54.3\\ 
K04581 & 5849 & 4.24 & $+$0.07 & 2.1 &  & 5873 & 4.27 & $+$0.08 & 2.1 &  & 5824 & 4.21 & $+$0.06 & 4.9 & $-$36.3\\ 
K04582 & 5637 & 4.44 & $-$0.19 & 2.1 &  & 5686 & 4.48 & $-$0.17 & 2.1 &  & 5588 & 4.40 & $-$0.20 & 4.8 & $-$3.4\\ 
K04585 & 6153 & 4.11 & $-$0.12 & 9.5 &  & 6142 & 4.16 & $-$0.11 & 9.5 &  & 6165 & 4.06 & $-$0.12 & 10.5 & $+$25.1\\ 
K04588 & 6204 & 4.10 & $-$0.14 & 7.3 &  & 6249 & 4.19 & $-$0.12 & 7.3 &  & 6158 & 4.02 & $-$0.17 & 8.3 & $-$36.2\\ 
K04601 & 6217 & 4.26 & $+$0.22 & 8.0 &  & 6217 & 4.26 & $+$0.22 & 8.0 &  & 5265 & 3.41 & $-$0.22 & 6.2 & $-$14.2\\ 
K04603 & 6245 & 4.26 & $+$0.19 & 8.1 &  & 6257 & 4.30 & $+$0.22 & 8.1 &  & 6233 & 4.22 & $+$0.15 & 9.1 & $+$27.8\\ 
K04605 & 6096 & 3.87 & $+$0.04 & 4.4 &  & 6034 & 3.97 & $+$0.03 & 4.4 &  & 6157 & 3.77 & $+$0.05 & 5.1 & $-$53.5\\ 
K04613 & 5443 & 4.55 & $-$0.13 & 0.8 &  & 5474 & 4.60 & $-$0.09 & 0.8 &  & 5412 & 4.49 & $-$0.16 & 4.3 & $+$33.5\\ 
K04614 & 6071 & 4.19 & $+$0.08 & 5.7 &  & 6045 & 4.20 & $+$0.09 & 5.7 &  & 6096 & 4.18 & $+$0.08 & 6.9 & $-$26.4\\ 
K04617 & 5903 & 4.17 & $-$0.12 & 2.0 &  & 5939 & 4.17 & $-$0.11 & 2.0 &  & 5866 & 4.16 & $-$0.13 & 4.8 & $-$9.8\\ 
K04633 & 5985 & 4.10 & $+$0.10 & 5.9 &  & 5973 & 4.11 & $+$0.11 & 5.9 &  & 5996 & 4.09 & $+$0.10 & 7.1 & $-$20.4\\ 
K04634 & 6058 & 4.24 & $+$0.12 & 3.2 &  & 6050 & 4.26 & $+$0.13 & 3.2 &  & 6067 & 4.22 & $+$0.11 & 5.4 & $-$8.7\\ 
K04637 & 6284 & 4.08 & $-$0.16 & 5.3 &  & 6265 & 4.16 & $-$0.17 & 5.3 &  & 6303 & 4.01 & $-$0.16 & 6.9 & $-$21.7\\ 
K04640 & 6430 & 4.19 & $-$0.06 & 10.7 &  & 6429 & 4.29 & $-$0.05 & 10.7 &  & 6430 & 4.09 & $-$0.07 & 11.8 & $-$22.1\\ 
K04647 & 5166 & 3.81 & $+$0.23 & 3.0 &  & 5168 & 3.83 & $+$0.26 & 3.0 &  & 5164 & 3.80 & $+$0.20 & 5.0 & $+$12.3\\ 
K04651 & 5715 & 4.57 & $+$0.04 & 2.7 &  & 5715 & 4.57 & $+$0.04 & 2.7 &  & 5428 & 4.11 & $-$0.51 & 2.9 & $-$8.4\\ 
K04653 & 6138 & 4.19 & $-$0.00 & 7.5 &  & 6156 & 4.21 & $+$0.02 & 7.5 &  & 6120 & 4.17 & $-$0.02 & 8.6 & $-$44.4\\ 
K04657 & 5318 & 4.48 & $-$0.05 & 0.5 &  & 5354 & 4.53 & $-$0.02 & 0.5 &  & 5281 & 4.43 & $-$0.08 & 4.2 & $-$48.3\\ 
K04659 & 5600 & 4.46 & $-$0.03 & 1.3 &  & 5633 & 4.51 & $-$0.00 & 1.3 &  & 5566 & 4.41 & $-$0.06 & 4.5 & $-$26.5\\ 
K04663 & 5545 & 3.88 & $+$0.30 & 3.6 &  & 5543 & 3.88 & $+$0.31 & 3.6 &  & 5547 & 3.88 & $+$0.29 & 5.3 & $-$24.5\\ 
K04665 & 5622 & 4.00 & $-$0.02 & 2.3 &  & 5668 & 4.00 & $+$0.00 & 2.3 &  & 5575 & 4.01 & $-$0.05 & 4.9 & $-$54.8\\ 
K04674 & 5700 & 4.23 & $+$0.20 & 1.4 &  & 5740 & 4.27 & $+$0.22 & 1.4 &  & 5659 & 4.19 & $+$0.18 & 4.7 & $-$58.6\\ 
K04686 & 5697 & 3.90 & $+$0.33 & 3.8 &  & 5704 & 3.92 & $+$0.34 & 3.8 &  & 5691 & 3.88 & $+$0.33 & 5.4 & $-$24.2\\ 
K04693 & 5650 & 4.20 & $-$0.27 & 1.4 &  & 5704 & 4.14 & $-$0.24 & 1.4 &  & 5595 & 4.26 & $-$0.29 & 4.5 & $-$17.0\\ 
K04699 & 6115 & 4.29 & $+$0.05 & 5.0 &  & 6115 & 4.29 & $+$0.05 & 5.0 &  & 6301 & 5.36 & $-$0.64 & $-$0.7 & $-$39.7\\ 
K04706 & 5920 & 4.26 & $-$0.28 & 2.5 &  & 5938 & 4.27 & $-$0.28 & 2.5 &  & 5902 & 4.24 & $-$0.28 & 4.9 & $-$28.9\\ 
K04715 & 6150 & 4.01 & $-$0.09 & 8.3 &  & 6125 & 4.06 & $-$0.09 & 8.3 &  & 6175 & 3.97 & $-$0.09 & 9.4 & $-$35.3\\ 
K04716 & 6028 & 4.15 & $+$0.06 & 4.7 &  & 6065 & 4.23 & $+$0.08 & 4.7 &  & 5992 & 4.08 & $+$0.05 & 6.3 & $-$75.6\\ 
K04717 & 5669 & 4.48 & $-$0.26 & 0.3 &  & 5669 & 4.48 & $-$0.26 & 0.3 &  & \nodata & \nodata & \nodata & \nodata & $+$0.0\\ 
K04725 & 4825 & 4.49 & $-$0.03 & 2.8 &  & 4803 & 4.53 & $-$0.02 & 2.8 &  & 4846 & 4.45 & $-$0.03 & 5.2 & $-$24.9\\ 
K04744 & 5739 & 4.04 & $+$0.25 & 3.2 &  & 5738 & 4.03 & $+$0.26 & 3.2 &  & 5740 & 4.04 & $+$0.25 & 5.3 & $-$15.2\\ 
K04745 & 4781 & 4.56 & $+$0.02 & 2.2 &  & 4781 & 4.56 & $+$0.02 & 2.2 &  & \nodata & \nodata & \nodata & \nodata & $-$24.0\\ 
K04746 & 4947 & 4.59 & $+$0.08 & 4.6 &  & 4947 & 4.59 & $+$0.08 & 4.6 &  & \nodata & \nodata & \nodata & \nodata & $-$28.1\\ 
K04763 & 5695 & 3.98 & $+$0.17 & 3.5 &  & 5679 & 3.95 & $+$0.15 & 3.5 &  & 5710 & 4.00 & $+$0.18 & 5.5 & $-$15.8\\ 
K04765 & 6188 & 4.30 & $+$0.10 & 6.8 &  & 6215 & 4.30 & $+$0.14 & 6.8 &  & 6161 & 4.30 & $+$0.07 & 7.9 & $-$19.0\\ 
K04771 & 6287 & 4.26 & $-$0.08 & 10.7 &  & 6299 & 4.33 & $-$0.07 & 10.7 &  & 6275 & 4.20 & $-$0.09 & 11.4 & $-$55.5\\ 
K04773 & 6191 & 4.04 & $-$0.22 & 6.1 &  & 6188 & 4.12 & $-$0.22 & 6.1 &  & 6194 & 3.97 & $-$0.22 & 7.4 & $-$22.0\\ 
K04774 & 5222 & 4.54 & $-$0.02 & 1.5 &  & 5248 & 4.57 & $+$0.02 & 1.5 &  & 5196 & 4.50 & $-$0.05 & 4.4 & $+$0.6\\ 
K04775 & 5210 & 3.80 & $+$0.46 & 2.9 &  & 5159 & 3.68 & $+$0.44 & 2.9 &  & 5260 & 3.93 & $+$0.49 & 5.0 & $-$87.7\\ 
K04792 & 5902 & 4.41 & $+$0.06 & 2.7 &  & 5911 & 4.42 & $+$0.07 & 2.7 &  & 5894 & 4.41 & $+$0.06 & 5.1 & $-$20.1\\ 
K04811 & 5572 & 3.90 & $+$0.05 & 2.7 &  & 5549 & 3.90 & $+$0.04 & 2.7 &  & 5594 & 3.89 & $+$0.06 & 4.9 & $+$3.4\\ 
K04822 & 5787 & 3.99 & $-$0.02 & 2.6 &  & 5790 & 4.00 & $-$0.02 & 2.6 &  & 5785 & 3.98 & $-$0.02 & 5.0 & $-$103.1\\ 
K04829 & 6002 & 4.21 & $-$0.07 & 3.0 &  & 6034 & 4.21 & $-$0.05 & 3.0 &  & 5971 & 4.20 & $-$0.09 & 5.3 & $-$33.7\\ 
K04833 & 5747 & 4.11 & $+$0.02 & 2.3 &  & 5712 & 4.04 & $+$0.01 & 2.3 &  & 5783 & 4.18 & $+$0.03 & 4.6 & $+$55.7\\ 
K04834 & 5030 & 3.75 & $+$0.40 & 3.1 &  & 5014 & 3.67 & $+$0.41 & 3.1 &  & 5045 & 3.84 & $+$0.39 & 4.9 & $+$2.4\\ 
K04839 & 6108 & 4.13 & $-$0.10 & 3.2 &  & 6135 & 4.20 & $-$0.09 & 3.2 &  & 6082 & 4.05 & $-$0.11 & 5.4 & $-$30.0\\ 
K04841 & 4801 & 4.61 & $-$0.01 & 2.7 &  & 4801 & 4.61 & $-$0.01 & 2.7 &  & \nodata & \nodata & \nodata & \nodata & $+$10.0\\ 
K04850 & 5571 & 4.41 & $+$0.05 & 1.4 &  & 5602 & 4.43 & $+$0.08 & 1.4 &  & 5539 & 4.39 & $+$0.02 & 4.6 & $-$9.8\\ 
K04864 & 5752 & 3.86 & $-$0.21 & 2.9 &  & 5760 & 3.94 & $-$0.23 & 2.9 &  & 5743 & 3.78 & $-$0.20 & 5.2 & $-$7.7\\ 
K04881 & 6286 & 4.25 & $-$0.02 & 9.4 &  & 6273 & 4.22 & $-$0.02 & 9.4 &  & 6300 & 4.28 & $-$0.02 & 10.2 & $-$19.2\\ 
K04887 & 5872 & 3.85 & $+$0.03 & 4.8 &  & 5824 & 3.85 & $+$0.01 & 4.8 &  & 5919 & 3.85 & $+$0.06 & 6.3 & $-$23.9\\ 
K04892 & 5552 & 3.82 & $-$0.36 & 2.7 &  & 5517 & 3.80 & $-$0.40 & 2.7 &  & 5587 & 3.83 & $-$0.32 & 5.1 & $+$44.7\\ 
K04898 & 5810 & 4.19 & $-$0.12 & 0.3 &  & 5810 & 4.19 & $-$0.12 & 0.3 &  & \nodata & \nodata & \nodata & \nodata & $-$21.4\\ 
K04902 & 4821 & 3.23 & $+$0.19 & 3.6 &  & 4821 & 3.23 & $+$0.19 & 3.6 &  & \nodata & \nodata & \nodata & \nodata & $-$59.2\\ 
K04907 & 5933 & 4.22 & $+$0.03 & 2.9 &  & 5959 & 4.25 & $+$0.05 & 2.9 &  & 5906 & 4.18 & $+$0.02 & 5.1 & $-$36.6\\ 
K04941 & 5099 & 3.91 & $-$0.13 & 4.5 &  & 5099 & 3.91 & $-$0.13 & 4.5 &  & \nodata & \nodata & \nodata & \nodata & $+$27.1\\ 
K04961 & 4826 & 4.55 & $+$0.25 & 2.8 &  & 4826 & 4.55 & $+$0.25 & 2.8 &  & \nodata & \nodata & \nodata & \nodata & $-$57.0\\ 
K04978 & 5546 & 4.60 & $+$0.18 & 1.9 &  & 5546 & 4.60 & $+$0.18 & 1.9 &  & \nodata & \nodata & \nodata & \nodata & $-$48.8\\ 
K05018 & 5481 & 4.35 & $+$0.39 & 1.5 &  & 5481 & 4.35 & $+$0.39 & 1.5 &  & \nodata & \nodata & \nodata & \nodata & $-$16.3\\ 
K05021 & 5675 & 4.26 & $+$0.05 & 1.5 &  & 5675 & 4.26 & $+$0.05 & 1.5 &  & \nodata & \nodata & \nodata & \nodata & $+$13.0\\ 
K05039 & 4835 & 4.58 & $+$0.02 & 1.7 &  & 4835 & 4.58 & $+$0.02 & 1.7 &  & \nodata & \nodata & \nodata & \nodata & $-$16.2\\ 
K05048 & 4941 & 3.36 & $+$0.09 & 3.0 &  & 4941 & 3.36 & $+$0.09 & 3.0 &  & \nodata & \nodata & \nodata & \nodata & $-$38.4\\ 
K05057 & 5004 & 3.30 & $+$0.00 & 3.0 &  & 5004 & 3.30 & $+$0.00 & 3.0 &  & \nodata & \nodata & \nodata & \nodata & $+$16.6\\ 
K05084 & 5586 & 3.97 & $+$0.24 & 1.9 &  & 5586 & 3.97 & $+$0.24 & 1.9 &  & \nodata & \nodata & \nodata & \nodata & $+$12.4\\ 
K05085 & 5713 & 4.49 & $-$0.01 & 0.9 &  & 5713 & 4.49 & $-$0.01 & 0.9 &  & \nodata & \nodata & \nodata & \nodata & $-$1.5\\ 
K05107 & 4933 & 3.04 & $-$0.13 & 3.7 &  & 4933 & 3.04 & $-$0.13 & 3.7 &  & \nodata & \nodata & \nodata & \nodata & $-$12.4\\ 
K05119 & 4984 & 3.26 & $+$0.08 & 3.8 &  & 4984 & 3.26 & $+$0.08 & 3.8 &  & \nodata & \nodata & \nodata & \nodata & $+$9.5\\ 
K05124 & 5301 & 4.37 & $+$0.04 & 0.8 &  & 5301 & 4.37 & $+$0.04 & 0.8 &  & \nodata & \nodata & \nodata & \nodata & $-$42.3\\ 
K05135 & 5168 & 4.54 & $+$0.04 & 3.1 &  & 5168 & 4.54 & $+$0.04 & 3.1 &  & \nodata & \nodata & \nodata & \nodata & $-$144.2\\ 
K05155 & 5728 & 4.18 & $-$0.01 & 1.3 &  & 5728 & 4.18 & $-$0.01 & 1.3 &  & \nodata & \nodata & \nodata & \nodata & $-$62.4\\ 
K05159 & 6121 & 4.36 & $+$0.14 & 4.4 &  & 6121 & 4.36 & $+$0.14 & 4.4 &  & \nodata & \nodata & \nodata & \nodata & $+$20.8\\ 
K05198 & 5349 & 4.59 & $+$0.03 & 0.8 &  & 5349 & 4.59 & $+$0.03 & 0.8 &  & \nodata & \nodata & \nodata & \nodata & $-$12.2\\ 
K05216 & 5596 & 4.51 & $-$0.02 & 0.8 &  & 5596 & 4.51 & $-$0.02 & 0.8 &  & \nodata & \nodata & \nodata & \nodata & $-$24.1\\ 
K05236 & 6093 & 4.47 & $-$0.20 & 3.0 &  & 6093 & 4.47 & $-$0.20 & 3.0 &  & \nodata & \nodata & \nodata & \nodata & $-$29.8\\ 
K05241 & 6111 & 4.17 & $-$0.26 & 2.6 &  & 6111 & 4.17 & $-$0.26 & 2.6 &  & \nodata & \nodata & \nodata & \nodata & $-$45.8\\ 
K05247 & 5963 & 4.08 & $+$0.12 & 2.8 &  & 5963 & 4.08 & $+$0.12 & 2.8 &  & \nodata & \nodata & \nodata & \nodata & $-$17.9\\ 
K05269 & 5343 & 4.61 & $-$0.03 & 1.7 &  & 5343 & 4.61 & $-$0.03 & 1.7 &  & \nodata & \nodata & \nodata & \nodata & $-$9.4\\ 
K05278 & 5024 & 3.47 & $+$0.22 & 11.6 &  & 5024 & 3.47 & $+$0.22 & 11.6 &  & \nodata & \nodata & \nodata & \nodata & $-$23.2\\ 
K05284 & 5666 & 4.05 & $+$0.40 & 1.6 &  & 5666 & 4.05 & $+$0.40 & 1.6 &  & \nodata & \nodata & \nodata & \nodata & $-$67.7\\ 
K05290 & 5516 & 4.39 & $+$0.08 & 0.9 &  & 5516 & 4.39 & $+$0.08 & 0.9 &  & \nodata & \nodata & \nodata & \nodata & $+$9.0\\ 
K05324 & 4977 & 3.32 & $-$0.10 & 3.5 &  & 4977 & 3.32 & $-$0.10 & 3.5 &  & \nodata & \nodata & \nodata & \nodata & $-$13.3\\ 
K05375 & 5017 & 3.37 & $-$0.19 & 5.3 &  & 5017 & 3.37 & $-$0.19 & 5.3 &  & \nodata & \nodata & \nodata & \nodata & $-$27.0\\ 
K05379 & 5042 & 3.34 & $+$0.02 & 3.4 &  & 5042 & 3.34 & $+$0.02 & 3.4 &  & \nodata & \nodata & \nodata & \nodata & $-$44.3\\ 
K05380 & 5577 & 4.53 & $-$0.20 & 0.0 &  & 5577 & 4.53 & $-$0.20 & 0.0 &  & \nodata & \nodata & \nodata & \nodata & $-$46.4\\ 
K05393 & 4815 & 3.12 & $+$0.02 & 3.6 &  & 4815 & 3.12 & $+$0.02 & 3.6 &  & \nodata & \nodata & \nodata & \nodata & $+$3.4\\ 
K05423 & 5722 & 4.14 & $+$0.35 & 2.5 &  & 5722 & 4.14 & $+$0.35 & 2.5 &  & \nodata & \nodata & \nodata & \nodata & $-$5.9\\ 
K05546 & 6240 & 4.50 & $-$0.03 & 5.0 &  & 6240 & 4.50 & $-$0.03 & 5.0 &  & \nodata & \nodata & \nodata & \nodata & $+$5.6\\ 
K05567 & 5580 & 4.12 & $+$0.17 & 3.4 &  & 5580 & 4.12 & $+$0.17 & 3.4 &  & \nodata & \nodata & \nodata & \nodata & $-$48.3\\ 
K05592 & 6130 & 4.28 & $-$0.00 & 5.7 &  & 6130 & 4.28 & $-$0.00 & 5.7 &  & \nodata & \nodata & \nodata & \nodata & $-$24.1\\ 
K05612 & 5196 & 4.54 & $+$0.03 & 0.5 &  & 5196 & 4.54 & $+$0.03 & 0.5 &  & \nodata & \nodata & \nodata & \nodata & $-$48.2\\ 
K05613 & 5511 & 3.96 & $+$0.09 & 48.5 &  & 5511 & 3.96 & $+$0.09 & 48.5 &  & \nodata & \nodata & \nodata & \nodata & $+$44.2\\ 
K05622 & 5240 & 4.45 & $+$0.06 & 0.7 &  & 5240 & 4.45 & $+$0.06 & 0.7 &  & \nodata & \nodata & \nodata & \nodata & $-$2.0\\ 
K05625 & 4867 & 3.31 & $-$0.23 & 3.1 &  & 4867 & 3.31 & $-$0.23 & 3.1 &  & \nodata & \nodata & \nodata & \nodata & $-$45.2\\ 
K05626 & 5949 & 4.21 & $-$0.02 & 2.4 &  & 5949 & 4.21 & $-$0.02 & 2.4 &  & \nodata & \nodata & \nodata & \nodata & $-$5.8\\ 
K05645 & 5459 & 4.54 & $-$0.03 & 0.5 &  & 5459 & 4.54 & $-$0.03 & 0.5 &  & \nodata & \nodata & \nodata & \nodata & $-$3.1\\ 
K05689 & 4670 & 4.54 & $+$0.03 & 1.5 &  & 4670 & 4.54 & $+$0.03 & 1.5 &  & \nodata & \nodata & \nodata & \nodata & $-$26.8\\ 
K05702 & 5819 & 4.61 & $+$0.03 & 2.9 &  & 5819 & 4.61 & $+$0.03 & 2.9 &  & \nodata & \nodata & \nodata & \nodata & $-$2.9\\ 
K05706 & 5726 & 4.19 & $+$0.19 & 1.3 &  & 5726 & 4.19 & $+$0.19 & 1.3 &  & \nodata & \nodata & \nodata & \nodata & $-$27.0\\ 
K05782 & 5046 & 3.57 & $+$0.11 & 2.9 &  & 5046 & 3.57 & $+$0.11 & 2.9 &  & \nodata & \nodata & \nodata & \nodata & $-$11.4\\ 
K05790 & 4877 & 4.59 & $+$0.14 & 2.1 &  & 4877 & 4.59 & $+$0.14 & 2.1 &  & \nodata & \nodata & \nodata & \nodata & $-$17.1\\ 
K05792 & 4820 & 4.55 & $+$0.01 & 2.3 &  & 4820 & 4.55 & $+$0.01 & 2.3 &  & \nodata & \nodata & \nodata & \nodata & $-$64.5\\ 
K05798 & 4966 & 4.55 & $+$0.04 & 1.4 &  & 4966 & 4.55 & $+$0.04 & 1.4 &  & \nodata & \nodata & \nodata & \nodata & $-$2.4\\ 
K05837 & 5735 & 4.32 & $+$0.12 & 2.1 &  & 5735 & 4.32 & $+$0.12 & 2.1 &  & \nodata & \nodata & \nodata & \nodata & $-$27.4\\ 
K05850 & 5615 & 4.42 & $+$0.09 & 1.8 &  & 5615 & 4.42 & $+$0.09 & 1.8 &  & \nodata & \nodata & \nodata & \nodata & $-$36.5\\ 
K05852 & 5654 & 4.03 & $+$0.01 & 0.9 &  & 5654 & 4.03 & $+$0.01 & 0.9 &  & \nodata & \nodata & \nodata & \nodata & $+$28.7\\ 
K05855 & 5702 & 4.47 & $+$0.14 & 1.4 &  & 5702 & 4.47 & $+$0.14 & 1.4 &  & \nodata & \nodata & \nodata & \nodata & $-$22.7\\ 
K05869 & 4766 & 2.94 & $-$0.25 & 3.3 &  & 4766 & 2.94 & $-$0.25 & 3.3 &  & \nodata & \nodata & \nodata & \nodata & $-$42.5\\ 
K05877 & 5502 & 4.57 & $+$0.05 & 0.5 &  & 5502 & 4.57 & $+$0.05 & 0.5 &  & \nodata & \nodata & \nodata & \nodata & $+$5.0\\ 
K05888 & 5174 & 4.59 & $-$0.08 & 1.0 &  & 5174 & 4.59 & $-$0.08 & 1.0 &  & \nodata & \nodata & \nodata & \nodata & $-$14.6\\ 
K05900 & 6371 & 4.40 & $-$0.06 & 12.8 &  & 6371 & 4.40 & $-$0.06 & 12.8 &  & \nodata & \nodata & \nodata & \nodata & $+$2.0\\ 
K05924 & 4977 & 4.01 & $-$0.02 & 1.5 &  & 4977 & 4.01 & $-$0.02 & 1.5 &  & \nodata & \nodata & \nodata & \nodata & $-$100.9\\ 
K05929 & 5504 & 4.28 & $-$0.07 & 1.3 &  & 5504 & 4.28 & $-$0.07 & 1.3 &  & \nodata & \nodata & \nodata & \nodata & $+$2.6\\ 
K05932 & 5431 & 4.07 & $-$0.17 & 1.3 &  & 5431 & 4.07 & $-$0.17 & 1.3 &  & \nodata & \nodata & \nodata & \nodata & $-$68.4\\ 
K05949 & 5791 & 4.41 & $-$0.24 & 0.7 &  & 5791 & 4.41 & $-$0.24 & 0.7 &  & \nodata & \nodata & \nodata & \nodata & $+$28.2\\ 
K05953 & 5094 & 4.42 & $+$0.33 & 1.7 &  & 5094 & 4.42 & $+$0.33 & 1.7 &  & \nodata & \nodata & \nodata & \nodata & $+$23.8\\ 
K06102 & 6323 & 3.38 & $-$0.13 & 11.8 &  & 6323 & 3.38 & $-$0.13 & 11.8 &  & \nodata & \nodata & \nodata & \nodata & $-$6.8\\ 
K06384 & 5774 & 4.40 & $+$0.19 & 1.3 &  & 5774 & 4.40 & $+$0.19 & 1.3 &  & \nodata & \nodata & \nodata & \nodata & $-$7.9\\ 
K06425 & 5756 & 4.11 & $+$0.08 & 0.8 &  & 5756 & 4.11 & $+$0.08 & 0.8 &  & \nodata & \nodata & \nodata & \nodata & $-$88.0\\ 
K06676 & 6493 & 4.18 & $-$0.19 & 26.4 &  & 6493 & 4.18 & $-$0.19 & 26.4 &  & \nodata & \nodata & \nodata & \nodata & $+$11.2\\ 
K06734 & 5434 & 4.48 & $+$0.40 & 2.1 &  & 5434 & 4.48 & $+$0.40 & 2.1 &  & \nodata & \nodata & \nodata & \nodata & $-$26.4\\ 
K06745 & 6537 & 4.44 & $+$0.13 & 6.8 &  & 6537 & 4.44 & $+$0.13 & 6.8 &  & \nodata & \nodata & \nodata & \nodata & $-$32.6\\ 
K06759 & 5494 & 3.90 & $+$0.36 & 2.5 &  & 5494 & 3.90 & $+$0.36 & 2.5 &  & \nodata & \nodata & \nodata & \nodata & $-$66.9\\ 
K06786 & 5743 & 4.49 & $-$0.04 & 1.9 &  & 5743 & 4.49 & $-$0.04 & 1.9 &  & \nodata & \nodata & \nodata & \nodata & $-$33.6\\ 
K06883 & 5446 & 4.25 & $+$0.04 & 1.9 &  & 5446 & 4.25 & $+$0.04 & 1.9 &  & \nodata & \nodata & \nodata & \nodata & $+$10.8\\ 
K06927 & 4931 & 4.61 & $+$0.13 & 1.9 &  & 4931 & 4.61 & $+$0.13 & 1.9 &  & \nodata & \nodata & \nodata & \nodata & $-$15.5\\ 
K06971 & 4898 & 4.73 & $-$0.17 & 1.7 &  & 4898 & 4.73 & $-$0.17 & 1.7 &  & \nodata & \nodata & \nodata & \nodata & $+$4.4\\ 
K06981 & 5913 & 4.29 & $-$0.38 & 3.9 &  & 5913 & 4.29 & $-$0.38 & 3.9 &  & \nodata & \nodata & \nodata & \nodata & $-$81.3\\ 
K07016 & 5769 & 4.29 & $+$0.24 & 1.6 &  & 5769 & 4.29 & $+$0.24 & 1.6 &  & \nodata & \nodata & \nodata & \nodata & $-$25.5\\ 
K07040 & 6215 & 4.16 & $-$0.33 & 7.7 &  & 6215 & 4.16 & $-$0.33 & 7.7 &  & \nodata & \nodata & \nodata & \nodata & $-$24.3\\ 
K07136 & 5518 & 4.35 & $+$0.33 & 1.2 &  & 5518 & 4.35 & $+$0.33 & 1.2 &  & \nodata & \nodata & \nodata & \nodata & $-$36.4\\ 
K07179 & 5726 & 4.26 & $+$0.03 & 1.7 &  & 5726 & 4.26 & $+$0.03 & 1.7 &  & \nodata & \nodata & \nodata & \nodata & $+$3.3\\ 
K07223 & 5474 & 4.65 & $-$0.41 & 3.1 &  & 5474 & 4.65 & $-$0.41 & 3.1 &  & \nodata & \nodata & \nodata & \nodata & $-$8.2\\ 
K07235 & 5416 & 4.47 & $-$0.02 & 0.8 &  & 5416 & 4.47 & $-$0.02 & 0.8 &  & \nodata & \nodata & \nodata & \nodata & $-$25.1\\ 
K07345 & 5698 & 4.39 & $-$0.05 & 1.9 &  & 5698 & 4.39 & $-$0.05 & 1.9 &  & \nodata & \nodata & \nodata & \nodata & $+$29.5\\ 
K07566 & 5708 & 4.10 & $+$0.21 & 2.7 &  & 5708 & 4.10 & $+$0.21 & 2.7 &  & \nodata & \nodata & \nodata & \nodata & $-$37.1\\ 
K07587 & 5763 & 4.46 & $+$0.03 & 2.9 &  & 5763 & 4.46 & $+$0.03 & 2.9 &  & \nodata & \nodata & \nodata & \nodata & $-$2.6\\ 
K07599 & 5792 & 4.59 & $+$0.24 & 2.2 &  & 5792 & 4.59 & $+$0.24 & 2.2 &  & \nodata & \nodata & \nodata & \nodata & $-$27.2\\ 
K07605 & 5900 & 4.52 & $-$0.10 & 3.9 &  & 5900 & 4.52 & $-$0.10 & 3.9 &  & \nodata & \nodata & \nodata & \nodata & $+$12.7\\ 
KIC8435766 & 5065 & 4.69 & $+$0.00 & 2.0 &  & 5065 & 4.69 & $+$0.00 & 2.0 &  & \nodata & \nodata & \nodata & \nodata & $-$3.5\\ 
KIC11187332 & 5572 & 4.40 & $-$0.09 & 0.5 &  & 5572 & 4.40 & $-$0.09 & 0.5 &  & \nodata & \nodata & \nodata & \nodata & $-$73.4\\ 
KIC2718885 & 5615 & 4.37 & $+$0.13 & 2.6 &  & 5615 & 4.37 & $+$0.13 & 2.6 &  & \nodata & \nodata & \nodata & \nodata & $-$18.3\\ 
KIC6359893 & 5698 & 4.46 & $-$0.37 & 0.6 &  & 5698 & 4.46 & $-$0.37 & 0.6 &  & \nodata & \nodata & \nodata & \nodata & $-$22.2\\ 


==> tab_dispositions.tex <==
% lists dispositions according to various sources
% name cks morton mullaly nea 
K00001.01 & CP & CP & CP & CP  \\ 
K00002.01 & CP & CP & CP & CP  \\ 
K00003.01 & CP & CP & CP & CP  \\ 
K00006.01 & FP & FP & FP & FP  \\ 
K00007.01 & CP & CP & CP & CP  \\ 
K00008.01 & FP & FP & FP & FP  \\ 
K00010.01 & CP & CP & CP & CP  \\ 
K00017.01 & CP & CP & CP & CP  \\ 
K00018.01 & CP & CP & CP & CP  \\ 
K00020.01 & CP & CP & CP & CP  \\ 
K00022.01 & CP & CP & CP & CP  \\ 
K00041.01 & CP & CP & CP & CP  \\ 
K00041.02 & CP & CP & CP & CP  \\ 
K00041.03 & CP & CP & CP & CP  \\ 
K00042.01 & CP & CP & CP & CP  \\ 
K00046.01 & CP & CP & CP & CP  \\ 
K00046.02 & CP & CP & CP & CP  \\ 
K00049.01 & CP & PC & CP & CP  \\ 
K00063.01 & CP & CP & CP & CP  \\ 
K00064.01 & PC & PC & ND & PC  \\ 
K00069.01 & CP & CP & CP & CP  \\ 
K00070.01 & CP & CP & CP & CP  \\ 
K00070.02 & CP & CP & CP & CP  \\ 
K00070.03 & CP & CP & CP & CP  \\ 
K00070.04 & CP & CP & CP & CP  \\ 
K00070.05 & CP & CP & CP & CP  \\ 
K00072.01 & CP & CP & CP & CP  \\ 
K00072.02 & CP & CP & CP & CP  \\ 
K00075.01 & PC & PC & PC & PC  \\ 
K00082.01 & CP & CP & CP & CP  \\ 
K00082.02 & CP & CP & CP & CP  \\ 
K00082.03 & CP & CP & CP & CP  \\ 
K00082.04 & CP & CP & CP & CP  \\ 
K00082.05 & CP & CP & CP & CP  \\ 
K00084.01 & CP & CP & CP & CP  \\ 
K00085.01 & CP & CP & CP & CP  \\ 
K00085.02 & CP & CP & CP & CP  \\ 
K00085.03 & CP & CP & CP & CP  \\ 
K00087.01 & CP & CP & CP & CP  \\ 
K00092.01 & PC & PC & PC & PC  \\ 
K00094.01 & CP & CP & CP & CP  \\ 
K00094.02 & CP & CP & CP & CP  \\ 
K00094.03 & CP & CP & CP & CP  \\ 
K00094.04 & CP & CP & CP & CP  \\ 
K00097.01 & CP & CP & CP & CP  \\ 
K00098.01 & CP & CP & CP & CP  \\ 
K00099.01 & PC & \nodata & ND & PC  \\ 
K00099.02 & FP & \nodata & FP & FP  \\ 
K00102.01 & PC & PC & ND & PC  \\ 
K00102.02 & FP & FP & ND & FP  \\ 
K00103.01 & PC & PC & ND & PC  \\ 
K00104.01 & CP & CP & CP & CP  \\ 
K00105.01 & CP & PC & CP & CP  \\ 
K00107.01 & CP & PC & CP & CP  \\ 
K00108.01 & CP & CP & CP & CP  \\ 
K00108.02 & CP & CP & CP & CP  \\ 
K00110.01 & CP & PC & CP & CP  \\ 
K00111.01 & CP & CP & CP & CP  \\ 
K00111.02 & CP & CP & CP & CP  \\ 
K00111.03 & CP & CP & CP & CP  \\ 
K00111.04 & FP & \nodata & ND & FP  \\ 
K00112.01 & CP & PC & CP & CP  \\ 
K00112.02 & CP & PC & CP & CP  \\ 
K00113.01 & FP & \nodata & FP & FP  \\ 
K00115.01 & CP & CP & CP & CP  \\ 
K00115.02 & CP & CP & CP & CP  \\ 
K00115.03 & PC & \nodata & ND & PC  \\ 
K00116.01 & CP & CP & CP & CP  \\ 
K00116.02 & CP & CP & CP & CP  \\ 
K00116.03 & CP & CP & CP & CP  \\ 
K00116.04 & CP & CP & CP & CP  \\ 
K00117.01 & CP & CP & CP & CP  \\ 
K00117.02 & CP & CP & CP & CP  \\ 
K00117.03 & CP & CP & CP & CP  \\ 
K00117.04 & CP & CP & CP & CP  \\ 
K00118.01 & CP & PC & CP & CP  \\ 
K00119.01 & CP & CP & CP & CP  \\ 
K00119.02 & CP & CP & CP & CP  \\ 
K00122.01 & CP & CP & CP & CP  \\ 
K00123.01 & CP & CP & CP & CP  \\ 
K00123.02 & CP & CP & CP & CP  \\ 
K00124.01 & CP & CP & CP & CP  \\ 
K00124.02 & CP & CP & CP & CP  \\ 
K00127.01 & CP & CP & CP & CP  \\ 
K00128.01 & CP & CP & CP & CP  \\ 
K00134.01 & FP & \nodata & ND & FP  \\ 
K00135.01 & CP & CP & CP & CP  \\ 
K00137.01 & CP & CP & CP & CP  \\ 
K00137.02 & CP & CP & CP & CP  \\ 
K00137.03 & CP & CP & CP & CP  \\ 
K00139.01 & CP & CP & CP & CP  \\ 
K00139.02 & CP & CP & CP & CP  \\ 
K00141.01 & PC & PC & ND & PC  \\ 
K00142.01 & CP & \nodata & CP & CP  \\ 
K00142.02 & FP & \nodata & ND & FP  \\ 
K00144.01 & CP & PC & CP & CP  \\ 
K00145.01 & PC & PC & PC & PC  \\ 
K00148.01 & CP & CP & CP & CP  \\ 
K00148.02 & CP & CP & CP & CP  \\ 
K00148.03 & CP & CP & CP & CP  \\ 
K00149.01 & CP & PC & CP & CP  \\ 
K00150.01 & CP & CP & CP & CP  \\ 
K00150.02 & CP & CP & CP & CP  \\ 
K00152.01 & CP & CP & CP & CP  \\ 
K00152.02 & CP & CP & CP & CP  \\ 
K00152.03 & CP & CP & CP & CP  \\ 
K00152.04 & CP & CP & CP & CP  \\ 
K00153.01 & CP & CP & CP & CP  \\ 
K00153.02 & CP & CP & CP & CP  \\ 
K00155.01 & CP & PC & CP & CP  \\ 
K00156.01 & CP & CP & CP & CP  \\ 
K00156.02 & CP & CP & CP & CP  \\ 
K00156.03 & CP & CP & CP & CP  \\ 
K00157.01 & CP & CP & CP & CP  \\ 
K00157.02 & CP & CP & CP & CP  \\ 
K00157.03 & CP & CP & CP & CP  \\ 
K00157.04 & CP & CP & CP & CP  \\ 
K00157.05 & CP & CP & CP & CP  \\ 
K00157.06 & CP & CP & CP & CP  \\ 
K00159.01 & CP & CP & CP & CP  \\ 
K00159.02 & CP & CP & CP & CP  \\ 
K00161.01 & CP & PC & CP & CP  \\ 
K00162.01 & CP & PC & CP & CP  \\ 
K00163.01 & CP & PC & CP & CP  \\ 
K00165.01 & CP & PC & CP & CP  \\ 
K00166.01 & CP & PC & CP & CP  \\ 
K00167.01 & CP & PC & CP & CP  \\ 
K00168.01 & CP & CP & CP & CP  \\ 
K00168.02 & CP & CP & CP & CP  \\ 
K00168.03 & CP & CP & CP & CP  \\ 
K00171.01 & CP & CP & CP & CP  \\ 
K00171.02 & CP & CP & CP & CP  \\ 
K00172.01 & CP & CP & CP & CP  \\ 
K00172.02 & CP & CP & CP & CP  \\ 
K00173.01 & CP & PC & CP & CP  \\ 
K00174.01 & CP & PC & CP & CP  \\ 
K00176.01 & CP & PC & CP & CP  \\ 
K00177.01 & PC & PC & ND & PC  \\ 
K00179.01 & CP & PC & CP & CP  \\ 
K00179.02 & CP & \nodata & CP & CP  \\ 
K00180.01 & CP & PC & CP & CP  \\ 
K00186.01 & CP & PC & CP & CP  \\ 
K00191.01 & CP & PC & CP & CP  \\ 
K00191.02 & PC & PC & ND & PC  \\ 
K00191.03 & PC & PC & ND & PC  \\ 
K00191.04 & CP & PC & CP & CP  \\ 
K00193.01 & FP & FP & ND & FP  \\ 
K00195.01 & CP & CP & CP & CP  \\ 
K00197.01 & CP & PC & CP & CP  \\ 
K00201.01 & CP & PC & CP & CP  \\ 
K00203.01 & CP & CP & CP & CP  \\ 
K00209.01 & CP & CP & CP & CP  \\ 
K00209.02 & CP & CP & CP & CP  \\ 
K00211.01 & PC & PC & PC & PC  \\ 
K00214.01 & CP & CP & CP & CP  \\ 
K00232.01 & CP & CP & CP & CP  \\ 
K00232.02 & CP & CP & CP & CP  \\ 
K00232.03 & CP & CP & CP & CP  \\ 
K00232.04 & CP & CP & CP & CP  \\ 
K00232.05 & CP & CP & CP & CP  \\ 
K00237.01 & CP & PC & CP & CP  \\ 
K00238.01 & CP & CP & CP & CP  \\ 
K00238.02 & CP & CP & CP & CP  \\ 
K00238.03 & FP & \nodata & FP & FP  \\ 
K00241.01 & CP & CP & CP & CP  \\ 
K00241.02 & CP & CP & CP & CP  \\ 
K00241.03 & CP & CP & CP & CP  \\ 
K00244.01 & CP & CP & CP & CP  \\ 
K00244.02 & CP & CP & CP & CP  \\ 
K00245.01 & CP & CP & CP & CP  \\ 
K00245.02 & CP & CP & CP & CP  \\ 
K00245.03 & CP & \nodata & CP & CP  \\ 
K00245.04 & FP & \nodata & CP & CP  \\ 
K00246.01 & CP & CP & CP & CP  \\ 
K00246.02 & CP & CP & CP & CP  \\ 
K00257.01 & CP & PC & CP & CP  \\ 
K00260.01 & CP & CP & CP & CP  \\ 
K00260.02 & CP & CP & CP & CP  \\ 
K00260.03 & CP & CP & CP & CP  \\ 
K00261.01 & CP & CP & CP & CP  \\ 
K00262.01 & CP & CP & CP & CP  \\ 
K00262.02 & CP & CP & CP & CP  \\ 
K00263.01 & FP & FP & FP & FP  \\ 
K00265.01 & CP & PC & CP & CP  \\ 
K00266.01 & CP & PC & CP & CP  \\ 
K00266.02 & PC & PC & PC & PC  \\ 
K00268.01 & PC & PC & PC & PC  \\ 
K00269.01 & PC & PC & ND & PC  \\ 
K00270.01 & CP & CP & CP & CP  \\ 
K00270.02 & CP & CP & CP & CP  \\ 
K00271.01 & CP & CP & CP & CP  \\ 
K00271.02 & CP & CP & CP & CP  \\ 
K00271.03 & CP & CP & CP & CP  \\ 
K00273.01 & CP & PC & CP & CP  \\ 
K00274.01 & CP & CP & CP & CP  \\ 
K00274.02 & CP & CP & CP & CP  \\ 
K00275.01 & CP & CP & CP & CP  \\ 
K00275.02 & CP & CP & CP & CP  \\ 
K00276.01 & CP & PC & CP & CP  \\ 
K00277.01 & CP & CP & CP & CP  \\ 
K00277.02 & CP & CP & CP & CP  \\ 
K00279.01 & CP & CP & CP & CP  \\ 
K00279.02 & CP & CP & CP & CP  \\ 
K00279.03 & CP & \nodata & CP & CP  \\ 
K00280.01 & PC & PC & ND & PC  \\ 
K00281.01 & CP & PC & CP & CP  \\ 
K00282.01 & CP & CP & CP & CP  \\ 
K00282.02 & CP & CP & CP & CP  \\ 
K00282.03 & CP & CP & CP & CP  \\ 
K00283.01 & CP & CP & CP & CP  \\ 
K00283.02 & CP & CP & CP & CP  \\ 
K00283.03 & PC & PC & \nodata & PC  \\ 
K00284.01 & CP & CP & CP & CP  \\ 
K00284.02 & CP & CP & CP & CP  \\ 
K00284.03 & CP & CP & CP & CP  \\ 
K00284.04 & CP & PC & CP & CP  \\ 
K00285.01 & CP & CP & CP & CP  \\ 
K00285.02 & CP & CP & CP & CP  \\ 
K00285.03 & CP & CP & CP & CP  \\ 
K00288.01 & FP & FP & ND & FP  \\ 
K00289.01 & PC & PC & PC & PC  \\ 
K00289.02 & CP & PC & CP & CP  \\ 
K00291.01 & CP & CP & CP & CP  \\ 
K00291.02 & CP & CP & CP & CP  \\ 
K00292.01 & CP & CP & CP & CP  \\ 
K00294.01 & CP & PC & CP & CP  \\ 
K00295.01 & CP & CP & CP & CP  \\ 
K00295.02 & CP & CP & CP & CP  \\ 
K00296.01 & CP & PC & CP & CP  \\ 
K00297.01 & CP & PC & CP & CP  \\ 
K00299.01 & CP & CP & CP & CP  \\ 
K00301.01 & CP & CP & CP & CP  \\ 
K00301.02 & CP & CP & CP & CP  \\ 
K00303.01 & CP & PC & CP & CP  \\ 
K00304.01 & CP & PC & CP & CP  \\ 
K00304.02 & PC & PC & ND & PC  \\ 
K00305.01 & CP & CP & CP & CP  \\ 
K00306.01 & CP & PC & CP & CP  \\ 
K00307.01 & CP & PC & CP & CP  \\ 
K00307.02 & CP & PC & CP & CP  \\ 
K00308.01 & PC & PC & ND & PC  \\ 
K00312.01 & CP & CP & CP & CP  \\ 
K00312.02 & CP & CP & CP & CP  \\ 
K00313.01 & CP & CP & CP & CP  \\ 
K00313.02 & CP & CP & CP & CP  \\ 
K00315.01 & PC & PC & ND & PC  \\ 
K00316.01 & CP & CP & CP & CP  \\ 
K00316.02 & CP & CP & CP & CP  \\ 
K00316.03 & PC & PC & PC & PC  \\ 
K00317.01 & CP & PC & CP & CP  \\ 
K00318.01 & CP & PC & CP & CP  \\ 
K00319.01 & PC & PC & ND & PC  \\ 
K00321.01 & CP & CP & CP & CP  \\ 
K00321.02 & CP & CP & CP & CP  \\ 
K00323.01 & CP & PC & CP & CP  \\ 
K00327.01 & CP & CP & CP & CP  \\ 
K00327.02 & CP & CP & CP & CP  \\ 
K00328.01 & FP & FP & ND & FP  \\ 
K00330.01 & CP & PC & CP & CP  \\ 
K00330.02 & CP & PC & CP & CP  \\ 
K00331.01 & CP & PC & CP & CP  \\ 
K00332.01 & CP & PC & CP & CP  \\ 
K00332.02 & PC & PC & ND & PC  \\ 
K00333.01 & CP & PC & CP & CP  \\ 
K00337.01 & CP & PC & CP & CP  \\ 
K00337.02 & PC & \nodata & PC & PC  \\ 
K00338.01 & CP & CP & CP & CP  \\ 
K00338.02 & CP & CP & CP & CP  \\ 
K00339.01 & CP & PC & CP & CP  \\ 
K00339.02 & CP & PC & CP & CP  \\ 
K00339.03 & PC & PC & ND & PC  \\ 
K00340.01 & FP & FP & ND & FP  \\ 
K00341.01 & CP & CP & CP & CP  \\ 
K00341.02 & CP & CP & CP & CP  \\ 
K00343.01 & CP & CP & CP & CP  \\ 
K00343.02 & CP & CP & CP & CP  \\ 
K00343.03 & CP & CP & CP & CP  \\ 
K00344.01 & CP & PC & CP & CP  \\ 
K00345.01 & CP & PC & CP & CP  \\ 
K00346.01 & CP & PC & CP & CP  \\ 
K00348.01 & CP & PC & CP & CP  \\ 
K00349.01 & PC & PC & ND & PC  \\ 
K00350.01 & PC & PC & ND & PC  \\ 
K00351.01 & CP & CP & CP & CP  \\ 
K00351.02 & CP & \nodata & CP & CP  \\ 
K00351.03 & CP & \nodata & CP & CP  \\ 
K00351.04 & CP & \nodata & CP & CP  \\ 
K00351.05 & CP & \nodata & CP & CP  \\ 
K00351.06 & CP & \nodata & CP & CP  \\ 
K00351.07 & PC & \nodata & ND & PC  \\ 
K00352.01 & CP & CP & CP & CP  \\ 
K00352.02 & CP & CP & CP & CP  \\ 
K00355.01 & CP & PC & CP & CP  \\ 
K00356.01 & CP & PC & CP & CP  \\ 
K00360.01 & FP & FP & FP & FP  \\ 
K00361.01 & CP & PC & CP & CP  \\ 
K00364.01 & PC & \nodata & ND & PC  \\ 
K00365.01 & CP & PC & CP & CP  \\ 
K00365.02 & FP & \nodata & FP & FP  \\ 
K00367.01 & PC & PC & ND & PC  \\ 
K00369.01 & CP & CP & CP & CP  \\ 
K00369.02 & CP & CP & CP & CP  \\ 
K00370.01 & CP & CP & CP & CP  \\ 
K00370.02 & CP & CP & CP & CP  \\ 
K00371.01 & PC & PC & PC & PC  \\ 
K00371.02 & FP & FP & \nodata & FP  \\ 
K00372.01 & CP & PC & CP & CP  \\ 
K00373.01 & PC & PC & PC & PC  \\ 
K00374.01 & CP & PC & CP & CP  \\ 
K00375.01 & PC & \nodata & ND & PC  \\ 
K00377.01 & CP & CP & CP & CP  \\ 
K00377.02 & CP & \nodata & CP & CP  \\ 
K00377.03 & CP & \nodata & CP & CP  \\ 
K00379.01 & FP & FP & ND & FP  \\ 
K00379.02 & PC & PC & ND & PC  \\ 
K00384.01 & CP & PC & CP & CP  \\ 
K00385.01 & CP & PC & CP & CP  \\ 
K00386.01 & CP & CP & CP & CP  \\ 
K00386.02 & CP & CP & CP & CP  \\ 
K00387.01 & CP & PC & CP & CP  \\ 
K00388.01 & PC & PC & ND & PC  \\ 
K00392.01 & CP & CP & CP & CP  \\ 
K00392.02 & CP & CP & CP & CP  \\ 
K00393.01 & CP & PC & CP & CP  \\ 
K00399.01 & FP & FP & ND & FP  \\ 
K00401.01 & CP & CP & CP & CP  \\ 
K00401.02 & CP & CP & CP & CP  \\ 
K00401.03 & CP & CP & CP & CP  \\ 
K00403.01 & FP & FP & ND & FP  \\ 
K00408.01 & CP & CP & CP & CP  \\ 
K00408.02 & CP & CP & CP & CP  \\ 
K00408.03 & CP & CP & CP & CP  \\ 
K00408.04 & CP & CP & CP & CP  \\ 
K00409.01 & CP & PC & CP & CP  \\ 
K00415.01 & PC & PC & PC & PC  \\ 
K00416.01 & CP & CP & CP & CP  \\ 
K00416.02 & CP & CP & CP & CP  \\ 
K00416.03 & PC & PC & PC & PC  \\ 
K00416.04 & PC & PC & \nodata & PC  \\ 
K00427.01 & PC & PC & PC & PC  \\ 
K00427.02 & CP & PC & CP & CP  \\ 
K00427.03 & CP & PC & CP & CP  \\ 
K00431.01 & CP & CP & CP & CP  \\ 
K00431.02 & CP & CP & CP & CP  \\ 
K00433.01 & CP & PC & CP & CP  \\ 
K00433.02 & CP & PC & CP & CP  \\ 
K00435.01 & CP & PC & CP & CP  \\ 
K00435.02 & PC & \nodata & ND & PC  \\ 
K00435.03 & CP & CP & CP & CP  \\ 
K00435.04 & CP & PC & CP & CP  \\ 
K00435.05 & CP & CP & CP & CP  \\ 
K00435.06 & CP & PC & CP & CP  \\ 
K00439.01 & CP & PC & CP & CP  \\ 
K00439.02 & FP & \nodata & ND & FP  \\ 
K00440.01 & CP & CP & CP & CP  \\ 
K00440.02 & CP & CP & CP & CP  \\ 
K00442.01 & CP & CP & CP & CP  \\ 
K00442.02 & CP & CP & CP & CP  \\ 
K00442.03 & CP & PC & CP & CP  \\ 
K00444.01 & CP & PC & CP & CP  \\ 
K00446.01 & CP & CP & CP & CP  \\ 
K00446.02 & CP & CP & CP & CP  \\ 
K00448.01 & CP & CP & CP & CP  \\ 
K00448.02 & CP & CP & CP & CP  \\ 
K00456.01 & CP & CP & CP & CP  \\ 
K00456.02 & CP & CP & CP & CP  \\ 
K00457.01 & CP & CP & CP & CP  \\ 
K00457.02 & CP & CP & CP & CP  \\ 
K00459.01 & CP & CP & CP & CP  \\ 
K00459.02 & CP & CP & CP & CP  \\ 
K00464.01 & CP & PC & CP & CP  \\ 
K00464.02 & CP & PC & CP & CP  \\ 
K00465.01 & FP & \nodata & ND & FP  \\ 
K00466.01 & PC & PC & ND & PC  \\ 
K00474.01 & CP & CP & CP & CP  \\ 
K00474.02 & CP & CP & CP & CP  \\ 
K00474.03 & PC & PC & PC & PC  \\ 
K00474.04 & CP & CP & CP & CP  \\ 
K00475.01 & CP & CP & CP & CP  \\ 
K00475.02 & CP & CP & CP & CP  \\ 
K00479.01 & CP & PC & CP & CP  \\ 
K00481.01 & CP & CP & CP & CP  \\ 
K00481.02 & CP & PC & CP & CP  \\ 
K00481.03 & CP & CP & CP & CP  \\ 
K00486.01 & CP & PC & CP & CP  \\ 
K00490.01 & CP & CP & CP & CP  \\ 
K00490.02 & CP & \nodata & CP & CP  \\ 
K00490.03 & CP & CP & CP & CP  \\ 
K00490.04 & CP & PC & CP & CP  \\ 
K00500.01 & CP & CP & CP & CP  \\ 
K00500.02 & CP & CP & CP & CP  \\ 
K00500.03 & CP & CP & CP & CP  \\ 
K00500.04 & CP & CP & CP & CP  \\ 
K00500.05 & CP & PC & CP & CP  \\ 
K00505.01 & CP & CP & CP & CP  \\ 
K00505.02 & CP & CP & CP & CP  \\ 
K00505.03 & CP & CP & CP & CP  \\ 
K00505.04 & CP & CP & CP & CP  \\ 
K00505.05 & CP & CP & CP & CP  \\ 
K00508.01 & CP & CP & CP & CP  \\ 
K00508.02 & CP & CP & CP & CP  \\ 
K00509.01 & CP & CP & CP & CP  \\ 
K00509.02 & CP & CP & CP & CP  \\ 
K00509.03 & CP & CP & CP & CP  \\ 
K00510.01 & CP & CP & CP & CP  \\ 
K00510.02 & CP & CP & CP & CP  \\ 
K00510.03 & CP & CP & CP & CP  \\ 
K00510.04 & CP & CP & CP & CP  \\ 
K00511.01 & CP & CP & CP & CP  \\ 
K00511.02 & CP & CP & CP & CP  \\ 
K00517.01 & CP & PC & CP & CP  \\ 
K00518.01 & CP & CP & CP & CP  \\ 
K00518.02 & CP & CP & CP & CP  \\ 
K00518.03 & CP & CP & CP & CP  \\ 
K00519.01 & CP & CP & CP & CP  \\ 
K00519.02 & CP & CP & CP & CP  \\ 
K00520.01 & CP & CP & CP & CP  \\ 
K00520.02 & CP & CP & CP & CP  \\ 
K00520.03 & CP & CP & CP & CP  \\ 
K00520.04 & CP & PC & CP & CP  \\ 
K00523.01 & CP & CP & CP & CP  \\ 
K00523.02 & CP & CP & CP & CP  \\ 
K00528.01 & CP & CP & CP & CP  \\ 
K00528.02 & CP & CP & CP & CP  \\ 
K00528.03 & CP & CP & CP & CP  \\ 
K00534.01 & CP & CP & CP & CP  \\ 
K00534.02 & CP & CP & CP & CP  \\ 
K00543.01 & CP & CP & CP & CP  \\ 
K00543.02 & CP & CP & CP & CP  \\ 
K00546.01 & CP & CP & CP & CP  \\ 
K00546.02 & CP & CP & CP & CP  \\ 
K00548.01 & CP & PC & CP & CP  \\ 
K00550.01 & CP & PC & CP & CP  \\ 
K00551.01 & CP & CP & CP & CP  \\ 
K00551.02 & CP & CP & CP & CP  \\ 
K00555.01 & CP & PC & CP & CP  \\ 
K00555.02 & PC & PC & PC & PC  \\ 
K00561.01 & CP & PC & CP & CP  \\ 
K00564.01 & CP & PC & CP & CP  \\ 
K00564.02 & CP & PC & CP & CP  \\ 
K00564.03 & CP & PC & CP & CP  \\ 
K00567.01 & CP & CP & CP & CP  \\ 
K00567.02 & CP & CP & CP & CP  \\ 
K00567.03 & CP & CP & CP & CP  \\ 
K00568.01 & CP & PC & CP & CP  \\ 
K00568.02 & CP & PC & CP & CP  \\ 
K00569.01 & CP & CP & CP & CP  \\ 
K00569.02 & CP & CP & CP & CP  \\ 
K00572.01 & CP & CP & CP & CP  \\ 
K00572.02 & CP & CP & CP & CP  \\ 
K00573.01 & CP & CP & CP & CP  \\ 
K00573.02 & CP & CP & CP & CP  \\ 
K00574.01 & CP & CP & CP & CP  \\ 
K00574.02 & CP & CP & CP & CP  \\ 
K00577.01 & PC & PC & ND & PC  \\ 
K00577.02 & CP & PC & CP & CP  \\ 
K00579.01 & CP & CP & CP & CP  \\ 
K00579.02 & CP & CP & CP & CP  \\ 
K00582.01 & CP & PC & CP & CP  \\ 
K00582.02 & CP & CP & CP & CP  \\ 
K00582.03 & CP & CP & CP & CP  \\ 
K00584.01 & CP & CP & CP & CP  \\ 
K00584.02 & CP & CP & CP & CP  \\ 
K00584.03 & CP & PC & CP & CP  \\ 
K00590.01 & CP & CP & CP & CP  \\ 
K00590.02 & CP & CP & CP & CP  \\ 
K00597.01 & CP & CP & CP & CP  \\ 
K00597.02 & CP & CP & CP & CP  \\ 
K00597.03 & CP & CP & CP & CP  \\ 
K00598.01 & CP & CP & CP & CP  \\ 
K00598.02 & CP & CP & CP & CP  \\ 
K00600.01 & CP & PC & CP & CP  \\ 
K00600.02 & PC & \nodata & PC & PC  \\ 
K00601.01 & CP & PC & CP & CP  \\ 
K00601.02 & PC & PC & ND & PC  \\ 
K00601.03 & CP & PC & CP & CP  \\ 
K00611.01 & PC & PC & ND & PC  \\ 
K00612.01 & CP & CP & CP & CP  \\ 
K00612.02 & CP & CP & CP & CP  \\ 
K00612.03 & PC & PC & PC & PC  \\ 
K00620.01 & CP & CP & CP & CP  \\ 
K00620.02 & CP & CP & CP & CP  \\ 
K00620.03 & CP & CP & CP & CP  \\ 
K00623.01 & CP & CP & CP & CP  \\ 
K00623.02 & CP & CP & CP & CP  \\ 
K00623.03 & CP & CP & CP & CP  \\ 
K00623.04 & CP & CP & CP & CP  \\ 
K00624.01 & CP & CP & CP & CP  \\ 
K00624.02 & CP & CP & CP & CP  \\ 
K00624.03 & CP & PC & CP & CP  \\ 
K00626.01 & CP & PC & CP & CP  \\ 
K00626.02 & PC & PC & ND & PC  \\ 
K00627.01 & CP & PC & CP & CP  \\ 
K00627.02 & CP & PC & CP & CP  \\ 
K00628.01 & CP & PC & CP & CP  \\ 
K00629.01 & CP & PC & CP & CP  \\ 
K00632.01 & CP & PC & CP & CP  \\ 
K00633.01 & CP & PC & CP & CP  \\ 
K00635.01 & PC & PC & ND & PC  \\ 
K00638.01 & CP & CP & CP & CP  \\ 
K00638.02 & CP & CP & CP & CP  \\ 
K00639.01 & CP & PC & CP & CP  \\ 
K00640.01 & CP & PC & CP & CP  \\ 
K00644.01 & FP & FP & ND & FP  \\ 
K00645.01 & CP & PC & CP & CP  \\ 
K00645.02 & PC & PC & ND & PC  \\ 
K00647.01 & CP & PC & CP & CP  \\ 
K00647.02 & PC & PC & ND & PC  \\ 
K00649.01 & CP & PC & CP & CP  \\ 
K00649.02 & PC & \nodata & PC & PC  \\ 
K00650.01 & PC & PC & ND & PC  \\ 
K00654.01 & CP & CP & CP & CP  \\ 
K00654.02 & CP & CP & CP & CP  \\ 
K00655.01 & CP & CP & CP & CP  \\ 
K00655.02 & CP & CP & CP & CP  \\ 
K00657.01 & CP & CP & CP & CP  \\ 
K00657.02 & CP & CP & CP & CP  \\ 
K00658.01 & CP & CP & CP & CP  \\ 
K00658.02 & CP & CP & CP & CP  \\ 
K00658.03 & CP & CP & CP & CP  \\ 
K00659.01 & CP & PC & CP & CP  \\ 
K00660.01 & CP & PC & CP & CP  \\ 
K00661.01 & CP & CP & CP & CP  \\ 
K00661.02 & CP & CP & CP & CP  \\ 
K00662.01 & CP & PC & CP & CP  \\ 
K00664.01 & CP & CP & CP & CP  \\ 
K00664.02 & CP & CP & CP & CP  \\ 
K00664.03 & CP & CP & CP & CP  \\ 
K00665.01 & CP & CP & CP & CP  \\ 
K00665.02 & CP & CP & CP & CP  \\ 
K00665.03 & CP & CP & CP & CP  \\ 
K00666.01 & CP & PC & CP & CP  \\ 
K00670.01 & CP & PC & CP & CP  \\ 
K00671.01 & CP & CP & CP & CP  \\ 
K00671.02 & CP & CP & CP & CP  \\ 
K00671.03 & CP & CP & CP & CP  \\ 
K00671.04 & CP & CP & CP & CP  \\ 
K00672.01 & CP & CP & CP & CP  \\ 
K00672.02 & CP & CP & CP & CP  \\ 
K00672.03 & FP & FP & ND & FP  \\ 
K00673.01 & CP & PC & CP & CP  \\ 
K00674.01 & CP & PC & CP & CP  \\ 
K00678.01 & CP & CP & CP & CP  \\ 
K00678.02 & CP & CP & CP & CP  \\ 
K00679.01 & CP & CP & CP & CP  \\ 
K00679.02 & CP & CP & CP & CP  \\ 
K00680.01 & CP & CP & CP & CP  \\ 
K00682.01 & PC & \nodata & ND & PC  \\ 
K00683.01 & PC & PC & PC & PC  \\ 
K00684.01 & PC & PC & ND & PC  \\ 
K00685.01 & CP & PC & CP & CP  \\ 
K00686.01 & PC & PC & PC & PC  \\ 
K00687.01 & PC & PC & ND & PC  \\ 
K00688.01 & CP & PC & CP & CP  \\ 
K00689.01 & CP & PC & CP & CP  \\ 
K00691.01 & PC & PC & ND & PC  \\ 
K00691.02 & CP & PC & CP & CP  \\ 
K00692.01 & CP & CP & CP & CP  \\ 
K00692.02 & CP & CP & CP & CP  \\ 
K00693.01 & CP & CP & CP & CP  \\ 
K00693.02 & CP & CP & CP & CP  \\ 
K00694.01 & CP & PC & CP & CP  \\ 
K00695.01 & CP & PC & CP & CP  \\ 
K00697.01 & CP & PC & CP & CP  \\ 
K00700.01 & CP & CP & CP & CP  \\ 
K00700.02 & CP & CP & CP & CP  \\ 
K00700.03 & CP & CP & CP & CP  \\ 
K00700.04 & CP & CP & CP & CP  \\ 
K00701.01 & CP & CP & CP & CP  \\ 
K00701.02 & CP & CP & CP & CP  \\ 
K00701.03 & CP & CP & CP & CP  \\ 
K00701.04 & CP & CP & CP & CP  \\ 
K00701.05 & CP & CP & CP & CP  \\ 
K00703.01 & FP & FP & ND & FP  \\ 
K00704.01 & PC & PC & ND & PC  \\ 
K00707.01 & CP & CP & CP & CP  \\ 
K00707.02 & CP & CP & CP & CP  \\ 
K00707.03 & CP & CP & CP & CP  \\ 
K00707.04 & CP & CP & CP & CP  \\ 
K00707.05 & CP & CP & CP & CP  \\ 
K00708.01 & CP & CP & CP & CP  \\ 
K00708.02 & CP & CP & CP & CP  \\ 
K00709.01 & CP & PC & CP & CP  \\ 
K00710.01 & CP & CP & CP & CP  \\ 
K00710.02 & CP & CP & CP & CP  \\ 
K00710.03 & CP & PC & CP & CP  \\ 
K00711.01 & CP & CP & CP & CP  \\ 
K00711.02 & CP & CP & CP & CP  \\ 
K00711.03 & CP & PC & CP & CP  \\ 
K00712.01 & FP & FP & FP & FP  \\ 
K00714.01 & CP & PC & CP & CP  \\ 
K00717.01 & CP & PC & CP & CP  \\ 
K00717.02 & CP & PC & CP & CP  \\ 
K00718.01 & CP & CP & CP & CP  \\ 
K00718.02 & CP & CP & CP & CP  \\ 
K00718.03 & CP & CP & CP & CP  \\ 
K00719.01 & CP & CP & CP & CP  \\ 
K00719.02 & CP & CP & CP & CP  \\ 
K00719.03 & CP & CP & CP & CP  \\ 
K00719.04 & CP & CP & CP & CP  \\ 
K00720.01 & CP & CP & CP & CP  \\ 
K00720.02 & CP & CP & CP & CP  \\ 
K00720.03 & CP & CP & CP & CP  \\ 
K00720.04 & CP & CP & CP & CP  \\ 
K00721.01 & CP & PC & CP & CP  \\ 
K00722.01 & CP & PC & CP & CP  \\ 
K00723.01 & CP & CP & CP & CP  \\ 
K00723.02 & CP & CP & CP & CP  \\ 
K00723.03 & CP & CP & CP & CP  \\ 
K00730.01 & CP & CP & CP & CP  \\ 
K00730.02 & CP & CP & CP & CP  \\ 
K00730.03 & CP & CP & CP & CP  \\ 
K00730.04 & CP & CP & CP & CP  \\ 
K00732.01 & CP & PC & CP & CP  \\ 
K00732.02 & PC & PC & ND & PC  \\ 
K00732.03 & PC & PC & ND & PC  \\ 
K00733.01 & CP & CP & CP & CP  \\ 
K00733.02 & CP & CP & CP & CP  \\ 
K00733.03 & CP & CP & CP & CP  \\ 
K00733.04 & CP & CP & CP & CP  \\ 
K00734.01 & CP & PC & CP & CP  \\ 
K00734.02 & PC & PC & PC & PC  \\ 
K00738.01 & CP & CP & CP & CP  \\ 
K00738.02 & CP & CP & CP & CP  \\ 
K00749.01 & CP & CP & CP & CP  \\ 
K00749.02 & CP & CP & CP & CP  \\ 
K00749.03 & CP & CP & CP & CP  \\ 
K00752.01 & CP & CP & CP & CP  \\ 
K00752.02 & CP & CP & CP & CP  \\ 
K00756.01 & CP & CP & CP & CP  \\ 
K00756.02 & CP & CP & CP & CP  \\ 
K00756.03 & CP & CP & CP & CP  \\ 
K00757.01 & CP & CP & CP & CP  \\ 
K00757.02 & CP & CP & CP & CP  \\ 
K00757.03 & CP & CP & CP & CP  \\ 
K00759.01 & CP & CP & CP & CP  \\ 
K00759.02 & CP & CP & CP & CP  \\ 
K00760.01 & PC & PC & ND & PC  \\ 
K00771.01 & PC & \nodata & ND & PC  \\ 
K00800.01 & CP & CP & CP & CP  \\ 
K00800.02 & CP & CP & CP & CP  \\ 
K00806.01 & CP & CP & CP & CP  \\ 
K00806.02 & CP & CP & CP & CP  \\ 
K00806.03 & CP & \nodata & CP & CP  \\ 
K00806.04 & FP & \nodata & ND & FP  \\ 
K00806.05 & FP & \nodata & ND & FP  \\ 
K00825.01 & CP & CP & CP & CP  \\ 
K00825.02 & CP & CP & CP & CP  \\ 
K00829.01 & CP & CP & CP & CP  \\ 
K00829.02 & CP & CP & CP & CP  \\ 
K00829.03 & CP & CP & CP & CP  \\ 
K00834.01 & CP & CP & CP & CP  \\ 
K00834.02 & CP & CP & CP & CP  \\ 
K00834.03 & CP & CP & CP & CP  \\ 
K00834.04 & CP & CP & CP & CP  \\ 
K00834.05 & CP & CP & CP & CP  \\ 
K00835.01 & CP & CP & CP & CP  \\ 
K00835.02 & CP & CP & CP & CP  \\ 
K00837.01 & CP & CP & CP & CP  \\ 
K00837.02 & CP & CP & CP & CP  \\ 
K00841.01 & CP & CP & CP & CP  \\ 
K00841.02 & CP & CP & CP & CP  \\ 
K00841.03 & PC & PC & PC & PC  \\ 
K00841.04 & PC & PC & PC & PC  \\ 
K00841.05 & FP & \nodata & FP & FP  \\ 
K00853.01 & CP & CP & CP & CP  \\ 
K00853.02 & CP & CP & CP & CP  \\ 
K00857.01 & CP & CP & CP & CP  \\ 
K00857.02 & CP & CP & CP & CP  \\ 
K00864.01 & CP & CP & CP & CP  \\ 
K00864.02 & CP & CP & CP & CP  \\ 
K00864.03 & CP & CP & CP & CP  \\ 
K00869.01 & CP & CP & CP & CP  \\ 
K00869.02 & CP & CP & CP & CP  \\ 
K00869.03 & CP & CP & CP & CP  \\ 
K00869.04 & CP & PC & CP & CP  \\ 
K00870.01 & CP & CP & CP & CP  \\ 
K00870.02 & CP & CP & CP & CP  \\ 
K00872.01 & CP & CP & CP & CP  \\ 
K00872.02 & CP & CP & CP & CP  \\ 
K00874.01 & CP & CP & CP & CP  \\ 
K00874.02 & CP & CP & CP & CP  \\ 
K00880.01 & CP & CP & CP & CP  \\ 
K00880.02 & CP & CP & CP & CP  \\ 
K00880.03 & CP & CP & CP & CP  \\ 
K00880.04 & CP & CP & CP & CP  \\ 
K00881.01 & CP & PC & CP & CP  \\ 
K00881.02 & CP & PC & CP & CP  \\ 
K00884.01 & CP & CP & CP & CP  \\ 
K00884.02 & CP & CP & CP & CP  \\ 
K00884.03 & CP & CP & CP & CP  \\ 
K00889.01 & CP & CP & CP & CP  \\ 
K00892.01 & CP & PC & CP & CP  \\ 
K00892.02 & PC & PC & ND & PC  \\ 
K00896.01 & CP & CP & CP & CP  \\ 
K00896.02 & CP & CP & CP & CP  \\ 
K00896.03 & PC & PC & PC & PC  \\ 
K00906.01 & CP & CP & CP & CP  \\ 
K00906.02 & CP & CP & CP & CP  \\ 
K00906.03 & CP & CP & CP & CP  \\ 
K00907.01 & CP & CP & CP & CP  \\ 
K00907.02 & CP & CP & CP & CP  \\ 
K00907.03 & CP & CP & CP & CP  \\ 
K00907.04 & CP & CP & CP & CP  \\ 
K00918.01 & CP & PC & CP & CP  \\ 
K00918.02 & FP & \nodata & ND & FP  \\ 
K00921.01 & CP & CP & CP & CP  \\ 
K00921.02 & CP & CP & CP & CP  \\ 
K00921.03 & CP & CP & CP & CP  \\ 
K00934.01 & CP & CP & CP & CP  \\ 
K00934.02 & CP & CP & CP & CP  \\ 
K00934.03 & CP & CP & CP & CP  \\ 
K00935.01 & CP & CP & CP & CP  \\ 
K00935.02 & CP & CP & CP & CP  \\ 
K00935.03 & CP & CP & CP & CP  \\ 
K00935.04 & PC & PC & ND & PC  \\ 
K00939.01 & CP & CP & CP & CP  \\ 
K00939.02 & CP & CP & CP & CP  \\ 
K00939.03 & CP & CP & CP & CP  \\ 
K00939.04 & CP & CP & CP & CP  \\ 
K00941.01 & CP & CP & CP & CP  \\ 
K00941.02 & CP & CP & CP & CP  \\ 
K00941.03 & CP & CP & CP & CP  \\ 
K00954.01 & CP & CP & CP & CP  \\ 
K00954.02 & CP & CP & CP & CP  \\ 
K00958.01 & PC & PC & ND & PC  \\ 
K00974.01 & PC & PC & PC & PC  \\ 
K00975.01 & CP & CP & CP & CP  \\ 
K00981.01 & FP & \nodata & ND & FP  \\ 
K00986.01 & CP & CP & CP & CP  \\ 
K00986.02 & CP & CP & CP & CP  \\ 
K00987.01 & CP & PC & CP & CP  \\ 
K00988.01 & CP & CP & CP & CP  \\ 
K00988.02 & CP & CP & CP & CP  \\ 
K00991.01 & CP & PC & CP & CP  \\ 
K00993.01 & CP & CP & CP & CP  \\ 
K00993.02 & CP & CP & CP & CP  \\ 
K00993.03 & PC & PC & PC & PC  \\ 
K00999.01 & CP & CP & CP & CP  \\ 
K00999.02 & CP & CP & CP & CP  \\ 
K01001.01 & CP & CP & CP & CP  \\ 
K01001.02 & CP & CP & CP & CP  \\ 
K01002.01 & CP & PC & CP & CP  \\ 
K01010.01 & FP & \nodata & ND & FP  \\ 
K01015.01 & CP & PC & CP & CP  \\ 
K01015.02 & CP & PC & CP & CP  \\ 
K01015.03 & PC & PC & PC & PC  \\ 
K01019.01 & FP & \nodata & ND & FP  \\ 
K01032.01 & PC & \nodata & ND & PC  \\ 
K01050.01 & CP & PC & CP & CP  \\ 
K01050.02 & CP & PC & CP & CP  \\ 
K01052.01 & CP & CP & CP & CP  \\ 
K01052.02 & CP & CP & CP & CP  \\ 
K01052.03 & CP & CP & CP & CP  \\ 
K01052.04 & CP & CP & CP & CP  \\ 
K01054.01 & FP & \nodata & ND & FP  \\ 
K01060.01 & CP & PC & CP & CP  \\ 
K01060.02 & CP & PC & CP & CP  \\ 
K01060.03 & CP & PC & CP & CP  \\ 
K01060.04 & CP & PC & CP & CP  \\ 
K01069.01 & CP & PC & CP & CP  \\ 
K01069.02 & CP & PC & CP & CP  \\ 
K01089.01 & CP & CP & CP & CP  \\ 
K01089.02 & PC & PC & PC & PC  \\ 
K01102.01 & CP & CP & CP & CP  \\ 
K01102.02 & CP & CP & CP & CP  \\ 
K01102.03 & CP & CP & CP & CP  \\ 
K01102.04 & CP & CP & CP & CP  \\ 
K01113.01 & CP & CP & CP & CP  \\ 
K01113.02 & CP & CP & CP & CP  \\ 
K01115.01 & CP & PC & CP & CP  \\ 
K01116.01 & CP & PC & CP & CP  \\ 
K01117.01 & CP & PC & CP & CP  \\ 
K01118.01 & PC & PC & ND & PC  \\ 
K01120.01 & FP & FP & ND & FP  \\ 
K01126.01 & FP & FP & FP & FP  \\ 
K01126.02 & PC & PC & \nodata & PC  \\ 
K01127.01 & CP & CP & CP & CP  \\ 
K01127.02 & CP & CP & CP & CP  \\ 
K01127.03 & PC & PC & ND & PC  \\ 
K01128.01 & CP & PC & CP & CP  \\ 
K01145.01 & PC & PC & ND & PC  \\ 
K01148.01 & CP & CP & CP & CP  \\ 
K01148.02 & CP & CP & CP & CP  \\ 
K01150.01 & CP & PC & CP & CP  \\ 
K01151.01 & CP & CP & CP & CP  \\ 
K01151.02 & CP & CP & CP & CP  \\ 
K01151.03 & CP & PC & CP & CP  \\ 
K01151.04 & PC & PC & ND & PC  \\ 
K01151.05 & PC & PC & ND & PC  \\ 
K01161.01 & CP & CP & CP & CP  \\ 
K01161.02 & CP & CP & CP & CP  \\ 
K01161.03 & CP & CP & CP & CP  \\ 
K01162.01 & CP & PC & CP & CP  \\ 
K01163.01 & CP & CP & CP & CP  \\ 
K01163.02 & CP & CP & CP & CP  \\ 
K01165.01 & PC & PC & ND & PC  \\ 
K01165.02 & CP & PC & CP & CP  \\ 
K01168.01 & PC & \nodata & ND & PC  \\ 
K01169.01 & PC & PC & ND & PC  \\ 
K01175.01 & CP & PC & CP & CP  \\ 
K01175.02 & PC & PC & ND & PC  \\ 
K01196.01 & FP & FP & FP & FP  \\ 
K01196.02 & CP & CP & CP & CP  \\ 
K01196.03 & CP & CP & CP & CP  \\ 
K01198.01 & CP & CP & CP & CP  \\ 
K01198.02 & CP & CP & CP & CP  \\ 
K01198.03 & CP & CP & CP & CP  \\ 
K01198.04 & PC & \nodata & ND & PC  \\ 
K01199.01 & CP & PC & CP & CP  \\ 
K01203.01 & CP & CP & CP & CP  \\ 
K01203.02 & CP & CP & CP & CP  \\ 
K01203.03 & CP & CP & CP & CP  \\ 
K01206.01 & PC & \nodata & ND & PC  \\ 
K01208.01 & PC & \nodata & ND & PC  \\ 
K01209.01 & PC & \nodata & ND & PC  \\ 
K01215.01 & CP & CP & CP & CP  \\ 
K01215.02 & CP & CP & CP & CP  \\ 
K01216.01 & CP & PC & CP & CP  \\ 
K01218.01 & CP & PC & CP & CP  \\ 
K01220.01 & CP & PC & CP & CP  \\ 
K01221.01 & CP & CP & CP & CP  \\ 
K01221.02 & CP & CP & CP & CP  \\ 
K01222.01 & FP & \nodata & ND & FP  \\ 
K01230.01 & PC & PC & PC & PC  \\ 
K01239.01 & PC & PC & ND & PC  \\ 
K01239.02 & PC & PC & ND & PC  \\ 
K01240.01 & CP & CP & CP & CP  \\ 
K01240.02 & CP & CP & CP & CP  \\ 
K01241.01 & CP & CP & CP & CP  \\ 
K01241.02 & CP & CP & CP & CP  \\ 
K01242.01 & PC & PC & PC & PC  \\ 
K01257.01 & CP & CP & CP & CP  \\ 
K01270.01 & CP & CP & CP & CP  \\ 
K01270.02 & CP & CP & CP & CP  \\ 
K01271.01 & PC & PC & PC & PC  \\ 
K01274.01 & CP & \nodata & CP & CP  \\ 
K01275.01 & CP & PC & CP & CP  \\ 
K01276.01 & PC & PC & ND & PC  \\ 
K01276.02 & PC & PC & ND & PC  \\ 
K01278.01 & CP & CP & CP & CP  \\ 
K01278.02 & CP & CP & CP & CP  \\ 
K01278.03 & CP & CP & CP & CP  \\ 
K01278.04 & CP & CP & CP & CP  \\ 
K01279.01 & CP & PC & CP & CP  \\ 
K01279.02 & CP & PC & CP & CP  \\ 
K01282.01 & CP & PC & CP & CP  \\ 
K01283.01 & CP & PC & CP & CP  \\ 
K01288.01 & CP & PC & CP & CP  \\ 
K01299.01 & CP & CP & CP & CP  \\ 
K01300.01 & CP & PC & CP & CP  \\ 
K01301.01 & CP & CP & CP & CP  \\ 
K01301.02 & CP & CP & CP & CP  \\ 
K01305.01 & CP & CP & CP & CP  \\ 
K01305.02 & CP & CP & CP & CP  \\ 
K01306.01 & CP & CP & CP & CP  \\ 
K01306.02 & CP & CP & CP & CP  \\ 
K01306.03 & CP & CP & CP & CP  \\ 
K01306.04 & CP & CP & CP & CP  \\ 
K01307.01 & CP & CP & CP & CP  \\ 
K01307.02 & CP & CP & CP & CP  \\ 
K01308.01 & CP & PC & CP & CP  \\ 
K01311.01 & PC & PC & PC & PC  \\ 
K01314.01 & CP & PC & CP & CP  \\ 
K01315.01 & PC & PC & ND & PC  \\ 
K01316.01 & PC & PC & ND & PC  \\ 
K01316.02 & PC & \nodata & ND & PC  \\ 
K01332.01 & CP & CP & CP & CP  \\ 
K01332.02 & CP & CP & CP & CP  \\ 
K01332.03 & CP & CP & CP & CP  \\ 
K01335.01 & CP & PC & CP & CP  \\ 
K01336.01 & CP & CP & CP & CP  \\ 
K01336.02 & CP & CP & CP & CP  \\ 
K01336.03 & CP & CP & CP & CP  \\ 
K01336.04 & PC & PC & ND & PC  \\ 
K01338.01 & CP & PC & CP & CP  \\ 
K01338.02 & FP & FP & ND & FP  \\ 
K01338.03 & FP & FP & ND & FP  \\ 
K01344.01 & CP & PC & CP & CP  \\ 
K01353.01 & CP & CP & CP & CP  \\ 
K01353.02 & CP & CP & CP & CP  \\ 
K01356.01 & PC & \nodata & ND & PC  \\ 
K01359.01 & PC & PC & PC & PC  \\ 
K01359.02 & PC & PC & PC & PC  \\ 
K01360.01 & CP & CP & CP & CP  \\ 
K01360.02 & CP & CP & CP & CP  \\ 
K01360.03 & PC & PC & ND & PC  \\ 
K01363.01 & CP & CP & CP & CP  \\ 
K01363.02 & CP & CP & CP & CP  \\ 
K01364.01 & CP & CP & CP & CP  \\ 
K01364.02 & CP & CP & CP & CP  \\ 
K01364.03 & CP & CP & CP & CP  \\ 
K01364.04 & CP & CP & CP & CP  \\ 
K01364.05 & CP & CP & CP & CP  \\ 
K01366.01 & CP & CP & CP & CP  \\ 
K01366.02 & CP & CP & CP & CP  \\ 
K01367.01 & CP & PC & CP & CP  \\ 
K01375.01 & PC & PC & PC & PC  \\ 
K01378.01 & PC & PC & ND & PC  \\ 
K01378.02 & FP & FP & ND & FP  \\ 
K01379.01 & CP & PC & CP & CP  \\ 
K01396.01 & CP & CP & CP & CP  \\ 
K01396.02 & CP & CP & CP & CP  \\ 
K01411.01 & PC & PC & ND & PC  \\ 
K01412.01 & CP & PC & CP & CP  \\ 
K01413.01 & CP & CP & CP & CP  \\ 
K01413.02 & CP & CP & CP & CP  \\ 
K01413.03 & CP & CP & CP & CP  \\ 
K01421.01 & PC & \nodata & ND & PC  \\ 
K01426.01 & CP & CP & CP & CP  \\ 
K01426.02 & CP & CP & CP & CP  \\ 
K01426.03 & PC & PC & PC & PC  \\ 
K01428.01 & CP & PC & CP & CP  \\ 
K01431.01 & PC & PC & PC & PC  \\ 
K01432.01 & CP & CP & CP & CP  \\ 
K01432.02 & CP & CP & CP & CP  \\ 
K01432.03 & CP & CP & CP & CP  \\ 
K01432.04 & CP & CP & CP & CP  \\ 
K01436.01 & CP & CP & CP & CP  \\ 
K01436.02 & CP & CP & CP & CP  \\ 
K01436.03 & CP & CP & CP & CP  \\ 
K01438.01 & CP & PC & CP & CP  \\ 
K01439.01 & CP & PC & CP & CP  \\ 
K01442.01 & CP & CP & CP & CP  \\ 
K01444.01 & CP & PC & CP & CP  \\ 
K01445.01 & CP & PC & CP & CP  \\ 
K01445.02 & PC & \nodata & ND & PC  \\ 
K01445.03 & PC & \nodata & ND & PC  \\ 
K01463.01 & PC & \nodata & ND & PC  \\ 
K01466.01 & PC & PC & PC & PC  \\ 
K01474.01 & CP & CP & CP & CP  \\ 
K01477.01 & PC & PC & PC & PC  \\ 
K01478.01 & CP & PC & CP & CP  \\ 
K01480.01 & CP & PC & CP & CP  \\ 
K01480.02 & PC & PC & ND & PC  \\ 
K01483.01 & PC & PC & PC & PC  \\ 
K01486.01 & CP & CP & CP & CP  \\ 
K01486.02 & CP & CP & CP & CP  \\ 
K01528.01 & CP & PC & CP & CP  \\ 
K01529.01 & CP & CP & CP & CP  \\ 
K01529.02 & CP & CP & CP & CP  \\ 
K01530.01 & CP & PC & CP & CP  \\ 
K01531.01 & CP & PC & CP & CP  \\ 
K01532.01 & CP & PC & CP & CP  \\ 
K01533.01 & CP & PC & CP & CP  \\ 
K01534.01 & CP & PC & CP & CP  \\ 
K01534.02 & CP & PC & CP & CP  \\ 
K01535.01 & CP & PC & CP & CP  \\ 
K01536.01 & CP & PC & CP & CP  \\ 
K01537.01 & PC & PC & ND & PC  \\ 
K01546.01 & PC & \nodata & ND & PC  \\ 
K01557.01 & CP & CP & CP & CP  \\ 
K01557.02 & CP & CP & CP & CP  \\ 
K01557.03 & CP & CP & CP & CP  \\ 
K01557.04 & CP & PC & CP & CP  \\ 
K01563.01 & CP & CP & CP & CP  \\ 
K01563.02 & CP & CP & CP & CP  \\ 
K01563.03 & PC & PC & ND & PC  \\ 
K01563.04 & CP & CP & CP & CP  \\ 
K01567.01 & CP & CP & CP & CP  \\ 
K01567.02 & CP & CP & CP & CP  \\ 
K01567.03 & CP & CP & CP & CP  \\ 
K01567.04 & CP & CP & CP & CP  \\ 
K01576.01 & CP & CP & CP & CP  \\ 
K01576.02 & CP & CP & CP & CP  \\ 
K01576.03 & PC & \nodata & ND & PC  \\ 
K01581.01 & PC & PC & PC & PC  \\ 
K01581.02 & CP & PC & CP & CP  \\ 
K01589.01 & CP & CP & CP & CP  \\ 
K01589.02 & CP & CP & CP & CP  \\ 
K01589.03 & CP & CP & CP & CP  \\ 
K01589.04 & CP & CP & CP & CP  \\ 
K01589.05 & CP & CP & CP & CP  \\ 
K01590.01 & PC & PC & ND & PC  \\ 
K01590.02 & PC & PC & ND & PC  \\ 
K01590.03 & PC & PC & ND & PC  \\ 
K01596.01 & CP & CP & CP & CP  \\ 
K01596.02 & CP & CP & CP & CP  \\ 
K01598.01 & CP & CP & CP & CP  \\ 
K01598.02 & CP & CP & CP & CP  \\ 
K01598.03 & CP & CP & CP & CP  \\ 
K01601.01 & CP & PC & CP & CP  \\ 
K01601.02 & CP & PC & CP & CP  \\ 
K01606.01 & CP & PC & CP & CP  \\ 
K01608.01 & CP & CP & CP & CP  \\ 
K01608.02 & CP & CP & CP & CP  \\ 
K01608.03 & PC & PC & PC & PC  \\ 
K01609.01 & CP & PC & CP & CP  \\ 
K01612.01 & CP & CP & CP & CP  \\ 
K01615.01 & CP & PC & CP & CP  \\ 
K01616.01 & CP & PC & CP & CP  \\ 
K01616.02 & PC & \nodata & PC & PC  \\ 
K01618.01 & CP & PC & CP & CP  \\ 
K01619.01 & PC & PC & ND & PC  \\ 
K01621.01 & CP & PC & CP & CP  \\ 
K01623.01 & FP & FP & FP & FP  \\ 
K01628.01 & CP & CP & CP & CP  \\ 
K01628.02 & CP & CP & CP & CP  \\ 
K01628.03 & FP & FP & FP & FP  \\ 
K01629.01 & CP & PC & CP & CP  \\ 
K01632.01 & CP & PC & CP & CP  \\ 
K01639.01 & FP & \nodata & ND & FP  \\ 
K01639.02 & PC & \nodata & ND & PC  \\ 
K01647.01 & CP & CP & CP & CP  \\ 
K01647.02 & CP & CP & CP & CP  \\ 
K01647.03 & PC & PC & ND & PC  \\ 
K01655.01 & CP & PC & CP & CP  \\ 
K01665.01 & CP & PC & CP & CP  \\ 
K01665.02 & PC & \nodata & ND & PC  \\ 
K01666.01 & FP & FP & ND & FP  \\ 
K01669.01 & CP & PC & CP & CP  \\ 
K01688.01 & CP & PC & CP & CP  \\ 
K01692.01 & CP & CP & CP & CP  \\ 
K01692.02 & CP & CP & CP & CP  \\ 
K01695.01 & CP & PC & CP & CP  \\ 
K01706.01 & CP & PC & CP & CP  \\ 
K01707.01 & CP & CP & CP & CP  \\ 
K01707.02 & CP & CP & CP & CP  \\ 
K01715.01 & PC & PC & PC & PC  \\ 
K01726.01 & CP & PC & CP & CP  \\ 
K01738.01 & PC & PC & ND & PC  \\ 
K01739.01 & PC & \nodata & ND & PC  \\ 
K01751.01 & CP & PC & CP & CP  \\ 
K01751.02 & PC & PC & ND & PC  \\ 
K01754.01 & PC & PC & ND & PC  \\ 
K01779.01 & CP & CP & CP & CP  \\ 
K01779.02 & CP & CP & CP & CP  \\ 
K01781.01 & CP & PC & CP & CP  \\ 
K01781.02 & CP & CP & CP & CP  \\ 
K01781.03 & PC & PC & PC & PC  \\ 
K01783.01 & PC & PC & PC & PC  \\ 
K01783.02 & PC & PC & PC & PC  \\ 
K01792.01 & CP & PC & CP & CP  \\ 
K01792.02 & FP & FP & FP & FP  \\ 
K01792.03 & CP & PC & CP & CP  \\ 
K01796.01 & PC & PC & ND & PC  \\ 
K01797.01 & CP & PC & CP & CP  \\ 
K01800.01 & CP & CP & CP & CP  \\ 
K01802.01 & CP & PC & CP & CP  \\ 
K01803.01 & PC & PC & ND & PC  \\ 
K01803.02 & FP & FP & FP & FP  \\ 
K01803.03 & FP & FP & \nodata & FP  \\ 
K01805.01 & CP & CP & CP & CP  \\ 
K01805.02 & CP & CP & CP & CP  \\ 
K01805.03 & CP & CP & CP & CP  \\ 
K01806.01 & FP & FP & FP & FP  \\ 
K01806.02 & CP & CP & CP & CP  \\ 
K01806.03 & CP & CP & CP & CP  \\ 
K01808.01 & PC & PC & PC & PC  \\ 
K01809.01 & CP & CP & CP & CP  \\ 
K01809.02 & CP & CP & CP & CP  \\ 
K01812.01 & PC & PC & ND & PC  \\ 
K01813.01 & CP & PC & CP & CP  \\ 
K01815.01 & CP & PC & CP & CP  \\ 
K01818.01 & CP & PC & CP & CP  \\ 
K01819.01 & CP & PC & CP & CP  \\ 
K01820.01 & CP & CP & CP & CP  \\ 
K01820.02 & CP & CP & CP & CP  \\ 
K01822.01 & PC & PC & PC & PC  \\ 
K01824.01 & CP & CP & CP & CP  \\ 
K01824.02 & CP & CP & CP & CP  \\ 
K01825.01 & CP & PC & CP & CP  \\ 
K01826.01 & CP & PC & CP & CP  \\ 
K01831.01 & CP & CP & CP & CP  \\ 
K01831.02 & CP & CP & CP & CP  \\ 
K01831.03 & PC & PC & ND & PC  \\ 
K01831.04 & PC & PC & PC & PC  \\ 
K01832.01 & CP & CP & CP & CP  \\ 
K01832.02 & CP & CP & CP & CP  \\ 
K01832.03 & CP & CP & CP & CP  \\ 
K01835.01 & CP & CP & CP & CP  \\ 
K01835.02 & CP & CP & CP & CP  \\ 
K01835.03 & CP & CP & CP & CP  \\ 
K01837.01 & CP & PC & CP & CP  \\ 
K01837.02 & CP & PC & CP & CP  \\ 
K01839.01 & CP & PC & CP & CP  \\ 
K01839.02 & PC & \nodata & PC & PC  \\ 
K01841.01 & CP & PC & CP & CP  \\ 
K01845.01 & CP & PC & CP & CP  \\ 
K01845.02 & PC & PC & ND & PC  \\ 
K01848.01 & CP & PC & CP & CP  \\ 
K01850.01 & CP & PC & CP & CP  \\ 
K01852.01 & CP & PC & CP & CP  \\ 
K01854.01 & CP & PC & CP & CP  \\ 
K01856.01 & PC & PC & ND & PC  \\ 
K01857.01 & PC & PC & PC & PC  \\ 
K01858.01 & CP & PC & CP & CP  \\ 
K01858.02 & PC & \nodata & ND & PC  \\ 
K01860.01 & CP & CP & CP & CP  \\ 
K01860.02 & CP & CP & CP & CP  \\ 
K01860.03 & PC & PC & PC & PC  \\ 
K01860.04 & PC & PC & PC & PC  \\ 
K01861.01 & PC & PC & ND & PC  \\ 
K01862.01 & CP & PC & CP & CP  \\ 
K01863.01 & PC & PC & ND & PC  \\ 
K01864.01 & PC & PC & ND & PC  \\ 
K01871.01 & PC & PC & PC & PC  \\ 
K01871.02 & PC & PC & PC & PC  \\ 
K01875.01 & CP & PC & CP & CP  \\ 
K01875.02 & CP & PC & CP & CP  \\ 
K01877.01 & CP & PC & CP & CP  \\ 
K01878.01 & PC & PC & ND & PC  \\ 
K01883.01 & CP & PC & CP & CP  \\ 
K01886.01 & CP & PC & CP & CP  \\ 
K01888.01 & CP & PC & CP & CP  \\ 
K01889.01 & CP & PC & CP & CP  \\ 
K01889.02 & PC & PC & ND & PC  \\ 
K01890.01 & CP & PC & CP & CP  \\ 
K01891.01 & CP & CP & CP & CP  \\ 
K01891.02 & CP & CP & CP & CP  \\ 
K01893.01 & CP & PC & CP & CP  \\ 
K01894.01 & CP & PC & CP & CP  \\ 
K01897.01 & PC & PC & PC & PC  \\ 
K01898.01 & CP & PC & CP & CP  \\ 
K01901.01 & PC & PC & PC & PC  \\ 
K01904.01 & CP & PC & CP & CP  \\ 
K01905.01 & CP & CP & CP & CP  \\ 
K01905.02 & CP & CP & CP & CP  \\ 
K01905.03 & CP & CP & CP & CP  \\ 
K01909.01 & CP & CP & CP & CP  \\ 
K01909.02 & CP & CP & CP & CP  \\ 
K01909.03 & CP & CP & CP & CP  \\ 
K01913.01 & CP & PC & CP & CP  \\ 
K01915.01 & CP & CP & CP & CP  \\ 
K01915.02 & CP & CP & CP & CP  \\ 
K01916.01 & CP & CP & CP & CP  \\ 
K01916.02 & CP & CP & CP & CP  \\ 
K01916.03 & CP & CP & CP & CP  \\ 
K01917.01 & PC & PC & ND & PC  \\ 
K01921.01 & CP & PC & CP & CP  \\ 
K01922.01 & CP & PC & CP & CP  \\ 
K01922.02 & PC & \nodata & ND & PC  \\ 
K01922.03 & CP & PC & CP & CP  \\ 
K01923.01 & CP & PC & CP & CP  \\ 
K01924.01 & FP & FP & FP & FP  \\ 
K01925.01 & CP & CP & CP & CP  \\ 
K01928.01 & PC & PC & PC & PC  \\ 
K01929.01 & CP & CP & CP & CP  \\ 
K01929.02 & CP & CP & CP & CP  \\ 
K01930.01 & CP & CP & CP & CP  \\ 
K01930.02 & CP & CP & CP & CP  \\ 
K01930.03 & CP & CP & CP & CP  \\ 
K01930.04 & CP & CP & CP & CP  \\ 
K01931.01 & CP & CP & CP & CP  \\ 
K01931.02 & CP & CP & CP & CP  \\ 
K01931.03 & CP & CP & CP & CP  \\ 
K01938.01 & CP & PC & CP & CP  \\ 
K01944.01 & PC & PC & ND & PC  \\ 
K01944.02 & FP & \nodata & FP & FP  \\ 
K01945.01 & CP & PC & CP & CP  \\ 
K01945.02 & PC & \nodata & ND & PC  \\ 
K01947.01 & PC & PC & ND & PC  \\ 
K01951.01 & CP & PC & CP & CP  \\ 
K01952.01 & CP & CP & CP & CP  \\ 
K01952.02 & CP & CP & CP & CP  \\ 
K01952.03 & CP & CP & CP & CP  \\ 
K01952.04 & CP & CP & CP & CP  \\ 
K01955.01 & CP & CP & CP & CP  \\ 
K01955.02 & CP & CP & CP & CP  \\ 
K01955.03 & CP & PC & CP & CP  \\ 
K01955.04 & CP & CP & CP & CP  \\ 
K01958.01 & CP & CP & CP & CP  \\ 
K01960.01 & CP & CP & CP & CP  \\ 
K01960.02 & CP & CP & CP & CP  \\ 
K01961.01 & CP & PC & CP & CP  \\ 
K01961.02 & FP & \nodata & ND & FP  \\ 
K01962.01 & PC & PC & ND & PC  \\ 
K01963.01 & PC & PC & ND & PC  \\ 
K01964.01 & PC & PC & ND & PC  \\ 
K01970.01 & CP & CP & CP & CP  \\ 
K01970.02 & CP & CP & CP & CP  \\ 
K01978.01 & CP & CP & CP & CP  \\ 
K01978.02 & CP & CP & CP & CP  \\ 
K01979.01 & CP & PC & CP & CP  \\ 
K01980.01 & CP & PC & CP & CP  \\ 
K01984.01 & PC & PC & ND & PC  \\ 
K01985.01 & PC & PC & ND & PC  \\ 
K01988.01 & CP & PC & CP & CP  \\ 
K01989.01 & CP & PC & CP & CP  \\ 
K01992.01 & CP & CP & CP & CP  \\ 
K01992.02 & CP & CP & CP & CP  \\ 
K01992.03 & FP & FP & ND & FP  \\ 
K02001.01 & PC & PC & ND & PC  \\ 
K02002.01 & CP & PC & CP & CP  \\ 
K02004.01 & CP & PC & CP & CP  \\ 
K02004.02 & CP & PC & CP & CP  \\ 
K02004.03 & PC & PC & ND & PC  \\ 
K02007.01 & CP & PC & CP & CP  \\ 
K02007.02 & CP & PC & CP & CP  \\ 
K02009.01 & PC & PC & PC & PC  \\ 
K02010.01 & CP & PC & CP & CP  \\ 
K02011.01 & CP & CP & CP & CP  \\ 
K02011.02 & CP & CP & CP & CP  \\ 
K02012.01 & CP & PC & CP & CP  \\ 
K02012.02 & PC & \nodata & PC & PC  \\ 
K02016.01 & CP & PC & CP & CP  \\ 
K02017.01 & CP & PC & CP & CP  \\ 
K02022.01 & CP & CP & CP & CP  \\ 
K02022.02 & CP & CP & CP & CP  \\ 
K02026.01 & CP & PC & CP & CP  \\ 
K02029.01 & CP & CP & CP & CP  \\ 
K02029.02 & CP & CP & CP & CP  \\ 
K02029.03 & PC & PC & ND & PC  \\ 
K02029.04 & PC & PC & ND & PC  \\ 
K02033.01 & CP & PC & CP & CP  \\ 
K02035.01 & CP & PC & CP & CP  \\ 
K02037.01 & PC & PC & PC & PC  \\ 
K02037.02 & PC & PC & PC & PC  \\ 
K02037.03 & PC & PC & PC & PC  \\ 
K02038.01 & CP & CP & CP & CP  \\ 
K02038.02 & CP & CP & CP & CP  \\ 
K02038.03 & CP & \nodata & CP & CP  \\ 
K02038.04 & CP & CP & CP & CP  \\ 
K02039.01 & PC & PC & ND & PC  \\ 
K02039.02 & CP & PC & CP & CP  \\ 
K02040.01 & PC & PC & ND & PC  \\ 
K02043.01 & PC & PC & PC & PC  \\ 
K02044.01 & CP & PC & CP & CP  \\ 
K02046.01 & CP & PC & CP & CP  \\ 
K02047.01 & CP & PC & CP & CP  \\ 
K02048.01 & CP & PC & CP & CP  \\ 
K02048.02 & FP & FP & PC & FP  \\ 
K02049.01 & CP & PC & CP & CP  \\ 
K02051.01 & CP & CP & CP & CP  \\ 
K02051.02 & CP & CP & CP & CP  \\ 
K02053.01 & CP & CP & CP & CP  \\ 
K02053.02 & CP & CP & CP & CP  \\ 
K02071.01 & CP & PC & CP & CP  \\ 
K02072.01 & CP & PC & CP & CP  \\ 
K02073.01 & CP & CP & CP & CP  \\ 
K02073.02 & CP & CP & CP & CP  \\ 
K02073.03 & CP & CP & CP & CP  \\ 
K02076.01 & PC & PC & PC & PC  \\ 
K02076.02 & CP & PC & CP & CP  \\ 
K02079.01 & CP & PC & CP & CP  \\ 
K02081.01 & PC & PC & PC & PC  \\ 
K02081.02 & FP & \nodata & FP & FP  \\ 
K02082.01 & PC & PC & ND & PC  \\ 
K02083.01 & PC & PC & ND & PC  \\ 
K02086.01 & CP & CP & CP & CP  \\ 
K02086.02 & CP & CP & CP & CP  \\ 
K02086.03 & CP & CP & CP & CP  \\ 
K02086.04 & FP & \nodata & FP & FP  \\ 
K02087.01 & CP & PC & CP & CP  \\ 
K02092.01 & CP & CP & CP & CP  \\ 
K02092.02 & CP & CP & CP & CP  \\ 
K02092.03 & CP & CP & CP & CP  \\ 
K02093.01 & PC & PC & ND & PC  \\ 
K02093.02 & PC & PC & ND & PC  \\ 
K02093.03 & PC & PC & ND & PC  \\ 
K02094.01 & PC & PC & PC & PC  \\ 
K02094.02 & CP & PC & CP & CP  \\ 
K02098.01 & CP & PC & CP & CP  \\ 
K02098.02 & CP & PC & CP & CP  \\ 
K02105.01 & CP & PC & CP & CP  \\ 
K02109.01 & CP & PC & CP & CP  \\ 
K02110.01 & CP & PC & CP & CP  \\ 
K02111.01 & CP & CP & CP & CP  \\ 
K02111.02 & CP & CP & CP & CP  \\ 
K02115.01 & CP & CP & CP & CP  \\ 
K02119.01 & CP & PC & CP & CP  \\ 
K02120.01 & PC & PC & ND & PC  \\ 
K02135.01 & CP & CP & CP & CP  \\ 
K02135.02 & PC & PC & PC & PC  \\ 
K02135.03 & CP & CP & CP & CP  \\ 
K02137.01 & CP & PC & CP & CP  \\ 
K02143.01 & CP & PC & CP & CP  \\ 
K02147.01 & CP & CP & CP & CP  \\ 
K02147.02 & CP & CP & CP & CP  \\ 
K02148.01 & CP & CP & CP & CP  \\ 
K02148.02 & CP & CP & CP & CP  \\ 
K02148.03 & CP & CP & CP & CP  \\ 
K02149.01 & CP & PC & CP & CP  \\ 
K02153.01 & CP & CP & CP & CP  \\ 
K02153.02 & CP & CP & CP & CP  \\ 
K02158.01 & PC & PC & ND & PC  \\ 
K02158.02 & PC & PC & ND & PC  \\ 
K02159.01 & PC & PC & ND & PC  \\ 
K02159.02 & FP & FP & ND & FP  \\ 
K02162.01 & CP & PC & CP & CP  \\ 
K02162.02 & PC & PC & PC & PC  \\ 
K02167.01 & CP & PC & CP & CP  \\ 
K02167.02 & PC & \nodata & ND & PC  \\ 
K02167.03 & CP & PC & CP & CP  \\ 
K02168.01 & CP & CP & CP & CP  \\ 
K02168.02 & CP & CP & CP & CP  \\ 
K02169.01 & CP & PC & CP & CP  \\ 
K02169.02 & PC & PC & ND & PC  \\ 
K02169.03 & PC & PC & ND & PC  \\ 
K02169.04 & PC & PC & ND & PC  \\ 
K02173.01 & CP & CP & CP & CP  \\ 
K02173.02 & CP & CP & CP & CP  \\ 
K02175.01 & CP & CP & CP & CP  \\ 
K02175.02 & CP & CP & CP & CP  \\ 
K02183.01 & CP & CP & CP & CP  \\ 
K02183.02 & CP & CP & CP & CP  \\ 
K02183.03 & PC & \nodata & PC & PC  \\ 
K02188.01 & FP & FP & FP & FP  \\ 
K02188.02 & PC & \nodata & ND & PC  \\ 
K02194.01 & CP & CP & CP & CP  \\ 
K02194.02 & CP & CP & CP & CP  \\ 
K02194.03 & PC & \nodata & PC & PC  \\ 
K02195.01 & CP & CP & CP & CP  \\ 
K02195.02 & CP & CP & CP & CP  \\ 
K02195.03 & CP & CP & CP & CP  \\ 
K02201.01 & PC & PC & PC & PC  \\ 
K02202.01 & CP & PC & CP & CP  \\ 
K02208.01 & CP & PC & CP & CP  \\ 
K02218.01 & CP & CP & CP & CP  \\ 
K02218.02 & CP & CP & CP & CP  \\ 
K02219.01 & PC & PC & ND & PC  \\ 
K02220.01 & CP & CP & CP & CP  \\ 
K02220.02 & CP & CP & CP & CP  \\ 
K02220.03 & CP & CP & CP & CP  \\ 
K02220.04 & PC & PC & ND & PC  \\ 
K02220.05 & PC & \nodata & ND & PC  \\ 
K02228.01 & FP & \nodata & FP & FP  \\ 
K02236.01 & CP & CP & CP & CP  \\ 
K02236.02 & CP & CP & CP & CP  \\ 
K02246.01 & CP & PC & CP & CP  \\ 
K02248.01 & PC & PC & ND & PC  \\ 
K02248.02 & PC & \nodata & ND & PC  \\ 
K02248.03 & FP & FP & ND & FP  \\ 
K02248.04 & PC & \nodata & ND & PC  \\ 
K02250.01 & PC & PC & ND & PC  \\ 
K02250.02 & PC & PC & ND & PC  \\ 
K02252.01 & CP & PC & CP & CP  \\ 
K02260.01 & CP & PC & CP & CP  \\ 
K02261.01 & CP & PC & CP & CP  \\ 
K02261.02 & PC & \nodata & ND & PC  \\ 
K02273.01 & CP & PC & CP & CP  \\ 
K02278.01 & CP & CP & CP & CP  \\ 
K02278.02 & CP & CP & CP & CP  \\ 
K02279.01 & CP & CP & CP & CP  \\ 
K02279.02 & CP & CP & CP & CP  \\ 
K02281.01 & CP & PC & CP & CP  \\ 
K02281.02 & FP & \nodata & FP & FP  \\ 
K02287.01 & CP & CP & CP & CP  \\ 
K02287.02 & CP & CP & CP & CP  \\ 
K02289.01 & CP & CP & CP & CP  \\ 
K02289.02 & CP & CP & CP & CP  \\ 
K02290.01 & PC & PC & PC & PC  \\ 
K02295.01 & PC & PC & ND & PC  \\ 
K02300.01 & CP & PC & CP & CP  \\ 
K02312.01 & PC & \nodata & ND & PC  \\ 
K02319.01 & PC & PC & ND & PC  \\ 
K02331.01 & CP & PC & CP & CP  \\ 
K02332.01 & PC & PC & ND & PC  \\ 
K02333.01 & CP & CP & CP & CP  \\ 
K02333.02 & CP & CP & CP & CP  \\ 
K02335.01 & CP & PC & CP & CP  \\ 
K02339.01 & CP & PC & CP & CP  \\ 
K02339.02 & PC & \nodata & ND & PC  \\ 
K02342.01 & CP & PC & CP & CP  \\ 
K02352.01 & CP & CP & CP & CP  \\ 
K02352.02 & CP & CP & CP & CP  \\ 
K02352.03 & PC & PC & ND & PC  \\ 
K02357.01 & PC & PC & ND & PC  \\ 
K02357.02 & PC & PC & ND & PC  \\ 
K02358.01 & PC & PC & PC & PC  \\ 
K02365.01 & CP & CP & CP & CP  \\ 
K02365.02 & CP & CP & CP & CP  \\ 
K02366.01 & CP & PC & CP & CP  \\ 
K02367.01 & PC & PC & ND & PC  \\ 
K02369.01 & CP & PC & CP & CP  \\ 
K02369.02 & PC & \nodata & ND & PC  \\ 
K02369.03 & PC & PC & \nodata & PC  \\ 
K02370.01 & PC & PC & PC & PC  \\ 
K02372.01 & CP & PC & CP & CP  \\ 
K02374.01 & CP & CP & CP & CP  \\ 
K02374.02 & CP & CP & CP & CP  \\ 
K02389.01 & CP & PC & CP & CP  \\ 
K02390.01 & CP & PC & CP & CP  \\ 
K02393.01 & PC & PC & PC & PC  \\ 
K02393.02 & PC & PC & PC & PC  \\ 
K02396.01 & FP & FP & ND & FP  \\ 
K02398.01 & PC & PC & ND & PC  \\ 
K02399.01 & CP & PC & CP & CP  \\ 
K02403.01 & CP & PC & CP & CP  \\ 
K02407.01 & CP & PC & CP & CP  \\ 
K02408.01 & CP & PC & CP & CP  \\ 
K02409.01 & CP & PC & CP & CP  \\ 
K02410.01 & PC & \nodata & ND & PC  \\ 
K02410.02 & PC & \nodata & ND & PC  \\ 
K02414.01 & CP & CP & CP & CP  \\ 
K02414.02 & CP & CP & CP & CP  \\ 
K02422.01 & CP & PC & CP & CP  \\ 
K02422.02 & PC & PC & PC & PC  \\ 
K02426.01 & CP & PC & CP & CP  \\ 
K02433.01 & CP & CP & CP & CP  \\ 
K02433.02 & CP & CP & CP & CP  \\ 
K02433.03 & PC & PC & PC & PC  \\ 
K02433.04 & PC & PC & PC & PC  \\ 
K02433.05 & FP & FP & ND & FP  \\ 
K02433.06 & PC & PC & PC & PC  \\ 
K02433.07 & PC & \nodata & PC & PC  \\ 
K02440.01 & CP & PC & CP & CP  \\ 
K02442.01 & CP & CP & CP & CP  \\ 
K02442.02 & CP & CP & CP & CP  \\ 
K02443.01 & CP & CP & CP & CP  \\ 
K02443.02 & CP & CP & CP & CP  \\ 
K02462.01 & PC & PC & ND & PC  \\ 
K02463.01 & CP & PC & CP & CP  \\ 
K02469.01 & PC & PC & PC & PC  \\ 
K02470.01 & FP & FP & ND & FP  \\ 
K02473.01 & CP & CP & CP & CP  \\ 
K02473.02 & FP & \nodata & ND & FP  \\ 
K02473.03 & CP & CP & CP & CP  \\ 
K02474.01 & PC & \nodata & ND & PC  \\ 
K02479.01 & PC & PC & ND & PC  \\ 
K02481.01 & PC & \nodata & ND & PC  \\ 
K02484.01 & CP & PC & CP & CP  \\ 
K02486.01 & PC & PC & ND & PC  \\ 
K02488.01 & CP & PC & CP & CP  \\ 
K02492.01 & CP & PC & CP & CP  \\ 
K02498.01 & CP & CP & CP & CP  \\ 
K02498.02 & CP & CP & CP & CP  \\ 
K02503.01 & PC & PC & ND & PC  \\ 
K02516.01 & PC & PC & ND & PC  \\ 
K02517.01 & CP & PC & CP & CP  \\ 
K02521.01 & CP & PC & CP & CP  \\ 
K02521.02 & PC & PC & ND & PC  \\ 
K02522.01 & PC & PC & ND & PC  \\ 
K02529.01 & CP & PC & CP & CP  \\ 
K02529.02 & CP & CP & CP & CP  \\ 
K02530.01 & CP & PC & CP & CP  \\ 
K02533.01 & CP & PC & CP & CP  \\ 
K02533.02 & FP & \nodata & ND & FP  \\ 
K02533.03 & PC & \nodata & PC & PC  \\ 
K02534.01 & CP & PC & CP & CP  \\ 
K02534.02 & PC & PC & ND & PC  \\ 
K02538.01 & PC & PC & ND & PC  \\ 
K02541.01 & CP & CP & CP & CP  \\ 
K02541.02 & CP & CP & CP & CP  \\ 
K02545.01 & CP & PC & CP & CP  \\ 
K02547.01 & PC & PC & ND & PC  \\ 
K02555.01 & CP & PC & CP & CP  \\ 
K02556.01 & CP & PC & CP & CP  \\ 
K02559.01 & PC & PC & ND & PC  \\ 
K02561.01 & CP & PC & CP & CP  \\ 
K02563.01 & CP & PC & CP & CP  \\ 
K02563.02 & PC & \nodata & ND & PC  \\ 
K02564.01 & CP & PC & CP & CP  \\ 
K02564.02 & PC & PC & \nodata & PC  \\ 
K02571.01 & PC & PC & ND & PC  \\ 
K02581.01 & PC & PC & ND & PC  \\ 
K02582.01 & PC & PC & ND & PC  \\ 
K02583.01 & PC & PC & ND & PC  \\ 
K02585.01 & CP & CP & CP & CP  \\ 
K02585.02 & CP & CP & CP & CP  \\ 
K02585.03 & PC & PC & ND & PC  \\ 
K02590.01 & FP & \nodata & ND & FP  \\ 
K02590.02 & PC & PC & ND & PC  \\ 
K02593.01 & CP & PC & CP & CP  \\ 
K02595.01 & CP & CP & CP & CP  \\ 
K02595.02 & CP & CP & CP & CP  \\ 
K02597.01 & CP & CP & CP & CP  \\ 
K02597.02 & CP & CP & CP & CP  \\ 
K02597.03 & PC & PC & ND & PC  \\ 
K02603.01 & PC & PC & PC & PC  \\ 
K02607.01 & PC & PC & ND & PC  \\ 
K02608.01 & CP & PC & CP & CP  \\ 
K02612.01 & PC & PC & ND & PC  \\ 
K02612.02 & PC & PC & ND & PC  \\ 
K02623.01 & CP & PC & CP & CP  \\ 
K02623.02 & PC & PC & \nodata & PC  \\ 
K02631.01 & PC & PC & ND & PC  \\ 
K02631.02 & FP & \nodata & ND & FP  \\ 
K02632.01 & CP & PC & CP & CP  \\ 
K02635.01 & CP & PC & CP & CP  \\ 
K02636.01 & PC & PC & ND & PC  \\ 
K02636.02 & PC & PC & \nodata & PC  \\ 
K02639.01 & PC & PC & ND & PC  \\ 
K02639.02 & PC & \nodata & ND & PC  \\ 
K02640.01 & PC & \nodata & ND & PC  \\ 
K02641.01 & PC & PC & ND & PC  \\ 
K02657.01 & PC & PC & ND & PC  \\ 
K02659.01 & PC & \nodata & ND & PC  \\ 
K02668.01 & CP & PC & CP & CP  \\ 
K02672.01 & CP & CP & CP & CP  \\ 
K02672.02 & CP & CP & CP & CP  \\ 
K02674.01 & FP & FP & PC & FP  \\ 
K02674.02 & CP & PC & CP & CP  \\ 
K02674.03 & CP & PC & CP & CP  \\ 
K02675.01 & CP & PC & CP & CP  \\ 
K02675.02 & PC & PC & ND & PC  \\ 
K02676.01 & FP & FP & FP & FP  \\ 
K02677.01 & PC & PC & PC & PC  \\ 
K02678.01 & CP & PC & CP & CP  \\ 
K02681.01 & CP & CP & CP & CP  \\ 
K02681.02 & CP & CP & CP & CP  \\ 
K02686.01 & PC & PC & PC & PC  \\ 
K02687.01 & PC & PC & ND & PC  \\ 
K02687.02 & PC & PC & ND & PC  \\ 
K02690.01 & FP & FP & ND & FP  \\ 
K02694.01 & CP & PC & CP & CP  \\ 
K02694.02 & PC & PC & ND & PC  \\ 
K02698.01 & CP & PC & CP & CP  \\ 
K02706.01 & PC & PC & ND & PC  \\ 
K02707.01 & CP & CP & CP & CP  \\ 
K02707.02 & CP & CP & CP & CP  \\ 
K02707.03 & CP & CP & CP & CP  \\ 
K02711.01 & CP & CP & CP & CP  \\ 
K02711.02 & CP & CP & CP & CP  \\ 
K02712.01 & PC & PC & ND & PC  \\ 
K02714.01 & CP & CP & CP & CP  \\ 
K02714.02 & CP & CP & CP & CP  \\ 
K02714.03 & CP & PC & CP & CP  \\ 
K02717.01 & CP & PC & CP & CP  \\ 
K02720.01 & PC & PC & ND & PC  \\ 
K02722.01 & CP & CP & CP & CP  \\ 
K02722.02 & CP & CP & CP & CP  \\ 
K02722.03 & CP & CP & CP & CP  \\ 
K02722.04 & CP & CP & CP & CP  \\ 
K02722.05 & PC & PC & ND & PC  \\ 
K02729.01 & CP & PC & CP & CP  \\ 
K02730.01 & CP & PC & CP & CP  \\ 
K02732.01 & CP & CP & CP & CP  \\ 
K02732.02 & CP & PC & CP & CP  \\ 
K02732.03 & CP & CP & CP & CP  \\ 
K02732.04 & PC & PC & PC & PC  \\ 
K02733.01 & PC & PC & ND & PC  \\ 
K02737.01 & FP & FP & ND & FP  \\ 
K02740.01 & FP & FP & ND & FP  \\ 
K02741.01 & FP & FP & FP & FP  \\ 
K02743.01 & CP & PC & CP & CP  \\ 
K02748.01 & CP & PC & CP & CP  \\ 
K02748.02 & CP & PC & CP & CP  \\ 
K02749.01 & FP & FP & ND & FP  \\ 
K02750.01 & PC & PC & PC & PC  \\ 
K02752.01 & FP & FP & ND & FP  \\ 
K02753.01 & CP & PC & CP & CP  \\ 
K02754.01 & CP & PC & CP & CP  \\ 
K02755.01 & PC & PC & ND & PC  \\ 
K02756.01 & CP & PC & CP & CP  \\ 
K02756.02 & PC & PC & \nodata & PC  \\ 
K02758.01 & PC & PC & PC & PC  \\ 
K02762.01 & CP & PC & CP & CP  \\ 
K02763.01 & FP & FP & ND & FP  \\ 
K02765.01 & FP & FP & ND & FP  \\ 
K02768.01 & CP & \nodata & CP & CP  \\ 
K02768.02 & CP & \nodata & CP & CP  \\ 
K02768.03 & FP & PC & FP & PC  \\ 
K02769.01 & FP & FP & FP & FP  \\ 
K02771.01 & FP & FP & FP & FP  \\ 
K02781.01 & FP & FP & ND & FP  \\ 
K02785.01 & CP & PC & CP & CP  \\ 
K02786.01 & CP & PC & CP & CP  \\ 
K02790.01 & CP & PC & CP & CP  \\ 
K02792.01 & CP & PC & CP & CP  \\ 
K02796.01 & FP & FP & ND & FP  \\ 
K02801.01 & PC & PC & ND & PC  \\ 
K02803.01 & PC & PC & ND & PC  \\ 
K02805.01 & CP & PC & CP & CP  \\ 
K02807.01 & PC & PC & ND & PC  \\ 
K02815.01 & PC & PC & ND & PC  \\ 
K02828.01 & CP & PC & CP & CP  \\ 
K02828.02 & FP & FP & PC & FP  \\ 
K02829.01 & PC & PC & ND & PC  \\ 
K02831.01 & FP & FP & ND & FP  \\ 
K02832.01 & CP & PC & CP & CP  \\ 
K02833.01 & PC & PC & ND & PC  \\ 
K02838.01 & CP & PC & CP & CP  \\ 
K02838.02 & CP & PC & CP & CP  \\ 
K02840.01 & PC & PC & ND & PC  \\ 
K02840.02 & PC & PC & ND & PC  \\ 
K02841.01 & PC & PC & PC & PC  \\ 
K02848.01 & PC & PC & ND & PC  \\ 
K02857.01 & CP & PC & CP & CP  \\ 
K02857.02 & CP & PC & CP & CP  \\ 
K02859.01 & CP & PC & CP & CP  \\ 
K02859.02 & CP & PC & CP & CP  \\ 
K02859.03 & PC & PC & ND & PC  \\ 
K02859.04 & PC & \nodata & ND & PC  \\ 
K02859.05 & PC & PC & \nodata & PC  \\ 
K02863.01 & FP & FP & FP & FP  \\ 
K02864.01 & FP & FP & ND & FP  \\ 
K02866.01 & CP & PC & CP & CP  \\ 
K02874.01 & FP & FP & ND & FP  \\ 
K02875.01 & FP & FP & ND & FP  \\ 
K02879.01 & FP & FP & ND & FP  \\ 
K02884.01 & FP & FP & ND & FP  \\ 
K02885.01 & FP & FP & ND & FP  \\ 
K02891.01 & FP & FP & FP & FP  \\ 
K02896.01 & FP & FP & ND & FP  \\ 
K02896.02 & FP & FP & \nodata & FP  \\ 
K02904.01 & CP & PC & CP & CP  \\ 
K02906.01 & CP & PC & CP & CP  \\ 
K02906.02 & PC & \nodata & PC & PC  \\ 
K02913.01 & CP & PC & CP & CP  \\ 
K02915.01 & PC & PC & ND & PC  \\ 
K02916.01 & PC & PC & ND & PC  \\ 
K02925.01 & PC & PC & ND & PC  \\ 
K02926.01 & CP & PC & CP & CP  \\ 
K02926.02 & CP & PC & CP & CP  \\ 
K02926.03 & CP & PC & CP & CP  \\ 
K02926.04 & CP & PC & CP & CP  \\ 
K02931.01 & CP & PC & CP & CP  \\ 
K02943.01 & CP & PC & CP & CP  \\ 
K02949.01 & PC & PC & ND & PC  \\ 
K02949.02 & PC & PC & ND & PC  \\ 
K02951.01 & CP & PC & CP & CP  \\ 
K02956.01 & CP & PC & CP & CP  \\ 
K02960.01 & FP & FP & ND & FP  \\ 
K02961.01 & CP & PC & CP & CP  \\ 
K02964.01 & CP & PC & CP & CP  \\ 
K02968.01 & PC & PC & ND & PC  \\ 
K02969.01 & FP & FP & FP & FP  \\ 
K02970.01 & PC & PC & ND & PC  \\ 
K02971.01 & PC & PC & PC & PC  \\ 
K02971.02 & PC & \nodata & PC & PC  \\ 
K02974.01 & FP & FP & ND & FP  \\ 
K02977.01 & CP & PC & CP & CP  \\ 
K02977.02 & CP & PC & CP & CP  \\ 
K02979.01 & FP & FP & ND & FP  \\ 
K02984.01 & PC & PC & ND & PC  \\ 
K03008.01 & CP & PC & CP & CP  \\ 
K03009.01 & CP & PC & CP & CP  \\ 
K03012.01 & FP & FP & ND & FP  \\ 
K03015.01 & CP & PC & CP & CP  \\ 
K03017.01 & PC & PC & ND & PC  \\ 
K03021.01 & FP & FP & ND & FP  \\ 
K03023.01 & FP & FP & ND & FP  \\ 
K03032.01 & CP & PC & CP & CP  \\ 
K03039.01 & CP & PC & CP & CP  \\ 
K03046.01 & FP & \nodata & ND & FP  \\ 
K03052.01 & PC & PC & ND & PC  \\ 
K03052.02 & PC & PC & ND & PC  \\ 
K03057.01 & CP & CP & CP & CP  \\ 
K03057.02 & CP & CP & CP & CP  \\ 
K03060.01 & CP & PC & CP & CP  \\ 
K03065.01 & PC & PC & ND & PC  \\ 
K03075.01 & PC & PC & ND & PC  \\ 
K03083.01 & PC & PC & ND & PC  \\ 
K03083.02 & PC & \nodata & ND & PC  \\ 
K03083.03 & PC & \nodata & ND & PC  \\ 
K03086.01 & PC & PC & PC & PC  \\ 
K03087.01 & FP & FP & ND & FP  \\ 
K03087.02 & FP & \nodata & ND & FP  \\ 
K03093.01 & CP & PC & CP & CP  \\ 
K03096.01 & CP & PC & CP & CP  \\ 
K03097.01 & CP & CP & CP & CP  \\ 
K03097.02 & CP & CP & CP & CP  \\ 
K03097.03 & CP & CP & CP & CP  \\ 
K03100.01 & FP & FP & FP & FP  \\ 
K03103.01 & FP & \nodata & ND & FP  \\ 
K03109.01 & CP & PC & CP & CP  \\ 
K03111.01 & PC & PC & ND & PC  \\ 
K03111.02 & PC & PC & ND & PC  \\ 
K03114.01 & PC & PC & ND & PC  \\ 
K03117.01 & PC & PC & ND & PC  \\ 
K03122.01 & CP & PC & CP & CP  \\ 
K03125.01 & CP & PC & CP & CP  \\ 
K03128.01 & PC & PC & ND & PC  \\ 
K03130.01 & PC & PC & ND & PC  \\ 
K03130.02 & PC & PC & ND & PC  \\ 
K03132.01 & FP & FP & ND & FP  \\ 
K03146.01 & CP & PC & CP & CP  \\ 
K03158.01 & CP & \nodata & CP & CP  \\ 
K03158.02 & CP & CP & CP & CP  \\ 
K03158.03 & CP & CP & CP & CP  \\ 
K03158.04 & CP & CP & CP & CP  \\ 
K03158.05 & CP & CP & CP & CP  \\ 
K03165.01 & PC & PC & ND & PC  \\ 
K03167.01 & FP & FP & ND & FP  \\ 
K03168.01 & PC & PC & PC & PC  \\ 
K03172.01 & FP & FP & ND & FP  \\ 
K03172.02 & FP & \nodata & ND & FP  \\ 
K03179.01 & PC & PC & ND & PC  \\ 
K03180.01 & FP & \nodata & ND & FP  \\ 
K03184.01 & PC & PC & ND & PC  \\ 
K03184.02 & FP & \nodata & ND & FP  \\ 
K03184.03 & PC & PC & \nodata & PC  \\ 
K03190.01 & PC & PC & ND & PC  \\ 
K03193.01 & PC & PC & ND & PC  \\ 
K03194.01 & PC & PC & ND & PC  \\ 
K03195.01 & FP & \nodata & ND & FP  \\ 
K03196.01 & PC & PC & ND & PC  \\ 
K03196.02 & PC & PC & ND & PC  \\ 
K03197.01 & PC & PC & ND & PC  \\ 
K03201.01 & FP & \nodata & ND & FP  \\ 
K03202.01 & FP & FP & PC & FP  \\ 
K03203.01 & PC & PC & PC & PC  \\ 
K03208.01 & PC & PC & ND & PC  \\ 
K03214.01 & PC & PC & PC & PC  \\ 
K03214.02 & PC & PC & PC & PC  \\ 
K03215.01 & FP & FP & ND & FP  \\ 
K03218.01 & FP & FP & FP & FP  \\ 
K03220.01 & CP & PC & CP & CP  \\ 
K03224.01 & PC & PC & ND & PC  \\ 
K03225.01 & PC & PC & ND & PC  \\ 
K03227.01 & FP & FP & ND & FP  \\ 
K03232.01 & PC & PC & ND & PC  \\ 
K03233.01 & FP & \nodata & ND & FP  \\ 
K03234.01 & CP & PC & CP & CP  \\ 
K03236.01 & PC & PC & ND & PC  \\ 
K03237.01 & CP & PC & CP & CP  \\ 
K03239.01 & FP & FP & ND & FP  \\ 
K03240.01 & FP & FP & FP & FP  \\ 
K03244.01 & FP & PC & FP & PC  \\ 
K03245.01 & CP & PC & CP & CP  \\ 
K03246.01 & CP & PC & CP & CP  \\ 
K03248.01 & PC & PC & ND & PC  \\ 
K03249.01 & FP & FP & FP & FP  \\ 
K03251.01 & FP & \nodata & ND & FP  \\ 
K03254.01 & FP & FP & ND & FP  \\ 
K03277.01 & CP & PC & CP & CP  \\ 
K03278.01 & FP & PC & FP & PC  \\ 
K03283.01 & FP & \nodata & ND & FP  \\ 
K03283.02 & PC & PC & PC & PC  \\ 
K03283.03 & PC & \nodata & PC & PC  \\ 
K03287.01 & CP & PC & CP & CP  \\ 
K03288.01 & CP & PC & CP & CP  \\ 
K03301.01 & PC & PC & ND & PC  \\ 
K03308.01 & CP & PC & CP & CP  \\ 
K03308.02 & CP & PC & CP & CP  \\ 
K03310.01 & PC & PC & ND & PC  \\ 
K03315.01 & CP & PC & CP & CP  \\ 
K03338.01 & FP & FP & FP & FP  \\ 
K03338.02 & FP & FP & FP & FP  \\ 
K03340.01 & PC & PC & ND & PC  \\ 
K03340.02 & PC & PC & ND & PC  \\ 
K03346.01 & CP & PC & CP & CP  \\ 
K03358.01 & PC & PC & ND & PC  \\ 
K03363.01 & CP & PC & CP & CP  \\ 
K03371.01 & PC & \nodata & PC & PC  \\ 
K03371.02 & CP & PC & CP & CP  \\ 
K03378.01 & FP & FP & ND & FP  \\ 
K03382.01 & FP & FP & ND & FP  \\ 
K03384.01 & PC & PC & ND & PC  \\ 
K03384.02 & CP & PC & CP & CP  \\ 
K03403.01 & CP & PC & CP & CP  \\ 
K03403.02 & PC & PC & ND & PC  \\ 
K03419.01 & PC & PC & PC & PC  \\ 
K03421.01 & PC & PC & ND & PC  \\ 
K03422.01 & PC & PC & ND & PC  \\ 
K03425.01 & PC & PC & ND & PC  \\ 
K03425.02 & PC & PC & ND & PC  \\ 
K03425.03 & PC & PC & \nodata & PC  \\ 
K03436.01 & CP & PC & CP & CP  \\ 
K03438.01 & CP & PC & CP & CP  \\ 
K03451.01 & PC & PC & ND & PC  \\ 
K03456.01 & CP & PC & CP & CP  \\ 
K03456.02 & PC & \nodata & PC & PC  \\ 
K03465.01 & CP & PC & CP & CP  \\ 
K03473.01 & PC & PC & ND & PC  \\ 
K03474.01 & PC & PC & PC & PC  \\ 
K03497.01 & CP & PC & CP & CP  \\ 
K03500.01 & PC & PC & PC & PC  \\ 
K03500.02 & FP & FP & ND & FP  \\ 
K03503.01 & PC & PC & PC & PC  \\ 
K03503.02 & PC & PC & PC & PC  \\ 
K03541.01 & PC & PC & PC & PC  \\ 
K03608.01 & PC & PC & PC & PC  \\ 
K03641.01 & FP & PC & FP & PC  \\ 
K03641.02 & FP & \nodata & FP & FP  \\ 
K03663.01 & CP & CP & CP & CP  \\ 
K03678.01 & CP & PC & CP & CP  \\ 
K03680.01 & PC & PC & PC & PC  \\ 
K03681.01 & CP & PC & CP & CP  \\ 
K03681.02 & PC & PC & PC & PC  \\ 
K03683.01 & CP & PC & CP & CP  \\ 
K03689.01 & PC & PC & ND & PC  \\ 
K03726.01 & PC & PC & PC & PC  \\ 
K03770.01 & PC & PC & ND & PC  \\ 
K03780.01 & PC & PC & ND & PC  \\ 
K03787.01 & PC & PC & PC & PC  \\ 
K03791.01 & CP & PC & CP & CP  \\ 
K03791.02 & CP & PC & CP & CP  \\ 
K03801.01 & PC & PC & PC & PC  \\ 
K03811.01 & PC & PC & PC & PC  \\ 
K03823.01 & PC & PC & PC & PC  \\ 
K03835.01 & CP & PC & CP & CP  \\ 
K03853.01 & PC & PC & ND & PC  \\ 
K03864.01 & PC & PC & ND & PC  \\ 
K03864.02 & PC & \nodata & ND & PC  \\ 
K03867.01 & CP & PC & CP & CP  \\ 
K03871.01 & FP & FP & FP & FP  \\ 
K03876.01 & PC & PC & ND & PC  \\ 
K03880.01 & PC & PC & ND & PC  \\ 
K03886.01 & PC & PC & ND & PC  \\ 
K03889.01 & FP & FP & FP & FP  \\ 
K03890.01 & PC & PC & PC & PC  \\ 
K03891.01 & PC & PC & ND & PC  \\ 
K03892.01 & CP & PC & CP & CP  \\ 
K03907.01 & PC & PC & ND & PC  \\ 
K03908.01 & PC & PC & PC & PC  \\ 
K03913.01 & PC & PC & ND & PC  \\ 
K03925.01 & PC & PC & ND & PC  \\ 
K03925.02 & CP & PC & CP & CP  \\ 
K03925.03 & CP & PC & CP & CP  \\ 
K03928.01 & CP & PC & CP & CP  \\ 
K03936.01 & FP & PC & FP & PC  \\ 
K03936.02 & PC & PC & PC & PC  \\ 
K03943.01 & PC & PC & ND & PC  \\ 
K03946.01 & CP & PC & CP & CP  \\ 
K03980.01 & FP & FP & ND & FP  \\ 
K03991.01 & PC & PC & ND & PC  \\ 
K04002.01 & PC & PC & ND & PC  \\ 
K04004.01 & PC & PC & ND & PC  \\ 
K04005.01 & CP & CP & CP & CP  \\ 
K04011.01 & FP & FP & ND & FP  \\ 
K04014.01 & PC & PC & PC & PC  \\ 
K04018.01 & FP & FP & ND & FP  \\ 
K04021.01 & PC & PC & ND & PC  \\ 
K04021.02 & PC & PC & ND & PC  \\ 
K04022.01 & FP & FP & ND & FP  \\ 
K04024.01 & CP & PC & CP & CP  \\ 
K04032.01 & CP & PC & CP & CP  \\ 
K04032.02 & CP & PC & CP & CP  \\ 
K04032.03 & CP & PC & CP & CP  \\ 
K04032.04 & CP & PC & CP & CP  \\ 
K04032.05 & PC & PC & \nodata & PC  \\ 
K04036.01 & CP & PC & CP & CP  \\ 
K04037.01 & PC & PC & PC & PC  \\ 
K04053.01 & PC & PC & ND & PC  \\ 
K04054.01 & PC & PC & PC & PC  \\ 
K04060.01 & PC & PC & PC & PC  \\ 
K04062.01 & FP & FP & ND & FP  \\ 
K04066.01 & PC & PC & PC & PC  \\ 
K04067.01 & PC & PC & ND & PC  \\ 
K04070.01 & FP & FP & ND & FP  \\ 
K04072.01 & CP & PC & CP & CP  \\ 
K04098.01 & PC & PC & ND & PC  \\ 
K04103.01 & CP & PC & CP & CP  \\ 
K04103.02 & PC & PC & PC & PC  \\ 
K04109.01 & PC & PC & ND & PC  \\ 
K04121.01 & CP & PC & CP & CP  \\ 
K04123.01 & PC & PC & ND & PC  \\ 
K04129.01 & PC & PC & ND & PC  \\ 
K04136.01 & PC & PC & ND & PC  \\ 
K04136.02 & PC & PC & ND & PC  \\ 
K04144.01 & PC & PC & ND & PC  \\ 
K04146.01 & CP & PC & CP & CP  \\ 
K04156.01 & PC & PC & ND & PC  \\ 
K04157.01 & PC & PC & ND & PC  \\ 
K04157.02 & PC & PC & \nodata & PC  \\ 
K04159.01 & CP & PC & CP & CP  \\ 
K04160.01 & CP & PC & CP & CP  \\ 
K04184.01 & PC & PC & ND & PC  \\ 
K04188.01 & PC & PC & ND & PC  \\ 
K04190.01 & CP & PC & CP & CP  \\ 
K04198.01 & FP & FP & ND & FP  \\ 
K04199.01 & CP & PC & CP & CP  \\ 
K04204.01 & CP & PC & CP & CP  \\ 
K04212.01 & CP & PC & CP & CP  \\ 
K04212.02 & PC & PC & ND & PC  \\ 
K04215.01 & CP & PC & CP & CP  \\ 
K04222.01 & CP & PC & CP & CP  \\ 
K04226.01 & PC & PC & ND & PC  \\ 
K04230.01 & CP & PC & CP & CP  \\ 
K04235.01 & PC & PC & PC & PC  \\ 
K04245.01 & PC & PC & ND & PC  \\ 
K04246.01 & CP & PC & CP & CP  \\ 
K04246.02 & PC & \nodata & PC & PC  \\ 
K04251.01 & PC & PC & ND & PC  \\ 
K04257.01 & FP & FP & ND & FP  \\ 
K04269.01 & PC & PC & ND & PC  \\ 
K04269.02 & FP & FP & ND & FP  \\ 
K04273.01 & PC & PC & ND & PC  \\ 
K04276.01 & CP & PC & CP & CP  \\ 
K04287.01 & PC & PC & PC & PC  \\ 
K04287.02 & PC & PC & PC & PC  \\ 
K04288.01 & CP & PC & CP & CP  \\ 
K04288.02 & PC & PC & ND & PC  \\ 
K04288.03 & FP & FP & \nodata & FP  \\ 
K04292.01 & CP & PC & CP & CP  \\ 
K04296.01 & PC & PC & ND & PC  \\ 
K04298.01 & FP & FP & ND & FP  \\ 
K04298.02 & FP & FP & \nodata & FP  \\ 
K04301.01 & CP & PC & CP & CP  \\ 
K04301.02 & PC & PC & \nodata & PC  \\ 
K04302.01 & PC & PC & ND & PC  \\ 
K04304.01 & CP & PC & CP & CP  \\ 
K04312.01 & CP & PC & CP & CP  \\ 
K04318.01 & PC & \nodata & ND & PC  \\ 
K04323.01 & PC & PC & PC & PC  \\ 
K04323.02 & FP & FP & FP & FP  \\ 
K04329.01 & PC & PC & ND & PC  \\ 
K04335.01 & CP & PC & CP & CP  \\ 
K04343.01 & PC & PC & ND & PC  \\ 
K04356.01 & CP & PC & CP & CP  \\ 
K04366.01 & PC & PC & ND & PC  \\ 
K04367.01 & PC & PC & PC & PC  \\ 
K04368.01 & FP & FP & FP & FP  \\ 
K04368.02 & PC & PC & ND & PC  \\ 
K04374.01 & PC & PC & ND & PC  \\ 
K04382.01 & CP & PC & CP & CP  \\ 
K04382.02 & PC & \nodata & ND & PC  \\ 
K04383.01 & CP & PC & CP & CP  \\ 
K04383.02 & PC & PC & \nodata & PC  \\ 
K04385.01 & PC & PC & PC & PC  \\ 
K04385.02 & CP & PC & CP & CP  \\ 
K04385.03 & PC & PC & PC & PC  \\ 
K04399.01 & PC & PC & ND & PC  \\ 
K04400.01 & CP & PC & CP & CP  \\ 
K04407.01 & PC & PC & ND & PC  \\ 
K04409.01 & PC & PC & ND & PC  \\ 
K04411.01 & CP & PC & CP & CP  \\ 
K04418.01 & PC & \nodata & ND & PC  \\ 
K04421.01 & PC & PC & ND & PC  \\ 
K04421.02 & PC & PC & \nodata & PC  \\ 
K04423.01 & PC & PC & ND & PC  \\ 
K04426.01 & PC & \nodata & ND & PC  \\ 
K04430.01 & FP & FP & ND & FP  \\ 
K04431.01 & PC & PC & ND & PC  \\ 
K04431.02 & FP & \nodata & ND & FP  \\ 
K04435.01 & PC & PC & PC & PC  \\ 
K04435.02 & PC & \nodata & PC & PC  \\ 
K04441.01 & CP & PC & CP & CP  \\ 
K04443.01 & PC & PC & ND & PC  \\ 
K04446.01 & CP & PC & CP & CP  \\ 
K04452.01 & PC & PC & ND & PC  \\ 
K04457.01 & PC & PC & PC & PC  \\ 
K04469.01 & FP & FP & ND & FP  \\ 
K04473.01 & CP & PC & CP & CP  \\ 
K04480.01 & PC & PC & PC & PC  \\ 
K04482.01 & PC & PC & ND & PC  \\ 
K04505.01 & PC & PC & ND & PC  \\ 
K04546.01 & PC & PC & ND & PC  \\ 
K04556.01 & FP & FP & ND & FP  \\ 
K04557.01 & PC & PC & ND & PC  \\ 
K04561.01 & CP & PC & CP & CP  \\ 
K04567.01 & PC & PC & PC & PC  \\ 
K04567.02 & PC & PC & PC & PC  \\ 
K04575.01 & PC & \nodata & PC & PC  \\ 
K04580.01 & PC & PC & ND & PC  \\ 
K04581.01 & PC & PC & ND & PC  \\ 
K04582.01 & PC & PC & ND & PC  \\ 
K04585.01 & CP & PC & CP & CP  \\ 
K04588.01 & PC & PC & ND & PC  \\ 
K04601.01 & PC & PC & ND & PC  \\ 
K04603.01 & PC & PC & ND & PC  \\ 
K04605.01 & PC & PC & ND & PC  \\ 
K04613.01 & PC & PC & ND & PC  \\ 
K04614.01 & PC & PC & ND & PC  \\ 
K04617.01 & CP & PC & CP & CP  \\ 
K04633.01 & PC & PC & ND & PC  \\ 
K04634.01 & PC & PC & ND & PC  \\ 
K04637.01 & PC & PC & ND & PC  \\ 
K04640.01 & CP & PC & CP & CP  \\ 
K04647.01 & PC & PC & PC & PC  \\ 
K04647.02 & PC & PC & PC & PC  \\ 
K04651.01 & PC & PC & ND & PC  \\ 
K04653.01 & PC & PC & ND & PC  \\ 
K04657.01 & FP & FP & PC & FP  \\ 
K04657.02 & PC & PC & PC & PC  \\ 
K04659.01 & PC & PC & ND & PC  \\ 
K04663.01 & PC & PC & ND & PC  \\ 
K04665.01 & FP & \nodata & FP & FP  \\ 
K04674.01 & PC & PC & ND & PC  \\ 
K04686.01 & PC & PC & ND & PC  \\ 
K04693.01 & CP & PC & CP & CP  \\ 
K04699.01 & PC & PC & ND & PC  \\ 
K04706.01 & CP & PC & CP & CP  \\ 
K04715.01 & PC & PC & PC & PC  \\ 
K04716.01 & PC & PC & ND & PC  \\ 
K04716.02 & PC & PC & \nodata & PC  \\ 
K04717.01 & PC & \nodata & ND & PC  \\ 
K04725.01 & PC & PC & ND & PC  \\ 
K04744.01 & FP & FP & ND & FP  \\ 
K04745.01 & CP & CP & CP & CP  \\ 
K04746.01 & FP & FP & ND & FP  \\ 
K04763.01 & PC & PC & PC & PC  \\ 
K04765.01 & CP & PC & CP & CP  \\ 
K04771.01 & PC & \nodata & PC & PC  \\ 
K04773.01 & PC & PC & ND & PC  \\ 
K04774.01 & PC & PC & PC & PC  \\ 
K04775.01 & PC & PC & ND & PC  \\ 
K04792.01 & PC & PC & ND & PC  \\ 
K04811.01 & PC & PC & ND & PC  \\ 
K04822.01 & PC & PC & ND & PC  \\ 
K04829.01 & PC & PC & ND & PC  \\ 
K04829.02 & FP & \nodata & ND & FP  \\ 
K04833.01 & PC & PC & ND & PC  \\ 
K04834.01 & PC & PC & ND & PC  \\ 
K04839.01 & PC & \nodata & ND & PC  \\ 
K04841.01 & FP & \nodata & ND & FP  \\ 
K04850.01 & PC & PC & ND & PC  \\ 
K04864.01 & PC & PC & ND & PC  \\ 
K04881.01 & PC & PC & ND & PC  \\ 
K04881.02 & FP & FP & \nodata & FP  \\ 
K04887.01 & FP & FP & ND & FP  \\ 
K04892.01 & PC & PC & ND & PC  \\ 
K04898.01 & PC & \nodata & PC & PC  \\ 
K04902.01 & PC & \nodata & PC & PC  \\ 
K04907.01 & PC & PC & ND & PC  \\ 
K04941.01 & FP & \nodata & FP & FP  \\ 
K04961.01 & PC & \nodata & PC & PC  \\ 
K04978.01 & PC & \nodata & PC & PC  \\ 
K05018.01 & PC & PC & PC & PC  \\ 
K05021.01 & PC & \nodata & PC & PC  \\ 
K05039.01 & FP & \nodata & FP & FP  \\ 
K05048.01 & PC & \nodata & PC & PC  \\ 
K05057.01 & PC & \nodata & PC & PC  \\ 
K05084.01 & CP & PC & CP & CP  \\ 
K05085.01 & PC & \nodata & PC & PC  \\ 
K05107.01 & PC & \nodata & PC & PC  \\ 
K05119.01 & PC & \nodata & PC & PC  \\ 
K05124.01 & PC & PC & PC & PC  \\ 
K05135.01 & PC & \nodata & PC & PC  \\ 
K05155.01 & PC & PC & PC & PC  \\ 
K05159.01 & FP & \nodata & FP & FP  \\ 
K05198.01 & FP & \nodata & FP & FP  \\ 
K05216.01 & PC & \nodata & PC & PC  \\ 
K05236.01 & PC & PC & PC & PC  \\ 
K05241.01 & PC & PC & PC & PC  \\ 
K05247.01 & PC & \nodata & PC & PC  \\ 
K05269.01 & PC & \nodata & PC & PC  \\ 
K05278.01 & PC & PC & PC & PC  \\ 
K05284.01 & PC & PC & PC & PC  \\ 
K05290.01 & PC & \nodata & PC & PC  \\ 
K05324.01 & PC & \nodata & PC & PC  \\ 
K05375.01 & PC & \nodata & PC & PC  \\ 
K05379.01 & PC & \nodata & PC & PC  \\ 
K05380.01 & PC & \nodata & PC & PC  \\ 
K05393.01 & PC & \nodata & PC & PC  \\ 
K05423.01 & PC & \nodata & PC & PC  \\ 
K05546.01 & PC & \nodata & PC & PC  \\ 
K05567.01 & PC & PC & PC & PC  \\ 
K05592.01 & PC & \nodata & PC & PC  \\ 
K05612.01 & PC & \nodata & PC & PC  \\ 
K05613.01 & PC & \nodata & PC & PC  \\ 
K05622.01 & CP & PC & CP & CP  \\ 
K05625.01 & PC & PC & PC & PC  \\ 
K05626.01 & PC & \nodata & PC & PC  \\ 
K05645.01 & PC & \nodata & PC & PC  \\ 
K05689.01 & PC & \nodata & PC & PC  \\ 
K05702.01 & PC & \nodata & PC & PC  \\ 
K05706.01 & CP & PC & CP & CP  \\ 
K05782.01 & PC & \nodata & PC & PC  \\ 
K05790.01 & PC & PC & PC & PC  \\ 
K05792.01 & PC & PC & PC & PC  \\ 
K05798.01 & PC & \nodata & PC & PC  \\ 
K05837.01 & PC & \nodata & PC & PC  \\ 
K05850.01 & PC & PC & PC & PC  \\ 
K05852.01 & PC & \nodata & PC & PC  \\ 
K05855.01 & PC & PC & PC & PC  \\ 
K05869.01 & PC & \nodata & PC & PC  \\ 
K05877.01 & PC & \nodata & PC & PC  \\ 
K05888.01 & PC & \nodata & PC & PC  \\ 
K05900.01 & FP & \nodata & FP & FP  \\ 
K05900.02 & FP & FP & \nodata & FP  \\ 
K05924.01 & PC & \nodata & PC & PC  \\ 
K05929.01 & PC & PC & PC & PC  \\ 
K05932.01 & PC & \nodata & PC & PC  \\ 
K05949.01 & PC & \nodata & PC & PC  \\ 
K05953.01 & PC & \nodata & PC & PC  \\ 
K06102.01 & PC & \nodata & PC & PC  \\ 
K06384.01 & PC & PC & \nodata & PC  \\ 
K06425.01 & PC & PC & \nodata & PC  \\ 
K06676.01 & PC & PC & \nodata & PC  \\ 
K06734.01 & PC & PC & \nodata & PC  \\ 
K06745.01 & PC & PC & \nodata & PC  \\ 
K06759.01 & PC & PC & \nodata & PC  \\ 
K06786.01 & PC & PC & \nodata & PC  \\ 
K06883.01 & FP & FP & \nodata & FP  \\ 
K06927.01 & FP & FP & \nodata & FP  \\ 
K06971.01 & PC & PC & \nodata & PC  \\ 
K06981.01 & FP & FP & \nodata & FP  \\ 
K07016.01 & CP & CP & \nodata & CP  \\ 
K07040.01 & PC & PC & \nodata & PC  \\ 
K07136.01 & PC & PC & \nodata & PC  \\ 
K07179.01 & PC & PC & \nodata & PC  \\ 
K07223.01 & PC & PC & \nodata & PC  \\ 
K07235.01 & PC & PC & \nodata & PC  \\ 
K07345.01 & PC & PC & \nodata & PC  \\ 
K07566.01 & FP & FP & \nodata & FP  \\ 
K07587.01 & PC & PC & \nodata & PC  \\ 
K07599.01 & PC & PC & \nodata & PC  \\ 
K07605.01 & FP & FP & \nodata & FP  \\ 
KIC8435766.01 & CP & \nodata & \nodata & \nodata  \\ 
KIC11187332.01 & CP & \nodata & \nodata & \nodata  \\ 
KIC2718885.01 & CP & \nodata & \nodata & \nodata  \\ 
KIC6359893.01 & CP & \nodata & \nodata & \nodata  \\ 


==> table3.tex <==
          1 &   1 &   0 &   0 &   0 &   0 &   0 \\
          2 &   1 &   0 &   0 &   0 &   0 &   0 \\
          3 &   1 &   0 &   0 &   0 &   0 &   0 \\
          6 &   1 &   0 &   0 &   0 &   0 &   1 \\
          7 &   1 &   0 &   0 &   0 &   0 &   0 \\
          8 &   1 &   0 &   0 &   0 &   0 &   1 \\
         10 &   1 &   0 &   0 &   0 &   0 &   0 \\
         17 &   1 &   0 &   0 &   0 &   0 &   0 \\
         18 &   1 &   0 &   0 &   0 &   0 &   0 \\
         20 &   1 &   0 &   0 &   0 &   0 &   0 \\
         22 &   1 &   0 &   0 &   0 &   0 &   0 \\
         41 &   1 &   1 &   0 &   0 &   0 &   0 \\
         42 &   1 &   0 &   0 &   0 &   0 &   0 \\
         46 &   1 &   1 &   0 &   0 &   0 &   0 \\
         49 &   1 &   0 &   0 &   0 &   0 &   0 \\
         63 &   1 &   0 &   0 &   0 &   0 &   0 \\
         64 &   1 &   0 &   0 &   0 &   0 &   0 \\
         69 &   1 &   0 &   0 &   0 &   0 &   0 \\
         70 &   1 &   1 &   0 &   0 &   0 &   0 \\
         72 &   1 &   1 &   0 &   1 &   0 &   0 \\
         75 &   1 &   0 &   0 &   0 &   0 &   0 \\
         82 &   1 &   1 &   0 &   0 &   0 &   0 \\
         84 &   1 &   0 &   0 &   0 &   0 &   0 \\
         85 &   1 &   1 &   0 &   0 &   0 &   0 \\
         87 &   1 &   0 &   1 &   0 &   0 &   0 \\
         92 &   1 &   0 &   0 &   0 &   0 &   0 \\
         94 &   1 &   1 &   0 &   0 &   0 &   0 \\
         97 &   1 &   0 &   0 &   0 &   0 &   0 \\
         98 &   1 &   0 &   0 &   0 &   0 &   0 \\
         99 &   1 &   1 &   0 &   0 &   0 &   0 \\
        102 &   1 &   1 &   0 &   0 &   0 &   0 \\
        103 &   1 &   0 &   0 &   0 &   0 &   0 \\
        104 &   1 &   0 &   0 &   0 &   0 &   0 \\
        105 &   1 &   0 &   0 &   0 &   0 &   0 \\
        107 &   1 &   0 &   0 &   0 &   0 &   0 \\
        108 &   1 &   1 &   0 &   0 &   0 &   0 \\
        110 &   1 &   0 &   0 &   0 &   0 &   0 \\
        111 &   1 &   1 &   0 &   0 &   0 &   0 \\
        112 &   1 &   1 &   0 &   0 &   0 &   0 \\
        113 &   1 &   0 &   1 &   0 &   0 &   1 \\
        115 &   1 &   1 &   0 &   0 &   0 &   0 \\
        116 &   1 &   1 &   0 &   0 &   0 &   0 \\
        117 &   1 &   1 &   0 &   0 &   0 &   0 \\
        118 &   1 &   0 &   0 &   0 &   0 &   0 \\
        119 &   1 &   1 &   1 &   0 &   0 &   0 \\
        122 &   1 &   0 &   0 &   0 &   0 &   0 \\
        123 &   1 &   1 &   0 &   0 &   0 &   0 \\
        124 &   1 &   1 &   0 &   0 &   0 &   0 \\
        127 &   1 &   0 &   0 &   0 &   0 &   0 \\
        128 &   1 &   0 &   0 &   0 &   0 &   0 \\
        134 &   1 &   0 &   0 &   0 &   0 &   1 \\
        135 &   1 &   0 &   0 &   0 &   0 &   0 \\
        137 &   1 &   1 &   0 &   0 &   0 &   0 \\
        139 &   1 &   1 &   1 &   0 &   0 &   0 \\
        141 &   1 &   0 &   0 &   0 &   0 &   0 \\
        142 &   1 &   1 &   0 &   0 &   0 &   0 \\
        144 &   1 &   0 &   0 &   0 &   0 &   0 \\
        145 &   1 &   0 &   0 &   0 &   0 &   0 \\
        148 &   1 &   1 &   0 &   0 &   0 &   0 \\
        149 &   1 &   0 &   0 &   0 &   0 &   0 \\
        150 &   1 &   1 &   0 &   0 &   0 &   0 \\
        152 &   1 &   1 &   0 &   0 &   0 &   0 \\
        153 &   1 &   1 &   0 &   0 &   0 &   0 \\
        155 &   1 &   0 &   0 &   0 &   0 &   0 \\
        156 &   1 &   1 &   0 &   0 &   0 &   0 \\
        157 &   1 &   1 &   0 &   0 &   0 &   0 \\
        159 &   1 &   1 &   0 &   0 &   0 &   0 \\
        161 &   1 &   0 &   0 &   0 &   0 &   0 \\
        162 &   1 &   0 &   0 &   0 &   0 &   0 \\
        163 &   1 &   0 &   0 &   0 &   0 &   0 \\
        165 &   1 &   0 &   0 &   0 &   0 &   0 \\
        166 &   1 &   0 &   0 &   0 &   0 &   0 \\
        167 &   1 &   0 &   0 &   0 &   0 &   0 \\
        168 &   1 &   1 &   0 &   0 &   0 &   0 \\
        171 &   1 &   1 &   0 &   0 &   0 &   0 \\
        172 &   1 &   1 &   1 &   0 &   0 &   0 \\
        173 &   1 &   0 &   0 &   0 &   0 &   0 \\
        174 &   1 &   0 &   0 &   0 &   0 &   0 \\
        176 &   1 &   0 &   0 &   0 &   0 &   0 \\
        177 &   1 &   0 &   0 &   0 &   0 &   0 \\
        179 &   1 &   1 &   1 &   0 &   0 &   0 \\
        180 &   1 &   0 &   0 &   0 &   0 &   0 \\
        186 &   0 &   0 &   0 &   0 &   1 &   0 \\
        191 &   0 &   1 &   0 &   1 &   0 &   0 \\
        193 &   0 &   0 &   0 &   0 &   1 &   1 \\
        195 &   0 &   0 &   0 &   0 &   1 &   0 \\
        197 &   1 &   0 &   0 &   0 &   0 &   0 \\
        201 &   1 &   0 &   0 &   0 &   0 &   0 \\
        203 &   1 &   0 &   0 &   0 &   0 &   0 \\
        209 &   0 &   1 &   0 &   0 &   0 &   0 \\
        211 &   0 &   0 &   1 &   0 &   0 &   0 \\
        214 &   0 &   0 &   0 &   0 &   1 &   0 \\
        232 &   0 &   1 &   0 &   0 &   0 &   0 \\
        237 &   1 &   0 &   0 &   0 &   0 &   0 \\
        238 &   1 &   1 &   0 &   0 &   0 &   0 \\
        241 &   1 &   1 &   0 &   0 &   0 &   0 \\
        244 &   1 &   1 &   0 &   0 &   0 &   0 \\
        245 &   1 &   1 &   0 &   0 &   0 &   0 \\
        246 &   1 &   1 &   0 &   0 &   0 &   0 \\
        257 &   1 &   0 &   0 &   0 &   0 &   0 \\
        260 &   1 &   1 &   0 &   0 &   0 &   0 \\
        261 &   1 &   0 &   0 &   0 &   0 &   0 \\
        262 &   1 &   1 &   0 &   0 &   0 &   0 \\
        263 &   1 &   0 &   0 &   0 &   0 &   1 \\
        265 &   1 &   0 &   0 &   0 &   0 &   0 \\
        266 &   1 &   1 &   0 &   0 &   0 &   0 \\
        268 &   1 &   0 &   1 &   0 &   0 &   0 \\
        269 &   1 &   0 &   0 &   0 &   0 &   0 \\
        270 &   1 &   1 &   0 &   0 &   0 &   0 \\
        271 &   1 &   1 &   0 &   0 &   0 &   0 \\
        273 &   1 &   0 &   0 &   0 &   0 &   0 \\
        274 &   1 &   1 &   0 &   0 &   0 &   0 \\
        275 &   1 &   1 &   0 &   0 &   0 &   0 \\
        276 &   1 &   0 &   0 &   0 &   0 &   0 \\
        277 &   1 &   1 &   0 &   0 &   0 &   0 \\
        279 &   1 &   1 &   0 &   0 &   0 &   0 \\
        280 &   1 &   0 &   0 &   0 &   0 &   0 \\
        281 &   1 &   0 &   0 &   0 &   0 &   0 \\
        282 &   1 &   1 &   0 &   0 &   0 &   0 \\
        283 &   1 &   1 &   0 &   0 &   0 &   0 \\
        284 &   1 &   1 &   0 &   0 &   0 &   0 \\
        285 &   1 &   1 &   0 &   0 &   0 &   0 \\
        288 &   1 &   0 &   0 &   0 &   0 &   1 \\
        289 &   1 &   1 &   0 &   0 &   0 &   0 \\
        291 &   1 &   1 &   0 &   0 &   0 &   0 \\
        292 &   1 &   0 &   0 &   0 &   0 &   0 \\
        294 &   1 &   0 &   0 &   0 &   0 &   0 \\
        295 &   1 &   1 &   0 &   0 &   0 &   0 \\
        296 &   1 &   0 &   0 &   0 &   0 &   0 \\
        297 &   1 &   0 &   0 &   0 &   0 &   0 \\
        299 &   1 &   0 &   0 &   0 &   0 &   0 \\
        301 &   1 &   1 &   0 &   0 &   0 &   0 \\
        303 &   1 &   0 &   0 &   0 &   0 &   0 \\
        304 &   1 &   1 &   0 &   0 &   0 &   0 \\
        305 &   1 &   0 &   0 &   0 &   0 &   0 \\
        306 &   1 &   0 &   0 &   0 &   0 &   0 \\
        307 &   1 &   1 &   0 &   0 &   0 &   0 \\
        308 &   1 &   0 &   0 &   0 &   0 &   0 \\
        312 &   1 &   1 &   0 &   0 &   0 &   0 \\
        313 &   1 &   1 &   0 &   0 &   0 &   0 \\
        315 &   1 &   0 &   0 &   0 &   0 &   0 \\
        316 &   1 &   1 &   0 &   0 &   0 &   0 \\
        317 &   1 &   0 &   0 &   0 &   0 &   0 \\
        318 &   1 &   0 &   0 &   0 &   0 &   0 \\
        319 &   1 &   0 &   0 &   0 &   0 &   0 \\
        321 &   1 &   1 &   0 &   0 &   0 &   0 \\
        323 &   1 &   0 &   0 &   0 &   0 &   0 \\
        327 &   1 &   1 &   0 &   0 &   0 &   0 \\
        328 &   1 &   0 &   0 &   0 &   0 &   1 \\
        330 &   1 &   1 &   0 &   0 &   0 &   0 \\
        331 &   1 &   0 &   0 &   0 &   0 &   0 \\
        332 &   1 &   1 &   0 &   0 &   0 &   0 \\
        333 &   1 &   0 &   0 &   0 &   0 &   0 \\
        337 &   1 &   1 &   0 &   0 &   0 &   0 \\
        338 &   1 &   1 &   0 &   0 &   0 &   0 \\
        339 &   1 &   1 &   0 &   0 &   0 &   0 \\
        340 &   1 &   0 &   0 &   0 &   0 &   1 \\
        341 &   1 &   1 &   0 &   0 &   0 &   0 \\
        343 &   1 &   1 &   0 &   0 &   0 &   0 \\
        344 &   1 &   0 &   0 &   0 &   0 &   0 \\
        345 &   1 &   0 &   0 &   0 &   0 &   0 \\
        346 &   1 &   0 &   0 &   0 &   0 &   0 \\
        348 &   1 &   0 &   0 &   0 &   0 &   0 \\
        349 &   1 &   0 &   0 &   0 &   0 &   0 \\
        350 &   1 &   0 &   0 &   0 &   0 &   0 \\
        351 &   1 &   1 &   1 &   0 &   0 &   0 \\
        352 &   1 &   1 &   0 &   0 &   0 &   0 \\
        355 &   1 &   0 &   0 &   0 &   0 &   0 \\
        356 &   1 &   0 &   0 &   0 &   0 &   0 \\
        360 &   1 &   0 &   0 &   0 &   0 &   1 \\
        361 &   1 &   0 &   0 &   0 &   0 &   0 \\
        364 &   1 &   0 &   0 &   0 &   0 &   0 \\
        365 &   1 &   1 &   1 &   0 &   0 &   0 \\
        367 &   1 &   0 &   0 &   0 &   0 &   0 \\
        369 &   1 &   1 &   0 &   0 &   0 &   0 \\
        370 &   1 &   1 &   0 &   0 &   0 &   0 \\
        371 &   1 &   1 &   0 &   0 &   0 &   0 \\
        372 &   1 &   0 &   0 &   0 &   0 &   0 \\
        373 &   1 &   0 &   0 &   0 &   0 &   0 \\
        374 &   1 &   0 &   0 &   0 &   0 &   0 \\
        375 &   1 &   0 &   1 &   0 &   0 &   0 \\
        377 &   1 &   1 &   0 &   0 &   0 &   0 \\
        379 &   1 &   1 &   0 &   0 &   0 &   0 \\
        384 &   1 &   0 &   0 &   0 &   0 &   0 \\
        385 &   1 &   0 &   0 &   0 &   0 &   0 \\
        386 &   1 &   1 &   0 &   0 &   0 &   0 \\
        387 &   1 &   0 &   0 &   0 &   0 &   0 \\
        388 &   1 &   0 &   0 &   0 &   0 &   0 \\
        392 &   1 &   1 &   0 &   0 &   0 &   0 \\
        393 &   1 &   0 &   0 &   0 &   0 &   0 \\
        399 &   1 &   0 &   0 &   0 &   0 &   1 \\
        401 &   1 &   1 &   0 &   0 &   0 &   0 \\
        403 &   1 &   0 &   0 &   0 &   0 &   1 \\
        408 &   0 &   1 &   0 &   0 &   0 &   0 \\
        409 &   1 &   0 &   0 &   0 &   0 &   0 \\
        415 &   1 &   0 &   0 &   0 &   0 &   0 \\
        416 &   0 &   1 &   0 &   0 &   0 &   0 \\
        427 &   0 &   1 &   0 &   0 &   0 &   0 \\
        431 &   0 &   1 &   0 &   0 &   0 &   0 \\
        433 &   0 &   1 &   1 &   0 &   0 &   0 \\
        435 &   0 &   1 &   1 &   0 &   0 &   0 \\
        439 &   0 &   1 &   0 &   0 &   0 &   0 \\
        440 &   1 &   1 &   0 &   0 &   0 &   0 \\
        442 &   1 &   1 &   0 &   0 &   0 &   0 \\
        444 &   1 &   0 &   0 &   0 &   0 &   0 \\
        446 &   0 &   1 &   0 &   0 &   0 &   0 \\
        448 &   0 &   1 &   1 &   0 &   0 &   0 \\
        456 &   0 &   1 &   0 &   0 &   0 &   0 \\
        457 &   1 &   1 &   0 &   0 &   0 &   0 \\
        459 &   0 &   1 &   0 &   0 &   0 &   0 \\
        464 &   0 &   1 &   0 &   0 &   0 &   0 \\
        465 &   1 &   0 &   1 &   0 &   0 &   1 \\
        466 &   0 &   0 &   0 &   0 &   1 &   0 \\
        474 &   0 &   1 &   0 &   0 &   0 &   0 \\
        475 &   0 &   1 &   0 &   0 &   0 &   0 \\
        479 &   1 &   0 &   0 &   0 &   0 &   0 \\
        481 &   0 &   1 &   0 &   0 &   0 &   0 \\
        486 &   1 &   0 &   0 &   0 &   0 &   0 \\
        490 &   1 &   1 &   1 &   0 &   0 &   0 \\
        500 &   0 &   1 &   0 &   1 &   0 &   0 \\
        505 &   1 &   1 &   0 &   0 &   0 &   0 \\
        508 &   0 &   1 &   0 &   0 &   0 &   0 \\
        509 &   0 &   1 &   0 &   0 &   0 &   0 \\
        510 &   0 &   1 &   0 &   0 &   0 &   0 \\
        511 &   0 &   1 &   0 &   0 &   0 &   0 \\
        517 &   1 &   0 &   0 &   0 &   0 &   0 \\
        518 &   0 &   1 &   1 &   0 &   0 &   0 \\
        519 &   0 &   1 &   0 &   0 &   0 &   0 \\
        520 &   0 &   1 &   0 &   0 &   0 &   0 \\
        523 &   0 &   1 &   0 &   0 &   0 &   0 \\
        528 &   0 &   1 &   0 &   0 &   0 &   0 \\
        534 &   0 &   1 &   0 &   0 &   0 &   0 \\
        543 &   0 &   1 &   0 &   0 &   0 &   0 \\
        546 &   0 &   1 &   0 &   0 &   0 &   0 \\
        548 &   1 &   0 &   0 &   0 &   0 &   0 \\
        550 &   1 &   0 &   0 &   0 &   0 &   0 \\
        551 &   0 &   1 &   0 &   0 &   0 &   0 \\
        555 &   0 &   1 &   0 &   0 &   0 &   0 \\
        561 &   1 &   0 &   0 &   0 &   0 &   0 \\
        564 &   0 &   1 &   0 &   0 &   0 &   0 \\
        567 &   0 &   1 &   0 &   0 &   0 &   0 \\
        568 &   1 &   1 &   0 &   0 &   0 &   0 \\
        569 &   0 &   1 &   0 &   0 &   0 &   0 \\
        572 &   1 &   1 &   0 &   0 &   0 &   0 \\
        573 &   0 &   1 &   0 &   0 &   0 &   0 \\
        574 &   0 &   1 &   0 &   0 &   0 &   0 \\
        577 &   0 &   1 &   0 &   1 &   0 &   0 \\
        579 &   1 &   1 &   0 &   0 &   0 &   0 \\
        582 &   0 &   1 &   0 &   0 &   0 &   0 \\
        584 &   1 &   1 &   0 &   0 &   0 &   0 \\
        590 &   0 &   1 &   0 &   0 &   0 &   0 \\
        597 &   0 &   1 &   0 &   0 &   0 &   0 \\
        598 &   0 &   1 &   0 &   0 &   0 &   0 \\
        600 &   0 &   1 &   1 &   0 &   0 &   0 \\
        601 &   0 &   1 &   0 &   0 &   0 &   0 \\
        611 &   1 &   0 &   0 &   0 &   0 &   0 \\
        612 &   1 &   1 &   0 &   0 &   0 &   0 \\
        620 &   0 &   1 &   0 &   0 &   0 &   0 \\
        623 &   1 &   1 &   0 &   0 &   0 &   0 \\
        624 &   1 &   1 &   0 &   0 &   0 &   0 \\
        626 &   1 &   1 &   0 &   0 &   0 &   0 \\
        627 &   1 &   1 &   0 &   0 &   0 &   0 \\
        628 &   1 &   0 &   0 &   0 &   0 &   0 \\
        629 &   1 &   0 &   0 &   0 &   0 &   0 \\
        632 &   1 &   0 &   0 &   0 &   0 &   0 \\
        633 &   1 &   0 &   0 &   0 &   0 &   0 \\
        635 &   1 &   0 &   0 &   0 &   0 &   0 \\
        638 &   1 &   1 &   0 &   0 &   0 &   0 \\
        639 &   1 &   0 &   0 &   0 &   0 &   0 \\
        640 &   1 &   0 &   0 &   0 &   0 &   0 \\
        644 &   1 &   0 &   0 &   0 &   0 &   1 \\
        645 &   1 &   1 &   0 &   0 &   0 &   0 \\
        647 &   1 &   1 &   0 &   0 &   0 &   0 \\
        649 &   1 &   1 &   0 &   0 &   0 &   0 \\
        650 &   1 &   0 &   0 &   0 &   0 &   0 \\
        654 &   1 &   1 &   0 &   0 &   0 &   0 \\
        655 &   1 &   1 &   0 &   0 &   0 &   0 \\
        657 &   1 &   1 &   0 &   0 &   0 &   0 \\
        658 &   1 &   1 &   0 &   0 &   0 &   0 \\
        659 &   1 &   0 &   0 &   0 &   0 &   0 \\
        660 &   1 &   0 &   0 &   0 &   0 &   0 \\
        661 &   1 &   1 &   0 &   0 &   0 &   0 \\
        662 &   1 &   0 &   0 &   0 &   0 &   0 \\
        664 &   1 &   1 &   0 &   0 &   0 &   0 \\
        665 &   1 &   1 &   0 &   0 &   0 &   0 \\
        666 &   1 &   0 &   0 &   0 &   0 &   0 \\
        670 &   1 &   0 &   0 &   0 &   0 &   0 \\
        671 &   1 &   1 &   0 &   0 &   0 &   0 \\
        672 &   1 &   1 &   0 &   0 &   0 &   0 \\
        673 &   1 &   0 &   0 &   0 &   0 &   0 \\
        674 &   1 &   0 &   0 &   0 &   0 &   0 \\
        678 &   1 &   1 &   0 &   0 &   0 &   0 \\
        679 &   1 &   1 &   0 &   0 &   0 &   0 \\
        680 &   1 &   0 &   0 &   0 &   0 &   0 \\
        682 &   1 &   0 &   1 &   0 &   0 &   0 \\
        683 &   1 &   0 &   1 &   0 &   0 &   0 \\
        684 &   1 &   0 &   0 &   0 &   0 &   0 \\
        685 &   1 &   0 &   0 &   0 &   0 &   0 \\
        686 &   1 &   0 &   0 &   0 &   0 &   0 \\
        687 &   1 &   0 &   0 &   0 &   0 &   0 \\
        688 &   1 &   0 &   0 &   0 &   0 &   0 \\
        689 &   1 &   0 &   0 &   0 &   0 &   0 \\
        691 &   1 &   1 &   0 &   0 &   0 &   0 \\
        692 &   1 &   1 &   0 &   0 &   0 &   0 \\
        693 &   1 &   1 &   0 &   0 &   0 &   0 \\
        694 &   1 &   0 &   0 &   0 &   0 &   0 \\
        695 &   1 &   0 &   0 &   0 &   0 &   0 \\
        697 &   1 &   0 &   0 &   0 &   0 &   0 \\
        700 &   1 &   1 &   0 &   0 &   0 &   0 \\
        701 &   1 &   1 &   1 &   0 &   0 &   0 \\
        703 &   1 &   0 &   0 &   0 &   0 &   1 \\
        704 &   1 &   0 &   0 &   0 &   0 &   0 \\
        707 &   1 &   1 &   0 &   0 &   0 &   0 \\
        708 &   1 &   1 &   0 &   0 &   0 &   0 \\
        709 &   1 &   0 &   0 &   0 &   0 &   0 \\
        710 &   1 &   1 &   0 &   0 &   0 &   0 \\
        711 &   1 &   1 &   0 &   0 &   0 &   0 \\
        712 &   1 &   0 &   0 &   0 &   0 &   1 \\
        714 &   1 &   0 &   0 &   0 &   0 &   0 \\
        717 &   1 &   1 &   0 &   1 &   0 &   0 \\
        718 &   1 &   1 &   0 &   0 &   0 &   0 \\
        719 &   1 &   1 &   0 &   0 &   0 &   0 \\
        720 &   1 &   1 &   0 &   0 &   0 &   0 \\
        721 &   1 &   0 &   0 &   0 &   0 &   0 \\
        722 &   1 &   0 &   0 &   0 &   0 &   0 \\
        723 &   0 &   1 &   0 &   0 &   0 &   0 \\
        730 &   0 &   1 &   0 &   0 &   0 &   0 \\
        732 &   0 &   1 &   0 &   0 &   0 &   0 \\
        733 &   0 &   1 &   0 &   0 &   0 &   0 \\
        734 &   0 &   1 &   0 &   0 &   0 &   0 \\
        738 &   0 &   1 &   0 &   0 &   0 &   0 \\
        749 &   0 &   1 &   0 &   0 &   0 &   0 \\
        752 &   0 &   1 &   0 &   0 &   0 &   0 \\
        756 &   0 &   1 &   0 &   0 &   0 &   0 \\
        757 &   0 &   1 &   0 &   0 &   0 &   0 \\
        759 &   0 &   1 &   0 &   0 &   0 &   0 \\
        760 &   0 &   0 &   0 &   0 &   1 &   0 \\
        771 &   0 &   0 &   1 &   0 &   0 &   0 \\
        800 &   0 &   1 &   0 &   0 &   0 &   0 \\
        806 &   0 &   1 &   0 &   0 &   0 &   0 \\
        825 &   0 &   1 &   0 &   0 &   0 &   0 \\
        829 &   0 &   1 &   0 &   0 &   0 &   0 \\
        834 &   0 &   1 &   0 &   0 &   0 &   0 \\
        835 &   0 &   1 &   0 &   0 &   0 &   0 \\
        837 &   0 &   1 &   0 &   0 &   0 &   0 \\
        841 &   0 &   1 &   1 &   0 &   0 &   0 \\
        853 &   0 &   1 &   0 &   0 &   0 &   0 \\
        857 &   0 &   1 &   0 &   0 &   0 &   0 \\
        864 &   0 &   1 &   0 &   0 &   0 &   0 \\
        869 &   0 &   1 &   0 &   0 &   0 &   0 \\
        870 &   0 &   1 &   0 &   0 &   0 &   0 \\
        872 &   0 &   1 &   0 &   0 &   0 &   0 \\
        874 &   0 &   1 &   0 &   0 &   0 &   0 \\
        880 &   0 &   1 &   0 &   0 &   0 &   0 \\
        881 &   0 &   1 &   1 &   0 &   0 &   0 \\
        884 &   0 &   1 &   0 &   0 &   0 &   0 \\
        889 &   0 &   0 &   0 &   0 &   1 &   0 \\
        892 &   0 &   1 &   0 &   0 &   0 &   0 \\
        896 &   0 &   1 &   0 &   0 &   0 &   0 \\
        906 &   0 &   1 &   0 &   0 &   0 &   0 \\
        907 &   0 &   1 &   0 &   0 &   0 &   0 \\
        918 &   0 &   1 &   0 &   0 &   0 &   0 \\
        921 &   0 &   1 &   0 &   0 &   0 &   0 \\
        934 &   0 &   1 &   0 &   0 &   0 &   0 \\
        935 &   0 &   1 &   0 &   0 &   0 &   0 \\
        939 &   0 &   1 &   0 &   0 &   0 &   0 \\
        941 &   0 &   1 &   0 &   0 &   0 &   0 \\
        954 &   0 &   1 &   0 &   0 &   0 &   0 \\
        958 &   1 &   0 &   0 &   0 &   0 &   0 \\
        974 &   1 &   0 &   0 &   0 &   0 &   0 \\
        975 &   1 &   0 &   0 &   0 &   0 &   0 \\
        981 &   1 &   0 &   0 &   0 &   0 &   1 \\
        986 &   1 &   1 &   1 &   0 &   0 &   0 \\
        987 &   1 &   0 &   0 &   0 &   0 &   0 \\
        988 &   1 &   1 &   0 &   0 &   0 &   0 \\
        991 &   1 &   0 &   0 &   0 &   0 &   0 \\
        993 &   0 &   1 &   0 &   0 &   0 &   0 \\
        999 &   0 &   1 &   0 &   0 &   0 &   0 \\
       1001 &   1 &   1 &   0 &   0 &   0 &   0 \\
       1002 &   1 &   0 &   0 &   0 &   0 &   0 \\
       1010 &   1 &   0 &   0 &   0 &   0 &   1 \\
       1015 &   0 &   1 &   0 &   0 &   0 &   0 \\
       1019 &   1 &   0 &   0 &   0 &   0 &   1 \\
       1032 &   1 &   0 &   1 &   0 &   0 &   0 \\
       1050 &   1 &   1 &   0 &   0 &   0 &   0 \\
       1052 &   0 &   1 &   0 &   0 &   0 &   0 \\
       1054 &   1 &   0 &   0 &   0 &   0 &   1 \\
       1060 &   0 &   1 &   0 &   0 &   0 &   0 \\
       1069 &   0 &   1 &   0 &   0 &   0 &   0 \\
       1089 &   0 &   1 &   0 &   0 &   0 &   0 \\
       1102 &   0 &   1 &   0 &   0 &   0 &   0 \\
       1113 &   1 &   1 &   0 &   0 &   0 &   0 \\
       1115 &   1 &   0 &   0 &   0 &   0 &   0 \\
       1116 &   1 &   0 &   0 &   0 &   0 &   0 \\
       1117 &   1 &   0 &   0 &   0 &   0 &   0 \\
       1118 &   1 &   0 &   0 &   0 &   0 &   0 \\
       1120 &   1 &   0 &   0 &   0 &   0 &   1 \\
       1126 &   0 &   1 &   0 &   0 &   0 &   0 \\
       1127 &   0 &   1 &   0 &   0 &   0 &   0 \\
       1128 &   1 &   0 &   0 &   1 &   0 &   0 \\
       1145 &   1 &   0 &   0 &   0 &   0 &   0 \\
       1148 &   1 &   1 &   0 &   0 &   0 &   0 \\
       1150 &   1 &   0 &   0 &   1 &   0 &   0 \\
       1151 &   1 &   1 &   0 &   0 &   0 &   0 \\
       1161 &   0 &   1 &   0 &   0 &   0 &   0 \\
       1162 &   1 &   0 &   0 &   0 &   0 &   0 \\
       1163 &   0 &   1 &   0 &   0 &   0 &   0 \\
       1165 &   1 &   1 &   0 &   0 &   0 &   0 \\
       1168 &   1 &   0 &   1 &   0 &   0 &   0 \\
       1169 &   1 &   0 &   0 &   1 &   0 &   0 \\
       1175 &   1 &   1 &   0 &   0 &   0 &   0 \\
       1196 &   0 &   1 &   0 &   0 &   0 &   0 \\
       1198 &   0 &   1 &   0 &   0 &   0 &   0 \\
       1199 &   0 &   0 &   0 &   0 &   1 &   0 \\
       1203 &   0 &   1 &   0 &   0 &   0 &   0 \\
       1206 &   1 &   0 &   1 &   0 &   0 &   0 \\
       1208 &   1 &   0 &   1 &   0 &   0 &   0 \\
       1209 &   0 &   0 &   1 &   0 &   0 &   0 \\
       1215 &   1 &   1 &   0 &   0 &   0 &   0 \\
       1216 &   1 &   0 &   0 &   0 &   0 &   0 \\
       1218 &   1 &   0 &   0 &   0 &   0 &   0 \\
       1220 &   1 &   0 &   0 &   0 &   0 &   0 \\
       1221 &   1 &   1 &   0 &   0 &   0 &   0 \\
       1222 &   1 &   0 &   0 &   0 &   0 &   1 \\
       1230 &   1 &   0 &   0 &   0 &   0 &   0 \\
       1239 &   0 &   1 &   0 &   1 &   0 &   0 \\
       1240 &   0 &   1 &   0 &   0 &   0 &   0 \\
       1241 &   1 &   1 &   0 &   0 &   0 &   0 \\
       1242 &   1 &   0 &   0 &   0 &   0 &   0 \\
       1257 &   0 &   0 &   0 &   0 &   1 &   0 \\
       1270 &   0 &   1 &   0 &   0 &   0 &   0 \\
       1271 &   1 &   0 &   0 &   0 &   0 &   0 \\
       1274 &   1 &   0 &   1 &   0 &   0 &   0 \\
       1275 &   1 &   0 &   0 &   0 &   0 &   0 \\
       1276 &   0 &   1 &   0 &   0 &   0 &   0 \\
       1278 &   0 &   1 &   0 &   0 &   0 &   0 \\
       1279 &   1 &   1 &   0 &   0 &   0 &   0 \\
       1282 &   1 &   0 &   0 &   0 &   0 &   0 \\
       1283 &   1 &   0 &   0 &   0 &   0 &   0 \\
       1288 &   0 &   0 &   0 &   0 &   1 &   0 \\
       1299 &   1 &   0 &   0 &   0 &   0 &   0 \\
       1300 &   0 &   0 &   0 &   1 &   0 &   0 \\
       1301 &   0 &   1 &   0 &   0 &   0 &   0 \\
       1305 &   0 &   1 &   0 &   0 &   0 &   0 \\
       1306 &   0 &   1 &   0 &   0 &   0 &   0 \\
       1307 &   0 &   1 &   0 &   0 &   0 &   0 \\
       1308 &   1 &   0 &   0 &   0 &   0 &   0 \\
       1311 &   1 &   0 &   0 &   0 &   0 &   0 \\
       1314 &   1 &   0 &   0 &   0 &   0 &   0 \\
       1315 &   1 &   0 &   0 &   0 &   0 &   0 \\
       1316 &   1 &   1 &   0 &   0 &   0 &   0 \\
       1332 &   0 &   1 &   0 &   0 &   0 &   0 \\
       1335 &   1 &   0 &   0 &   0 &   0 &   0 \\
       1336 &   0 &   1 &   0 &   0 &   0 &   0 \\
       1338 &   0 &   1 &   0 &   0 &   0 &   0 \\
       1344 &   1 &   0 &   0 &   0 &   0 &   0 \\
       1353 &   1 &   1 &   0 &   0 &   0 &   0 \\
       1356 &   0 &   0 &   1 &   0 &   0 &   0 \\
       1359 &   0 &   1 &   0 &   0 &   0 &   0 \\
       1360 &   0 &   1 &   0 &   1 &   0 &   0 \\
       1363 &   0 &   1 &   0 &   0 &   0 &   0 \\
       1364 &   0 &   1 &   0 &   0 &   0 &   0 \\
       1366 &   0 &   1 &   0 &   0 &   0 &   0 \\
       1367 &   0 &   0 &   0 &   1 &   0 &   0 \\
       1375 &   1 &   0 &   1 &   0 &   0 &   0 \\
       1378 &   1 &   1 &   0 &   0 &   0 &   0 \\
       1379 &   1 &   0 &   0 &   0 &   0 &   0 \\
       1396 &   0 &   1 &   0 &   0 &   0 &   0 \\
       1411 &   1 &   0 &   1 &   0 &   0 &   0 \\
       1412 &   1 &   0 &   0 &   0 &   0 &   0 \\
       1413 &   0 &   1 &   0 &   0 &   0 &   0 \\
       1421 &   0 &   0 &   1 &   0 &   0 &   0 \\
       1426 &   0 &   1 &   0 &   0 &   0 &   0 \\
       1428 &   0 &   0 &   0 &   1 &   0 &   0 \\
       1431 &   1 &   0 &   1 &   0 &   0 &   0 \\
       1432 &   0 &   1 &   0 &   0 &   0 &   0 \\
       1436 &   0 &   1 &   0 &   0 &   0 &   0 \\
       1438 &   1 &   0 &   0 &   0 &   0 &   0 \\
       1439 &   1 &   0 &   0 &   0 &   0 &   0 \\
       1442 &   1 &   0 &   0 &   1 &   0 &   0 \\
       1444 &   1 &   0 &   0 &   0 &   0 &   0 \\
       1445 &   1 &   1 &   0 &   0 &   0 &   0 \\
       1463 &   1 &   0 &   1 &   0 &   0 &   0 \\
       1466 &   0 &   0 &   1 &   0 &   0 &   0 \\
       1474 &   1 &   0 &   0 &   0 &   0 &   0 \\
       1477 &   0 &   0 &   1 &   0 &   0 &   0 \\
       1478 &   1 &   0 &   1 &   0 &   0 &   0 \\
       1480 &   0 &   1 &   0 &   0 &   0 &   0 \\
       1483 &   0 &   0 &   0 &   0 &   1 &   0 \\
       1486 &   0 &   1 &   1 &   0 &   0 &   0 \\
       1528 &   1 &   0 &   0 &   0 &   0 &   0 \\
       1529 &   0 &   1 &   0 &   0 &   0 &   0 \\
       1530 &   1 &   0 &   0 &   0 &   0 &   0 \\
       1531 &   1 &   0 &   0 &   0 &   0 &   0 \\
       1532 &   1 &   0 &   0 &   0 &   0 &   0 \\
       1533 &   1 &   0 &   0 &   0 &   0 &   0 \\
       1534 &   1 &   1 &   0 &   0 &   0 &   0 \\
       1535 &   1 &   0 &   0 &   0 &   0 &   0 \\
       1536 &   1 &   0 &   0 &   0 &   0 &   0 \\
       1537 &   1 &   0 &   0 &   0 &   0 &   0 \\
       1546 &   0 &   0 &   0 &   0 &   1 &   0 \\
       1557 &   0 &   1 &   0 &   0 &   0 &   0 \\
       1563 &   0 &   1 &   0 &   0 &   0 &   0 \\
       1567 &   0 &   1 &   0 &   0 &   0 &   0 \\
       1576 &   1 &   1 &   0 &   0 &   0 &   0 \\
       1581 &   0 &   1 &   0 &   0 &   0 &   0 \\
       1589 &   0 &   1 &   0 &   0 &   0 &   0 \\
       1590 &   0 &   1 &   0 &   0 &   0 &   0 \\
       1596 &   0 &   1 &   1 &   0 &   0 &   0 \\
       1598 &   0 &   1 &   0 &   0 &   0 &   0 \\
       1601 &   0 &   1 &   0 &   0 &   0 &   0 \\
       1606 &   1 &   0 &   0 &   0 &   0 &   0 \\
       1608 &   1 &   1 &   0 &   0 &   0 &   0 \\
       1609 &   1 &   0 &   0 &   0 &   0 &   0 \\
       1612 &   1 &   0 &   0 &   0 &   0 &   0 \\
       1615 &   1 &   0 &   0 &   0 &   0 &   0 \\
       1616 &   1 &   1 &   0 &   0 &   0 &   0 \\
       1618 &   1 &   0 &   0 &   0 &   0 &   0 \\
       1619 &   1 &   0 &   0 &   0 &   0 &   0 \\
       1621 &   1 &   0 &   0 &   0 &   0 &   0 \\
       1623 &   1 &   0 &   0 &   0 &   0 &   1 \\
       1628 &   1 &   1 &   0 &   0 &   0 &   0 \\
       1629 &   1 &   0 &   0 &   0 &   0 &   0 \\
       1632 &   1 &   0 &   0 &   0 &   0 &   0 \\
       1639 &   1 &   1 &   0 &   0 &   0 &   0 \\
       1647 &   1 &   1 &   0 &   0 &   0 &   0 \\
       1655 &   1 &   0 &   0 &   1 &   0 &   0 \\
       1665 &   1 &   1 &   0 &   0 &   0 &   0 \\
       1666 &   0 &   0 &   0 &   1 &   0 &   1 \\
       1669 &   1 &   0 &   0 &   0 &   0 &   0 \\
       1688 &   0 &   0 &   0 &   1 &   0 &   0 \\
       1692 &   1 &   1 &   0 &   0 &   0 &   0 \\
       1695 &   1 &   0 &   0 &   0 &   0 &   0 \\
       1706 &   1 &   0 &   0 &   0 &   0 &   0 \\
       1707 &   0 &   1 &   1 &   0 &   0 &   0 \\
       1715 &   1 &   0 &   0 &   0 &   0 &   0 \\
       1726 &   1 &   0 &   0 &   0 &   0 &   0 \\
       1738 &   1 &   0 &   0 &   0 &   0 &   0 \\
       1739 &   0 &   0 &   1 &   0 &   0 &   0 \\
       1751 &   0 &   1 &   0 &   0 &   0 &   0 \\
       1754 &   1 &   0 &   0 &   0 &   0 &   0 \\
       1779 &   1 &   1 &   0 &   0 &   0 &   0 \\
       1781 &   1 &   1 &   0 &   0 &   0 &   0 \\
       1783 &   1 &   1 &   1 &   0 &   0 &   0 \\
       1792 &   1 &   1 &   0 &   0 &   0 &   0 \\
       1796 &   1 &   0 &   0 &   0 &   0 &   0 \\
       1797 &   1 &   0 &   0 &   0 &   0 &   0 \\
       1800 &   1 &   0 &   0 &   0 &   0 &   0 \\
       1802 &   1 &   0 &   0 &   0 &   0 &   0 \\
       1803 &   1 &   1 &   0 &   0 &   0 &   0 \\
       1805 &   1 &   1 &   0 &   0 &   0 &   0 \\
       1806 &   1 &   1 &   0 &   0 &   0 &   0 \\
       1808 &   1 &   0 &   0 &   0 &   0 &   0 \\
       1809 &   1 &   1 &   0 &   0 &   0 &   0 \\
       1812 &   1 &   0 &   0 &   0 &   0 &   0 \\
       1813 &   1 &   0 &   0 &   0 &   0 &   0 \\
       1815 &   1 &   0 &   0 &   0 &   0 &   0 \\
       1818 &   1 &   0 &   0 &   0 &   0 &   0 \\
       1819 &   1 &   0 &   0 &   0 &   0 &   0 \\
       1820 &   1 &   1 &   0 &   0 &   0 &   0 \\
       1822 &   1 &   0 &   0 &   0 &   0 &   0 \\
       1824 &   1 &   1 &   0 &   0 &   0 &   0 \\
       1825 &   1 &   0 &   0 &   0 &   0 &   0 \\
       1826 &   1 &   0 &   0 &   0 &   0 &   0 \\
       1831 &   1 &   1 &   0 &   0 &   0 &   0 \\
       1832 &   0 &   1 &   0 &   0 &   0 &   0 \\
       1835 &   1 &   1 &   0 &   0 &   0 &   0 \\
       1837 &   1 &   1 &   0 &   0 &   0 &   0 \\
       1839 &   1 &   1 &   0 &   0 &   0 &   0 \\
       1841 &   1 &   0 &   0 &   0 &   0 &   0 \\
       1845 &   0 &   1 &   0 &   0 &   0 &   0 \\
       1848 &   1 &   0 &   0 &   0 &   0 &   0 \\
       1850 &   1 &   0 &   0 &   0 &   0 &   0 \\
       1852 &   1 &   0 &   0 &   0 &   0 &   0 \\
       1854 &   1 &   0 &   0 &   0 &   0 &   0 \\
       1856 &   1 &   0 &   0 &   0 &   0 &   0 \\
       1857 &   1 &   0 &   0 &   0 &   0 &   0 \\
       1858 &   0 &   1 &   0 &   0 &   0 &   0 \\
       1860 &   1 &   1 &   0 &   0 &   0 &   0 \\
       1861 &   1 &   0 &   0 &   0 &   0 &   0 \\
       1862 &   1 &   0 &   0 &   0 &   0 &   0 \\
       1863 &   1 &   0 &   0 &   0 &   0 &   0 \\
       1864 &   1 &   0 &   0 &   0 &   0 &   0 \\
       1871 &   0 &   1 &   1 &   0 &   0 &   0 \\
       1875 &   0 &   1 &   0 &   1 &   0 &   0 \\
       1877 &   1 &   0 &   0 &   0 &   0 &   0 \\
       1878 &   1 &   0 &   0 &   0 &   0 &   0 \\
       1883 &   1 &   0 &   0 &   0 &   0 &   0 \\
       1886 &   1 &   0 &   0 &   0 &   0 &   0 \\
       1888 &   1 &   0 &   0 &   0 &   0 &   0 \\
       1889 &   0 &   1 &   0 &   0 &   0 &   0 \\
       1890 &   1 &   0 &   0 &   0 &   0 &   0 \\
       1891 &   0 &   1 &   0 &   0 &   0 &   0 \\
       1893 &   1 &   0 &   0 &   0 &   0 &   0 \\
       1894 &   1 &   0 &   0 &   0 &   0 &   0 \\
       1897 &   1 &   0 &   0 &   0 &   0 &   0 \\
       1898 &   1 &   0 &   0 &   0 &   0 &   0 \\
       1901 &   1 &   0 &   0 &   0 &   0 &   0 \\
       1904 &   1 &   0 &   0 &   0 &   0 &   0 \\
       1905 &   1 &   1 &   0 &   0 &   0 &   0 \\
       1909 &   1 &   1 &   0 &   0 &   0 &   0 \\
       1913 &   1 &   0 &   0 &   0 &   0 &   0 \\
       1915 &   1 &   1 &   0 &   0 &   0 &   0 \\
       1916 &   1 &   1 &   0 &   0 &   0 &   0 \\
       1917 &   1 &   0 &   0 &   0 &   0 &   0 \\
       1921 &   1 &   0 &   0 &   0 &   0 &   0 \\
       1922 &   0 &   1 &   0 &   0 &   0 &   0 \\
       1923 &   1 &   0 &   0 &   0 &   0 &   0 \\
       1924 &   1 &   0 &   0 &   0 &   0 &   1 \\
       1925 &   1 &   0 &   0 &   0 &   0 &   0 \\
       1928 &   1 &   0 &   0 &   0 &   0 &   0 \\
       1929 &   1 &   1 &   0 &   0 &   0 &   0 \\
       1930 &   1 &   1 &   0 &   0 &   0 &   0 \\
       1931 &   0 &   1 &   0 &   0 &   0 &   0 \\
       1938 &   1 &   0 &   1 &   0 &   0 &   0 \\
       1944 &   1 &   1 &   0 &   0 &   0 &   0 \\
       1945 &   0 &   1 &   0 &   0 &   0 &   0 \\
       1947 &   1 &   0 &   0 &   0 &   0 &   0 \\
       1951 &   1 &   0 &   0 &   0 &   0 &   0 \\
       1952 &   0 &   1 &   0 &   0 &   0 &   0 \\
       1955 &   1 &   1 &   0 &   0 &   0 &   0 \\
       1958 &   0 &   0 &   0 &   0 &   1 &   0 \\
       1960 &   1 &   1 &   0 &   0 &   0 &   0 \\
       1961 &   1 &   1 &   0 &   0 &   0 &   0 \\
       1962 &   1 &   0 &   0 &   0 &   0 &   0 \\
       1963 &   1 &   0 &   0 &   0 &   0 &   0 \\
       1964 &   1 &   0 &   0 &   0 &   0 &   0 \\
       1970 &   0 &   1 &   0 &   0 &   0 &   0 \\
       1978 &   0 &   1 &   0 &   0 &   0 &   0 \\
       1979 &   1 &   0 &   0 &   0 &   0 &   0 \\
       1980 &   1 &   0 &   0 &   0 &   0 &   0 \\
       1984 &   1 &   0 &   0 &   0 &   0 &   0 \\
       1985 &   1 &   0 &   0 &   0 &   0 &   0 \\
       1988 &   1 &   0 &   0 &   0 &   0 &   0 \\
       1989 &   1 &   0 &   0 &   0 &   0 &   0 \\
       1992 &   0 &   1 &   0 &   0 &   0 &   0 \\
       2001 &   1 &   0 &   0 &   0 &   0 &   0 \\
       2002 &   1 &   0 &   0 &   0 &   0 &   0 \\
       2004 &   1 &   1 &   0 &   0 &   0 &   0 \\
       2007 &   1 &   1 &   0 &   0 &   0 &   0 \\
       2009 &   1 &   0 &   0 &   0 &   0 &   0 \\
       2010 &   1 &   0 &   0 &   0 &   0 &   0 \\
       2011 &   1 &   1 &   0 &   0 &   0 &   0 \\
       2012 &   0 &   1 &   0 &   0 &   0 &   0 \\
       2016 &   1 &   0 &   0 &   0 &   0 &   0 \\
       2017 &   1 &   0 &   0 &   0 &   0 &   0 \\
       2022 &   0 &   1 &   0 &   0 &   0 &   0 \\
       2026 &   1 &   0 &   0 &   0 &   0 &   0 \\
       2029 &   1 &   1 &   0 &   0 &   0 &   0 \\
       2033 &   1 &   0 &   0 &   0 &   0 &   0 \\
       2035 &   1 &   0 &   0 &   0 &   0 &   0 \\
       2037 &   0 &   1 &   0 &   0 &   0 &   0 \\
       2038 &   0 &   1 &   0 &   0 &   0 &   0 \\
       2039 &   0 &   1 &   0 &   1 &   0 &   0 \\
       2040 &   1 &   0 &   0 &   0 &   0 &   0 \\
       2043 &   1 &   0 &   0 &   0 &   0 &   0 \\
       2044 &   0 &   0 &   0 &   0 &   1 &   0 \\
       2046 &   1 &   0 &   0 &   0 &   0 &   0 \\
       2047 &   1 &   0 &   0 &   0 &   0 &   0 \\
       2048 &   0 &   1 &   0 &   0 &   0 &   0 \\
       2049 &   1 &   0 &   0 &   0 &   0 &   0 \\
       2051 &   0 &   1 &   0 &   0 &   0 &   0 \\
       2053 &   1 &   1 &   0 &   0 &   0 &   0 \\
       2071 &   1 &   0 &   0 &   0 &   0 &   0 \\
       2072 &   1 &   0 &   0 &   0 &   0 &   0 \\
       2073 &   0 &   1 &   0 &   0 &   0 &   0 \\
       2076 &   0 &   1 &   0 &   0 &   0 &   0 \\
       2079 &   1 &   0 &   0 &   1 &   0 &   0 \\
       2081 &   1 &   1 &   0 &   0 &   0 &   0 \\
       2082 &   1 &   0 &   0 &   0 &   0 &   0 \\
       2083 &   1 &   0 &   0 &   0 &   0 &   0 \\
       2086 &   1 &   1 &   0 &   0 &   0 &   0 \\
       2087 &   1 &   0 &   0 &   0 &   0 &   0 \\
       2092 &   0 &   1 &   0 &   0 &   0 &   0 \\
       2093 &   0 &   1 &   0 &   1 &   0 &   0 \\
       2094 &   0 &   1 &   1 &   0 &   0 &   0 \\
       2098 &   1 &   1 &   0 &   0 &   0 &   0 \\
       2105 &   1 &   0 &   0 &   0 &   0 &   0 \\
       2109 &   1 &   0 &   0 &   0 &   0 &   0 \\
       2110 &   1 &   0 &   0 &   0 &   0 &   0 \\
       2111 &   0 &   1 &   0 &   0 &   0 &   0 \\
       2115 &   0 &   0 &   0 &   0 &   1 &   0 \\
       2119 &   1 &   0 &   0 &   1 &   0 &   0 \\
       2120 &   1 &   0 &   0 &   0 &   0 &   0 \\
       2135 &   1 &   1 &   0 &   0 &   0 &   0 \\
       2137 &   1 &   0 &   0 &   0 &   0 &   0 \\
       2143 &   1 &   0 &   0 &   0 &   0 &   0 \\
       2147 &   0 &   1 &   0 &   0 &   0 &   0 \\
       2148 &   1 &   1 &   0 &   0 &   0 &   0 \\
       2149 &   1 &   0 &   0 &   0 &   0 &   0 \\
       2153 &   1 &   1 &   0 &   0 &   0 &   0 \\
       2158 &   1 &   1 &   0 &   0 &   0 &   0 \\
       2159 &   1 &   1 &   0 &   0 &   0 &   0 \\
       2162 &   1 &   1 &   0 &   0 &   0 &   0 \\
       2167 &   0 &   1 &   0 &   0 &   0 &   0 \\
       2168 &   0 &   1 &   0 &   0 &   0 &   0 \\
       2169 &   1 &   1 &   0 &   0 &   0 &   0 \\
       2173 &   1 &   1 &   0 &   0 &   0 &   0 \\
       2175 &   1 &   1 &   0 &   0 &   0 &   0 \\
       2183 &   0 &   1 &   0 &   0 &   0 &   0 \\
       2188 &   0 &   1 &   0 &   0 &   0 &   0 \\
       2194 &   1 &   1 &   1 &   0 &   0 &   0 \\
       2195 &   0 &   1 &   0 &   0 &   0 &   0 \\
       2201 &   1 &   0 &   0 &   0 &   0 &   0 \\
       2202 &   1 &   0 &   0 &   1 &   0 &   0 \\
       2208 &   1 &   0 &   0 &   0 &   0 &   0 \\
       2218 &   0 &   1 &   0 &   0 &   0 &   0 \\
       2219 &   1 &   0 &   0 &   0 &   0 &   0 \\
       2220 &   0 &   1 &   0 &   0 &   0 &   0 \\
       2228 &   1 &   0 &   0 &   0 &   0 &   1 \\
       2236 &   0 &   1 &   0 &   0 &   0 &   0 \\
       2246 &   1 &   0 &   0 &   0 &   0 &   0 \\
       2248 &   0 &   1 &   0 &   1 &   0 &   0 \\
       2250 &   0 &   1 &   0 &   1 &   0 &   0 \\
       2252 &   1 &   0 &   0 &   0 &   0 &   0 \\
       2260 &   1 &   0 &   0 &   0 &   0 &   0 \\
       2261 &   1 &   1 &   0 &   0 &   0 &   0 \\
       2273 &   1 &   0 &   0 &   0 &   0 &   0 \\
       2278 &   1 &   1 &   0 &   0 &   0 &   0 \\
       2279 &   1 &   1 &   0 &   0 &   0 &   0 \\
       2281 &   1 &   1 &   0 &   1 &   0 &   0 \\
       2287 &   1 &   1 &   0 &   0 &   0 &   0 \\
       2289 &   1 &   1 &   0 &   0 &   0 &   0 \\
       2290 &   0 &   0 &   1 &   0 &   0 &   0 \\
       2295 &   1 &   0 &   0 &   0 &   0 &   0 \\
       2300 &   1 &   0 &   0 &   0 &   0 &   0 \\
       2312 &   1 &   0 &   0 &   0 &   0 &   0 \\
       2319 &   1 &   0 &   0 &   0 &   0 &   0 \\
       2331 &   1 &   0 &   0 &   0 &   0 &   0 \\
       2332 &   1 &   0 &   0 &   0 &   0 &   0 \\
       2333 &   1 &   1 &   0 &   0 &   0 &   0 \\
       2335 &   1 &   0 &   0 &   0 &   0 &   0 \\
       2339 &   0 &   1 &   0 &   0 &   0 &   0 \\
       2342 &   1 &   0 &   0 &   0 &   0 &   0 \\
       2352 &   1 &   1 &   0 &   0 &   0 &   0 \\
       2357 &   0 &   1 &   0 &   0 &   0 &   0 \\
       2358 &   1 &   0 &   0 &   0 &   0 &   0 \\
       2365 &   1 &   1 &   0 &   0 &   0 &   0 \\
       2366 &   1 &   0 &   0 &   0 &   0 &   0 \\
       2367 &   1 &   0 &   0 &   0 &   0 &   0 \\
       2369 &   0 &   1 &   0 &   0 &   0 &   0 \\
       2370 &   1 &   0 &   0 &   0 &   0 &   0 \\
       2372 &   1 &   0 &   0 &   0 &   0 &   0 \\
       2374 &   0 &   1 &   0 &   0 &   0 &   0 \\
       2389 &   1 &   0 &   0 &   0 &   0 &   0 \\
       2390 &   1 &   0 &   0 &   0 &   0 &   0 \\
       2393 &   0 &   1 &   0 &   1 &   0 &   0 \\
       2396 &   0 &   0 &   0 &   1 &   0 &   1 \\
       2398 &   1 &   0 &   0 &   0 &   0 &   0 \\
       2399 &   1 &   0 &   0 &   0 &   0 &   0 \\
       2403 &   1 &   0 &   0 &   0 &   0 &   0 \\
       2407 &   1 &   0 &   0 &   0 &   0 &   0 \\
       2408 &   1 &   0 &   0 &   0 &   0 &   0 \\
       2409 &   0 &   0 &   0 &   1 &   0 &   0 \\
       2410 &   0 &   1 &   0 &   0 &   0 &   0 \\
       2414 &   1 &   1 &   0 &   0 &   0 &   0 \\
       2422 &   0 &   1 &   0 &   0 &   0 &   0 \\
       2426 &   1 &   0 &   0 &   0 &   0 &   0 \\
       2433 &   0 &   1 &   0 &   0 &   0 &   0 \\
       2440 &   1 &   0 &   0 &   0 &   0 &   0 \\
       2442 &   0 &   1 &   0 &   0 &   0 &   0 \\
       2443 &   1 &   1 &   0 &   0 &   0 &   0 \\
       2462 &   1 &   0 &   0 &   0 &   0 &   0 \\
       2463 &   1 &   0 &   0 &   0 &   0 &   0 \\
       2469 &   0 &   0 &   1 &   0 &   0 &   0 \\
       2470 &   1 &   0 &   0 &   0 &   0 &   1 \\
       2473 &   0 &   1 &   0 &   0 &   0 &   0 \\
       2474 &   1 &   0 &   1 &   0 &   0 &   0 \\
       2479 &   1 &   0 &   0 &   0 &   0 &   0 \\
       2481 &   1 &   0 &   0 &   0 &   0 &   0 \\
       2484 &   1 &   0 &   0 &   0 &   0 &   0 \\
       2486 &   1 &   0 &   0 &   0 &   0 &   0 \\
       2488 &   1 &   0 &   0 &   0 &   0 &   0 \\
       2492 &   1 &   0 &   0 &   1 &   0 &   0 \\
       2498 &   1 &   1 &   0 &   0 &   0 &   0 \\
       2503 &   1 &   0 &   0 &   0 &   0 &   0 \\
       2516 &   1 &   0 &   0 &   0 &   0 &   0 \\
       2517 &   0 &   0 &   0 &   1 &   0 &   0 \\
       2521 &   0 &   1 &   0 &   0 &   0 &   0 \\
       2522 &   1 &   0 &   0 &   0 &   0 &   0 \\
       2529 &   0 &   1 &   1 &   0 &   0 &   0 \\
       2530 &   1 &   0 &   0 &   0 &   0 &   0 \\
       2533 &   1 &   1 &   0 &   0 &   0 &   0 \\
       2534 &   1 &   1 &   0 &   0 &   0 &   0 \\
       2538 &   1 &   0 &   0 &   0 &   0 &   0 \\
       2541 &   1 &   1 &   0 &   0 &   0 &   0 \\
       2545 &   1 &   0 &   0 &   0 &   0 &   0 \\
       2547 &   1 &   0 &   0 &   0 &   0 &   0 \\
       2555 &   1 &   0 &   0 &   0 &   0 &   0 \\
       2556 &   1 &   0 &   0 &   0 &   0 &   0 \\
       2559 &   1 &   0 &   0 &   0 &   0 &   0 \\
       2561 &   1 &   0 &   0 &   0 &   0 &   0 \\
       2563 &   1 &   1 &   0 &   0 &   0 &   0 \\
       2564 &   1 &   1 &   0 &   0 &   0 &   0 \\
       2571 &   0 &   0 &   0 &   1 &   0 &   0 \\
       2581 &   1 &   0 &   0 &   0 &   0 &   0 \\
       2582 &   1 &   0 &   0 &   0 &   0 &   0 \\
       2583 &   1 &   0 &   0 &   0 &   0 &   0 \\
       2585 &   1 &   1 &   0 &   0 &   0 &   0 \\
       2590 &   1 &   1 &   0 &   0 &   0 &   0 \\
       2593 &   1 &   0 &   0 &   0 &   0 &   0 \\
       2595 &   1 &   1 &   0 &   0 &   0 &   0 \\
       2597 &   0 &   1 &   0 &   0 &   0 &   0 \\
       2603 &   1 &   0 &   0 &   0 &   0 &   0 \\
       2607 &   0 &   0 &   0 &   1 &   0 &   0 \\
       2608 &   1 &   0 &   0 &   0 &   0 &   0 \\
       2612 &   1 &   1 &   0 &   0 &   0 &   0 \\
       2623 &   1 &   1 &   0 &   0 &   0 &   0 \\
       2631 &   1 &   1 &   0 &   0 &   0 &   0 \\
       2632 &   1 &   0 &   0 &   0 &   0 &   0 \\
       2635 &   1 &   0 &   0 &   0 &   0 &   0 \\
       2636 &   1 &   1 &   0 &   0 &   0 &   0 \\
       2639 &   0 &   1 &   0 &   0 &   0 &   0 \\
       2640 &   1 &   0 &   0 &   0 &   0 &   0 \\
       2641 &   1 &   0 &   0 &   0 &   0 &   0 \\
       2657 &   1 &   0 &   0 &   0 &   0 &   0 \\
       2659 &   1 &   0 &   0 &   0 &   0 &   0 \\
       2668 &   1 &   0 &   0 &   1 &   0 &   0 \\
       2672 &   1 &   1 &   0 &   0 &   0 &   0 \\
       2674 &   1 &   1 &   0 &   0 &   0 &   0 \\
       2675 &   1 &   1 &   0 &   0 &   0 &   0 \\
       2676 &   1 &   0 &   0 &   0 &   0 &   1 \\
       2677 &   1 &   0 &   0 &   0 &   0 &   0 \\
       2678 &   1 &   0 &   0 &   0 &   0 &   0 \\
       2681 &   0 &   1 &   1 &   0 &   0 &   0 \\
       2686 &   1 &   0 &   1 &   0 &   0 &   0 \\
       2687 &   1 &   1 &   0 &   0 &   0 &   0 \\
       2690 &   1 &   0 &   0 &   0 &   0 &   1 \\
       2694 &   0 &   1 &   0 &   1 &   0 &   0 \\
       2698 &   1 &   0 &   0 &   0 &   0 &   0 \\
       2706 &   1 &   0 &   0 &   0 &   0 &   0 \\
       2707 &   0 &   1 &   0 &   0 &   0 &   0 \\
       2711 &   1 &   1 &   0 &   0 &   0 &   0 \\
       2712 &   1 &   0 &   0 &   0 &   0 &   0 \\
       2714 &   1 &   1 &   0 &   0 &   0 &   0 \\
       2717 &   1 &   0 &   0 &   1 &   0 &   0 \\
       2720 &   1 &   0 &   0 &   0 &   0 &   0 \\
       2722 &   1 &   1 &   0 &   0 &   0 &   0 \\
       2729 &   1 &   0 &   0 &   0 &   0 &   0 \\
       2730 &   1 &   0 &   0 &   0 &   0 &   0 \\
       2732 &   1 &   1 &   0 &   0 &   0 &   0 \\
       2733 &   1 &   0 &   0 &   0 &   0 &   0 \\
       2737 &   1 &   0 &   0 &   0 &   0 &   1 \\
       2740 &   1 &   0 &   0 &   0 &   0 &   1 \\
       2741 &   1 &   0 &   0 &   0 &   0 &   1 \\
       2743 &   1 &   0 &   0 &   0 &   0 &   0 \\
       2748 &   1 &   1 &   0 &   0 &   0 &   0 \\
       2749 &   1 &   0 &   0 &   0 &   0 &   1 \\
       2750 &   0 &   0 &   1 &   0 &   0 &   0 \\
       2752 &   1 &   0 &   0 &   0 &   0 &   1 \\
       2753 &   1 &   0 &   0 &   1 &   0 &   0 \\
       2754 &   1 &   0 &   0 &   0 &   0 &   0 \\
       2755 &   1 &   0 &   0 &   0 &   0 &   0 \\
       2756 &   0 &   1 &   0 &   1 &   0 &   0 \\
       2758 &   1 &   0 &   0 &   0 &   0 &   0 \\
       2762 &   0 &   0 &   1 &   0 &   0 &   0 \\
       2763 &   0 &   0 &   0 &   1 &   0 &   1 \\
       2765 &   1 &   0 &   0 &   0 &   0 &   1 \\
       2768 &   0 &   1 &   0 &   0 &   0 &   0 \\
       2769 &   1 &   0 &   0 &   0 &   0 &   1 \\
       2771 &   1 &   0 &   0 &   0 &   0 &   1 \\
       2781 &   1 &   0 &   0 &   0 &   0 &   1 \\
       2785 &   1 &   0 &   0 &   0 &   0 &   0 \\
       2786 &   1 &   0 &   0 &   0 &   0 &   0 \\
       2790 &   1 &   0 &   0 &   0 &   0 &   0 \\
       2792 &   1 &   0 &   0 &   0 &   0 &   0 \\
       2796 &   0 &   0 &   0 &   1 &   0 &   1 \\
       2801 &   1 &   0 &   0 &   0 &   0 &   0 \\
       2803 &   1 &   0 &   0 &   0 &   0 &   0 \\
       2805 &   1 &   0 &   0 &   0 &   0 &   0 \\
       2807 &   1 &   0 &   0 &   0 &   0 &   0 \\
       2815 &   1 &   0 &   0 &   0 &   0 &   0 \\
       2828 &   0 &   1 &   1 &   0 &   0 &   0 \\
       2829 &   1 &   0 &   0 &   0 &   0 &   0 \\
       2831 &   1 &   0 &   0 &   0 &   0 &   1 \\
       2832 &   1 &   0 &   0 &   0 &   0 &   0 \\
       2833 &   1 &   0 &   0 &   0 &   0 &   0 \\
       2838 &   1 &   1 &   0 &   0 &   0 &   0 \\
       2840 &   1 &   1 &   0 &   0 &   0 &   0 \\
       2841 &   0 &   0 &   1 &   0 &   0 &   0 \\
       2848 &   1 &   0 &   0 &   0 &   0 &   0 \\
       2857 &   1 &   1 &   0 &   0 &   0 &   0 \\
       2859 &   1 &   1 &   0 &   0 &   0 &   0 \\
       2863 &   1 &   0 &   0 &   0 &   0 &   1 \\
       2864 &   1 &   0 &   0 &   0 &   0 &   1 \\
       2866 &   1 &   0 &   0 &   0 &   0 &   0 \\
       2874 &   0 &   0 &   0 &   1 &   0 &   1 \\
       2875 &   0 &   0 &   0 &   1 &   0 &   1 \\
       2879 &   1 &   0 &   0 &   1 &   0 &   1 \\
       2884 &   1 &   0 &   0 &   0 &   0 &   1 \\
       2885 &   1 &   0 &   0 &   0 &   0 &   1 \\
       2891 &   1 &   0 &   0 &   0 &   0 &   1 \\
       2896 &   1 &   1 &   0 &   0 &   0 &   1 \\
       2904 &   1 &   0 &   0 &   0 &   0 &   0 \\
       2906 &   1 &   1 &   0 &   0 &   0 &   0 \\
       2913 &   1 &   0 &   0 &   0 &   0 &   0 \\
       2915 &   1 &   0 &   0 &   0 &   0 &   0 \\
       2916 &   0 &   0 &   0 &   1 &   0 &   0 \\
       2925 &   1 &   0 &   0 &   1 &   0 &   0 \\
       2926 &   0 &   1 &   1 &   0 &   0 &   0 \\
       2931 &   0 &   0 &   1 &   0 &   0 &   0 \\
       2943 &   1 &   0 &   0 &   0 &   0 &   0 \\
       2949 &   1 &   1 &   0 &   0 &   0 &   0 \\
       2951 &   1 &   0 &   0 &   0 &   0 &   0 \\
       2956 &   1 &   0 &   0 &   0 &   0 &   0 \\
       2960 &   1 &   0 &   0 &   0 &   0 &   1 \\
       2961 &   1 &   0 &   0 &   0 &   0 &   0 \\
       2964 &   1 &   0 &   0 &   0 &   0 &   0 \\
       2968 &   1 &   0 &   0 &   0 &   0 &   0 \\
       2969 &   1 &   0 &   0 &   0 &   0 &   1 \\
       2970 &   1 &   0 &   0 &   0 &   0 &   0 \\
       2971 &   1 &   1 &   0 &   0 &   0 &   0 \\
       2974 &   1 &   0 &   0 &   0 &   0 &   1 \\
       2977 &   1 &   1 &   0 &   0 &   0 &   0 \\
       2979 &   1 &   0 &   0 &   0 &   0 &   1 \\
       2984 &   1 &   0 &   0 &   0 &   0 &   0 \\
       3008 &   1 &   0 &   0 &   0 &   0 &   0 \\
       3009 &   0 &   0 &   0 &   1 &   0 &   0 \\
       3012 &   1 &   0 &   0 &   0 &   0 &   1 \\
       3015 &   1 &   0 &   0 &   0 &   0 &   0 \\
       3017 &   1 &   0 &   0 &   0 &   0 &   0 \\
       3021 &   1 &   0 &   0 &   0 &   0 &   1 \\
       3023 &   1 &   0 &   0 &   0 &   0 &   1 \\
       3032 &   0 &   0 &   0 &   1 &   0 &   0 \\
       3039 &   1 &   0 &   0 &   0 &   0 &   0 \\
       3046 &   1 &   0 &   0 &   0 &   0 &   1 \\
       3052 &   1 &   1 &   0 &   0 &   0 &   0 \\
       3057 &   0 &   1 &   0 &   0 &   0 &   0 \\
       3060 &   1 &   0 &   0 &   0 &   0 &   0 \\
       3065 &   0 &   0 &   0 &   1 &   0 &   0 \\
       3075 &   1 &   0 &   0 &   0 &   0 &   0 \\
       3083 &   1 &   1 &   0 &   0 &   0 &   0 \\
       3086 &   0 &   0 &   1 &   0 &   0 &   0 \\
       3087 &   1 &   1 &   0 &   0 &   0 &   1 \\
       3093 &   1 &   0 &   0 &   0 &   0 &   0 \\
       3096 &   1 &   0 &   0 &   0 &   0 &   0 \\
       3097 &   1 &   1 &   0 &   0 &   0 &   0 \\
       3100 &   1 &   0 &   0 &   0 &   0 &   1 \\
       3103 &   1 &   0 &   0 &   0 &   0 &   1 \\
       3109 &   1 &   0 &   0 &   0 &   0 &   0 \\
       3111 &   1 &   1 &   0 &   0 &   0 &   0 \\
       3114 &   1 &   0 &   0 &   0 &   0 &   0 \\
       3117 &   1 &   0 &   0 &   0 &   0 &   0 \\
       3122 &   1 &   0 &   0 &   0 &   0 &   0 \\
       3125 &   1 &   0 &   0 &   0 &   0 &   0 \\
       3128 &   1 &   0 &   0 &   0 &   0 &   0 \\
       3130 &   1 &   1 &   0 &   0 &   0 &   0 \\
       3132 &   1 &   0 &   0 &   0 &   0 &   1 \\
       3146 &   1 &   0 &   0 &   0 &   0 &   0 \\
       3158 &   1 &   1 &   0 &   0 &   0 &   0 \\
       3165 &   1 &   0 &   0 &   0 &   0 &   0 \\
       3167 &   1 &   0 &   0 &   0 &   0 &   1 \\
       3168 &   1 &   0 &   0 &   0 &   0 &   0 \\
       3172 &   1 &   1 &   0 &   0 &   0 &   1 \\
       3179 &   1 &   0 &   0 &   0 &   0 &   0 \\
       3180 &   1 &   0 &   0 &   0 &   0 &   1 \\
       3184 &   1 &   1 &   0 &   0 &   0 &   0 \\
       3190 &   1 &   0 &   0 &   0 &   0 &   0 \\
       3193 &   1 &   0 &   0 &   0 &   0 &   0 \\
       3194 &   1 &   0 &   0 &   0 &   0 &   0 \\
       3195 &   1 &   0 &   0 &   0 &   0 &   1 \\
       3196 &   1 &   1 &   0 &   0 &   0 &   0 \\
       3197 &   1 &   0 &   0 &   0 &   0 &   0 \\
       3201 &   1 &   0 &   0 &   0 &   0 &   1 \\
       3202 &   1 &   0 &   0 &   0 &   0 &   1 \\
       3203 &   1 &   0 &   0 &   0 &   0 &   0 \\
       3208 &   1 &   0 &   0 &   0 &   0 &   0 \\
       3214 &   1 &   1 &   0 &   0 &   0 &   0 \\
       3215 &   1 &   0 &   0 &   0 &   0 &   1 \\
       3218 &   1 &   0 &   0 &   0 &   0 &   1 \\
       3220 &   1 &   0 &   0 &   0 &   0 &   0 \\
       3224 &   1 &   0 &   0 &   0 &   0 &   0 \\
       3225 &   1 &   0 &   0 &   0 &   0 &   0 \\
       3227 &   1 &   0 &   0 &   0 &   0 &   1 \\
       3232 &   1 &   0 &   0 &   0 &   0 &   0 \\
       3233 &   1 &   0 &   0 &   0 &   0 &   1 \\
       3234 &   1 &   0 &   0 &   0 &   0 &   0 \\
       3236 &   1 &   0 &   0 &   0 &   0 &   0 \\
       3237 &   1 &   0 &   0 &   0 &   0 &   0 \\
       3239 &   1 &   0 &   0 &   0 &   0 &   1 \\
       3240 &   1 &   0 &   0 &   0 &   0 &   1 \\
       3244 &   1 &   0 &   0 &   0 &   0 &   1 \\
       3245 &   1 &   0 &   0 &   0 &   0 &   0 \\
       3246 &   1 &   0 &   0 &   1 &   0 &   0 \\
       3248 &   1 &   0 &   0 &   0 &   0 &   0 \\
       3249 &   1 &   0 &   0 &   0 &   0 &   1 \\
       3251 &   1 &   0 &   0 &   0 &   0 &   1 \\
       3254 &   1 &   0 &   0 &   0 &   0 &   1 \\
       3277 &   1 &   0 &   0 &   0 &   0 &   0 \\
       3278 &   0 &   0 &   0 &   0 &   1 &   1 \\
       3283 &   0 &   1 &   0 &   0 &   0 &   0 \\
       3287 &   1 &   0 &   0 &   0 &   0 &   0 \\
       3288 &   1 &   0 &   0 &   0 &   0 &   0 \\
       3301 &   1 &   0 &   0 &   0 &   0 &   0 \\
       3308 &   1 &   1 &   0 &   0 &   0 &   0 \\
       3310 &   1 &   0 &   0 &   0 &   0 &   0 \\
       3315 &   1 &   0 &   0 &   0 &   0 &   0 \\
       3338 &   1 &   1 &   0 &   0 &   0 &   1 \\
       3340 &   1 &   1 &   0 &   0 &   0 &   0 \\
       3346 &   1 &   0 &   0 &   0 &   0 &   0 \\
       3358 &   1 &   0 &   0 &   0 &   0 &   0 \\
       3363 &   1 &   0 &   0 &   0 &   0 &   0 \\
       3371 &   1 &   1 &   0 &   0 &   0 &   0 \\
       3378 &   1 &   0 &   0 &   0 &   0 &   1 \\
       3382 &   1 &   0 &   0 &   0 &   0 &   1 \\
       3384 &   1 &   1 &   0 &   0 &   0 &   0 \\
       3403 &   1 &   1 &   0 &   0 &   0 &   0 \\
       3419 &   1 &   0 &   0 &   0 &   0 &   0 \\
       3421 &   1 &   0 &   0 &   0 &   0 &   0 \\
       3422 &   1 &   0 &   0 &   0 &   0 &   0 \\
       3425 &   1 &   1 &   0 &   0 &   0 &   0 \\
       3436 &   1 &   0 &   0 &   0 &   0 &   0 \\
       3438 &   1 &   0 &   0 &   0 &   0 &   0 \\
       3451 &   1 &   0 &   0 &   0 &   0 &   0 \\
       3456 &   1 &   1 &   0 &   0 &   0 &   0 \\
       3465 &   1 &   0 &   0 &   0 &   0 &   0 \\
       3473 &   1 &   0 &   0 &   0 &   0 &   0 \\
       3474 &   1 &   0 &   0 &   0 &   0 &   0 \\
       3497 &   1 &   0 &   0 &   0 &   0 &   0 \\
       3500 &   1 &   1 &   0 &   0 &   0 &   0 \\
       3503 &   1 &   1 &   0 &   0 &   0 &   0 \\
       3541 &   1 &   0 &   0 &   0 &   0 &   0 \\
       3608 &   1 &   0 &   0 &   0 &   0 &   0 \\
       3641 &   1 &   1 &   0 &   0 &   0 &   1 \\
       3663 &   1 &   0 &   1 &   0 &   0 &   0 \\
       3678 &   1 &   0 &   0 &   0 &   0 &   0 \\
       3680 &   0 &   0 &   0 &   0 &   1 &   0 \\
       3681 &   1 &   1 &   0 &   0 &   0 &   0 \\
       3683 &   1 &   0 &   0 &   0 &   0 &   0 \\
       3689 &   1 &   0 &   0 &   0 &   0 &   0 \\
       3726 &   0 &   0 &   1 &   0 &   0 &   0 \\
       3770 &   1 &   0 &   0 &   0 &   0 &   0 \\
       3780 &   1 &   0 &   0 &   0 &   0 &   0 \\
       3787 &   1 &   0 &   0 &   0 &   0 &   0 \\
       3791 &   1 &   1 &   0 &   0 &   0 &   0 \\
       3801 &   0 &   0 &   1 &   0 &   0 &   0 \\
       3811 &   1 &   0 &   1 &   0 &   0 &   0 \\
       3823 &   1 &   0 &   1 &   0 &   0 &   0 \\
       3835 &   1 &   0 &   0 &   0 &   0 &   0 \\
       3853 &   1 &   0 &   0 &   0 &   0 &   0 \\
       3864 &   1 &   1 &   0 &   0 &   0 &   0 \\
       3867 &   0 &   0 &   0 &   1 &   0 &   0 \\
       3871 &   1 &   0 &   0 &   0 &   0 &   1 \\
       3876 &   1 &   0 &   0 &   0 &   0 &   0 \\
       3880 &   1 &   0 &   0 &   0 &   0 &   0 \\
       3886 &   1 &   0 &   0 &   0 &   0 &   0 \\
       3889 &   1 &   0 &   0 &   0 &   0 &   1 \\
       3890 &   1 &   0 &   0 &   0 &   0 &   0 \\
       3891 &   1 &   0 &   0 &   0 &   0 &   0 \\
       3892 &   1 &   0 &   0 &   0 &   0 &   0 \\
       3907 &   1 &   0 &   0 &   0 &   0 &   0 \\
       3908 &   1 &   0 &   0 &   0 &   0 &   0 \\
       3913 &   0 &   0 &   0 &   1 &   0 &   0 \\
       3925 &   1 &   1 &   0 &   0 &   0 &   0 \\
       3928 &   1 &   0 &   0 &   0 &   0 &   0 \\
       3936 &   1 &   1 &   0 &   0 &   0 &   0 \\
       3943 &   1 &   0 &   0 &   0 &   0 &   0 \\
       3946 &   1 &   0 &   1 &   0 &   0 &   0 \\
       3980 &   0 &   0 &   0 &   1 &   0 &   1 \\
       3991 &   1 &   0 &   0 &   0 &   0 &   0 \\
       4002 &   0 &   0 &   0 &   1 &   0 &   0 \\
       4004 &   1 &   0 &   0 &   0 &   0 &   0 \\
       4005 &   0 &   0 &   1 &   0 &   0 &   0 \\
       4011 &   1 &   0 &   0 &   0 &   0 &   1 \\
       4014 &   1 &   0 &   0 &   0 &   0 &   0 \\
       4018 &   0 &   0 &   0 &   1 &   0 &   1 \\
       4021 &   1 &   1 &   0 &   0 &   0 &   0 \\
       4022 &   1 &   0 &   0 &   0 &   0 &   1 \\
       4024 &   1 &   0 &   0 &   0 &   0 &   0 \\
       4032 &   1 &   1 &   0 &   0 &   0 &   0 \\
       4036 &   1 &   0 &   1 &   0 &   0 &   0 \\
       4037 &   1 &   0 &   0 &   0 &   0 &   0 \\
       4053 &   1 &   0 &   0 &   0 &   0 &   0 \\
       4054 &   0 &   0 &   1 &   0 &   0 &   0 \\
       4060 &   1 &   0 &   1 &   0 &   0 &   0 \\
       4062 &   1 &   0 &   0 &   0 &   0 &   1 \\
       4066 &   1 &   0 &   0 &   0 &   0 &   0 \\
       4067 &   1 &   0 &   0 &   0 &   0 &   0 \\
       4070 &   0 &   0 &   0 &   1 &   0 &   1 \\
       4072 &   1 &   0 &   0 &   1 &   0 &   0 \\
       4098 &   1 &   0 &   0 &   0 &   0 &   0 \\
       4103 &   0 &   1 &   1 &   0 &   0 &   0 \\
       4109 &   0 &   0 &   0 &   1 &   0 &   0 \\
       4121 &   0 &   0 &   1 &   0 &   0 &   0 \\
       4123 &   1 &   0 &   0 &   0 &   0 &   0 \\
       4129 &   1 &   0 &   0 &   0 &   0 &   0 \\
       4136 &   1 &   1 &   0 &   0 &   0 &   0 \\
       4144 &   0 &   0 &   0 &   1 &   0 &   0 \\
       4146 &   1 &   0 &   0 &   0 &   0 &   0 \\
       4156 &   1 &   0 &   0 &   0 &   0 &   0 \\
       4157 &   1 &   1 &   0 &   0 &   0 &   0 \\
       4159 &   0 &   0 &   0 &   1 &   0 &   0 \\
       4160 &   1 &   0 &   0 &   0 &   0 &   0 \\
       4184 &   1 &   0 &   0 &   0 &   0 &   0 \\
       4188 &   1 &   0 &   0 &   0 &   0 &   0 \\
       4190 &   1 &   0 &   0 &   0 &   0 &   0 \\
       4198 &   1 &   0 &   0 &   0 &   0 &   1 \\
       4199 &   0 &   0 &   0 &   1 &   0 &   0 \\
       4204 &   1 &   0 &   0 &   0 &   0 &   0 \\
       4212 &   1 &   1 &   0 &   0 &   0 &   0 \\
       4215 &   1 &   0 &   0 &   0 &   0 &   0 \\
       4222 &   1 &   0 &   0 &   0 &   0 &   0 \\
       4226 &   1 &   0 &   0 &   0 &   0 &   0 \\
       4230 &   1 &   0 &   0 &   0 &   0 &   0 \\
       4235 &   1 &   0 &   0 &   0 &   0 &   0 \\
       4245 &   1 &   0 &   0 &   0 &   0 &   0 \\
       4246 &   1 &   1 &   0 &   0 &   0 &   0 \\
       4251 &   1 &   0 &   0 &   0 &   0 &   0 \\
       4257 &   1 &   0 &   0 &   0 &   0 &   1 \\
       4269 &   1 &   1 &   0 &   0 &   0 &   0 \\
       4273 &   1 &   0 &   0 &   0 &   0 &   0 \\
       4276 &   1 &   0 &   0 &   0 &   0 &   0 \\
       4287 &   1 &   1 &   0 &   0 &   0 &   0 \\
       4288 &   1 &   1 &   0 &   0 &   0 &   0 \\
       4292 &   1 &   0 &   0 &   0 &   0 &   0 \\
       4296 &   1 &   0 &   0 &   0 &   0 &   0 \\
       4298 &   1 &   1 &   0 &   0 &   0 &   1 \\
       4301 &   1 &   1 &   0 &   0 &   0 &   0 \\
       4302 &   1 &   0 &   0 &   0 &   0 &   0 \\
       4304 &   1 &   0 &   0 &   0 &   0 &   0 \\
       4312 &   1 &   0 &   0 &   0 &   0 &   0 \\
       4318 &   1 &   0 &   0 &   0 &   0 &   0 \\
       4323 &   1 &   1 &   0 &   0 &   0 &   0 \\
       4329 &   1 &   0 &   0 &   0 &   0 &   0 \\
       4335 &   1 &   0 &   0 &   0 &   0 &   0 \\
       4343 &   1 &   0 &   0 &   0 &   0 &   0 \\
       4356 &   0 &   0 &   1 &   0 &   0 &   0 \\
       4366 &   0 &   0 &   0 &   1 &   0 &   0 \\
       4367 &   1 &   0 &   0 &   0 &   0 &   0 \\
       4368 &   1 &   1 &   0 &   0 &   0 &   0 \\
       4374 &   1 &   0 &   0 &   0 &   0 &   0 \\
       4382 &   1 &   1 &   0 &   0 &   0 &   0 \\
       4383 &   1 &   1 &   0 &   0 &   0 &   0 \\
       4385 &   0 &   1 &   1 &   0 &   0 &   0 \\
       4399 &   1 &   0 &   0 &   0 &   0 &   0 \\
       4400 &   1 &   0 &   0 &   0 &   0 &   0 \\
       4407 &   1 &   0 &   0 &   0 &   0 &   0 \\
       4409 &   1 &   0 &   0 &   0 &   0 &   0 \\
       4411 &   1 &   0 &   0 &   0 &   0 &   0 \\
       4418 &   0 &   0 &   1 &   0 &   0 &   0 \\
       4421 &   1 &   1 &   0 &   0 &   0 &   0 \\
       4423 &   1 &   0 &   0 &   0 &   0 &   0 \\
       4426 &   1 &   0 &   0 &   0 &   0 &   0 \\
       4430 &   0 &   0 &   0 &   1 &   0 &   1 \\
       4431 &   1 &   1 &   0 &   0 &   0 &   0 \\
       4435 &   1 &   1 &   0 &   0 &   0 &   0 \\
       4441 &   0 &   0 &   0 &   1 &   0 &   0 \\
       4443 &   1 &   0 &   0 &   0 &   0 &   0 \\
       4446 &   1 &   0 &   0 &   0 &   0 &   0 \\
       4452 &   1 &   0 &   0 &   0 &   0 &   0 \\
       4457 &   1 &   0 &   0 &   0 &   0 &   0 \\
       4469 &   0 &   0 &   0 &   1 &   0 &   1 \\
       4473 &   1 &   0 &   0 &   0 &   0 &   0 \\
       4480 &   1 &   0 &   0 &   0 &   0 &   0 \\
       4482 &   1 &   0 &   0 &   0 &   0 &   0 \\
       4505 &   1 &   0 &   0 &   0 &   0 &   0 \\
       4546 &   1 &   0 &   0 &   0 &   0 &   0 \\
       4556 &   1 &   0 &   0 &   0 &   0 &   1 \\
       4557 &   1 &   0 &   0 &   0 &   0 &   0 \\
       4561 &   1 &   0 &   0 &   0 &   0 &   0 \\
       4567 &   1 &   1 &   0 &   0 &   0 &   0 \\
       4575 &   1 &   0 &   0 &   0 &   0 &   0 \\
       4580 &   1 &   0 &   0 &   0 &   0 &   0 \\
       4581 &   1 &   0 &   0 &   0 &   0 &   0 \\
       4582 &   1 &   0 &   0 &   0 &   0 &   0 \\
       4585 &   1 &   0 &   0 &   0 &   0 &   0 \\
       4588 &   1 &   0 &   0 &   0 &   0 &   0 \\
       4601 &   1 &   0 &   0 &   0 &   0 &   0 \\
       4603 &   1 &   0 &   0 &   0 &   0 &   0 \\
       4605 &   1 &   0 &   0 &   0 &   0 &   0 \\
       4613 &   1 &   0 &   0 &   0 &   0 &   0 \\
       4614 &   1 &   0 &   0 &   0 &   0 &   0 \\
       4617 &   1 &   0 &   0 &   0 &   0 &   0 \\
       4633 &   1 &   0 &   0 &   0 &   0 &   0 \\
       4634 &   1 &   0 &   0 &   0 &   0 &   0 \\
       4637 &   1 &   0 &   0 &   0 &   0 &   0 \\
       4640 &   1 &   0 &   0 &   0 &   0 &   0 \\
       4647 &   1 &   1 &   0 &   0 &   0 &   0 \\
       4651 &   1 &   0 &   0 &   0 &   0 &   0 \\
       4653 &   1 &   0 &   0 &   0 &   0 &   0 \\
       4657 &   1 &   1 &   0 &   0 &   0 &   0 \\
       4659 &   1 &   0 &   0 &   0 &   0 &   0 \\
       4663 &   1 &   0 &   0 &   0 &   0 &   0 \\
       4665 &   1 &   0 &   0 &   0 &   0 &   1 \\
       4674 &   1 &   0 &   0 &   0 &   0 &   0 \\
       4686 &   1 &   0 &   0 &   0 &   0 &   0 \\
       4693 &   1 &   0 &   0 &   0 &   0 &   0 \\
       4699 &   1 &   0 &   0 &   0 &   0 &   0 \\
       4706 &   1 &   0 &   0 &   0 &   0 &   0 \\
       4715 &   1 &   0 &   0 &   0 &   0 &   0 \\
       4716 &   1 &   1 &   0 &   0 &   0 &   0 \\
       4717 &   0 &   0 &   1 &   0 &   0 &   0 \\
       4725 &   1 &   0 &   0 &   0 &   0 &   0 \\
       4744 &   1 &   0 &   0 &   0 &   0 &   1 \\
       4745 &   0 &   0 &   1 &   0 &   0 &   0 \\
       4746 &   0 &   0 &   0 &   1 &   0 &   1 \\
       4763 &   1 &   0 &   0 &   0 &   0 &   0 \\
       4765 &   1 &   0 &   0 &   0 &   0 &   0 \\
       4771 &   1 &   0 &   0 &   0 &   0 &   0 \\
       4773 &   1 &   0 &   0 &   0 &   0 &   0 \\
       4774 &   1 &   0 &   0 &   0 &   0 &   0 \\
       4775 &   1 &   0 &   0 &   0 &   0 &   0 \\
       4792 &   1 &   0 &   0 &   0 &   0 &   0 \\
       4811 &   1 &   0 &   0 &   0 &   0 &   0 \\
       4822 &   1 &   0 &   0 &   0 &   0 &   0 \\
       4829 &   1 &   1 &   0 &   0 &   0 &   0 \\
       4833 &   1 &   0 &   0 &   0 &   0 &   0 \\
       4834 &   1 &   0 &   0 &   0 &   0 &   0 \\
       4839 &   1 &   0 &   0 &   0 &   0 &   0 \\
       4841 &   0 &   0 &   0 &   1 &   0 &   1 \\
       4850 &   1 &   0 &   0 &   0 &   0 &   0 \\
       4864 &   1 &   0 &   0 &   0 &   0 &   0 \\
       4881 &   1 &   1 &   0 &   0 &   0 &   0 \\
       4887 &   1 &   0 &   0 &   0 &   0 &   1 \\
       4892 &   1 &   0 &   0 &   0 &   0 &   0 \\
       4898 &   0 &   0 &   1 &   0 &   0 &   0 \\
       4902 &   0 &   0 &   1 &   0 &   0 &   0 \\
       4907 &   1 &   0 &   0 &   0 &   0 &   0 \\
       4941 &   0 &   0 &   1 &   0 &   0 &   1 \\
       4961 &   0 &   0 &   1 &   0 &   0 &   0 \\
       4978 &   0 &   0 &   1 &   0 &   0 &   0 \\
       5018 &   0 &   0 &   1 &   0 &   0 &   0 \\
       5021 &   0 &   0 &   1 &   0 &   0 &   0 \\
       5039 &   0 &   0 &   1 &   0 &   0 &   1 \\
       5048 &   1 &   0 &   0 &   0 &   0 &   0 \\
       5057 &   1 &   0 &   0 &   0 &   0 &   0 \\
       5084 &   0 &   0 &   1 &   0 &   0 &   0 \\
       5085 &   0 &   0 &   1 &   0 &   0 &   0 \\
       5107 &   1 &   0 &   0 &   0 &   0 &   0 \\
       5119 &   1 &   0 &   0 &   0 &   0 &   0 \\
       5124 &   0 &   0 &   1 &   0 &   0 &   0 \\
       5135 &   0 &   0 &   1 &   0 &   0 &   0 \\
       5155 &   0 &   0 &   0 &   0 &   1 &   0 \\
       5159 &   0 &   0 &   1 &   0 &   0 &   1 \\
       5198 &   0 &   0 &   1 &   0 &   0 &   1 \\
       5216 &   0 &   0 &   1 &   0 &   0 &   0 \\
       5236 &   1 &   0 &   1 &   0 &   0 &   0 \\
       5241 &   0 &   0 &   1 &   0 &   0 &   0 \\
       5247 &   0 &   0 &   0 &   0 &   1 &   0 \\
       5269 &   0 &   0 &   1 &   0 &   0 &   0 \\
       5278 &   0 &   0 &   1 &   0 &   0 &   0 \\
       5284 &   0 &   0 &   1 &   0 &   0 &   0 \\
       5290 &   0 &   0 &   1 &   0 &   0 &   0 \\
       5324 &   1 &   0 &   0 &   0 &   0 &   0 \\
       5375 &   1 &   0 &   0 &   0 &   0 &   0 \\
       5379 &   1 &   0 &   0 &   0 &   0 &   0 \\
       5380 &   0 &   0 &   1 &   0 &   0 &   0 \\
       5393 &   1 &   0 &   0 &   0 &   0 &   0 \\
       5423 &   0 &   0 &   1 &   0 &   0 &   0 \\
       5546 &   0 &   0 &   1 &   0 &   0 &   0 \\
       5567 &   0 &   0 &   1 &   0 &   0 &   0 \\
       5592 &   0 &   0 &   1 &   0 &   0 &   0 \\
       5612 &   0 &   0 &   1 &   0 &   0 &   0 \\
       5613 &   0 &   0 &   1 &   0 &   0 &   0 \\
       5622 &   0 &   0 &   1 &   0 &   0 &   0 \\
       5625 &   0 &   0 &   0 &   0 &   1 &   0 \\
       5626 &   0 &   0 &   1 &   0 &   0 &   0 \\
       5645 &   0 &   0 &   1 &   0 &   0 &   0 \\
       5689 &   0 &   0 &   1 &   0 &   0 &   0 \\
       5702 &   0 &   0 &   1 &   0 &   0 &   0 \\
       5706 &   0 &   0 &   1 &   0 &   0 &   0 \\
       5782 &   1 &   0 &   0 &   0 &   0 &   0 \\
       5790 &   0 &   0 &   1 &   0 &   0 &   0 \\
       5792 &   0 &   0 &   1 &   0 &   0 &   0 \\
       5798 &   0 &   0 &   1 &   0 &   0 &   0 \\
       5837 &   0 &   0 &   1 &   0 &   0 &   0 \\
       5850 &   0 &   0 &   1 &   0 &   0 &   0 \\
       5852 &   0 &   0 &   0 &   0 &   1 &   0 \\
       5855 &   0 &   0 &   1 &   0 &   0 &   0 \\
       5869 &   0 &   0 &   1 &   0 &   0 &   0 \\
       5877 &   0 &   0 &   1 &   0 &   0 &   0 \\
       5888 &   0 &   0 &   1 &   0 &   0 &   0 \\
       5900 &   1 &   1 &   0 &   1 &   0 &   1 \\
       5924 &   0 &   0 &   1 &   0 &   0 &   0 \\
       5929 &   0 &   0 &   1 &   0 &   0 &   0 \\
       5932 &   0 &   0 &   1 &   0 &   0 &   0 \\
       5949 &   1 &   0 &   1 &   0 &   0 &   0 \\
       5953 &   0 &   0 &   1 &   0 &   0 &   0 \\
       6102 &   1 &   0 &   0 &   0 &   0 &   0 \\
       6384 &   0 &   0 &   0 &   0 &   1 &   0 \\
       6425 &   1 &   0 &   0 &   0 &   0 &   0 \\
       6676 &   1 &   0 &   0 &   0 &   0 &   0 \\
       6734 &   0 &   0 &   0 &   0 &   1 &   0 \\
       6745 &   0 &   0 &   0 &   0 &   1 &   0 \\
       6759 &   0 &   0 &   0 &   0 &   1 &   0 \\
       6786 &   0 &   0 &   0 &   0 &   1 &   0 \\
       6883 &   0 &   0 &   0 &   0 &   1 &   1 \\
       6927 &   0 &   0 &   0 &   0 &   1 &   1 \\
       6971 &   0 &   0 &   0 &   0 &   1 &   0 \\
       6981 &   0 &   0 &   0 &   0 &   1 &   1 \\
       7016 &   1 &   0 &   0 &   0 &   0 &   0 \\
       7040 &   0 &   0 &   0 &   0 &   1 &   0 \\
       7136 &   0 &   0 &   0 &   0 &   1 &   0 \\
       7179 &   1 &   0 &   0 &   0 &   0 &   0 \\
       7223 &   0 &   0 &   0 &   0 &   1 &   0 \\
       7235 &   0 &   0 &   0 &   0 &   1 &   0 \\
       7345 &   0 &   0 &   0 &   0 &   1 &   0 \\
       7566 &   0 &   0 &   0 &   0 &   1 &   1 \\
       7587 &   1 &   0 &   0 &   0 &   0 &   0 \\
       7599 &   0 &   0 &   0 &   0 &   1 &   0 \\
       7605 &   0 &   0 &   0 &   0 &   1 &   1 \\
 KIC8435766 &   1 &   0 &   0 &   1 &   0 &   0 \\
KIC11187332 &   0 &   0 &   0 &   1 &   0 &   0 \\
 KIC2718885 &   0 &   0 &   0 &   1 &   0 &   0 \\
 KIC6359893 &   0 &   0 &   0 &   1 &   0 &   0 \\

